Stochastic Top-$K$ Subset Bandits with Linear Space and Non-Linear Feedback

Many real-world problems like Social Influence Maximization face the dilemma of choosing the best $K$ out of $N$ options at a given time instant. This setup can be modeled as a combinatorial bandit which chooses $K$ out of $N$ arms at each time, with an aim to achieve an efficient trade-off between exploration and exploitation. This is the first work for combinatorial bandits where the feedback received can be a non-linear function of the chosen $K$ arms. The direct use of multi-armed bandit requires choosing among $N$-choose-$K$ options making the state space large. In this paper, we present a novel algorithm which is computationally efficient and the storage is linear in $N$. The proposed algorithm is a divide-and-conquer based strategy, that we call CMAB-SM. Further, the proposed algorithm achieves a \textit{regret bound} of $\tilde O(K^{\frac{1}{2}}N^{\frac{1}{3}}T^{\frac{2}{3}})$ for a time horizon $T$, which is \textit{sub-linear} in all parameters $T$, $N$, and $K$. %When applied to the problem of Social Influence Maximization, the performance of the proposed algorithm surpasses the UCB algorithm and some more sophisticated domain-specific methods.

==> algo_update_round.tex <==
	\begin{algorithm} [htb]
		\small
		\begin{algorithmic}
		    \STATE \bf{Input} $r$
            \STATE $r = r+1$
            \STATE $\Delta_r = 2^{-r}$
            \STATE $n_r = \frac{2\log{\left(TNK\right)}}{\Delta^2_r}$
            \STATE \bf{Output} $n_r, \Delta_r, r$
		\end{algorithmic}
		\caption{UPDATE\_ROUND}\label{alg:update_round_param}
	\end{algorithm}

==> explore_time.tex <==
\subsection{Bounds on exploitation regret and exploration time}

In this subsection, we will bound the regret in the exploitation phase, which indicates the loss in reward due to choosing an incorrect action at the end of the MERGE algorithm. We will also bound the time spent in the SORT and the MERGE subroutines, which is the exploration phase. 

In order to bound the regret in the exploitation phase, we first characterize the probability that the action decided by \NAM\ is not the best action.  

\begin{lemma}[Total error probability] \label{algorithm_error_event_prob}
The probability that the action selected by \NAM\ is not the best action (action with the highest reward) is at most $\frac{1}{NT^2}$. 
\end{lemma} 
\begin{proof}
To bound the probability of error of \cref{alg:dama}, we define the event $\mathcal{E}$ which is the event when the algorithm makes an error. The algorithm makes an error when either SORT subroutine, or MERGE subroutine, or both make an error. So, we can write the error event as a union of error events in sorting and error events in merging. Let $\mathcal{E}_{s}$ the event where at least one of the $\frac{N}{K+1}$ calls made to \cref{alg:da} resulted in an incorrect list, and $\mathcal{E}_m$ be the event where at least one of the $\frac{N}{K+1} - 1$ merges is in error.
\begin{eqnarray}
    \mathcal{E} &=& \mathcal{E}_s \cup \mathcal{E}_m
\end{eqnarray}
Since the probability of the union of events is upper bounded by the sum of probabilities of individual events, we get
\begin{eqnarray}
    P\left(\mathcal{E}\right) &\leq& P\left(\mathcal{E}_s\right) + P\left(\mathcal{E}_m\right) \label{ref:algo_error_sum}
\end{eqnarray}
We now identify upper bounds for $P\left(\mathcal{E}_s\right)$ and $P\left(\mathcal{E}_m\right)$ by breaking down the error events into error in each call to SORT and MERGE subroutine.

Let us define an event $\mathcal{E}_{s,i}$ which denotes that there was an error in the sorted list given by \cref{alg:da} for $i^{th}$ group, or 
\begin{eqnarray}
\mathcal{E}_{s,i} &\triangleq& \left\{\text{at least two arms are incorrectly placed in sorting } i^{th} \text{ group}\right\}
\end{eqnarray}

 Hence, $\mathcal{E}_{s}$ is a union of $\mathcal{E}_{s,i}$ for all  $i \in \{1, 2, \cdots, \frac{N}{K+1}\}$, or  $\mathcal{E}_s = \bigcup_{k = 1}^{\frac{N}{K+1}}\mathcal{E}_{s,i}$. 
Probability of error in any of the sorting operations is thus given as
\begin{eqnarray}
    P\left(\mathcal{E}_s\right) &=& P\left(\bigcup_{k = 1}^{\frac{N}{K+1}}\mathcal{E}_{s,i}\right) \label{eq:sort_union_bound}\\
    &\leq& \sum^{\frac{N}{K+1}}_{k = 1}P\left(\mathcal{E}_{s,i}\right)\label{eq:sort_union_bound_sum}\\
    &<& \sum^{\frac{N}{K+1}}_{k = 1}\frac{K}{2N^2T^2} \label{eq:replace_prob_sort_val}\\
    &=& \frac{N}{K+1}\frac{K}{2NT^2}\\
    &<& \frac{1}{2NT^2},
\end{eqnarray}
where (\ref{eq:sort_union_bound}), and (\ref{eq:sort_union_bound_sum}) follow from the definition of events and the union bound, respectively, and  (\ref{eq:replace_prob_sort_val}) follows from Lemma \ref{sort_requirements}.

Similarly we define event $\mathcal{E}_{m,i}$ representing that  \cref{alg:da} incorrectly merges the merged group up to group $i$ and $(i+1)^{th}$ group. Let $G_M^i$ be the merged sorted group formed by merging sorted groups $G_M^{i-1}$ and $G_i$ for $i>1$, with $G_M^1 = G_1$. Then, we have
\begin{eqnarray}
\mathcal{E}_{m,i} = \left\{\text{error occurred while merging } G_M^{i} \text{ and } G_{i+1}\right\} . 
\end{eqnarray}

We note that $\mathcal{E}_{m}$ is a union of $\mathcal{E}_{m,i}$ for all $i \in \{1, 2, \cdots, \frac{N}{K+1}-1\}$, or   $ \mathcal{E}_m = \bigcup_{k = 1}^{\frac{N}{K+1}-1}\mathcal{E}_{m,i}$. 
Probability of error in the MERGE subroutine is given as 
\begin{eqnarray}
    P\left(\mathcal{E}_m\right) &=& P\left(\bigcup_{k = 1}^{\frac{N}{K+1}-1}\mathcal{E}_{m,i}\right) \label{eq:merge_union_bound}\\
    &\leq& \sum^{\frac{N}{K+1}-1}_{k = 1}P\left(\mathcal{E}_{m,i}\right)\label{eq:merge_union_bound_sum}\\
    &<& \sum^{\frac{N}{K+1}-1}_{k = 1}\frac{K}{2N^2T^2} \label{eq:replace_prob_merge_val}\\
    &<& \frac{N}{K+1}\frac{K}{2NT^2}\\
    &<& \frac{1}{2NT^2},
\end{eqnarray}
where (\ref{eq:merge_union_bound}) and (\ref{eq:merge_union_bound_sum}) follow from the definition of events and union bound, respectively, and (\ref{eq:replace_prob_merge_val}) follows from Lemma \ref{Merge_requirements}.% and rest follows from algebra.

Substituting bounds obtained on $P\left(\mathcal{E}_m\right)$ and $P\left(\mathcal{E}_s\right)$ in  (\ref{ref:algo_error_sum}), we have
\begin{eqnarray}
    P\left(\mathcal{E}\right) &<& \frac{1}{2NT^2} + \frac{1}{2NT^2}\\
    &=& \frac{1}{NT^2}
\end{eqnarray}
The total error probability of the algorithm is thus bounded by $\frac{1}{NT^2}$, proving the statement of the Lemma. 
\end{proof}

In the following result, we bound the expected regret in the exploitation phase, caused by \NAM\ selecting incorrect action. 

\begin{lemma}[ Bounded exploitation regret] \label{exploitation_regret_bound}
The expected regret when a sub-optimal action ${\bf \hat{a}}^*$ is returned by \NAM\ is bounded as 
\begin{eqnarray}
    \mathbb{E}\left[\Delta_{{\bf \hat{a}}^*}\right] \leq U\lambda\sqrt{K} + \frac{U\sqrt{K}}{NT^2}
\end{eqnarray}
\end{lemma} 
\begin{proof}
We will bound the expected regret where the suboptimal action is returned by \NAM, which includes an error from \cref{alg:da} or from \cref{alg:ma}. Let the chosen action be ${{\bf \hat{a}}^*} = (\hat{a}^*_1, \cdots, \hat{a}^*_K)$ and  optimal action be ${\bf a}^* = ({a}^*_1, \cdots, {a}^*_K)$. Then, the gap in the actions is $P=\sqrt{\min_{\Pi}(\sum_{i=1}^K ({\bf d}_{{ \hat{a}}^*_i} - {\bf d}_{{a}^*_{\Pi(i)}}) )^2}$, where $\Pi$ is any possible permutation of $\{1, \cdots, K\}$. Also, let $\Pi^*$ be the permutation that optimizes the above minimization. Using \ref{continuous_assumption}, and $U$ defined in \ref{double_sided_continuity}, we have 

\begin{eqnarray}
\mathbb{E}\left[r_{{\bf a}^*} - r_{{\bf \hat{a}}^*}\right] &\leq& U P \label{eq:pbound}
\end{eqnarray}
\if 0
We also note that since ${\bf d}_{\bf a} \in [0,1]^K$ for any action ${\bf a}$, we also have from \ref{continuous_assumption}
\begin{eqnarray}
\mathbb{E}\left[r_{{\bf a}^*} - r_{{\bf \hat{a}}^*}\right] &\leq& U 
\sqrt{K}. 
\end{eqnarray}

Combining the two, we have
\begin{eqnarray}
\mathbb{E}\left[r_{{\bf a}^*} - r_{{\bf \hat{a}}^*}\right] &\leq& U \min(P, \sqrt{K})\\
&=&U\sqrt{K} \label{eq:bnd_1}
\end{eqnarray}
\fi

%{\bf Mridul, check the above and see - seems you will not get the additional $\sqrt{K}$. Your part is in commented below, and I am rewriting it separately. }

We consider two possible cases. Case 1 corresponds to the scenario where for some $i$, $ {\bf d}_{{\hat{a}}^*_i} - {\bf d}_{{a}^*_{\Pi^*(i)}} >\lambda$. The second case is when for all $i$, $ {\bf d}_{{\hat{a}}^*_i} - {\bf d}_{{a}^*_{\Pi^*(i)}} \le \lambda$.

% corresponding to whether $P> \lambda$ or $P\le \lambda$.

{\bf Case 1: For some $i$, $ {\bf d}_{{\hat{a}}^*_i} - {\bf d}_{{a}^*_{\Pi^*(i)}} >\lambda$. } In this case, the incorrect action has arms which could have been separated without hitting the threshold $\lambda$, but did not do so because of an error in the SORT or MERGE subroutine. We note that since ${\bf d}_{{ \hat{a}}^*_i}$ and  ${\bf d}_{{a}^*_{\Pi(i)}}$ are both in $[0,1]$, $P\le \sqrt{K}$. The expected regret at time $t$  can be written as

%Let the chosen sub-optimal action be ${{\bf \hat{a}}^*}$ and true optimal action ${\bf a}^*$. The expected value of arms which are different in ${{\bf \hat{a}}^*}$ and ${\bf a}^*$ are at least $\lambda$. The maximum difference between expected of any two arms can be $1$ as the rewards are bounded in $[0,1]$. Then using assumption \ref{continuous_assumption} and equation (\ref{eq:cont_upper_defn}) we have,
%\begin{eqnarray}
%\mathbb{E}\left[r_{{\bf a}^*} - r_{{\bf \hat{a}}^*}\right] &\leq& U\big|\big|\mathbb{E}[{\bf d}_{{\bf a}^*}] - \mathbb{E}[{\bf d}_{{\bf \hat{a}}^*}]\big|\big|_2\\
%&\leq& U\sqrt{K} \label{eq:max_arm_separation}
%\end{eqnarray}
%Where (\ref{eq:max_arm_separation}) is obtained by making expectation of all $K$ arms in ${{\bf \hat{a}}^*}$  at max $1$ separated in expectation from all arms of ${{\bf a}^*}$. 


\begin{eqnarray}
\mathbb{E}\left[R(t)\right] &=& \mathbb{E}\left[r_{{\bf a}^*} - r_{{\bf \hat{a}}^*}\big|{\bf a}_t \neq {\bf a}^*\right]  \times P\left(\left\{{\bf a}_t \neq {\bf a}^*\right\}\right) \label{eq:conditional_regret}\\
&\leq& U\sqrt{K} \times P\left(\left\{{\bf a}_t \neq {\bf a}^*\right\}\right) \label{eq:cond_regret_expd}\\
&\le& \frac{U\sqrt{K}}{NT^2} \label{eq:cond_regret_final}, 
\end{eqnarray}
where (\ref{eq:cond_regret_expd}) follows from \eqref{eq:pbound} with $P\le \sqrt{K}$, and \eqref{eq:cond_regret_final} follows from \cref{algorithm_error_event_prob}. 


{\bf Case 2:  For all $i$, $ {\bf d}_{{\hat{a}}^*_i} - {\bf d}_{{a}^*_{\Pi^*(i)}} \le \lambda$.} In this case,  the SORT or MERGE subroutines will not be able to differentiate between the two actions. Thus, $P\left(\left\{{\bf a}_t \neq {\bf a}^*\right\}\right) $ will no longer be bounded by $1/{NT^2}$ in this case, since the individual rewards are bounded by $\lambda$, we have $P\le \lambda \sqrt{K}$.  Thus, we have 

%Where the difference between the expected value is less than precision threshold $\lambda$ and the SORT or MERGE subroutine were not able to identify the correct arm.

%Let the chosen sub-optimal action be ${{\bf \hat{a}}^*}$ and true optimal action ${\bf a}^*$. The expected value of arms which are different in ${{\bf \hat{a}}^*}$ and ${\bf a}^*$ are at max $\lambda$. Then using assumption \ref{continuous_assumption} and equation (\ref{eq:cont_upper_defn}) we have,
\begin{eqnarray}
\mathbb{E}\left[R(t)\right] &=& \mathbb{E}\left[r_{{\bf a}^*} - r_{{\bf \hat{a}}^*}\big|{\bf a}_t \neq {\bf a}^*\right] \times P\left(\left\{{\bf a}_t \neq {\bf a}^*\right\}\right) \label{eq:conditional_regret_good_event}\\
&\leq& U\lambda \sqrt{K} \times P\left(\left\{{\bf a}_t \neq {\bf a}^*\right\}\right) \label{eq:cond_regret_expd_good_event}\\
&\le & U\lambda \sqrt{K}, \label{eq:cond_regret_final_good_event}
\end{eqnarray}
where  (\ref{eq:cond_regret_expd_good_event}) follows from \eqref{eq:pbound} and $P\le \lambda \sqrt{K}$. 



%the maximum regret any sub-optimal action can incur, and (\ref{eq:cond_regret_final_good_event}) comes from the fact that probability of any event cannot exceed $1$



Combining both the cases, the maximum regret the algorithm can incur is bounded by $U\lambda\sqrt{K} + \frac{U\sqrt{K}}{NT^2}$, this proving the result. 
\end{proof}

In the next result, we bound the time spent in exploring, including the SORT and MERGE subroutines for all groups. 

\begin{lemma}[Bound on exploration time steps] \label{exploration_time_bound}
Total time-steps used to SORT all $\frac{N}{K+1}$ groups, and merge these sorted groups one after the other is bounded as 
\begin{eqnarray}
    T_{exp} \le \frac{128NU^2\log{2NT}}{\lambda^2}
\end{eqnarray}
\end{lemma}
\begin{proof}
    Exploration in \cref{alg:dama} is done using SORT and MERGE subroutines, so we will analyze the maximum time taken by the two subroutines. To sort all groups, \cref{alg:dama} runs SORT $\frac{N}{K+1}$ times, and to merge the groups, \cref{alg:dama} runs  $\frac{N}{K+1}-1$ times. Let $i^{th}$ run of SORT uses $T_{SORT, i}$ time steps, and $j^{th}$ run of MERGE uses $T_{MERGE,j}$ time steps. The total number of time-steps used for exploration can be written as
    \begin{eqnarray}
        T_{exp} &=& \sum_{s = 1}^{\frac{N}{K+1}}T_{SORT,s} + \sum_{m = 1}^{\frac{N}{K+1}-1}T_{MERGE,m}\\
        &\leq& \sum_{s = 1}^{\frac{N}{K+1}}\max_{s}{\left(T_{SORT,s}\right)} + \sum_{m = 1}^{\frac{N}{K+1}-1}\max_{m}{\left(T_{MERGE,m}\right)}\\
        &=& \frac{N}{K+1}\max_{s}{\left(T_{SORT,s}\right)} + \left(\frac{N}{K+1}-1\right)\max_{m}{\left(T_{MERGE,m}\right)}
    \end{eqnarray}
    We use Lemma \ref{sort_requirements} to find $\max_{s}{\left(T_{SORT,s}\right)}$ as follows. 
    \begin{eqnarray}
        T_{SORT,s} &=& \sum_{j=1}^{K+1}\frac{64U^2\log{2NT}}{\left(\max{\left(\lambda,\delta_{s,j}\right)}\right)^2}\\
        &\leq& \sum_{j, \delta_{s,j} > \lambda}^{K+1}\frac{64U^2\log{2NT}}{\lambda^2} + \sum_{j, \delta_{s,j} < \lambda}^{K+1}\frac{64U^2\log{2NT}}{\lambda^2} \label{eq:lower_bound_delta}\\
        &=& \sum_{j=1}^{K+1}\frac{64U^2\log{2NT}}{\lambda^2}\\
        &=& \frac{64\left(K+1\right)U^2\log{2NT}}{\lambda^2}.  \label{eq:sort_time_bound}
    \end{eqnarray}
%    Where equation (\ref{eq:lower_bound_delta}) follows by reducing difference of expected reward of arms of the groups to precision threshold. Since time required for any run of SORT is at most by the right hand side of (\ref{eq:sort_time_bound}), the maximum time for sorting any group is bounded by the same expression.
    Similarly,  we use Lemma \ref{Merge_requirements} to find $\max_s\left(T_{MERGE_s}\right)$ as follows. 
    \begin{eqnarray}
        T_{MERGE,m} &=& \sum_{j=1}^{K+1}\frac{64U^2\log{2NT}}{\left(\max{\left(\lambda,\delta_{m,j}\right)}\right)^2} \\
        &\leq& \sum_{j, \delta_{m,j} > \lambda}^{K+1}\frac{64U^2\log{2NT}}{\lambda^2} + \sum_{j, \delta_{m,j} < \lambda}^{K+1}\frac{64U^2\log{2NT}}{\lambda^2} \label{eq:lower_bound_delta_merge}\\
        &=& \sum_{j=1}^{K+1}\frac{64U^2\log{2NT}}{\lambda^2}\\
        &=& \frac{64\left(K+1\right)U^2\log{2NT}}{\lambda^2}
    \end{eqnarray}
    Total exploration time can now be bounded by using the values for maximum time taken for SORT and MERGE as,
    \begin{eqnarray}
        T_{exp} &\leq& \frac{N}{K+1}\max_{s}{\left(T_{SORT,s}\right)} + \left(\frac{N}{K+1}-1\right)\max_{s}{\left(T_{SORT,s}\right)}\\
        &\leq& \frac{N}{K+1}\frac{64\left(K+1\right)U^2\log{2NT}}{\lambda^2} + \left(\frac{N}{K+1}-1\right)\frac{64\left(K+1\right)U^2\log{2NT}}{\lambda^2}\\
        &<& \frac{N}{K+1}\frac{64\left(K+1\right)U^2\log{2NT}}{\lambda^2} + \left(\frac{N}{K+1}\right)\frac{64\left(K+1\right)U^2\log{2NT}}{\lambda^2}\\
        &\leq& \frac{64NU^2\log{2NT}}{\lambda^2} + \frac{64NU^2\log{2NT}}{\lambda^2}\\
        &\leq& \frac{128NU^2\log{2NT}}{\lambda^2}
    \end{eqnarray}
\end{proof}


==> keylemmas.tex <==
\subsection{Key results used in the proof of Theorem \ref{final_theorem_for_regret_bound}}

In this subsection, we will describe some key results that will be later used to prove the regret bound in Theorem \ref{final_theorem_for_regret_bound}. The following lemma relates the expected value of a random variable to the complementary cumulative distribution function. 
\begin{lemma}[Chapter 5, Lemma 2.1, \citealt{ross2006first}] \label{exp_from_ccdf} 
    Expected value of a positive random variable $X$ is the area under the curve of the complementary cumulative distribution function of the random variable
    \begin{equation}
        \mathbb{E}\left[g\left(X\right)\right] = \int^{\infty}_{0}P\left(g\left(X\right) > t\right)dt \label{eq:exp_from_ccdf}
    \end{equation}
\end{lemma}


The next result shows that the property of FSD is preserved by strictly increasing functions. 
\begin{lemma} \label{ordering_on_increasing_fn}
    Suppose that a random variable $X$ has FSD over another random variable $Y$ (or 
    $X \succ Y$).  Further, let $g'(.)$ be a strictly increasing function, or $g':\mathbb{R}\to \mathbb{R} \text{ s.t. } g'(x) > g'(y) \text{ } \forall \text{ }x>y, \text{ } x,y \in \mathbb{R}$. Then, $g'(X)$ has FSD over $g'(Y)$, or 
    \begin{equation}
         g'(X)\succ g'(Y)
    \end{equation}
\end{lemma}

\begin{proof}
%    Let $X$ and $Y$ be two random variables such that $X$ majorizes $Y$, and $g:\mathbb{R}\to\mathbb{R}$ be a strictly increasing function, then we have
 %   \begin{eqnarray}
 %       X &\succ& Y \label{eq:def_maj_1}\\
  %      g'(x) &>&g'(y) \text{ }\forall \text{ } x > y, \text{ }x,y \in \mathbb{R}
  %  \end{eqnarray}    
 Since $X \succ Y$, we have 
    \begin{eqnarray}
        P\left(X\ge x\right) &\geq& P\left(Y\ge x\right) \label{eq:def_maj_2}
    \end{eqnarray}
    Transforming $X$ and $Y$ using the function $g$, and using the strict monotonicity of $g$, we have
    \begin{eqnarray}
        P\left(g'(X) \ge  g'(x)\right) &\geq& P\left(g'(Y) \ge g'(x)\right) \label{eq:RV_transform}
    \end{eqnarray}
    Taking $t \triangleq g'(x)$, we have,
    \begin{eqnarray}
        P\left(g'(X) \ge  t\right) &\geq& P\left(g'(Y) \ge  t\right) \label{eq:def_maj_RV_transform_1}
    \end{eqnarray}
    By the same arguments, if there is a $x$ where $P\left(X\ge x\right) > P\left(Y\ge x\right)$, for $t=g'(x)$, $P\left(g'(X) \ge  t\right) > P\left(g'(Y) \ge  t\right)$. Thus, we have $g'(X) \succ g'(Y)$. 
    
%    From the definition of majorization, and equation (\ref{eq:def_maj_RV_transform_1}) we obtain the required result.
 %   \begin{eqnarray}
  %      g'(X) \succ g'(Y)
  %  \end{eqnarray}
\end{proof}

The FSD implies second order stochastic dominance, which indicates that the mean of the dominating random variable is at least as much as the mean of the dominated random variable \cite{hadar1969rules,bawa1975optimal}. This is summarized in the following lemma. 
\begin{lemma}[\cite{hadar1969rules,bawa1975optimal}] \label{expectation_from_majorization}
    If a random variable $X$ has FSD over another random variable $Y$ 
    (or, $X \succ Y$ ), then the expected value of $X$ is at least the expected value of $Y$, or 
    \begin{eqnarray}
        \mathbb{E}\left[X\right] \geq \mathbb{E}\left[Y\right]
    \end{eqnarray}
\end{lemma}
\if 0
\begin{proof}
    Let $X$, and $Y$ be two random variables such that $X \succ Y$, then from the definition of majorization we have,
    \begin{eqnarray}
        P\left(X>x\right) &geq& P\left(Y > x\right)
    \end{eqnarray}
    Integrating both sides with respect to $x$, and using lemma \ref{exp_from_ccdf}, we have,
    \begin{eqnarray}
        \int_{0}^{\infty}P\left(X>x\right)dx &\geq& \int_{0}^{\infty}P\left(Y>x\right)dx\\
        \mathbb{E}\left[X\right] &\geq& \mathbb{E}\left[Y\right]
    \end{eqnarray}
\end{proof}
\fi 

%In the following result, we consider the SORT subroutine and 

In the SORT subroutine, we picked $K$ arms from $K+1$ arms at each time. Let $G(i)$ $\forall i \in {1, 2, \cdots, K+1}$ be the arms selected for group $G$. Let ${\bf a}^G_{-i}$ be an action in group $G$ with $G(i)^{th}$ arm left out. Then, the individual reward vector with the action ${\bf a}^G_{-i}$ is 
	\begin{eqnarray}
	    {\bf d}_{{\bf a}^G_{-i}}(k) = \bigg\{\begin{array}{cr}X_{G_k}, &k < i\\
	                                                      X_{G_{k+1}}, &i \leq k < K+1 \end{array} 
	\end{eqnarray}
	The (random) reward obtained at any time with this action is $r_{{\bf a}^G_{-i}} = f\left({\bf d}_{{\bf a}^G_{-i}}\right)$, with a mean reward of $\mu_{{\bf a}^G_{-i}} = \mathbb{E}\left[f\left({\bf d}_{{\bf a}^G_{-i}}\right)\right]$. The following result shows that the ordering on the $K$ sized super-arms gives an ordering on the individual arm rewards. 

	
%	From the definition of reward of an action, and the arms in group $G$, we get the reward of action ${\bf a}^G_{-i}$, and its expectation as follows
%	\begin{eqnarray}
%	    {\bf d}_{{\bf a}^G_{-i}}(k) &=& \bigg\{\begin{array}{cr}X_{G_k}, &k < i\\
%	                                                      X_{G_{k+1}}, &i \leq k < K+1 \end{array} \\
%	    r_{{\bf a}^G_{-i}} &=& f\left({\bf d}_{{\bf a}^G_{-i}}\right) \\
%	    \mu_{{\bf a}^G_{-i}} = \mathbb{E}\left[f\left({\bf d}_{{\bf a}^G_{-i}}\right)\right]
%	\end{eqnarray}


\begin{lemma} \label{ordering_from_expectation}
    An ordering on $\binom{K+1}{K}$ actions, in group $G$, made using  $K+1$ arms gives an ordering on $K+1$ arms. In other words, if an ordering exists between actions ${\bf a}^G_{-i}$ and ${\bf a}^G_{-j}$, then an ordering exists between arm $G(i)$ and $G(j)$. More precisely, 
     \begin{eqnarray}
        \mu_{{\bf a}^G_{-i}} > \mu_{{\bf a}^G_{-j}}\Rightarrow \mathbb{E}\left[X_{G(j)}\right] > \mathbb{E}\left[X_{G(i)}\right]
    \end{eqnarray}
\end{lemma} 
\begin{proof}
	
 %   We need to prove that, if an ordering exists between actions ${\bf a}^G_{-i}$ and ${\bf a}^G_{-j}$, then an ordering exists between arm $G(i)$ and $G(j)$, or, 
   
    Note we can write the actions using replacement function $h$ to replace reward of $G(j)$ arm by the reward of $G(i)$ arm, and obtain 
    \begin{eqnarray}
        {\bf d}_{{\bf a}^G_{-j}} &=& h\left({\bf d}_{{\bf a}^G_{-i}},j, X_{G(i)}\right)\text{ }\forall\text{ }j \label{eq:replace_by_i}
    \end{eqnarray}
    The expectation of the reward of an action formed using replacement can be written as expected value of the conditional expectation of the replaced reward value of arm $G(i)$. More precisely, 
    \begin{eqnarray}
        \mathbb{E}\left[f\left({\bf d}_{{\bf a}^G_{-j}}\right)\right] &=& \mathbb{E}\left[\mathbb{E}\left[f\left(h\left({\bf d}_{{\bf a}^G_{-i}},j, X_{G(i)}\right)\right) \Big| X_{G(i)}\right]\right] \label{eq:reward_given_X_g_i}
    \end{eqnarray}
    In right hand side of Equation (\ref{eq:reward_given_X_g_i}), the outer expectation is taken over $X_{G(i)}$ while the inner expectation is over ${\bf d_{a^G_{-i}}}$. In addition, we can replace the reward of an arm $G(j)$ in ${\bf d}_{{\bf a}^G_{-i}}$ by itself to obtain 
    \begin{eqnarray}
        {\bf d}_{{\bf a}^G_{-i}} &=& h\left({\bf d}_{{\bf a}^G_{-i}},j, X_{G(j)}\right) \label{eq:replace_by_j}
    \end{eqnarray}
    Similar to \eqref{eq:reward_given_X_g_i}, we can write the expected reward of the action as the expectation of conditional expectation of reward of arm $G(j)$. Thus, we have
    \begin{eqnarray}
        \mathbb{E}\left[f\left({\bf d}_{{\bf a}^G_{-i}}\right)\right] &=& \mathbb{E}\left[\mathbb{E}\left[f\left(h\left({\bf d}_{{\bf a}^G_{-i}},j, X_{G(j)}\right)\right) \Big| X_{G(j)} \right]\right] \label{eq:reward_given_X_g_j}
    \end{eqnarray}
    The ordering between actions ${\bf a}^G_{-i}$ and ${\bf a}^G_{-j}$ is defined as an order between the expected rewards of the respective actions. We assume that ${\bf a}^G_{-i}$ provides a higher expected reward than ${\bf a}^G_{-j}$, hence we have $\mu_{{\bf a}^G_{-i}} > \mu_{{\bf a}^G_{-j}}$. This further implies 
    
%    the following equations (\ref{eq:order_action_reward}) and (\ref{eq:order_arm_reward_function})
    \begin{eqnarray}
 %       \mu_{{\bf a}^G_{-i}} &>& \mu_{{\bf a}^G_{-j}} \label{eq:order_action_reward}\\
        \mathbb{E}\left[f\left({\bf d_{a^G_{-i}}}\right)\right] &>& \mathbb{E}\left[f\left({\bf d_{a^G_{-j}}}\right)\right] \label{eq:order_arm_reward_function}
    \end{eqnarray}
    Replacing right hand side of   (\ref{eq:order_arm_reward_function}) by  (\ref{eq:reward_given_X_g_i}) and left hand side of (\ref{eq:order_arm_reward_function}) by (\ref{eq:reward_given_X_g_j}, we have 
    
    %, we obtain%, equation (\ref{eq:order_reward_given_X_g_i})
    %\begin{eqnarray}
     %   \mathbb{E}\left[f\left({\bf d_{a^G_{-i}}}\right)\right] &>& \mathbb{E}\left[\mathbb{E}\left[f\left(h\left({\bf d_{a^G_{-i}}},j, X_{G(i)}\right)\right) \Big| X_{G(i)}\right]\right] \label{eq:order_reward_given_X_g_i}
%    \end{eqnarray}
  %  Replacing left hand side of the equation (\ref{eq:order_reward_given_X_g_i}) by equation (\ref{eq:reward_given_X_g_j}), we obtain, equation (\ref{eq:exp_reward_double_exp})
    \begin{eqnarray}
        \mathbb{E}\left[\mathbb{E}\left[f\left(h\left({\bf d_{a^G_{-i}}},j, X_{G(j)}\right)\right) \Big| X_{G(j)}\right]\right] &>& \mathbb{E}\left[\mathbb{E}\left[f\left(h\left({\bf d_{a^G_{-i}}},j, X_{G(i)}\right)\right) \Big| X_{G(i)}\right]\right] \label{eq:exp_reward_double_exp}
    \end{eqnarray}
    We define a function $g(x)$ as  the conditional expectation of reward function $f(\cdot)$ with respect to the reward of the $j^{th}$ arm being $x$. More precisely, 
    \begin{eqnarray}
         g(x) \triangleq \mathbb{E}\left[f\left(h\left({\bf d_{a^G_{-i}}},j, X\right)\right) \Big| X = x\right] \label{eq:g_as_cond_exp}
    \end{eqnarray}
    Replacing the conditional expectations in  (\ref{eq:exp_reward_double_exp}), by $g$ as defined in  (\ref{eq:g_as_cond_exp}), we get
    \begin{eqnarray}
        \mathbb{E}_{X_{G(j)}}\left[g\left(X_{G(j)}\right)\right] &>& \mathbb{E}_{X_{G(i)}}\left[g\left(X_{G(i)}\right)\right]\label{eq:order_exp_with_g}
    \end{eqnarray}
    From Assumption \ref{monotone_assumption}, $g(x)$ is a strictly increasing function of $x$, and from Assumption \ref{majorized_arms}, rewards of individual arms have FSD relationships. Using Assumption \ref{monotone_assumption} and Assumption \ref{majorized_arms} along with equation (\ref{eq:order_exp_with_g}), we want to prove that arm $G(j)$ has FSD over arm $G(i)$. Let us assume the converse where arm $G(i)$ has FSD over arm $G(j)$, or $X_{G(i)} \succ X_{G(j)}$. 
%    \begin{eqnarray}
 %       X_{G(i)} &\succ& X_{G(j)} \label{eq:converse_assumption}
 %   \end{eqnarray}
 Due to the strict increasing nature of $g(\cdot)$ and Lemma \ref{ordering_on_increasing_fn}, we have 
%    \begin{eqnarray}
 $       g\left(X_{G(i)}\right) \succ g\left(X_{G(j)}\right)$.  %\label{eq:exp_to_ccdf}
 %   \end{eqnarray}
Using Lemma \ref{expectation_from_majorization}, we further have
    \begin{eqnarray}
        \mathbb{E}\left[g\left(X_{G(i)}\right)\right] &\geq& \mathbb{E}\left[g\left(X_{G(j)}\right)\right] \label{eq:incorrect_exp_order}
    \end{eqnarray}
    This inequality (\ref{eq:incorrect_exp_order}) does not agree with the inequality obtained from the original assumption (\ref{eq:order_exp_with_g}) thus disproving $X_{G(i)} \succ X_{G(j)}$. Since every two arms have FSD relation and $X_{G(i)} \succ X_{G(j)}$ does not hold, we have 
%    and hence the FSD exists the other way, or arm $G(j)$ majorizes arm $G(i)$
    \begin{equation}
        X_{G(j)} \succ X_{G(j)}
    \end{equation}
    Hence, an ordering on the expected rewards of the $K+1$ actions constructed by leaving one arm aside, gives an ordering on the $K+1$ arms of the group.
\end{proof}

The next lemma is the Hoeffding's Inequality, which will be used in the results in this paper. 
\begin{lemma}[Hoeffding's Inequality \cite{krafft1969note}] \label{Hoeffding_lemma}
     Let $\mathbb{X}$ be a bounded random variable between $[a, b]$, and expected value of $\mathbb{X}$ be $\bar{\mathbb{X}}$. Further, let$\mathbb{X}$ is estimated using $n$ time steps to obtain  $\hat{\bar{\mathbb{X}}}$. Then, for any $\epsilon>0$, we have 
    \begin{eqnarray}
        P\left(\big|\bar{\mathbb{X}} - \hat{\bar{\mathbb{X}}} \big| \geq \epsilon  \right) &\leq& 2e^{-\frac{2n\epsilon^2}{\left(b-a\right)^2}}
    \end{eqnarray}
\end{lemma} 

To reduce the notation clutter, we assume that in each group $G$, expected individual rewards of arms are ordered as $X_{G(1)} \succ X_{G(2)} \succ \cdots \succ X_{G(K+1)}$ From Lemma \ref{exp_from_ccdf}, we have $\mathbb{E}\left[X_{G(1)}\right] > \mathbb{E}\left[X_{G(2)}\right] > \cdots > \mathbb{E}\left[X_{G(K+1)}\right]$.


==> latexmk <==
#!/usr/bin/env perl

use warnings;

## Copyright John Collins 1998-2021
##           (username jcc8 at node psu.edu)
##      (and thanks to David Coppit (username david at node coppit.org) 
##           for suggestions) 
## Copyright Evan McLean
##         (modifications up to version 2)
## Copyright 1992 by David J. Musliner and The University of Michigan.
##         (original version)
##
##    This program is free software; you can redistribute it and/or modify
##    it under the terms of the GNU General Public License as published by
##    the Free Software Foundation; either version 2 of the License, or
##    (at your option) any later version.
##
##    This program is distributed in the hope that it will be useful,
##    but WITHOUT ANY WARRANTY; without even the implied warranty of
##    MERCHANTABILITY or FITNESS FOR A PARTICULAR PURPOSE.  See the
##    GNU General Public License for more details.
##
##    You should have received a copy of the GNU General Public License
##    along with this program; if not, write to the Free Software
##    Foundation, Inc., 59 Temple Place, Suite 330, Boston, MA  02111-1307
##
##
##
##   Modification log from 14 Apr 2021 onwards in detail
##
## 23 Sep 2021 John Collins  Option -time: times for all rules reported now
## 18 Sep 2021 John Collins  For biber: parse blg file for config file use
##                           V. 4.75.
## 27 Aug 2021 John Collins  Modified "missing file" message (when parsing
#                              log file). 
## 29 May 2021 John Collins  When emulating aux_dir, put .synctex.gz .synctex
##                             files in out_dir (as done by MiKTeX, and needed
##                             for their use).
##                           Turn emulate aux_dir off by default, to match older
##                             behavior.  (BACKWARDS INCOMPATIBLE with 4.73 and
##                             4.74.)
##                           Add end-of-all-runs warning if emulate aux_dir needed
##                             to be turned on, when it was initially off.
##                           Add .synctex to list of extensions to clear by default.
## 20 May 2021 John Collins  Turn back on default to report rc files read.
##                           Add options -rc-report, -rc-report-, 
##                             -dir_report, -dir_report-.
## 16 May 2021 John Collins  Deal with some variable used only once warnings
##                           Remove by default informational messages on rc
##                           files read, and aux_dir and out_dir setting.
##  5-6 May 2021 John Collins  Correct normalization of aux and out dirs.
##                           Version 4.74
##  3 May 2021 John Collins  Minor corrections.  Submit to CTAN.
## 30 Apr 2021 John Collins  Revert the change of 14-15 Apr, by removing the
##                           of cwd().  That gave sometimes obnoxiously slow
##                           parsing of big log files, because of the slowness
##                           of large number of calls to cwd() caused by calls
##                           to sub normalize_filename. I think I am mistaken
##                           that cwd() could possibly give a different result
##                           than getcwd(), whose cached result is used by
##                           my goodcwd(). That idea was my motivation on 14 Apr.
## 22 Apr 2021 John Collins  Clean up aux and out_dir code.
## 21 Apr 2021 John Collins  Clean up some comments
##                           Add in emulation of -aux-directory.  On by
##                           default.
## 20 Apr 2021 John Collins  Add -dALLOWPSTRANSPARENCY option to ps2pdf and
##                           dvi2pdf. That avoids problems with recent
##                           ghostscript versions when, e.g., pstricks is used.
## 16 Apr 2021 John Collins  Better normalization of aux_dir and out_dir, so
##                that TEXMFOUTPUT, and the source and dest names for bibtex
##                and makeindex allow them to work always when the aux_dir
##                is **not** below cwd, at least under TeX Live. With MiKTeX
##                bibtex works even without special precautions for aux_dir
##                not below cwd.  But makeindex doesn't work in this case,
##                even if TEXMFOUTPUT is set correctly.
## 14-15 Apr 2021 John Collins  In normalize_filename, try both good_cwd() and
##                           cwd() for removing directory component.
##                           That improves clean up.  At least it could.
##                V. 4.73.
##
##
## 1998-2021, John Collins:  Many improvements and fixes.
##   See CHANGE-log.txt for full list, and CHANGES for summaries
##
## Modified by Evan McLean (no longer available for support)
## Original script (RCS version 2.3) called "go" written by David J. Musliner
##
##-----------------------------------------------------------------------

## Explicit exit codes: 
##             10 = bad command line arguments
##             11 = file specified on command line not found
##                  or other file not found
##             12 = failure in some part of making files
##             13 = error in initialization file
##             20 = probable bug
##             or retcode from called program.

$my_name = 'latexmk';
$My_name = 'Latexmk';
$version_num = '4.75';
$version_details = "$My_name, John Collins, 21 September 2021";

use Config;
use File::Basename;
use File::Copy;
use File::Spec;

# If possible, use better glob, which does not use space as item separator.
# It's either File::Glob::bsd_glob or File::Glob::glob
# The first does not exist in old versions of Perl, while the second
# is deprecated in more recent versions and will be removed
$have_bsd_glob = 0;
use File::Glob;
if ( eval{ File::Glob->import('bsd_glob'); 1; } ) {
    # Success in importing bsd_glob
    $have_bsd_glob = 1;
}
elsif ( eval{ File::Glob->import('glob'); 1; } ) {
    warn "$My_name: I could not import File::Glob:bsd_glob, probably because your\n",
         "  Perl is too old.  I have arranged to use the deprecated File::Glob:glob\n",
         "  instead.\n",
         "  WARNING: It may malfunction on clean up operation on filenames containing\n",
         "           spaces.\n";
    $have_bsd_glob = 0;
}
else {
    die "Could not import 'File::Glob:bsd_glob' or 'File::Glob:glob'\n";
}
# How I use the result of loading glob routines:
sub my_glob {
    if ($have_bsd_glob) { return bsd_glob( $_[0] ); }
    else { return glob( $_[0] ); }
}

use File::Path 2.08 qw( make_path );
use FileHandle;
use File::Find;
use List::Util qw( max );
use Cwd;
use Cwd "abs_path"; 
use Cwd "chdir";    # Ensure $ENV{PWD}  tracks cwd.
use Digest::MD5;

#use strict;

# The following variables are assigned once and then used in symbolic 
#     references, so we need to avoid warnings 'name used only once':
use vars qw( $dvi_update_command $ps_update_command $pdf_update_command $out_dir_requested );

# Translation of signal names to numbers and vv:
%signo = ();
@signame = ();
if ( defined $Config{sig_name} ) {
   $i = 0;
   foreach $name (split('\s+', $Config{sig_name})) {
      $signo{$name} = $i;
      $signame[$i] = $name;
      $i++;
   }
}
else {
   warn "Something wrong with the perl configuration: No signals?\n";
}


# Line length in log file that indicates wrapping.  
# This number EXCLUDES line-end characters, and is one-based.
# It is the parameter max_print_line in the TeX program.  (tex.web)
$log_wrap = 79;

#########################################################################
## Default parsing and file-handling settings

## Array of reg-exps for patterns in log-file for file-not-found
## Each item is the string in a regexp, without the enclosing slashes.
## First parenthesized part is the filename.
## Note the need to quote slashes and single right quotes to make them 
## appear in the regexp.
## Add items by push, e.g.,
##     push @file_not_found, '^No data file found `([^\\\']*)\\\'';
## will give match to line starting "No data file found `filename'"
@file_not_found = (
    '^No file\\s*(.*)\\.$',
    '^\\! LaTeX Error: File `([^\\\']*)\\\' not found\\.',
    '^\\! I can\\\'t find file `([^\\\']*)\\\'\\.',
    '.*?:\\d*: LaTeX Error: File `([^\\\']*)\\\' not found\\.',
    '^LaTeX Warning: File `([^\\\']*)\\\' not found',
    '^Package .* [fF]ile `([^\\\']*)\\\' not found',
    '^Package .* No file `([^\\\']*)\\\'',
    'Error: pdflatex \(file ([^\)]*)\): cannot find image file',
    ': File (.*) not found:\s*$',
    '! Unable to load picture or PDF file \\\'([^\\\']+)\\\'.',
);

# Characters that we won't allow in the name of a TeX file.
# Notes: Some are disallowed by TeX itself.
#        '\' results in TeX macro expansion
#        '$' results in possible variable substitution by kpsewhich called from tex.
#        '"' gets special treatment.
#        See subroutine test_fix_texnames and its call for their use.
$illegal_in_texname = "\x00\t\f\n\r\$%\\~\x7F";

# Whether to normalize aux_dir and out_dir where possible.
# This is important when these directories aren't subdirectories of the cwd,
# and TeXLive's makeindex and/or bibtex are used.
$normalize_names = 2;  # Strongest kind.

## Hash mapping file extension (w/o period, e.g., 'eps') to a single regexp,
#  whose matching by a line in a file with that extension indicates that the 
#  line is to be ignored in the calculation of the hash number (md5 checksum)
#  for the file.  Typically used for ignoring datestamps in testing whether 
#  a file has changed.
#  Add items e.g., by
#     $hash_calc_ignore_pattern{'eps'} = '^%%CreationDate: ';
#  This makes the hash calculation for an eps file ignore lines starting with
#  '%%CreationDate: '
#  ?? Note that a file will be considered changed if 
#       (a) its size changes
#    or (b) its hash changes
#  So it is useful to ignore lines in the hash calculation only if they
#  are of a fixed size (as with a date/time stamp).
%hash_calc_ignore_pattern =();

# Specification of templates for extra rules.
# See subroutine rdb_initialize_rules for examples of rule templates, and
# how they get used to construct rules.
# (Documentation obviously needs to be improved!)
%extra_rule_spec = ();


# Hooks for customized extra processing on aux files.  The following
# variable is an array of references to functions.  Each function is
# invoked in turn when a line of an aux file is processed (if none
# of the built-in actions have been done).  On entry to the function,
# the following variables are set:
#    $_ = current line of aux file
#    $rule = name of rule during the invocation of which, the aux file
#            was supposed to have been generated.
@aux_hooks = ();
# Hooks for customized processing on lists of source and missing files.
# The following variable is an array of references to functions.  Each 
# function is invoked in turn after a run of latex (or pdflatex etc) and
# latexmk has analyzed the .log and .fls files for dependency information.
# On entry to each called function, the following variables are set:
#    $rule = name of *latex rule
#    %dependents: maps source files and possible source files to a status.
#                 See begining of sub parse_log for possible values.
@latex_file_hooks = ();

#########################################################################
## Default document processing programs, and related settings,
## These are mostly the same on all systems.
## Most of these variables represents the external command needed to 
## perform a certain action.  Some represent switches.


## Which TeX distribution is being used
## E.g., "MiKTeX 2.9", "TeX Live 2018"
## "" means not determined. Obtain from first line of .log file.
$tex_distribution = '';

&std_tex_cmds;

# Possible code to execute by *latex before inputting source file.
# Not used by default.
$pre_tex_code = '';

## Default switches:
$latex_default_switches = '';
$pdflatex_default_switches = '';
$lualatex_default_switches = '';
    # Note that xelatex is used to give xdv file, not pdf file, hence 
    # we need the -no-pdf option.
$xelatex_default_switches = '-no-pdf';

## Switch(es) to make them silent:
$latex_silent_switch  = '-interaction=batchmode';
$pdflatex_silent_switch  = '-interaction=batchmode';
$lualatex_silent_switch  = '-interaction=batchmode';
$xelatex_silent_switch  = '-interaction=batchmode';

# Whether to emulate -aux-directory, so we can use it on system(s) (TeXLive)
# that don't support it:
$emulate_aux = 0;
# Whether emulate_aux had to be switched on during a run:
$emulate_aux_switched = 0;

%input_extensions = ();
# %input_extensions maps primary_rule_name to pointer to hash of file extensions
#    used for extensionless files specified in the source file by constructs
#    like \input{file}  \includegraphics{file}
set_input_ext( 'latex', 'tex', 'eps' );
set_input_ext( 'pdflatex', 'tex', 'jpg', 'pdf', 'png' );
$input_extensions{lualatex} = $input_extensions{pdflatex};
$input_extensions{xelatex} = $input_extensions{pdflatex};
# Save these values as standards to be used when switching output,
# i.e., when actual primary rule differs from standard.
%standard_input_extensions = %input_extensions;

%allowed_output_ext = ( ".dvi" => 1, ".xdv" => 1, ".pdf" => 1 );
# Extensions of files preserved when clean up is by -c rather than -C:
%small_cleanup_preserved_exts = ();
foreach ( 'dvi', 'dviF', 'ps', 'psF', 'pdf', 'synctex', 'synctex.gz', 'xdv' ) {
    $small_cleanup_preserved_exts{$_} = 1;
}


# Information about options to latex and pdflatex that latexmk will simply
#   pass through to *latex
# Option without arg. maps to itself.
# Option with arg. maps the option part to the full specification
#  e.g., -kpathsea-debug => -kpathsea-debug=NUMBER
%allowed_latex_options = ();
%allowed_latex_options_with_arg = ();
foreach ( 
  #####
  # TeXLive options
    "-draftmode              switch on draft mode (generates no output PDF)",
    "-enc                    enable encTeX extensions such as \\mubyte",
    "-etex                   enable e-TeX extensions",
    "-file-line-error        enable file:line:error style messages",
    "-no-file-line-error     disable file:line:error style messages",
    "-fmt=FMTNAME            use FMTNAME instead of program name or a %& line",
    "-halt-on-error          stop processing at the first error",
    "-interaction=STRING     set interaction mode (STRING=batchmode/nonstopmode/\n".
    "                           scrollmode/errorstopmode)",
    "-ipc                    send DVI output to a socket as well as the usual\n".
    "                           output file",
    "-ipc-start              as -ipc, and also start the server at the other end",
    "-kpathsea-debug=NUMBER  set path searching debugging flags according to\n".
    "                           the bits of NUMBER",
    "-mktex=FMT              enable mktexFMT generation (FMT=tex/tfm/pk)",
    "-no-mktex=FMT           disable mktexFMT generation (FMT=tex/tfm/pk)",
    "-mltex                  enable MLTeX extensions such as \charsubdef",
    "-output-comment=STRING  use STRING for DVI file comment instead of date\n".
    "                           (no effect for PDF)",
    "-parse-first-line       enable parsing of first line of input file",
    "-no-parse-first-line    disable parsing of first line of input file",
    "-progname=STRING        set program (and fmt) name to STRING",
    "-shell-escape           enable \\write18{SHELL COMMAND}",
    "-no-shell-escape        disable \\write18{SHELL COMMAND}",
    "-shell-restricted       enable restricted \\write18",
    "-src-specials           insert source specials into the DVI file",
    "-src-specials=WHERE     insert source specials in certain places of\n".
    "                           the DVI file. WHERE is a comma-separated value\n".
    "                           list: cr display hbox math par parend vbox",
    "-synctex=NUMBER         generate SyncTeX data for previewers if nonzero",
    "-translate-file=TCXNAME use the TCX file TCXNAME",
    "-8bit                   make all characters printable by default",

  #####
  # MikTeX options not in TeXLive
    "-alias=app              pretend to be app",
    "-buf-size=n             maximum number of characters simultaneously present\n".
    "                           in current lines",
    "-c-style-errors         C-style error messages",
    "-disable-installer      disable automatic installation of missing packages",
    "-disable-pipes          disable input (output) from (to) child processes",
    "-disable-write18        disable the \\write18{command} construct",
    "-dont-parse-first-line  disable checking whether the first line of the main\n".
    "                           input file starts with %&",
    "-enable-enctex          enable encTeX extensions such as \\mubyte",
    "-enable-installer       enable automatic installation of missing packages",
    "-enable-mltex           enable MLTeX extensions such as \charsubdef",
    "-enable-pipes           enable input (output) from (to) child processes",
    "-enable-write18         fully enable the \\write18{command} construct",
    "-error-line=n           set the width of context lines on terminal error\n".
    "                           messages",
    "-extra-mem-bot=n        set the extra size (in memory words) for large data\n".
    "                           structures",
    "-extra-mem-top=n        set the extra size (in memory words) for chars,\n".
    "                           tokens, et al",
    "-font-max=n             set the maximum internal font number",
    "-font-mem-size=n        set the size, in TeX memory words, of the font memory",
    "-half-error-line=n      set the width of first lines of contexts in terminal\n".
    "                           error messages",
    "-hash-extra=n           set the extra space for the hash table of control\n".
    "                           sequences",
    "-job-time=file          set the time-stamp of all output files equal to\n".
    "                           file's time-stamp",
    "-main-memory=n          change the total size (in memory words) of the main\n".
    "                           memory array",
    "-max-in-open=n          set the maximum number of input files and error\n".
    "                           insertions that can be going on simultaneously",
    "-max-print-line=n       set the width of longest text lines output",
    "-max-strings=n          set the maximum number of strings",
    "-nest-size=n            set the maximum number of semantic levels\n".
    "                           simultaneously active",
    "-no-c-style-errors      standard error messages",
    "-param-size=n           set the the maximum number of simultaneous macro\n".
    "                           parameters",
    "-pool-size=n            set the maximum number of characters in strings",
    "-record-package-usages=file record all package usages and write them into\n".
    "                           file",
    "-restrict-write18       partially enable the \\write18{command} construct",
    "-save-size=n            set the the amount of space for saving values\n".
    "                           outside of current group",
    "-stack-size=n           set the maximum number of simultaneous input sources",
    "-string-vacancies=n     set the minimum number of characters that should be\n".
    "                           available for the user's control sequences and font\n".
    "                           names",
    "-tcx=name               process the TCX table name",
    "-time-statistics        show processing time statistics",
    "-trace                  enable trace messages",
    "-trace=tracestreams     enable trace messages. The tracestreams argument is\n".
    "                           a comma-separated list of trace stream names",
    "-trie-size=n            set the amount of space for hyphenation patterns",
    "-undump=name            use name as the name of the format to be used,\n".
    "                           instead of the name by which the program was\n".
    "                           called or a %& line.",

  #####
    # Options passed to *latex that have special processing by latexmk,
    #   so they are commented out here.
    #-jobname=STRING         set the job name to STRING
    #-aux-directory=dir    Set the directory dir to which auxiliary files are written
    #-output-directory=DIR   use existing DIR as the directory to write files in
    # "-output-format=FORMAT   use FORMAT for job output; FORMAT is `dvi\" or `pdf\"",
    #-quiet
    #-recorder               enable filename recorder
    #
    # Options with different processing by latexmk than *latex
    #-help
    #-version
    #
    # Options NOT used by latexmk
    #-includedirectory=dir    prefix dir to the search path
    #-initialize              become the INI variant of the compiler
    #-ini                     be pdfinitex, for dumping formats; this is implicitly
    #                          true if the program name is `pdfinitex'
) {
    if ( /^([^\s=]+)=/ ) {
        $allowed_latex_options_with_arg{$1} = $_;
    }
    elsif ( /^([^\s=]+)\s/ ) {
        $allowed_latex_options{$1} = $_;
    }
    else {
        $allowed_latex_options{$_} = $_;
    }
}

# Arrays of options that will be added to latex and pdflatex.
# These need to be stored until after the command line parsing is finished,
#  in case the values of $latex and/or $pdflatex change after an option
#  is added.
@extra_latex_options = ();
@extra_pdflatex_options = ();
@extra_lualatex_options = ();
@extra_xelatex_options = ();


## Command to invoke biber & bibtex
$biber  = 'biber %O %S';
$bibtex  = 'bibtex %O %S';
# Switch(es) to make biber & bibtex silent:
$biber_silent_switch  = '--onlylog';
$bibtex_silent_switch  = '-terse';
$bibtex_use = 1;   # Whether to actually run bibtex to update bbl files.
                   # This variable is also used in deciding whether to
                   #   delete bbl files in clean up operations.
                   # 0:  Never run bibtex.
                   #     Do NOT delete bbl files on clean up.
                   # 1:  Run bibtex only if the bibfiles exists 
                   #     according to kpsewhich, and the bbl files
                   #     appear to be out-of-date.
                   #     Do NOT delete bbl files on clean up.
                   # 1.5:  Run bibtex only if the bibfiles exists 
                   #     according to kpsewhich, and the bbl files
                   #     appear to be out-of-date.
                   #     Only delete bbl files on clean up if bibfiles exist.
                   # 2:  Run bibtex when the bbl files are out-of-date
                   #     Delete bbl files on clean up.
                   #
                   # In any event bibtex is only run if the log file
                   #   indicates that the document uses bbl files.
$bibtex_fudge = 1; #  Whether or not to cd to aux dir when running bibtex.
                   #  If the cd is not done, and bibtex is passed a
                   #  filename with a path component, then it can easily
                   #  happen that (a) bibtex refuses to write bbl and blg
                   #  files to the aux directory, for security reasons,
                   #  and/or (b) bibtex in pre-2019 versions fails to find
                   #  some input file(s).  But in some other cases, the cd
                   #  method fails. 

## Command to invoke makeindex
$makeindex  = 'makeindex %O -o %D %S';
# Switch(es) to make makeinex silent:
$makeindex_silent_switch  = '-q';
$makeindex_fudge = 1; # Whether or not to cd to aux dir when running makeindex.
                      # Set to 1 to avoid security-related prohibition on
                      # makeindex writing to aux_dir when it is not specified
                      # as a subdirectory of cwd.

## Command to convert dvi file to pdf file directly.
#   Use option -dALLOWPSTRANSPARENCY so that it works with documents
#   using pstricks etc:
$dvipdf  = 'dvipdf -dALLOWPSTRANSPARENCY %O %S %D';
# N.B. Standard dvipdf runs dvips and gs with their silent switch, so for
#      standard dvipdf $dvipdf_silent_switch is unneeded, but innocuous. 
#      But dvipdfmx can be used instead, and it has a silent switch (-q).
#      So implementing $dvipdf_silent_switch is useful.
$dvipdf_silent_switch  = '-q';

## Command to convert dvi file to ps file:
$dvips  = 'dvips %O -o %D %S';
## Command to convert dvi file to ps file in landscape format:
$dvips_landscape = 'dvips -tlandscape %O -o %D %S';
# Switch(es) to get dvips to make ps file suitable for conversion to good pdf:
#    (If this is not used, ps file and hence pdf file contains bitmap fonts
#       (type 3), which look horrible under acroread.  An appropriate switch
#       ensures type 1 fonts are generated.  You can put this switch in the 
#       dvips command if you prefer.)
$dvips_pdf_switch = '-P pdf';
# Switch(es) to make dvips silent:
$dvips_silent_switch  = '-q';

## Command to convert ps file to pdf file.
#   Use option -dALLOWPSTRANSPARENCY so that it works with documents
#   using pstricks etc:
$ps2pdf = 'ps2pdf -dALLOWPSTRANSPARENCY %O %S %D';

## Command to convert xdv file to pdf file
$xdvipdfmx  = 'xdvipdfmx -E -o %D %O %S';
$xdvipdfmx_silent_switch  = '-q';


## Command to search for tex-related files
$kpsewhich = 'kpsewhich %S';

## Command to run make:
$make = 'make';

##Printing:
$print_type = 'auto';   # When printing, print the postscript file.
                        # Possible values: 'dvi', 'ps', 'pdf', 'auto', 'none'
                        # 'auto' ==> set print type according to the printable
                        # file(s) being made: priority 'ps', 'pdf', 'dvi'

# Viewers.  These are system dependent, so default to none:
$pdf_previewer = $ps_previewer  = $ps_previewer_landscape  = $dvi_previewer  = $dvi_previewer_landscape = "NONE";

$dvi_update_signal = undef;
$ps_update_signal = undef;
$pdf_update_signal = undef;

$dvi_update_command = undef;
$ps_update_command = undef;
$pdf_update_command = undef;

$allow_subdir_creation = 1;

$new_viewer_always = 0;     # If 1, always open a new viewer in pvc mode.
                            # If 0, only open a new viewer if no previous
                            #     viewer for the same file is detected.

# Commands for use in pvc mode for compiling, success, warnings, and failure;
# they default to empty, i.e., not to use:
$compiling_cmd = $success_cmd = $warning_cmd = $failure_cmd = "";

# Commands for printing are highly system dependent, so default to NONE:
$lpr = 'NONE $lpr variable is not configured to allow printing of ps files';
$lpr_dvi = 'NONE $lpr_dvi variable is not configured to allow printing of dvi files';
$lpr_pdf = 'NONE $lpr_pdf variable is not configured to allow printing of pdf files';


# The $pscmd below holds a **system-dependent** command to list running
# processes.  It is used to find the process ID of the viewer looking at
# the current output file.  The output of the command must include the
# process number and the command line of the processes, since the
# relevant process is identified by the name of file to be viewed.
# Its use is not essential.
$pscmd =  'NONE $pscmd variable is not configured to detect running processes';
$pid_position = -1;     # offset of PID in output of pscmd.  
                        # Negative means I cannot use ps


$quote_filenames = 1;       # Quote filenames in external commands

$del_dir = '';        # Directory into which cleaned up files are to be put.
                      # If $del_dir is '', just delete the files

@rc_system_files = ();

#########################################################################

################################################################
##  Special variables for system-dependent fudges, etc.
$log_file_binary = 0;   # Whether to treat log file as binary
                        # Normally not, since the log file SHOULD be pure text.
                        # But Miktex 2.7 sometimes puts binary characters
                        #    in it.  (Typically in construct \OML ... after
                        #    overfull box with mathmode.)
                        # Sometimes there is ctrl/Z, which is not only non-text, 
                        #    but is end-of-file marker for MS-Win in text mode.  

$MSWin_fudge_break = 1; # Give special treatment to ctrl/C and ctrl/break
                        #    in -pvc mode under MSWin
                        # Under MSWin32 (at least with perl 5.8 and WinXP)
                        #   when latexmk is running another program, and the 
                        #   user gives ctrl/C or ctrl/break, to stop the 
                        #   daughter program, not only does it reach
                        #   the daughter, but also latexmk/perl, so
                        #   latexmk is stopped also.  In -pvc mode,
                        #   this is not normally desired.  So when the
                        #   $MSWin_fudge_break variable is set,
                        #   latexmk arranges to ignore ctrl/C and
                        #   ctrl/break during processing of files;
                        #   only the daughter programs receive them.
                        # This fudge is not applied in other
                        #   situations, since then having latexmk also
                        #   stopping because of the ctrl/C or
                        #   ctrl/break signal is desirable.
                        # The fudge is not needed under UNIX (at least
                        #   with Perl 5.005 on Solaris 8).  Only the
                        #   daughter programs receive the signal.  In
                        #   fact the inverse would be useful: In
                        #   normal processing, as opposed to -pvc, if
                        #   force mode (-f) is set, a ctrl/C is
                        #   received by a daughter program does not
                        #   also stop latexmk.  Under tcsh, we get
                        #   back to a command prompt, while latexmk
                        #   keeps running in the background!

## Substitute backslashes in file and directory names for
##  MSWin command line
$MSWin_back_slash = 1;

## Separator of elements in search_path.  Default is unix value
$search_path_separator = ':'; 


# Directory for temporary files.  Default to current directory.
$tmpdir = ".";


# When the aux_dir is on a network share (or the like), its system
# time may differ from the system time on which latexmk is running.
# This complicates the tests of whether particular files have been
# made in a current run of a program or are left over from a previous
# run.  One test, which is needed under some situations, is that a
# file was made on a previous run when the files modification time is
# less than the system time when the program is started.  (See
# subroutine test_gen_file; this is only needed in a couple of
# situations.)  The comparison between file and system times must be
# corrected if there is an offset between system times on the computer
# running latexmk and the computer hosting the file system containing
# aux_dir.  The offset is measured in subroutine get_filetime_offset
# by writing a temporary file; the test only needs to be done once.
#
# The following variables are used.  Since the system-independent
# values of system and file time are only accurate to a second (or 2
# seconds for FAT file systems), the offset is also accurate only to a
# second or two.  So thresholds are needed below which differences
# are insignificant.
#
# Note that the making or not making of a file is controlled by the
# state of the document being compiled and by latexmk's configuration.
# So a file that is left over from a previous run and not overwritten
# on the current run will have a file time at least many seconds less
# than the current time, corresponding to the time scale for a human
# run-edit-run cycle.
#
$filetime_offset_measured = 0;       # Measurement not yet done.
$filetime_offset = 0;                # Filetime relative to system time.
$filetime_causality_threshold = 5;   # Threshold for detection of left-over file.
                                     # Should be non-negative always, and should
                                     # be bigger than 2 secs if a remote
                                     # filesystem or network share is used.
$filetime_offset_report_threshold = 30; # Threshold beyond which filetime offsets
                                     # are reported; large offsets indicate
                                     # incorrect system time on at least one system.


################################################################


# System-dependent overrides:
# Currently, the cases I have tests for are: MSWin32, cygwin, linux and 
#   darwin, msys, with the main complications being for MSWin32 and cygwin.
# Further special treatment may also be useful for MSYS (for which $^O reports 
#   "msys").  This is another *nix-emulation/system for MSWindows.  At
#   present it is treated as unix-like, but the environment variables
#   are those of Windows.  (The test for USERNAME as well as USER was
#   to make latexmk work under MSYS's perl.)
#
if ( $^O eq "MSWin32" ) {
# Pure MSWindows configuration
    ## Configuration parameters:

    ## Use first existing case for $tmpdir:
    $tmpdir = $ENV{TMPDIR} || $ENV{TEMP} || '.';
    $log_file_binary = 1;   # Protect against ctrl/Z in log file from
                            # Miktex 2.7.

    ## List of possibilities for the system-wide initialization file.  
    ## The first one found (if any) is used.
    @rc_system_files = ( "C:/latexmk/LatexMk", "C:/latexmk/latexmkrc" );

    $search_path_separator = ';';  # Separator of elements in search_path

    # For a pdf-file, "start x.pdf" starts the pdf viewer associated with
    #   pdf files, so no program name is needed:
    $pdf_previewer = 'start %O %S';
    $ps_previewer  = 'start %O %S';
    $ps_previewer_landscape  = $ps_previewer;
    $dvi_previewer  = 'start %O %S';
    $dvi_previewer_landscape = "$dvi_previewer";
    # Viewer update methods: 
    #    0 => auto update: viewer watches file (e.g., gv)
    #    1 => manual update: user must do something: e.g., click on window.
    #         (e.g., ghostview, MSWIN previewers, acroread under UNIX)
    #    2 => send signal.  Number of signal in $dvi_update_signal,
    #                         $ps_update_signal, $pdf_update_signal
    #    3 => viewer can't update, because it locks the file and the file 
    #         cannot be updated.  (acroread under MSWIN)
    #    4 => run a command to force the update.  The commands are 
    #         specified by the variables $dvi_update_command, 
    #         $ps_update_command, $pdf_update_command
    $dvi_update_method = 1;
    $ps_update_method = 1;
    $pdf_update_method = 3; # acroread locks the pdf file
}
elsif ( $^O eq "cygwin" ) {
    # The problem is a mixed MSWin32 and UNIX environment. 
    # Perl decides the OS is cygwin in two situations:
    # 1. When latexmk is run from a cygwin shell under a cygwin
    #    environment.  Perl behaves in a UNIX way.  This is OK, since
    #    the user is presumably expecting UNIXy behavior.  
    # 2. When CYGWIN exectuables are in the path, but latexmk is run
    #    from a native NT shell.  Presumably the user is expecting NT
    #    behavior. But perl behaves more UNIXy.  This causes some
    #    clashes. 
    # The issues to handle are:
    # 1.  Perl sees both MSWin32 and cygwin filenames.  This is 
    #     normally only an advantage.
    # 2.  Perl uses a UNIX shell in the system command
    #     This is a nasty problem: under native NT, there is a
    #     start command that knows about NT file associations, so that
    #     we can do, e.g., (under native NT) system("start file.pdf");
    #     But this won't work when perl has decided the OS is cygwin,
    #     even if it is invoked from a native NT command line.  An
    #     NT command processor must be used to deal with this.
    # 3.  External executables can be native NT (which only know
    #     NT-style file names) or cygwin executables (which normally
    #     know both cygwin UNIX-style file names and NT file names,
    #     but not always; some do not know about drive names, for
    #     example).
    #     Cygwin executables for tex and latex may only know cygwin
    #     filenames. 
    # 4.  The BIBINPUTS environment variables may be
    #     UNIX-style or MSWin-style depending on whether native NT or
    #     cygwin executables are used.  They are therefore parsed
    #     differently.  Here is the clash:
    #        a. If a user is running under an NT shell, is using a
    #           native NT installation of tex (e.g., fptex or miktex),
    #           but has the cygwin executables in the path, then perl
    #           detects the OS as cygwin, but the user needs NT
    #           behavior from latexmk.
    #        b. If a user is running under an UNIX shell in a cygwin
    #           environment, and is using the cygwin installation of
    #           tex, then perl detects the OS as cygwin, and the user
    #           needs UNIX behavior from latexmk.
    #     Latexmk has no way of detecting the difference.  The two
    #     situations may even arise for the same user on the same
    #     computer simply by changing the order of directories in the
    #     path environment variable


    ## Configuration parameters: We'll assume native NT executables.
    ## The user should override if they are not.

    # This may fail: perl converts MSWin temp directory name to cygwin
    # format. Names containing this string cannot be handled by native
    # NT executables.
    $tmpdir = $ENV{TMPDIR} || $ENV{TEMP} || '.';

    # Which rc files did I read?
    @rc_files_read = ();
    ## List of possibilities for the system-wide initialization file.  
    ## The first one found (if any) is used.
    ## We could stay with MSWin files here, since cygwin perl understands them
    ## @rc_system_files = ( 'C:/latexmk/LatexMk', 'C:/latexmk/latexmkrc' );
    ## But they are deprecated in v. 1.7.  So use the UNIX version, prefixed
    ##   with a cygwin equivalent of the MSWin location
    ## In addition, we need to add the same set of possible locations as with
    ## unix, so that the user use a unix-style setup.
    @rc_system_files = ();
    foreach ( 'LatexMk', 'latexmkrc' ) {
       push @rc_system_files,
            ( "/cygdrive/c/latexmk/$_", 
              "/opt/local/share/latexmk/$_", 
              "/usr/local/share/latexmk/$_",
              "/usr/local/lib/latexmk/$_" );
    }
    $search_path_separator = ';';  # Separator of elements in search_path
    # This is tricky.  The search_path_separator depends on the kind
    # of executable: native NT v. cygwin.  
    # So the user will have to override this.

    # We will assume that files can be viewed by native NT programs.
    #  Then we must fix the start command/directive, so that the
    #  NT-native start command of a cmd.exe is used.
    # For a pdf-file, "start x.pdf" starts the pdf viewer associated with
    #   pdf files, so no program name is needed:
    $start_NT = "cmd /c start \"\"";
    $pdf_previewer = "$start_NT %O %S";
    $ps_previewer  = "$start_NT %O %S";
    $ps_previewer_landscape  = $ps_previewer;
    $dvi_previewer  = "$start_NT %O %S";
    $dvi_previewer_landscape = $dvi_previewer;
    # Viewer update methods: 
    #    0 => auto update: viewer watches file (e.g., gv)
    #    1 => manual update: user must do something: e.g., click on window.
    #         (e.g., ghostview, MSWIN previewers, acroread under UNIX)
    #    2 => send signal.  Number of signal in $dvi_update_signal,
    #                         $ps_update_signal, $pdf_update_signal
    #    3 => viewer can't update, because it locks the file and the file 
    #         cannot be updated.  (acroread under MSWIN)
    $dvi_update_method = 1;
    $ps_update_method = 1;
    $pdf_update_method = 3; # acroread locks the pdf file
}
elsif ( $^O eq "msys" ) {
    $search_path_separator = ';';  # Separator of elements in search_path
                                   # I think MS-Win value is OK, since
                                   # msys is running under MS-Win
    $pdf_previewer = q[sh -c 'start %S'];
    $ps_previewer = q[sh -c 'start %S'];
    $dvi_previewer = q[sh -c 'start %S'];
    $ps_previewer_landscape  = $ps_previewer;
    $dvi_previewer_landscape = "$dvi_previewer";
}
else {
    # Assume anything else is UNIX or clone
    # Do special cases (e.g., linux, darwin (i.e., OS-X)) inside this block.

    ## Use first existing case for $tmpdir:
    $tmpdir = $ENV{TMPDIR} || '/tmp';

    ## List of possibilities for the system-wide initialization file.  
    ## The first one found (if any) is used.
    ## Normally on a UNIX it will be in a subdirectory of /opt/local/share or
    ## /usr/local/share, depending on the local conventions.
    ## But /usr/local/lib/latexmk is put in the list for
    ## compatibility with older versions of latexmk.
    @rc_system_files = ();
    foreach ( 'LatexMk', 'latexmkrc' ) {
       push @rc_system_files,
            ( "/opt/local/share/latexmk/$_", 
              "/usr/local/share/latexmk/$_",
              "/usr/local/lib/latexmk/$_" );
    }
    $search_path_separator = ':';  # Separator of elements in search_path

    $dvi_update_signal = $signo{USR1} 
         if ( defined $signo{USR1} ); # Suitable for xdvi
    $ps_update_signal = $signo{HUP} 
         if ( defined $signo{HUP} );  # Suitable for gv
    $pdf_update_signal = $signo{HUP} 
         if ( defined $signo{HUP} );  # Suitable for gv
    ## default document processing programs.
    # Viewer update methods: 
    #    0 => auto update: viewer watches file (e.g., gv)
    #    1 => manual update: user must do something: e.g., click on window.
    #         (e.g., ghostview, MSWIN previewers, acroread under UNIX)
    #    2 => send signal.  Number of signal in $dvi_update_signal,
    #                         $ps_update_signal, $pdf_update_signal
    #    3 => viewer can't update, because it locks the file and the file 
    #         cannot be updated.  (acroread under MSWIN)
    #    4 => Run command to update.  Command in $dvi_update_command, 
    #    $ps_update_command, $pdf_update_command.
    $dvi_previewer  = 'start xdvi %O %S';
    $dvi_previewer_landscape = 'start xdvi -paper usr %O %S';
    if ( defined $dvi_update_signal ) { 
        $dvi_update_method = 2;  # xdvi responds to signal to update
    } else {
        $dvi_update_method = 1;  
    }
#    if ( defined $ps_update_signal ) { 
#        $ps_update_method = 2;  # gv responds to signal to update
#        $ps_previewer  = 'start gv -nowatch';
#        $ps_previewer_landscape  = 'start gv -swap -nowatch';
#    } else {
#        $ps_update_method = 0;  # gv -watch watches the ps file
#        $ps_previewer  = 'start gv -watch';
#        $ps_previewer_landscape  = 'start gv -swap -watch';
#    }
    # Turn off the fancy options for gv.  Regular gv likes -watch etc
    #   GNU gv likes --watch etc.  User must configure
    $ps_update_method = 0;  # gv -watch watches the ps file
    $ps_previewer  = 'start gv %O %S';
    $ps_previewer_landscape  = 'start gv -swap %O %S';
    $pdf_previewer = 'start acroread %O %S';
    $pdf_update_method = 1;  # acroread under unix needs manual update
    $lpr = 'lpr %O %S';         # Assume lpr command prints postscript files correctly
    $lpr_dvi =
        'NONE $lpr_dvi variable is not configured to allow printing of dvi files';
    $lpr_pdf =
        'NONE $lpr_pdf variable is not configured to allow printing of pdf files';
    # The $pscmd below holds a command to list running processes.  It
    # is used to find the process ID of the viewer looking at the
    # current output file.  The output of the command must include the
    # process number and the command line of the processes, since the
    # relevant process is identified by the name of file to be viewed.
    # Uses:
    #   1.  In preview_continuous mode, to save running a previewer
    #       when one is already running on the relevant file.
    #   2.  With xdvi in preview_continuous mode, xdvi must be
    #       signalled to make it read a new dvi file.
    #
    # The following works on Solaris, LINUX, HP-UX, IRIX
    # Use -f to get full listing, including command line arguments.
    # Use -u $ENV{USER} to get all processes started by current user (not just
    #   those associated with current terminal), but none of other users' 
    #   processes. 
    # However, the USER environment variable may not exist.  Windows uses 
    #   USERNAME instead.  (And this propagates to a situation of 
    #   unix-emulation software running under Windows.) 
    if ( exists $ENV{USER} ) {
       $pscmd = "ps -f -u $ENV{USER}"; 
    }
    elsif ( exists $ENV{USERNAME} ) {
       $pscmd = "ps -f -u $ENV{USERNAME}"; 
    }
    else {
       $pscmd = "ps -f"; 
    }
    $pid_position = 1; # offset of PID in output of pscmd; first item is 0.  
    if ( $^O eq "linux" ) {
        # Ps on Redhat (at least v. 7.2) appears to truncate its output
        #    at 80 cols, so that a long command string is truncated.
        # Fix this with the --width option.  This option works under 
        #    other versions of linux even if not necessary (at least 
        #    for SUSE 7.2). 
        # However the option is not available under other UNIX-type 
        #    systems, e.g., Solaris 8.
        # But (19 Aug 2010), the truncation doesn't happen on RHEL4 and 5,
        #    unless the output is written to a terminal.  So the --width 
        #    option is now unnecessary
        # $pscmd = "ps --width 200 -f -u $ENV{USER}"; 
    }
    elsif ( $^O eq "darwin" ) {
        # OS-X on Macintosh
        # open starts command associated with a file.
        # For pdf, this is set by default to OS-X's preview, which is suitable.
        #     Manual update is simply by clicking on window etc, which is OK.
        # For ps, this is set also to preview.  This works, but since it
        #     converts the file to pdf and views the pdf file, it doesn't
        #     see updates, and a refresh cannot be done.  This is far from
        #     optimal.
        # For a full installation of MacTeX, which is probably the most common
        #     on OS-X, an association is created between dvi files and TeXShop.
        #     This also converts the file to pdf, so again while it works, it
        #     does not deal with changed dvi files, as far as I can see.
        $pdf_previewer = 'open %S';
        $pdf_update_method = 1;     # manual
        $dvi_previewer = $dvi_previewer_landscape = 'NONE';
        $ps_previewer = $ps_previewer_landscape = 'NONE';
        # Others
        $lpr_pdf  = 'lpr %O %S';
        $pscmd = "ps -ww -u $ENV{USER}"; 
    }
}

## default parameters
$auto_rc_use = 1;       # Whether to read rc files automatically
$max_repeat = 5;        # Maximum times I repeat latex.  Normally
                        # 3 would be sufficient: 1st run generates aux file,
                        # 2nd run picks up aux file, and maybe toc, lof which 
                        # contain out-of-date information, e.g., wrong page
                        # references in toc, lof and index, and unresolved
                        # references in the middle of lines.  But the 
                        # formatting is more-or-less correct.  On the 3rd
                        # run, the page refs etc in toc, lof, etc are about
                        # correct, but some slight formatting changes may
                        # occur, which mess up page numbers in the toc and lof,
                        # Hence a 4th run is conceivably necessary. 
                        # At least one document class (JHEP.cls) works
                        # in such a way that a 4th run is needed.  
                        # We allow an extra run for safety for a
                        # maximum of 5. Needing further runs is
                        # usually an indication of a problem; further
                        # runs may not resolve the problem, and
                        # instead could cause an infinite loop.
$clean_ext = "";        # space separated extensions of files that are
                        # to be deleted when doing cleanup, beyond
                        # standard set
$clean_full_ext = "";   # space separated extensions of files that are
                        # to be deleted when doing cleanup_full, beyond
                        # standard set and those in $clean_ext
@cus_dep_list = ();     # Custom dependency list
@default_files = ( '*.tex' );   # Array of LaTeX files to process when 
                        # no files are specified on the command line.
                        # Wildcards allowed
                        # Best used for project specific files.
@default_excluded_files = ( );   
                        # Array of LaTeX files to exclude when using
                        # @default_files, i.e., when no files are specified
                        # on the command line.
                        # Wildcards allowed
                        # Best used for project specific files.
$texfile_search = "";   # Specification for extra files to search for
                        # when no files are specified on the command line
                        # and the @default_files variable is empty.
                        # Space separated, and wildcards allowed.
                        # These files are IN ADDITION to *.tex in current 
                        # directory. 
                        # This variable is obsolete, and only in here for
                        # backward compatibility.

$fdb_ext = 'fdb_latexmk'; # Extension for the file for latexmk's
                          # file-database
                          # Make it long to avoid possible collisions.
$fdb_ver = 3;             # Version number for kind of fdb_file.

$jobname = '';          # Jobname: as with current tex, etc indicates
                        # basename of generated files.  Defined so
                        # that --jobname=STRING on latexmk's command
                        # line has same effect as with current tex,
                        # etc, with the exception listed below.  (If
                        # $jobname is non-empty, then the
                        # --jobname=... option is used on tex.)
                        # Extension: $jobname is allowed to contain
                        # placeholder(s) (currently only %A),
                        # which allows construction of jobnames
                        # dependent on name of main TeX file; this is
                        # useful when a jobname is used and latexmk is
                        # invoked on multiple files.
$out_dir = '';          # Directory for output files.  
                        # Cf. --output-directory of current *latex
                        # Blank means default, i.e., cwd.
$aux_dir = '';          # Directory for aux files (log, aux, etc).
                        # Cf. --aux-directory of current *latex in MiKTeX.
                        # Blank means default, i.e., same as $out_dir.
                        # Note that these values get modified when
                        # processing a .tex file.

## default flag settings.
$recorder = 1;          # Whether to use recorder option on latex/pdflatex
$silent = 0;            # Whether fo silence latex's messages (and others)
$warnings_as_errors = 0;# Treat warnings as errors and exit with non-zero exit code
$silence_logfile_warnings = 0; # Do list warnings in log file
$rc_report = 1;         # Whether to report on rc files read
$aux_out_dir_report = 0; # Whether to report on aux_dir & out_dir after
                         # initialization and normalization

$kpsewhich_show = 0;    # Show calls to and results from kpsewhich
$landscape_mode = 0;    # default to portrait mode
$analyze_input_log_always = 1; # Always analyze .log for input files in the
                        #  <...> and (...) constructions.  Otherwise, only
                        # do the analysis when fls file doesn't exist or is
                        # out of date.
                        # Under normal circumstances, the data in the fls file
                        # is reliable, and the test of the log file gets lots
                        # of false positives; usually $analyze_input_log_always
                        # is best set to zero.  But the test of the log file
                        # is needed at least in the following situation:
                        # When a user needs to persuade latexmk that a certain
                        # file is a source file, and latexmk doesn't otherwise
                        # find it.  User code causes line with (...) to be
                        # written to log file.  One important case is for 
                        # lualatex, which doesn't always generate lines in the
                        # .fls file for input lua files.  (The situation with
                        # lualatex is HIGHLY version dependent, e.g., between
                        # 2016 and 2017.)
                        # To keep backward compatibility with older versions
                        # of latexmk, the default is to set
                        # $analyze_input_log_always to 1.

# The following two arrays contain lists of extensions (without
# period) for files that are read in during a *LaTeX run but that
# are generated automatically from the previous run, as opposed to
# being user generated files (directly or indirectly from a custom
# dependency).  These files get two kinds of special treatment:
#     1.  In clean up, where depending on the kind of clean up, some
#         or all of these generated files are deleted.
#         (Note that special treatment is given to aux files.)
#     2.  In analyzing the results of a run of *LaTeX, to
#         determine if another run is needed.  With an error free run,
#         a rerun should be provoked by a change in any source file,
#         whether a user file or a generated file.  But with a run
#         that ends in an error, only a change in a user file during
#         the run (which might correct the error) should provoke a
#         rerun, but a change in a generated file should not.
# These arrays can be user-configured.

@generated_exts = ( 'aux', 'bcf', 'fls', 'idx', 'ind', 'lof', 'lot', 
                    'out', 'toc' );
     # N.B. 'out' is generated by hyperref package

# Which kinds of file do I have requests to make?
# If no requests at all are made, then I will make dvi file
# If particular requests are made then other files may also have to be
# made.  E.g., ps file requires a dvi file
$dvi_mode = 0;          # No dvi file requested
$postscript_mode = 0;           # No postscript file requested
$pdf_mode = 0;          # No pdf file requested to be made by pdflatex
                        # Possible values: 
                        #     0 don't create pdf file
                        #     1 to create pdf file by pdflatex
                        #     2 to create pdf file by ps2pdf
                        #     3 to create pdf file by dvipdf
                        #     4 to create pdf file by lualatex
                        #     5 to create pdf file by xelatex + xdvipdfmx
$view = 'default';      # Default preview is of highest of dvi, ps, pdf
$sleep_time = 2;        # time to sleep b/w checks for file changes in -pvc mode
$banner = 0;            # Non-zero if we have a banner to insert
$banner_scale = 220;    # Original default scale
$banner_intensity = 0.95;  # Darkness of the banner message
$banner_message = 'DRAFT'; # Original default message
$do_cd = 0;     # Do not do cd to directory of source file.
                #   Thus behave like latex.
$dependents_list = 0;   # Whether to display list(s) of dependencies
$dependents_phony = 0;  # Whether list(s) of dependencies includes phony targets
                        # (as with 'gcc -MP').
$deps_file = '-';       # File for dependency list output.  Default stdout.
$rules_list = 0;        # Whether to display list(s) of dependencies
@dir_stack = ();        # Stack of pushed directories, each of form of 
                        # pointer to array  [ cwd, good_cwd ], where
                        # good_cwd differs from cwd by being converted
                        # to native MSWin path when cygwin is used.
$cleanup_mode = 0;      # No cleanup of nonessential LaTex-related files.
                        # $cleanup_mode = 0: no cleanup
                        # $cleanup_mode = 1: full cleanup 
                        # $cleanup_mode = 2: cleanup except for dvi,
                        #                    dviF, pdf, ps, psF & xdv
$cleanup_fdb  = 0;      # No removal of file for latexmk's file-database
$cleanup_only = 0;      # When doing cleanup, do not go on to making files
$cleanup_includes_generated = 0; 
                        # Determines whether cleanup deletes files generated by
                        #    *latex (found from \openout lines in log file).
                        # It's more than that.  BUG
$cleanup_includes_cusdep_generated = 0;
                        # Determines whether cleanup deletes files generated by
                        #    custom dependencies
$diagnostics = 0;
$dvi_filter = '';       # DVI filter command
$ps_filter = '';        # Postscript filter command

$force_mode = 0;        # =1 to force processing past errors
$go_mode = 0;           # =1 to force processing regardless of time-stamps
                        # =2 full clean-up first
$preview_mode = 0;
$preview_continuous_mode  = 0;
$printout_mode = 0;     # Don't print the file

## Control pvc inactivity timeout:
$pvc_timeout = 0;
$pvc_timeout_mins = 30;

$show_time = 0;
@timings = ();
$processing_time1 = processing_time();

$use_make_for_missing_files = 0;   # Whether to use make to try to make missing files.

# Do we make view file in temporary then move to final destination?
#  (To avoid premature updating by viewer).
$always_view_file_via_temporary = 0;      # Set to 1 if  viewed file is always
                                   #    made through a temporary.
$pvc_view_file_via_temporary = 1;  # Set to 1 if only in -pvc mode is viewed 
                                   #    file made through a temporary.

# State variables initialized here:

$updated = 0;           # Flags when something has been remade
                        # Used to allow convenient user message in -pvc mode
$waiting = 0;           # Flags whether we are in loop waiting for an event
                        # Used to avoid unnecessary repeated o/p in wait loop

# The following are used for some results of parsing log file
# Global variables, so results can be reported in main program. 
$reference_changed = 0;
$mult_defined = 0;
$bad_reference = 0;
$bad_character = 0;
$bad_citation = 0;
@primary_warning_summary = ();

# Cache of expensive-to-compute state variables, e.g., cwd in form
# fixed to deal with cygwin issues.
%cache = ();
&cache_good_cwd;

# Set search paths for includes.
# Set them early so that they can be overridden
$BIBINPUTS = $ENV{'BIBINPUTS'};
if (!$BIBINPUTS) { $BIBINPUTS = '.'; }

# Convert search paths to arrays:
# If any of the paths end in '//' then recursively search the
# directory.  After these operations, @BIBINPUTS  should
# have all the directories that need to be searched

@BIBINPUTS = find_dirs1( $BIBINPUTS );


######################################################################
######################################################################
#
#  ???  UPDATE THE FOLLOWING!!
#
# We will need to determine whether source files for runs of various
# programs are out of date.  In a normal situation, this is done by
# asking whether the times of the source files are later than the
# destination files.  But this won't work for us, since a common
# situation is that a file is written on one run of latex, for
# example, and read back in on the next run (e.g., an .aux file).
# Some situations of this kind are standard in latex generally; others
# occur with particular macro packages or with particular
# postprocessors. 
#
# The correct criterion for whether a source is out-of-date is
# therefore NOT that its modification time is later than the
# destination file, but whether the contents of the source file have
# changed since the last successful run.  This also handles the case
# that the user undoes some changes to a source file by replacing the
# source file by reverting to an earlier version, which may well have
# an older time stamp.  Since a direct comparison of old and new files
# would involve storage and access of a large number of backup files,
# we instead use the md5 signature of the files.  (Previous versions
# of latexmk used the backup file method, but restricted to the case
# of .aux and .idx files, sufficient for most, but not all,
# situations.)
#
# We will have a database of (time, size, md5) for the relevant
# files. If the time and size of a file haven't changed, then the file
# is assumed not to have changed; this saves us from having to
# determine its md5 signature, which would involve reading the whole 
# file, which is naturally time-consuming, especially if network file
# access to a server is needed, and many files are involved, when most
# of them don't change.  It is of course possible to change a file
# without changing its size, but then to adjust its timestamp 
# to what it was previously; this requires a certain amount of
# perversity.  We can safely assume that if the user edits a file or
# changes its contents, then the file's timestamp changes.  The
# interesting case is that the timestamp does change, because the file
# has actually been written to, but that the contents do not change;
# it is for this that we use the md5 signature.  However, since
# computing the md5 signature involves reading the whole file, which
# may be large, we should avoid computing it more than necessary. 
#
# So we get the following structure:
#
#     1.  For each relevant run (latex, pdflatex, each instance of a
#         custom dependency) we have a database of the state of the
#         source files that were last used by the run.
#     2.  On an initial startup, the database for a primary tex file
#         is read that was created by a previous run of latex or
#         pdflatex, if this exists.  
#     3.  If the file doesn't exist, then the criterion for
#         out-of-dateness for an initial run is that it goes by file
#         timestamps, as in previous versions of latexmk, with due
#         (dis)regard to those files that are known to be generated by
#         latex and re-read on the next run.
#     4.  Immediately before a run, the database is updated to
#         represent the current conditions of the run's source files.
#     5.  After the run, it is determined whether any of the source
#         files have changed.  This covers both files written by the
#         run, which are therefore in a dependency loop, and files that
#         the user may have updated during the run.  (The last often
#         happens when latex takes a long time, for a big document,
#         and the user makes edits before latex has finished.  This is
#         particularly prevalent when latexmk is used with
#         preview-continuous mode.)
#     6.  In the case of latex or pdflatex, the custom dependencies
#         must also be checked and redone if out-of-date.
#     7.  If any source files have changed, the run is redone,
#         starting at step 1.
#     8.  There is naturally a limit on the number of reruns, to avoid
#         infinite loops from bugs and from pathological or unforeseen
#         conditions. 
#     9.  After the run is done, the run's file database is updated.
#         (By hypothesis, the sizes and md5s are correct, if the run
#         is successful.)
#    10.  To allow reuse of data from previous runs, the file database
#         is written to a file after every complete set of passes
#         through latex or pdflatex.  (Note that there is separate
#         information for latex and pdflatex; the necessary
#         information won't coincide: Out-of-dateness for the files
#         for each program concerns the properties of the files when
#         the other program was run, and the set of source files could
#         be different, e.g., for graphics files.)  
#
# We therefore maintain the following data structures.:
#
#     a.  For each run (latex, pdflatex, each custom dependency) a
#         database is maintained.  This is a hash from filenames to a
#         reference to an array:  [time, size, md5].  The semantics of
#         the database is that it represents the state of the source
#         files used in the run.  During a run it represents the state
#         immediately before the run; after a run, with all reruns, it
#         represents the state of the files used, modified by having
#         the latest timestamps for generated files.
#     b.  There is a global database for all files, which represents
#         the current state.  This saves having to recompute the md5
#         signatures of a changed file used in more than one run
#         (e.g., latex and pdflatex).
#     c.  Each of latex and pdflatex has a list of the relevant custom
#         dependencies. 
#
# In all the following a fdb-hash is a hash of the form:
#                      filename -> [time, size, md5] 
# If a file is found to disappear, its entry is removed from the hash.
# In returns from fdb access routines, a size entry of -1 indicates a
# non-existent file.


# List of known rules.  Rule types: primary, 
#     external (calls program), internal (calls routine), cusdep.

%possible_primaries = ( 'latex'  => 'primary',  'pdflatex'  => 'primary',
                        'lualatex'  => 'primary', 'xelatex'  => 'primary' );

# Hashes, whose keys give names of particular kinds of rule, and targets.
# We use hashes for ease of lookup.
%possible_one_time = ( 'view' => 1, 'print' => 1, 'update_view' => 1,  );
%target_files      = (); # Hash for target files.
                    # The keys are the filenames and the value is 
                    # currently irrelevant.
%target_rules      = (); # Hash for target rules beyond those corresponding to files.
                    # The keys are the rule names and the value is 
                    # currently irrelevant.
# The target **files** can only be set inside the FILE loop.
$current_primary  = 'latex';   # Rule to compile .tex file.
                    # Subject to document-dependent override if .tex document
                    # uses metcommands andobeying them is enabled.
$pdf_method       = '';  # How to make pdf file.  '' if not requested,
                    # else 'ps2pdf', 'dvipdf', 'pdflatex', 'lualatex' or 'xelatex'
                    # Subject to document-dependent override if .tex document
                    #uses \pdfoutput or c.
%requested_filetypes = (); # Hash of requested file types (dvi, dviF, etc)
%one_time = ();     # Hash for requested one-time-only rules, currently
                    # possible values 'print' and 'view'.  

%actives = ();      # Hash of active rules

$allow_switch = 1;  # Allow switch of rule structure to accommodate
                    # changed output file name of primary. Even if
                    # this flag is set on, the switch may be
                    # prohibited by other issues.

%rule_db = ();      # Database of all rules:
                    # Hash: rulename -> [array of rule data]
                    # Rule data:
                    #   0: [ cmd_type, ext_cmd, int_cmd, test_kind, 
                    #       source, dest, base,
                    #       out_of_date, out_of_date_user,
                    #       time_of_last_run, time_of_last_file_check,
                    #       changed
                    #       last_result, last_message,
                    #       default_extra_generated,
                    #      ]
                    # where 
                    #     cmd_type is 'primary', 'external', or 'cusdep'
                    #     ext_cmd is string for associated external command
                    #       with substitutions (%D for destination, %S
                    #       for source, %B for base of current rule,
                    #       %R for base of primary tex file, %T for
                    #       texfile name, %O for options,
                    #       %V=$aux_dir, %W=$out_dir,
                    #       %Y for $aux_dir1, and %Z for $out_dir1
                    #     int_cmd specifies any internal command to be
                    #       used to implement the application of the
                    #       rule.  If this is present, it overrides
                    #       **direct** execution of the external command, and
                    #       it is the responsibility of the perl subroutine
                    #       specified in intcmd to execute the specified
                    #       external command if this is appropriate.
                    #       This variable intcmd is a reference to an array,  
                    #       $$intcmd[0] = internal routine
                    #       $$intcmd[1...] = its arguments (if any)
                    #     test_kind specifies method of determining
                    #       whether a file is out-of-date:
                    #         0 for never
                    #         1 for usual: whether there is a source
                    #              file change 
                    #         2 for dest earlier than source
                    #         3 for method 2 at first run, 1 thereafter
                    #              (used when don't have file data from
                    #              previous run).
                    #     source = name of primary source file, if any
                    #     dest   = name of primary destination file,
                    #              if any
                    #     base   = base name, if any, of files for
                    #              this rule
                    #     out_of_date = 1 if it has been detected that
                    #                     this rule needs to be run
                    #                     (typically because a source
                    #                     file has changed).
                    #                   Other values may be used for special cases.
                    #                   0 otherwise
                    #     out_of_date_user is like out_of_date, except
                    #         that the detection of out-of-dateness
                    #         has been made from a change of a
                    #         putative user file, i.e., one that is
                    #         not a generated file (e.g., aux). This
                    #         kind of out-of-dateness should provoke a
                    #         rerun whether or not there was an error
                    #         during a run of *LaTeX.  Normally,
                    #         if there is an error, one should wait
                    #         for the user to correct the error.  But
                    #         it is possible the error condition is
                    #         already corrected during the run, e.g.,
                    #         by the user changing a source file in
                    #         response to an error message. 
                    #     time_of_last_run = time that this rule was
                    #              last applied.  (In standard units
                    #              from perl, to be directly compared
                    #              with file modification times.)
                    #     time_of_last_file_check = last time that a check
                    #              was made for changes in source files.
                    #     changed flags whether special changes have been made
                    #          that require file-existence status to be ignored
                    #     last_result is 
                    #                 -1 if no run has been made,
                    #                  0 if the last run was successful
                    #                  1 if last run was successful, but
                    #                    failed to create an output file
                    #                  2 if last run failed
                    #                  200 if last run gave a warning that is
                    #                    important enough to be reported with 
                    #                    the error summary.  The warning
                    #                    message is stored in last_message.
                    #     last_message is error message for last run
                    #     default_extra_generated is a reference to an array
                    #       of specifications of extra generated files (beyond
                    #       the main dest file.  Standard place holders are used.
                    #   1: {Hash sourcefile -> [source-file data] }
                    # Source-file data array: 
                    #   0: time
                    #   1: size
                    #   2: md5
                    #   3: name of rule to make this file
                    #   4: whether the file is of the kind made by epstopdf.sty 
                    #      during a primary run.  It will have been read during
                    #      the run, so that even though the file changes during
                    #      a primary run, there is no need to trigger another 
                    #      run because of this.
                    #  Size and md5 correspond to the values at the last run.
                    #  But time may be updated to correspond to the time
                    #  for the file, if the file is otherwise unchanged.
                    #  This saves excessive md5 calculations, which would
                    #  otherwise be done everytime the file is checked, 
                    #  in the following situation:
                    #     When the file has been rewritten after a run
                    #     has started (commonly aux, bbl files etc),
                    #     but the actual file contents haven't
                    #     changed.  Then because the filetime has
                    #     changed, on every file-change check latexmk
                    #     would normally redo the md5 calculation to
                    #     test for actual changes.  Once one such
                    #     check is done, and the contents are
                    #     unchanged, later checks are superfluous, and
                    #     can be avoided by changing the file's time
                    #     in the source-file list.
                    #   2: {Hash generated_file -> 1 }
                    #      This lists all generated files; the values
                    #          are currently unused, only the keys
                    #   3: {Hash source_rule -> last_pass }
                    #      This lists rules that are to be considered source
                    #      rules for the current rule, separately from the 
                    #      from_rules of the source files. It maps the name
                    #      of each of these rules to the pass number of the
                    #      current rule when it was last run. The current rule
                    #      is out-of-date if the last_pass for a source rule
                    #      is less than the pass number for the rule.
                    #      The purpose of this is when the source file list
                    #      is expected to be inaccurate, because the source
                    #      files are hard to determine.  Typical needs are
                    #      for rules applied to dvi and xdv files, when
                    #      graphics files are involved.  Their names are coded
                    #      inside the dvi/xdv file, but not the contents.
                    #      It would need parsing of the contents of the file
                    #      to determine the actual source files.
                    #      An implication of using a source_rule is that this
                    #      rule passes files to the current rule and that the
                    #      current rule can be considered out-of-date whenever
                    #      the source_rule has been run.  Effectively these 
                    #      files are unconditionallyconsidered changed when
                    #      the source_rule runs.

%fdb_current = ();  # Hash of information for all files used.
                    # It maps filename to a reference to an array
                    #  (time, size, md5_checksum).
@nofile = (0,-1,0); # What we use for initializing a new entry in fdb
                    # or flagging non-existent file.

# The following provide information about the structure of the network of rules
# and files.  They are set by the routine rdb_set_rule_net
%from_rules = ();        # Used to optimize test for whether a file is generated.
                         # This maps files to rules that generate them.  (Files
                         # anywhere in %$PHdest.)
%from_rules_main = ();   # Used to optimize test for whether a file is generated.
                         # This maps files to rules that generate them as the 
                         # MAIN output.  (I.e., file $$Pdest only.)
# Classification of rules, for determining order of application
%current_primaries = ();   # Keys are primary rules (latex, etc) that are currently in use.
@pre_primary = ();         # Array of rules that are thought of as pre-primary
@post_primary = ();        # Array of rules that are thought of as post-primary
@unusual_one_time = ();    # Array of rules that are special cases of one-time rules.
                           # Currently not used.


# User's home directory
$HOME = '';
if (exists $ENV{'HOME'} ) {
    $HOME = $ENV{'HOME'};
}
elsif (exists $ENV{'USERPROFILE'} ) {
    $HOME = $ENV{'USERPROFILE'};
}
# XDG configuration home
$XDG_CONFIG_HOME = '';
if (exists $ENV{'XDG_CONFIG_HOME'} ) {
    $XDG_CONFIG_HOME = $ENV{'XDG_CONFIG_HOME'};
}
elsif ($HOME ne '') {
    if ( -d "$HOME/.config") {
        $XDG_CONFIG_HOME = "$HOME/.config";
    }
}


#==================================================

# Options that are to be obeyed before rc files are read:

foreach $_ ( @ARGV )
{
    if (/^-{1,2}norc$/ ) {
        $auto_rc_use = 0;
    }
}

#==================================================
## Read rc files with this subroutine

sub read_first_rc_file_in_list {
    foreach my $rc_file ( @_ ) {
        #print "===Testing for rc file \"$rc_file\" ...\n";
        if ( -d $rc_file ) {
            warn "$My_name: I have found a DIRECTORY named \"$rc_file\".\n",
                 "   Have you perhaps misunderstood latexmk's documentation?\n",
                 "   This name is normally used for a latexmk configuration (rc) file,\n",
                 "   and in that case it should be a regular text file, not a directory.\n";
        }
        elsif ( -e $rc_file ) {
            process_rc_file( $rc_file );
            return;
        }
    }
}

# Note that each rc file may unset $auto_rc_use to
# prevent lower-level rc files from being read.
# So test on $auto_rc_use in each case.
if ( $auto_rc_use ) {
    # System rc file:
    if (exists $ENV{LATEXMKRCSYS} ) {
        push @rc_system_files, $ENV{LATEXMKRCSYS};
        if ( !-e $ENV{LATEXMKRCSYS} ) {
            warn "$My_name: you've specified a system rc file `$ENV{LATEXMKRCSYS}`\n",
                 "   in environment variable LATEXMKRCSYS, but the file doesn't exist.\n",
                 "   I won't read any system rc file.\n";
        }
        else {
           process_rc_file( $ENV{LATEXMKRCSYS} );
        }
    }
    else {
        read_first_rc_file_in_list( @rc_system_files );
    }
}
if ( $auto_rc_use && ($HOME ne "" ) ) {
    # User rc file:
    @user_rc = ();
    if ( $XDG_CONFIG_HOME ) { 
       push @user_rc, "$XDG_CONFIG_HOME/latexmk/latexmkrc";
    }
    # N.B. $HOME equals "" if latexmk couldn't determine a home directory.
    # In that case, we shouldn't look for an rc file there.
    if ( $HOME ) { 
       push @user_rc, "$HOME/.latexmkrc";
    }
    read_first_rc_file_in_list( @user_rc );
}
if ( $auto_rc_use ) { 
    # Rc file in current directory:
    read_first_rc_file_in_list( ".latexmkrc", "latexmkrc" );
}

## Process command line args.
@command_line_file_list = ();
$bad_options = 0;

while ($_ = $ARGV[0])
{
  # Make -- and - equivalent at beginning of option,
  # but save original for possible use in *latex command line
  $original = $_;
  s/^--/-/;
  shift;
  if ( /^-aux-directory=(.*)$/ || /^-auxdir=(.*)$/ ) {
      $aux_dir = $1;
  }
  elsif (/^-bib(tex|)fudge$/) { $bibtex_fudge = 1; }
  elsif (/^-bib(tex|)fudge-$/) { $bibtex_fudge = 0; }
  elsif (/^-bibtex$/) { $bibtex_use = 2; }
  elsif (/^-bibtex-$/) { $bibtex_use = 0; }
  elsif (/^-nobibtex$/) { $bibtex_use = 0; }
  elsif (/^-bibtex-cond$/) { $bibtex_use = 1; }
  elsif (/^-bibtex-cond1$/) { $bibtex_use = 1.5; }
  elsif (/^-c$/)        { $cleanup_mode = 2; $cleanup_fdb = 1; $cleanup_only = 1; }
  elsif (/^-C$/ || /^-CA$/ ) { $cleanup_mode = 1; $cleanup_fdb = 1; $cleanup_only = 1; }
  elsif (/^-CF$/)    { $cleanup_fdb = 1; }
  elsif (/^-cd$/)    { $do_cd = 1; }
  elsif (/^-cd-$/)   { $do_cd = 0; }
  elsif (/^-commands$/) { &print_commands; exit; }
  elsif (/^-d$/)     { $banner = 1; }
  elsif (/^-dependents$/ || /^-deps$/ || /^-M$/ ) { $dependents_list = 1; }
  elsif (/^-nodependents$/ || /^-dependents-$/ || /^-deps-$/) { $dependents_list = 0; }
  elsif (/^-deps-out=(.*)$/) {
      $deps_file = $1;
      $dependents_list = 1; 
  }
  elsif (/^-diagnostics/) { $diagnostics = 1; }
  elsif (/^-dir-report$/)    { $aux_out_dir_report = 1; }
  elsif (/^-dir-report-$/)   { $aux_out_dir_report = 0; }
  elsif (/^-dvi$/)   { $dvi_mode = 1; }
  elsif (/^-dvi-$/)  { $dvi_mode = 0; }
  elsif (/^-emulate-aux-dir$/) { $emulate_aux = 1; }
  elsif (/^-emulate-aux-dir-$/) { $emulate_aux = 0; }
  elsif (/^-f$/)     { $force_mode = 1; }
  elsif (/^-f-$/)    { $force_mode = 0; }
  elsif (/^-g$/)     { $go_mode = 1; }
  elsif (/^-g-$/)    { $go_mode = 0; }
  elsif (/^-gg$/)    { 
     $go_mode = 2; $cleanup_mode = 1; $cleanup_fdb = 1; $cleanup_only = 0; 
  }
  elsif ( /^-h$/ || /^-help$/ )   { &print_help; exit;}
  elsif (/^-jobname=(.*)$/) {
      $jobname = $1;
  }
  elsif (/^-l$/)     { $landscape_mode = 1; }
  elsif (/^-l-$/)    { $landscape_mode = 0; }
  elsif ( /^-latex$/ )      { 
      $pdf_mode = 0;
      $postscript_mode = 0; 
      $dvi_mode = 1;
  }
  elsif (/^-latex=(.*)$/) {
      $latex = $1;
  }
  elsif (/^-latexoption=(.*)$/) {
      push @extra_latex_options, $1;
      push @extra_pdflatex_options, $1;
      push @extra_lualatex_options, $1;
      push @extra_xelatex_options, $1;
  }
  elsif ( /^-logfilewarninglist$/ || /^-logfilewarnings$/ )
      { $silence_logfile_warnings = 0; }
  elsif ( /^-logfilewarninglist-$/ || /^-logfilewarnings-$/ )
      { $silence_logfile_warnings = 1; }
  elsif ( /^-lualatex$/ || /^-pdflualatex$/ )      { 
      $pdf_mode = 4;
      $dvi_mode = $postscript_mode = 0; 
  }
# See below for -lualatex=...
# See above for -M
  elsif (/^-MF$/) {
     if ( $ARGV[0] eq '' ) {
        &exit_help( "No file name specified after -MF switch");
     }
     $deps_file = $ARGV[0];
     shift; 
  }
  elsif ( /^-MP$/ ) { $dependents_phony = 1; }
  elsif (/^-(make|)indexfudge$/) { $makeindex_fudge = 1; }
  elsif (/^-(make|)indexfudge-$/) { $makeindex_fudge = 0; }
  elsif ( /-MSWinBackSlash$/ ) { $MSWin_back_slash = 1; }
  elsif ( /-MSWinBackSlash-$/ ) { $MSWin_back_slash = 0; }
  elsif (/^-new-viewer$/) {
      $new_viewer_always = 1; 
  }
  elsif (/^-new-viewer-$/) {
      $new_viewer_always = 0;
  }
  elsif (/^-norc$/ ) {
      $auto_rc_use = 0;
      # N.B. This has already been obeyed.
  }
  elsif (/^-nobib(tex|)fudge$/) { $bibtex_fudge = 0; }
  elsif (/^-noemulate-aux-dir$/) { $emulate_aux = 0; }
  elsif (/^-no(make|)indexfudge$/) { $makeindex_fudge = 0; }
  elsif ( /^-output-directory=(.*)$/ ||/^-outdir=(.*)$/ ) {
      $out_dir = $1;
  }
  elsif ( /^-output-format=(.*)$/ ) {
      my $format = $1;
      if ($format eq 'dvi' ) {
          $dvi_mode = 1;
          $pdf_mode = $postscript_mode = 0;
      }
      elsif ($format eq 'pdf' ) {
          $pdf_mode = 1;
          $dvi_mode = $postscript_mode = 0;
      }
      else {
          warn "$My_name: unknown format in option '$_'\n";
          $bad_options++;
      }
  }
  elsif (/^-p$/)     { $printout_mode = 1; 
                       $preview_continuous_mode = 0; # to avoid conflicts
                       $preview_mode = 0;  
                     }
  elsif (/^-p-$/)    { $printout_mode = 0; }
  elsif (/^-pdf$/)   { $pdf_mode = 1; }
  elsif (/^-pdf-$/)  { $pdf_mode = 0; }
  elsif (/^-pdfdvi$/){ $pdf_mode = 3; }
  elsif (/^-pdflua$/){ $pdf_mode = 4; }
  elsif (/^-pdfps$/) { $pdf_mode = 2; }
  elsif (/^-pdfxe$/) { $pdf_mode = 5; }
  elsif (/^-pdflatex$/) {
      $pdflatex = "pdflatex %O %S";
      $pdf_mode = 1;
      $dvi_mode = $postscript_mode = 0; 
  }
  elsif (/^-pdflatex=(.*)$/) {
      $pdflatex = $1;
  }
  elsif ( /^-pdflualatex=(.*)$/ || /^-lualatex=(.*)$/ ) {
      $lualatex = $1;
  }
  elsif ( /^-pdfxelatex=(.*)$/ || /^-xelatex=(.*)$/ ) {
      $xelatex = $1;
  }
  elsif (/^-pretex=(.*)$/) {
      $pre_tex_code = $1;
  }
  elsif (/^-print=(.*)$/) {
      $value = $1;
      if ( $value =~ /^dvi$|^ps$|^pdf$|^auto$/ ) {
          $print_type = $value;
          $printout_mode = 1;
      }
      else {
          &exit_help("$My_name: unknown print type '$value' in option '$_'");
      }
  }
  elsif (/^-ps$/)    { $postscript_mode = 1; }
  elsif (/^-ps-$/)   { $postscript_mode = 0; }
  elsif (/^-pv$/)    { $preview_mode = 1; 
                       $preview_continuous_mode = 0; # to avoid conflicts
                       $printout_mode = 0; 
                     }
  elsif (/^-pv-$/)   { $preview_mode = 0; }
  elsif (/^-pvc$/)   { $preview_continuous_mode = 1;
                       $force_mode = 0;    # So that errors do not cause loops
                       $preview_mode = 0;  # to avoid conflicts
                       $printout_mode = 0; 
                     }
  elsif (/^-pvc-$/)  { $preview_continuous_mode = 0; }
  elsif (/^-pvctimeout$/) { $pvc_timeout = 1; }
  elsif (/^-pvctimeout-$/) { $pvc_timeout = 0; }
  elsif (/^-pvctimeoutmins=(.*)$/) { $pvc_timeout_mins = $1; }
  elsif (/^-rc-report$/)    { $rc_report = 1; }
  elsif (/^-rc-report-$/)   { $rc_report = 0; }
  elsif (/^-recorder$/ ){ $recorder = 1; }
  elsif (/^-recorder-$/ ){ $recorder = 0; }
  elsif (/^-rules$/ ) { $rules_list = 1; }
  elsif (/^-norules$/ || /^-rules-$/ ) { $rules_list = 0; }
  elsif (/^-showextraoptions$/) {
     print "List of extra latex and pdflatex options recognized by $my_name.\n",
           "These are passed as is to *latex.  They may not be recognized by\n",
           "particular versions of *latex.  This list is a combination of those\n",
           "for TeXLive and MikTeX.\n",
           "\n",
           "Note that in addition to the options in this list, there are several\n",
           "options known to the *latex programs that are also recognized by\n",
           "latexmk and trigger special behavior by latexmk.  Since these options\n",
           "appear in the main list given by running 'latexmk --help', they do not\n",
           "appear in the following list\n",
           "NOTE ALSO: Not all of these options are supported by all versions of *latex.\n",
           "\n";
     foreach $option ( sort( keys %allowed_latex_options, keys %allowed_latex_options_with_arg ) ) {
       if (exists $allowed_latex_options{$option} ) { print "   $allowed_latex_options{$option}\n"; }
       if (exists $allowed_latex_options_with_arg{$option} ) { print "   $allowed_latex_options_with_arg{$option}\n"; }
     }
     exit;
  }
  elsif (/^-silent$/ || /^-quiet$/ ){ $silent = 1; }
  elsif (/^-stdtexcmds$/) { &std_tex_cmds; }
  elsif (/^-time$/) { $show_time = 1;}
  elsif (/^-time-$/) { $show_time = 0;}
  elsif (/^-use-make$/)  { $use_make_for_missing_files = 1; }
  elsif (/^-use-make-$/)  { $use_make_for_missing_files = 0; }
  elsif (/^-usepretex$/) { &alt_tex_cmds; }
  elsif (/^-usepretex=(.*)$/) {
      &alt_tex_cmds;
      $pre_tex_code = $1;
  }
  elsif (/^-v$/ || /^-version$/)   { 
      print "\n$version_details. Version $version_num\n";
      exit;
  }
  elsif (/^-verbose$/)  { $silent = 0; }
  elsif (/^-view=default$/) { $view = "default";}
  elsif (/^-view=dvi$/)     { $view = "dvi";}
  elsif (/^-view=none$/)    { $view = "none";}
  elsif (/^-view=ps$/)      { $view = "ps";}
  elsif (/^-view=pdf$/)     { $view = "pdf"; }
  elsif (/^-Werror$/){ $warnings_as_errors = 1; }
  elsif ( /^-xelatex$/ || /^-pdfxelatex$/ )      { 
      $pdf_mode = 5;
      $dvi_mode = $postscript_mode = 0; 
  }
# See above for -xelatex=...
  elsif (/^-e$/) {  
     if ( $#ARGV < 0 ) {
        &exit_help( "No code to execute specified after -e switch"); 
     }
     execute_code_string( $ARGV[0] );
     shift;
  }
  elsif (/^-r$/) {  
     if ( $ARGV[0] eq '' ) {
        &exit_help( "No RC file specified after -r switch"); 
     }
     if ( -e $ARGV[0] ) {
        process_rc_file( $ARGV[0] );
     } 
     else {
        die "$My_name: RC file [$ARGV[0]] does not exist\n"; 
     }
     shift; 
  }
  elsif (/^-bm$/) {
     if ( $ARGV[0] eq '' ) {
        &exit_help( "No message specified after -bm switch");
     }
     $banner = 1; $banner_message = $ARGV[0];
     shift; 
  }
  elsif (/^-bi$/) {
     if ( $ARGV[0] eq '' ) {
        &exit_help( "No intensity specified after -bi switch");
     }
     $banner_intensity = $ARGV[0];
     shift; 
  }
  elsif (/^-bs$/) {
     if ( $ARGV[0] eq '' ) {
        &exit_help( "No scale specified after -bs switch");
     }
     $banner_scale = $ARGV[0];
     shift; 
  }
  elsif (/^-dF$/) {
     if ( $ARGV[0] eq '' ) {
        &exit_help( "No dvi filter specified after -dF switch");
     }
     $dvi_filter = $ARGV[0];
     shift; 
  }
  elsif (/^-pF$/) {
     if ( $ARGV[0] eq '' ) {
        &exit_help( "No ps filter specified after -pF switch");
     }
     $ps_filter = $ARGV[0];
     shift; 
  }
  elsif ( ( exists( $allowed_latex_options{$_} ) )
          || ( /^(-.+)=/ && exists( $allowed_latex_options_with_arg{$1} ) )
        )
  {
      push @extra_latex_options, $original;
      push @extra_pdflatex_options, $original;
      push @extra_lualatex_options, $original;
      push @extra_xelatex_options, $original;
  }
  elsif (/^-/) {
     warn "$My_name: $_ unknown option\n"; 
     $bad_options++;
  }
  else {
     push @command_line_file_list, $_ ; 
  }
}

if ( $diagnostics || $rc_report ) {
    show_array( "Rc files read:", @rc_files_read );
}

if ( $bad_options > 0 ) {
    &exit_help( "Bad options specified" );
}

warn "$My_name: This is $version_details, version: $version_num.\n",
   unless $silent;

if ($out_dir eq '' ){
    # Default to cwd
    $out_dir = '.';
}
if ( $aux_dir eq '' ){
    # Default to out_dir
    #  ?? This is different than MiKTeX
    $aux_dir = $out_dir;
}
# Save original values for use in diagnositics.
# We may change $aux_dir and $out_dir after a detection
#  of results of misconfiguration.
$aux_dir_requested = $aux_dir;
$out_dir_requested = $out_dir;


# The following reports results of diagnostics on location of .log file
#   after the first run of a latex engine, when actually used aux_dir
#   may not be the expected one, due to a configuration error.
# Values: -1 uninitialized (before first run)
#          0 log file not found;
#          1 log file in aux_dir;
#          2 log file **not** in aux_dir but in out_dir;
#          3 log file **not** in aux_dir or out_dir, but in cwd.
$where_log = -1;  

if ($bibtex_use > 1) {
    push @generated_exts, 'bbl';
}

# For backward compatibility, convert $texfile_search to @default_files
# Since $texfile_search is initialized to "", a nonzero value indicates
# that an initialization file has set it.
if ( $texfile_search ne "" ) {
    @default_files = split /\s+/, "*.tex $texfile_search";
}

#Glob the filenames command line if the script was not invoked under a 
#   UNIX-like environment.
#   Cases: (1) MS/MSwin native    Glob
#                      (OS detected as MSWin32)
#          (2) MS/MSwin cygwin    Glob [because we do not know whether
#                  the cmd interpreter is UNIXy (and does glob) or is
#                  native MS-Win (and does not glob).]
#                      (OS detected as cygwin)
#          (3) UNIX               Don't glob (cmd interpreter does it)
#                      (Currently, I assume this is everything else)
if ( ($^O eq "MSWin32") || ($^O eq "cygwin") ) {
    # Preserve ordering of files
    @file_list = glob_list1(@command_line_file_list);
#print "A1:File list:\n";
#for ($i = 0; $i <= $#file_list; $i++ ) {  print "$i: '$file_list[$i]'\n"; }
}
else {
    @file_list = @command_line_file_list;
}
@file_list = uniq1( @file_list );


# Check we haven't selected mutually exclusive modes.
# Note that -c overrides all other options, but doesn't cause
# an error if they are selected.
if (($printout_mode && ( $preview_mode || $preview_continuous_mode ))
    || ( $preview_mode && $preview_continuous_mode ))
{
  # Each of the options -p, -pv, -pvc turns the other off.
  # So the only reason to arrive here is an incorrect inititalization
  #   file, or a bug.
  &exit_help( "Conflicting options (print, preview, preview_continuous) selected");
}

if ( @command_line_file_list ) {   
    # At least one file specified on command line (before possible globbing).
    if ( !@file_list ) {
        &exit_help( "Wildcards in file names didn't match any files");
    }
}
else {
    # No files specified on command line, try and find some
    # Evaluate in order specified.  The user may have some special
    #   for wanting processing in a particular order, especially
    #   if there are no wild cards.
    # Preserve ordering of files
    my @file_list1 = uniq1( glob_list1(@default_files) );
    my @excluded_file_list = uniq1( glob_list1(@default_excluded_files) );
    # Make hash of excluded files, for easy checking:
    my %excl = ();
    foreach my $file (@excluded_file_list) {
        $excl{$file} = '';
    }
    foreach my $file (@file_list1) {
        push( @file_list, $file)  unless ( exists $excl{$file} );
    }    
    if ( !@file_list ) {
        &exit_help( "No file name specified, and I couldn't find any");
    }
}

$num_files = $#file_list + 1;
$num_specified = $#command_line_file_list + 1;

#print "Command line file list:\n";
#for ($i = 0; $i <= $#command_line_file_list; $i++ ) {  print "$i: '$command_line_file_list[$i]'\n"; }
#print "File list:\n";
#for ($i = 0; $i <= $#file_list; $i++ ) {  print "$i: '$file_list[$i]'\n"; }


# If selected a preview-continuous mode, make sure exactly one filename was specified
if ($preview_continuous_mode && ($num_files != 1) ) {
    if ($num_specified > 1) {
        &exit_help( 
          "Need to specify exactly one filename for ".
              "preview-continuous mode\n".
          "    but $num_specified were specified"
        );
    }
    elsif ($num_specified == 1) {
        &exit_help( 
          "Need to specify exactly one filename for ".
              "preview-continuous mode\n".
          "    but wildcarding produced $num_files files"
        );
    }
    else {
        &exit_help( 
          "Need to specify exactly one filename for ".
              "preview-continuous mode.\n".
          "    Since none were specified on the command line, I looked for \n".
          "    files in '@default_files'.\n".
          "    But I found $num_files files, not 1."
        );
    }
}

# If selected jobname, can only apply that to one file:
if ( ($jobname ne '') && ($jobname !~ /%A/) && ($num_files > 1) ) {
    &exit_help( 
          "Need to specify at most one filename if ".
          "jobname specified without a %A, \n".
          "    but $num_files were found (after defaults and wildcarding)."
        );
}
if ( $jobname =~ /%[^A]/ ) {
    &exit_help( 
         "Jobname '$jobname' contains placeholder other than %A."
        );
}

# Normalize the commands, to have place-holders for source, dest etc:
&fix_cmds;

# Add common options
add_option( $latex_default_switches,    \$latex );
add_option( $pdflatex_default_switches, \$pdflatex );
add_option( $lualatex_default_switches, \$lualatex );
add_option( $xelatex_default_switches,  \$xelatex );

foreach (@extra_latex_options)    { add_option( $_, \$latex ); }
foreach (@extra_pdflatex_options) { add_option( $_, \$pdflatex ); }
foreach (@extra_lualatex_options) { add_option( $_, \$lualatex ); }
foreach (@extra_xelatex_options)  { add_option( $_, \$xelatex ); }


# If landscape mode, change dvips processor, and the previewers:
if ( $landscape_mode )
{
  $dvips = $dvips_landscape;
  $dvi_previewer = $dvi_previewer_landscape;
  $ps_previewer = $ps_previewer_landscape;
}

if ( $silent ) { 
    add_option( "$latex_silent_switch", \$latex );
    add_option( "$pdflatex_silent_switch", \$pdflatex );
    add_option( "$lualatex_silent_switch", \$lualatex );
    add_option( "$xelatex_silent_switch", \$xelatex );
    add_option( "$biber_silent_switch", \$biber );
    add_option( "$bibtex_silent_switch", \$bibtex );
    add_option( "$makeindex_silent_switch", \$makeindex );
    add_option( "$dvipdf_silent_switch", \$dvipdf );
    add_option( "$dvips_silent_switch", \$dvips );
    add_option( "$xdvipdfmx_silent_switch", \$xdvipdfmx );
}

if ( $recorder ) {
    add_option( "-recorder", \$latex, \$pdflatex, \$lualatex, \$xelatex );
}

# If the output and/or aux directories are specified, fix the *latex
#   commands to use them.
# N.B. We'll ensure that the directories actually exist only after a
#   possible cd to the document directory, since the directories can be
#   relative to the document.

if ( $jobname ne '' ) {
    # Since $jobname may include placeholder(s), put %R placeholder
    # in option, and let %R be substituted by actual jobname at runtime.
    add_option( "--jobname=%R", \$latex, \$lualatex, \$pdflatex, \$xelatex );
}

# Which kind of file do we preview?
if ( $view eq "default" ) {
    # If default viewer requested, use "highest" of dvi, ps and pdf
    #    that was requested by user.  
    # No explicit request means view dvi.
    $view = "dvi";
    if ( $postscript_mode ) { $view = "ps"; }
    if ( $pdf_mode ) { $view = "pdf"; }
}

# Make sure we make the kind of file we want to view:
if ($view eq 'dvi') { $dvi_mode = 1; }
if ($view eq 'ps') { $postscript_mode = 1; }
if ( ($view eq 'pdf') && ($pdf_mode == 0) ) { 
    $pdf_mode = 1; 
}

# Make sure that we make something if all requests are turned off
if ( ! ( $dvi_mode || $pdf_mode || $postscript_mode || $printout_mode) ) {
    print "No specific requests made, so default to dvi by latex\n";
    $dvi_mode = 1;
}

# Determine requests.
if ( $banner ) { $postscript_mode = 1; }
if ( $dvi_mode ) {
    $current_primary = 'latex';
    $requested_filetypes{'dvi'} = 1;
    if ( length($dvi_filter) != 0 ) { $requested_filetypes{'dviF'} = 1; }
}
if ( $postscript_mode ) {
    $current_primary = 'latex';
    $requested_filetypes{'ps'} = 1;
    if ( length($ps_filter) != 0 )  { $requested_filetypes{'psF'} = 1; }
}

if ($pdf_mode > 5) {
    warn "$My_name: Non-allowed value of \$pdf_mode = $pdf_mode,",
        " replaced by 1.\n";
    $pdf_mode = 1;
}
if ( ($dvi_mode || $postscript_mode) && $pdf_mode ) {
    my %disallowed = ();
    foreach (1,4,5) { $disallowed{$_} = 1; }
    if ($disallowed{$pdf_mode}) {
        warn "$My_name: \$pdf_mode = $pdf_mode is incompatible with dvi and postscript modes\n",
             "  which are required by other requests.\n";
        if ($postscript_mode) {$pdf_mode = 2;}
        else { $pdf_mode = 3; }
        warn "  I replaced it by $pdf_mode.\n";
    }
}
if ( $pdf_mode == 0 ) {
    $pdf_method = '';
}
elsif ( $pdf_mode == 1 ) { 
    $requested_filetypes{'pdf'} = 1;
    $pdf_method = 'pdflatex';
}
elsif ( $pdf_mode == 2 ) { 
    $requested_filetypes{'pdf'} = 1;
    $pdf_method = 'ps2pdf';
}
elsif ( $pdf_mode == 3 ) { 
    $requested_filetypes{'pdf'} = 1;
    $pdf_method = 'dvipdf';
}
elsif ( $pdf_mode == 4 ) { 
    $requested_filetypes{'pdf'} = 1;
    $pdf_method = 'lualatex';
}
elsif ( $pdf_mode == 5 ) { 
    $requested_filetypes{'pdf'} = 1;
    $pdf_method = 'xelatex';
}

if ($print_type eq 'auto') {
    if ( $postscript_mode ) { $print_type = 'ps'; }
    elsif ( $pdf_mode )     { $print_type = 'pdf'; }
    elsif ( $dvi_mode )     { $print_type = 'dvi'; }
    else                    { $print_type = 'none'; }
}
if ( $printout_mode ) {
    $one_time{'print'} = 1;
    if ($print_type eq 'none'){
        warn "$My_name: You have requested printout, but \$print_type is set to 'none'\n";
    }
}
if ( $preview_continuous_mode || $preview_mode ) { $one_time{'view'} = 1; }

$can_switch = $allow_switch;
if ( $dvi_mode || $postscript_mode
     || ( $printout_mode && ($print_type eq 'ps') || ($print_type eq 'dvi') )
     || ( ($preview_mode || $preview_continuous_mode)  &&  ( ($view eq 'ps') || ($view eq 'dvi') ) )
   ) {
    # Automatic switching (e.g., pdf<->dvi o/p) requires pdf files to be
    # the only destinations.  So if ps or dvi files needed, we cannot
    # allow switching.  (There will then be an error condition if a TeX
    # engine fails to produce the correct type of output file.)
    if ($diagnostics) {
        warn "$My_name: Disallowing switch of output file as incompatible\n",
             "    with file requests.\n";
    }
    $can_switch = 0;
}


if ( $pdf_mode == 2 ) {
    # We generate pdf from ps.  Make sure we have the correct kind of ps.
    add_option( "$dvips_pdf_switch", \$dvips );
}

# Restrict variables to allowed values:

if ($filetime_causality_threshold < 0) {
    warn "$My_name: Correcting negative value of \$filetime_causality_threshold to zero.\n";
    $filetime_causality_threshold = 0;
}

# Note sleep has granularity of 1 second.
# Sleep periods 0 < $sleep_time < 1 give zero delay,
#    which is probably not what the user intended.
# Sleep periods less than zero give infinite delay
if ( $sleep_time < 0 ) {
     warn "$My_name: Correcting negative sleep_time to 1 sec.\n";
     $sleep_time = 1;
}
elsif ( ($sleep_time < 1) && ( $sleep_time != 0 ) ) {
     warn "$My_name: Correcting nonzero sleep_time of less than 1 sec to 1 sec.\n";
     $sleep_time = 1;
}
elsif ( $sleep_time == 0 ) {
     warn "$My_name: sleep_time was configured to zero.\n",
    "    Do you really want to do this?  It will give 100% CPU usage.\n";
}

# Make convenient forms for lookup.
# Extensions always have period.

# Convert @generated_exts to a hash for ease of look up and deletion
# Keep extension without period!
%generated_exts_all = ();
foreach (@generated_exts ) {
    $generated_exts_all{$_} = 1;
}

$quell_uptodate_msgs = $silent; 
   # Whether to quell informational messages when files are uptodate
   # Will turn off in -pvc mode

$failure_count = 0;
@failed_primaries = ();

if ($deps_file eq '' ) {
    # Standardize name used for stdout
    $deps_file = '-';
}

# Since deps_file is global (common to all processed files), we must
# delete it here when doing a clean up, and not in the FILE loop, where
# per-file processing (including clean-up) is done
if ( ($cleanup_mode > 0) &&  $dependents_list && ( $deps_file ne '-' ) ) {
    unlink_or_move( $deps_file );
}

# In non-pvc mode, the dependency list is global to all processed TeX files,
#   so we open a single file here, and add items to it after processing
#   each file.  But in -pvc mode, the dependency list should be written
#   after round of processing the single TeX file (as if each round were
#   a separate run of latexmk).
# If we are cleaning up ($cleanup_mode != 0) AND NOT continuing to
#   make files (--gg option and $go_mode == 2), deps_file should not be
#   created.
# I will use definedness of $deps_handle as flag for global deps file having
#   been opened and therefore being available to be written to after
#   compiling a file.
$deps_handle = undef;
if ( $dependents_list
     && ! $preview_continuous_mode
     && ( ($cleanup_mode == 0) || ($go_mode == 2) )
   ) {
    $deps_handle = new FileHandle "> $deps_file";
    if (! $deps_handle ) {
        die "Cannot open '$deps_file' for output of dependency information\n";
    }
}

# Remove leading and trailing space in the following space-separated lists,
#   and collapse multiple spaces to one,
#   to avoid getting incorrect blank items when they are split.
foreach ($clean_ext, $clean_full_ext) { s/^\s+//; s/\s+$//; s/\s+/ /g; }

# Deal with illegal and problematic characters in filename:
test_fix_texnames( @file_list );

$quote = $quote_filenames ? '"' : '';

FILE:
foreach $filename ( @file_list )
{
    # Global variables for making of current file:
    $updated = 0;
    $failure = 0;        # Set nonzero to indicate failure at some point of 
                         # a make.  Use value as exit code if I exit.
    $failure_msg = '';   # Indicate reason for failure

    if ( $do_cd ) {
       ($filename, $path) = fileparse( $filename );
       warn "$My_name: Changing directory to '$path'\n"
           if !$silent;
       pushd( dirname_no_tail( $path ) );
    }
    else {
        $path = '';
    }
    
    local $aux_dir = $aux_dir;
    local $out_dir = $out_dir;
    local $latex = $latex;
    local $lualatex = $lualatex;
    local $pdflatex = $pdflatex;
    local $xelatex = $xelatex;

    &normalize_aux_out_ETC;
    # Set -output-directory and -aux-directory options for *latex
    &set_aux_out_options;

    &set_names;
    
    # For use under error conditions:
    @default_includes = ($texfile_name, $aux_main);
    # N.B. Do **not** apply local %rule_db here.  It might appear appropriate,
    #      but %rule_db is needed in the continue block, which is not in the
    #      scope of a local declaration here.
    &rdb_initialize_rules;
    $view_file = '';
    rdb_one_rule( 'view', sub{ $view_file = $$Psource; } );

    if ( $cleanup_mode > 0 ) {
        my %other_generated = ();
        my @index_bibtex_generated = ();
        my @aux_files = ();
        my @missing_bib_files = ();
        my $bibs_all_exist = 0;
        my %final_output_files = ();
        foreach (keys %small_cleanup_preserved_exts) {
            $final_output_files{"$out_dir1$root_filename.$_"} = 1;
        }
        $have_fdb = 0;
        if ( -e $fdb_name ) {
            print "$My_name: Examining fdb file '$fdb_name' for rules ...\n"
              if $diagnostics;
            $have_fdb = ( 0 == rdb_read( $fdb_name ) );
        }
        if ( $have_fdb ) {
            rdb_for_actives(
                sub {  # Find generated files at rule level
                    my ($base, $path, $ext) = fileparseA( $$Psource );
                    $base = $path.$base;
                    if ( $rule =~ /^makeindex/ ) {
                        push @index_bibtex_generated, $$Psource, $$Pdest, "$base.ilg";
                    }
                    elsif ( $rule =~ /^(bibtex|biber)/ ) {
                        push @index_bibtex_generated, $$Pdest, "$base.blg";
                        push @aux_files, $$Psource;
                        if ( $bibtex_use == 1.5) {
                            foreach ( keys %$PHsource ) {
                                if ( ( /\.bib$/ ) && (! -e $_) ) {
                                    push @missing_bib_files, $_;
                                }
                            }
                        }
                    }
                    elsif ( exists $other_generated{$$Psource} ) {
#                       print "=========== CHECKING: source file of rule '$rule', '$$Psource'\n",
#                              "  is a generated file.\n";
                        ## OLD with apparent bug:
                        #$other_generated{$$Pdest};
                    }
                    foreach my $key (keys %$PHdest) {
                        $other_generated{$key} = 1;
                    }
                },
                sub {  # Find generated files at source file level
                    if ( $file =~ /\.aux$/ ) { push @aux_files, $file; }
                }
            );
            if ($#missing_bib_files == -1) { $bibs_all_exist = 1; }
        }
        elsif ( -e $log_name ) {
            # No fdb file, but log file exists, so do inferior job by parse_log
            print "$My_name: Examining log file '$log_name' for generated files...\n"
              if $diagnostics;
            # Variables set by parse_log. Can I remove them?
            local %generated_log = ();
            local %dependents = ();    # Maps files to status.  Not used here.
            local @bbl_files = ();     # Not used here.
            local %idx_files = ();     # Maps idx_file to (ind_file, base). Not used here.
            local %conversions = ();   # *latex-performed conversions.  Not used here.
                         # Maps output file created and read by *latex
                         #    to source file of conversion.
            local $primary_out = '';   # Actual output file (dvi or pdf). Not used here.
            local $fls_file_analyzed = 0;
            &parse_log;
            %other_generated = %generated_log;
        }
        else {
            print "$My_name: No fdb or log file, so clean up default set of files ...\n"
              if $diagnostics;
        }
        
        if ( ($go_mode == 2) && !$silent ) {
            warn "$My_name: Removing all generated files\n" unless $silent;
        }
        my $keep_bbl = 1;
        if ( ($bibtex_use > 1.6)
             ||
             (  ($bibtex_use == 1.5) && ($bibs_all_exist) )
           ) {
               $keep_bbl = 0;
        }
        if ($keep_bbl) {
            delete $generated_exts_all{'bbl'}; 
        }
        # Convert two arrays to hashes:
        my %index_bibtex_generated = ();
        my %aux_files = ();
        my %aux_files_to_save = ();
        foreach (@index_bibtex_generated) {
            $index_bibtex_generated{$_} = 1
               unless ( /\.bbl$/ && ($keep_bbl) );
            delete( $other_generated{$_} );
        }
        foreach (@aux_files) {
            if (exists $other_generated{$_} ) {
                $aux_files{$_} = 1;
            }
            else {
                $aux_files_to_save{$_} = 1;
            }
        }

        foreach (keys %final_output_files) { delete $other_generated{$_}; }
        
        if ($diagnostics) {
            show_array( "For deletion, the following were determined from fdb file or log file:\n"
                       ." Generated (from makeindex and bibtex):", 
                        keys %index_bibtex_generated );
            show_array( " Aux files:", keys %aux_files );
            show_array( " Other generated files:\n"
                       ." (only deleted if \$cleanup_includes_generated is set): ",
                        keys %other_generated );
            show_array( " Yet other generated files are specified by patterns:\n".
                        " Explicit pattern with %R or root-filename.extension:",
                        keys %generated_exts_all );
            show_array( " Aux files to SAVE and not delete:", keys %aux_files_to_save );
        }

        my @clean_args = ( 'blg', 'ilg', 'log', 'aux.bak', 'idx.bak',
                   split('\s+',$clean_ext), keys %generated_exts_all );
        cleanup1( $aux_dir1, @clean_args );
        if ( $out_dir1 ne $aux_dir1 ) { cleanup1( $out_dir1, @clean_args ); }
        if ( $cleanup_mode == 1 ) {
            my @clean_args = ( keys %small_cleanup_preserved_exts, split('\s+', $clean_full_ext) );
            cleanup1( $aux_dir1, @clean_args );
            if ( $out_dir1 ne $aux_dir1 ) { cleanup1( $out_dir1, @clean_args ); }
        }
        unlink_or_move( 'texput.log', "texput.aux", "missfont.log",
                keys %index_bibtex_generated, 
                        keys %aux_files );
        if ($cleanup_includes_generated) {
            unlink_or_move( keys %other_generated );
        }
        if ( $cleanup_includes_cusdep_generated) {
            &cleanup_cusdep_generated;
        }
    }
    if ($cleanup_fdb) {
       unlink_or_move( $fdb_name );
       # If the fdb file exists, it will have been read, and therefore changed
       #   rule database.  But deleting the fdb file implies we also want
       #   a virgin rule database, so we must reset it:
       &rdb_initialize_rules;
    }
    if ($cleanup_only) { next FILE; }

    if ( $diagnostics ) {
       print "$My_name: Rules after start up for '$texfile_name'\n";
       rdb_show();
    }

    $have_fdb = 0;
    if (! -e $aux_main ) {
        # No aux file => set up trivial aux file 
        #    and corresponding fdb_file.  Arrange them to provoke one run 
        #    as minimum, but no more if actual aux file is trivial.
        #    (Useful on big files without cross references.)
        # If aux file doesn't exist, then any fdb file is surely
        #    wrong.
        # Previously, I had condition for this as being both aux and
        #    fdb files failing to exist.  But it's not obvious what to
        #    do if aux exists and fdb doesn't.  So I won't do anything.
        &set_trivial_aux_fdb;
    }

    if ( -e $fdb_name ) {
        $rdb_errors = rdb_read( $fdb_name );
        $have_fdb = ($rdb_errors == 0);
    }
    if (!$have_fdb) { 
        # We didn't get a valid set of data on files used in
        # previous run.  So use filetime criterion for make
        # instead of change from previous run, until we have
        # done our own make.
        rdb_recurse( [keys %possible_primaries],
                      sub{ if ( $$Ptest_kind == 1 ) { $$Ptest_kind = 3;} }
        );
        if ( -e $log_name ) {
            rdb_for_some( [keys %current_primaries], \&rdb_set_latex_deps );
        }
    }
    # At this point, we assume that the file database was correctly
    # initialized from fdb_latexmk database (corresponding to the state at
    # the end of the previous run of latexmk, if the fdb_latexmk file exists.
    # PERHAPS if fdb_latexmk doesn't exist we ought to assume there was
    # a previous run that completed, if the appropriate output files exist,
    # so a new run of *latex etc isn't needed; then we should set the file
    # data from the on-disk state.
    if ($go_mode) {
        # Force everything to be remade.
        rdb_recurse( [ &rdb_target_array], sub{$$Pout_of_date=1;}  );
    }


    if ( $diagnostics ) {
       print "$My_name: Rules after initialization\n";
       rdb_show();
    }

    #************************************************************

    if ( $preview_continuous_mode ) { 
        &make_preview_continuous; 
        next FILE;
    }


## Handling of failures:
##    Variable $failure is set to indicate a failure, with information
##       put in $failure_msg.  
##    These variables should be set to 0 and '' at any point at which it
##       should be assumed that no failures have occurred.
##    When after a routine is called it is found that $failure is set, then
##       processing should normally be aborted, e.g., by return.
##    Then there is a cascade of returns back to the outermost level whose 
##       responsibility is to handle the error.
##    Exception: An outer level routine may reset $failure and $failure_msg
##       after initial processing, when the error condition may get 
##       ameliorated later.
    #Initialize failure flags now.
    $failure = 0;
    $failure_msg = '';
    if ($compiling_cmd) { Run_subst( $compiling_cmd ); }
    $failure = &rdb_make;
    if ( ( $failure <= 0 ) || $force_mode ) {
      rdb_for_some( [keys %one_time], \&rdb_run1 );
    }
    if ($#primary_warning_summary > -1) {
        # N.B. $mult_defined, $bad_reference, $bad_character, $bad_citation also available here.
        if ($warnings_as_errors) {
            $failure = 1;
            $failure_msg = "Warning(s) from latex (or c.) for '$filename'; treated as error";
        }
    }
    
    if ($failure > 0) {
        if ($failure_cmd) { Run_subst( $failure_cmd ); }
        next FILE;
    } else {
        if ($success_cmd) { Run_subst( $success_cmd ); }
    }
} # end FILE
continue {
    if ($deps_handle) { deps_list($deps_handle); }
    # If requested, print the list of rules.  But don't do this in -pvc
    # mode, since the rules list has already been printed.
    if ($rules_list && ! $preview_continuous_mode) { rdb_list(); }
    # Handle any errors
    $error_message_count = rdb_show_rule_errors();
    if ( ($error_message_count == 0) || ($failure > 0) ) {
        if ( $failure_msg ) {
            #Remove trailing space
            $failure_msg =~ s/\s*$//;
            warn "----------------------\n";
            warn "This message may duplicate earlier message.\n";
            warn "$My_name: Failure in processing file '$filename':\n",
                 "   $failure_msg\n";
            warn "----------------------\n";
            $failure = 1;
        }
    }
    if ( ($failure > 0) || ($error_message_count > 0) ) {
        $failure_count ++;
        push @failed_primaries, $filename;
    }
    &ifcd_popd;
}
close($deps_handle) if ( $deps_handle );

if ($show_time) { show_timing();}

sub show_timing {
    my $processing_time = processing_time() - $processing_time1;
    print @timings, "Accumulated processing time = $processing_time\n"; 
    @timings = (); 
    $processing_time1 = processing_time();
}

# If we get here without going through the continue section:
if ( $do_cd && ($#dir_stack > -1) ) {
   # Just in case we did an abnormal exit from the loop
   warn "$My_name: Potential bug: dir_stack not yet unwound, undoing all directory changes now\n";
   &finish_dir_stack;
}

if ($failure_count > 0) {
    if ( $#file_list > 0 ) {
        # Error occured, but multiple files were processed, so
        #     user may not have seen all the error messages
        warn "\n------------\n";
        show_array( 
           "$My_name: Some operations failed, for the following tex file(s)", 
           @failed_primaries);
    }
    if ( !$force_mode ) {
      warn "$My_name: Use the -f option to force complete processing,\n",
           " unless error was exceeding maximum runs, or warnings treated as errors.\n";
    }
    exit 12;
}

if ( $where_log == 2 ) {
    warn "$My_name: You requested aux_dir '$aux_dir_requested',\n",
         "  but '$out_dir' was used for the .log file etc, and I couldn't\n",
         "  correct the problem, even by setting emulation of aux_dir on.\n",
         "  There is a strong suspicion of a bug in $my_name or a configuration error.\n";
}
if ( $emulate_aux_switched ) {
    warn "$My_name: I had to switch -aux-directory on after it was initially off,\n",
         "  because your *latex program appeared not to support it. You probably\n",
         "  should either use the option -emulate-aux-dir, or in a latexmkrc file\n",
         "  set \$emulate_aux = 1;\n";
}

# end MAIN PROGRAM
#############################################################
#############################################################

sub set_tex_cmds {
    # Usage, e.g., set_tex_cmds( '%O %S' )
    my $args = $_[0];
    foreach my $cmd ('latex', 'lualatex', 'pdflatex', 'xelatex' ) {
        ${$cmd} = "$cmd $args";
    }
    # N.B. See setting of $latex_default_switches, ...,
    # $xelatex_default_switches, etc, for any special options needed.
}

sub std_tex_cmds { set_tex_cmds( '%O %S' ); }

sub alt_tex_cmds { set_tex_cmds( '%O %P' ); }

#========================

sub test_fix_texnames {
    my $illegal_char = 0;
    my $unbalanced_quote = 0;
    my $balanced_quote = 0;
    foreach (@_) {
        if ( ($^O eq "MSWin32") || ($^O eq "msys") ) {
            # On MS-Win, change directory separator '\' to '/', as needed
            # by the TeX engines, for which '\' introduces a macro name.
            # Remember that '/' is a valid directory separator in MS-Win.
            s[\\][/]g;
        }
        if ($do_cd) {
           my ($filename, $path) = fileparse( $_ );
           if ($filename =~ /[\Q$illegal_in_texname\E]/ )  {
              $illegal_char++;
              warn "$My_name: Filename '$filename' contains character not allowed for TeX file.\n";
           }
           if ($filename =~ /^&/) {
              $illegal_char++;
              warn "$My_name: Filename '$filename' contains initial '&', which is\n",
                   "   not allowed for TeX file.\n";
           }
        }
        else {
           if ( /[\Q$illegal_in_texname\E]/ ) {
              $illegal_char++;
              warn "$My_name: Filename '$_' contains character not allowed for TeX file.\n";
           }
           if (/^&/ ) {
              $illegal_char++;
              warn "$My_name: Filename '$_' contains initial '&', which is not allowed\n",
                   "   for TeX file.\n";
           }
        }
        my $count_q = ($_ =~ tr/\"//);
        if ( ($count_q % 2) != 0 ) {
            warn "$My_name: Filename '$_' contains unbalanced quotes, not allowed.\n";
            $unbalanced_quote++;
        }
        elsif ( $count_q > 0 ) {
            warn "$My_name: Removed (balanced quotes) from filename '$_',\n";
            s/\"//g;
            warn "   and obtained '$_'.\n";
            $balanced_quote++;
        }
    }
    if ($illegal_char || $unbalanced_quote) {
        die "$My_name: Stopping because of bad filename(s).\n";
    }
}

#############################################################

sub ensure_path {
    # Usage: ensure_path( $var, values ...)
    # $ENV{$var} is an environment variable (e.g. $ENV{TEXINPUTS}.
    # Ensure the values are in it, prepending them if not, and
    # creating the environment variable if it doesn't already exist.
    my $var = shift;
    my %cmpts = ();
    if ( exists $ENV{$var} ) {
        foreach ( split $search_path_separator, $ENV{$var} ) {
            if ($_ ne '') { $cmpts{$_} = 1; }
        }
    }
    foreach (@_) {
        next if ( ($_ eq '') || (exists $cmpts{$_}) );
        if (exists $ENV{$var}) {
            $ENV{$var} = $_ . $search_path_separator . $ENV{$var};
        }
        else {
            $ENV{$var} = $_ . $search_path_separator;
        }
        if ($diagnostics) {
            print "Set environment variable $var='$ENV{$var}'\n";
        }
    }
} #END ensure_path

#############################################################

sub normalize_aux_out_ETC {
    # 1. Normalize $out_dir and $aux_dir, so that if they have a non-trivial last
    #    component, any trailing '/' is removed.
    # 2. They should be non-empty.
    # 3. Set $out_dir1 and $aux_dir1 to have a directory separator character
    #    '/' added if needed to give forms suitable for direct concatenation with
    #    a filename.  These are needed for substitutions like %Y%R.
    #    Nasty cases of dir_name: "/"  on all systems,  "A:", "A:/" etc on MS-Win
    # 4. Set some TeX-related environment variables.
    # 5. Ensure the aux and out directories exist

    # Ensure the output/auxiliary directories exist, if need be
    my $ret1 = 0;
    my $ret2 = 0;
    eval {
        if ( $out_dir ) {
            $ret1 = make_path_mod( $out_dir,  'output' );
        }
        if ( $aux_dir && ($aux_dir ne $out_dir) ) {
            $ret2 = make_path_mod( $aux_dir,  'auxiliary' );
        }
    };
    if ($ret1 || $ret2 || $@ ) {
        if ($@) { print "Error message:\n  $@"; }
        die "$My_name: Since there was trouble making the output (and aux) dirs, I'll stop\n"
    }

    if ($normalize_names) {
        foreach ( $aux_dir, $out_dir ) { $_ = normalize_filename_abs($_); }
    }
    $aux_dir1 = $aux_dir;
    $out_dir1 = $out_dir;
    foreach ( $aux_dir1, $out_dir1 ) {
        if ($_ eq '.') {$_ = '';}
        if ( ($_ ne '')  && ! m([\\/\:]$) ) {
            # Add a trailing '/' if necessary to give a string that can be
            # correctly concatenated with a filename:
            $_ .= '/';
        }
    }
    if ($aux_dir) {
        # Ensure $aux_dir is in BIBINPUTS and TEXINPUTS search paths.
        # TEXINPUTS is used by dvips for files generated by mpost.
        # For BIBINPUTS, 
        # at least one widely package (revtex4-1) generates a bib file
        # (which is used in revtex4-1 for putting footnotes in the reference
        # list), and bibtex must be run to use it.  But latexmk needs to
        # determine the existence of the bib file by use of kpsewhich, otherwise
        # there is an error.  So cope with this situation (and any analogous
        # cases by adding the aux_dir to the relevant path search environment
        # variables.  BIBINPUTS seems to be the only one currently affected.
        # Convert $aux_dir to absolute path to make the search path invariant
        # under change of directory.
        foreach ( 'BIBINPUTS', 'TEXINPUTS' ) {
            ensure_path( $_, $aux_dir );
        }
        # Set TEXMFOUTPUT  so that when the aux_dir is not a subdirectory
        # of the cwd (or below), bibtex and makeindex can write to it.
        # Otherwise, security precautions in these programs will prevent
        # them from writing there, on TeXLive.  MiKTeX is different: see
        # below.
        # The security issues concern **document-controlled** writing of
        # files, when bibtex or makeindex is invoked directly by a
        # document. In contrast, here $aux_dir is set by latexmk, not by
        # the document. (See the main texmf.cnf file in a TeXLive
        # distribution for some information on security issues.)
        #
        # PROPERTIES:
        # 1. In TeXLive, the use of TEXMFOUTPUT works if
        #    (a) the directory given is an an absolute path,
        #    AND (b) the path contains no .. pieces
        #    AND (c) the directory component of the filename(s) on the command
        #       line for makeindex and bibtex is exactly the same string as
        #       for the directory named in TEXMFOUTPUT.
        # 2. In MiKTeX, bibtex has none of the security restrictions; but
        #    makeindex has, and the use of TEXMFOUTPUT has no effect.
        # So the following is only needed for TeXLive.
        $ENV{TEXMFOUTPUT} = $aux_dir;
    }
    
    if ($diagnostics || $aux_out_dir_report ) {
        warn "$My_name: Cwd: '", good_cwd(), "'\n";
        warn "$My_name: Normalized aux dir and out dir: '$aux_dir', '$out_dir'\n";
        warn "$My_name: and combining forms: '$aux_dir1', '$out_dir1'\n";
    }

}  #END normalize_aux_out_ETC

#############################################################

sub set_aux_out_options {
    # Set -output-directory and -aux-directory options for *latex.  Use
    # placeholders for substitutions so that correct value is put in at
    # runtime.
    # N.B. At this point, $aux_dir and $out_dir should be non-empty, unlike the
    #      case after the reading of latexmkrc files, where empty string means
    #      use default.  Let's be certain, however:
    if ($out_dir eq '') { $out_dir = '.'; $out_dir1 = ''; }
    if ($aux_dir eq '') { $aux_dir = $out_dir; $aux_dir1 = $out_dir1; }
    
    if ($emulate_aux) {
        if ( $aux_dir ne '.' ) {
            # N.B. Set **output** directory to **aux_dir**, rather than
            # out_dir. If aux and out dirs are are different, then we'll move
            # the relevant files (.pdf, .ps, .dvi, .xdv, .fls to the output
            # directory after running *latex.
            add_option( "-output-directory=%V",
                        \$latex, \$pdflatex, \$lualatex, \$xelatex );
        }
    }
    else {
        if ( $out_dir && ($out_dir ne '.') ) {
            add_option( "-output-directory=%W",
                        \$latex, \$pdflatex, \$lualatex, \$xelatex );
        }
        if ( $aux_dir ne $out_dir ) {
            # N.B. If $aux_dir and $out_dir are the same, then the
            # -output-directory option is sufficient, especially because
            # the -aux-directory exists only in MiKTeX, not in TeXLive.
            add_option( "-aux-directory=%V",
                            \$latex, \$pdflatex, \$lualatex, \$xelatex );
        }
    }
} #END set_aux_out_options

#############################################################

sub fix_cmds {
   # If commands do not have placeholders for %S etc, put them in
    foreach ($latex, $lualatex, $pdflatex, $xelatex, $lpr, $lpr_dvi, $lpr_pdf,
             $pdf_previewer, $ps_previewer, $ps_previewer_landscape,
             $dvi_previewer, $dvi_previewer_landscape,
             $kpsewhich
    ) {
        # Source only
        if ( $_ && ! /%/ ) { $_ .= " %O %S"; }
    }
    foreach ($pdf_previewer, $ps_previewer, $ps_previewer_landscape,
             $dvi_previewer, $dvi_previewer_landscape,
    ) {
        # Run previewers detached
        if ( $_ && ! /^(nostart|NONE|internal) / ) {
            $_ = "start $_";
        }
    }
    foreach ($biber, $bibtex) {
        # Base only
        if ( $_ && ! /%/ ) { $_ .= " %O %B"; }
    }
    foreach ($dvipdf, $ps2pdf) {
        # Source and dest without flag for destination
        if ( $_ && ! /%/ ) { $_ .= " %O %S %D"; }
    }
    foreach ($dvips, $makeindex) {
        # Source and dest with -o dest before source
        if ( $_ && ! /%/ ) { $_ .= " %O -o %D %S"; }
    }
    foreach ($dvi_filter, $ps_filter) {
        # Source and dest, but as filters
        if ( $_ && ! /%/ ) { $_ .= " %O <%S >%D"; }
    }
} #END fix_cmds

#############################################################

sub add_option {
    # Call add_option( $opt, \$cmd ... )
    # Add option to one or more commands
    my $option = shift;
    while (@_) {
        if ( ${$_[0]} !~ /%/ ) { &fix_cmds; }
        ${$_[0]} =~ s/%O/$option %O/;
        shift;
    }
} #END add_option

#############################################################

sub rdb_initialize_rules {
    # Initialize rule database.
    #   (The rule database may get overridden/extended after the fdb_latexmk
    #    file is read, and after running commands to adjust to dependencies
    #    determined from document.
    %rule_db = ();
    %target_rules = ();
    %target_files = ();

    local %rule_list = ();
    &rdb_set_rule_templates;

    my %rule_template = %rule_list;
    while ( my ($key, $value) = each %extra_rule_spec ) {
        $rule_template{$key} = $value;
    }
    foreach my $rule ( keys %rule_template ) {
        my ( $cmd_type, $ext_cmd, $int_cmd, $source, $dest, $base, $test_kind, $PA_extra_gen ) = @{$rule_template{$rule}};
        if ( ! $PA_extra_gen ) { $PA_extra_gen = []; }
        my $needs_making = 0;
        # Substitute in the filename variables, since we will use
        # those for determining filenames.  But delay expanding $cmd 
        # until run time, in case of changes.
        foreach ($base, $source, $dest, @$PA_extra_gen ) {
            s/%R/$root_filename/g;
            s/%Y/$aux_dir1/;
            s/%Z/$out_dir1/;
        }
        foreach ($source, $dest ) { 
            s/%B/$base/;
            s/%T/$texfile_name/;
        }
        rdb_create_rule( $rule, $cmd_type, $ext_cmd, $int_cmd, $test_kind, 
                         $source, $dest, $base,
                         $needs_making, undef, undef, 1, $PA_extra_gen );
    } # End rule iteration

    # Ensure we only have one way to make pdf file, and that it is appropriate. Remove other incompatibilities
    if    ($pdf_mode == 1) { rdb_deactivate( 'dvipdf', 'ps2pdf', 'latex', 'lualatex', 'xdvipdfmx', 'xelatex' ); }
    elsif ($pdf_mode == 2) { rdb_deactivate( 'dvipdf', 'pdflatex', 'lualatex', 'xdvipdfmx', 'xelatex' ); }
    elsif ($pdf_mode == 3) { rdb_deactivate( 'pdflatex', 'ps2pdf', 'lualatex', 'xdvipdfmx', 'xelatex' ); }
    elsif ($pdf_mode == 4) { rdb_deactivate( 'pdflatex', 'ps2pdf', 'dvipdf', 'xdvipdfmx', 'xelatex' ); }
    elsif ($pdf_mode == 5) { rdb_deactivate( 'pdflatex', 'ps2pdf', 'dvipdf', 'lualatex' ); }
    else                   { rdb_deactivate( 'dvipdf', 'pdflatex', 'ps2pdf', 'lualatex', 'xdvipdfmx', 'xelatex' ); }

    if ($dvi_mode == 1) {
        rdb_activate( 'latex' );
        $target_files{$dvi_final} = 1;
    }
    if ($postscript_mode == 1) {
        rdb_activate( 'latex' );
        $target_files{$ps_final} = 1;
    }
    if ($pdf_mode) { $target_files{$pdf_final} = 1; }
    &rdb_set_rule_net;
} # END rdb_initialize_rules

#************************************************************

sub rdb_set_rule_templates {
# Set up specifications for standard rules, adjusted to current conditions
# Substitutions: %S = source, %D = dest, %B = this rule's base
#                %T = texfile, %R = root = base for latex.
#                %Y for $aux_dir1, %Z for $out_dir1


    my $print_file = '';
    my $print_cmd = 'NONE';
    if ( $print_type eq 'dvi' ) {
        $print_file = $dvi_final;
        $print_cmd = $lpr_dvi;
    }
    elsif ( $print_type eq 'pdf' ) {
        $print_file = $pdf_final;
        $print_cmd = $lpr_pdf;
    }
    elsif ( $print_type eq 'ps' ) {
        $print_file = $ps_final;
        $print_cmd = $lpr;
    }
    elsif ( $print_type eq 'none' ) {
        $print_cmd = 'NONE echo NO PRINTING CONFIGURED';
    }

    my $view_file = '';
    my $viewer = '';
    my $viewer_update_method = 0;
    my $viewer_update_signal = undef;
    my $viewer_update_command = undef;

    if ( ($view eq 'dvi') || ($view eq 'pdf') || ($view eq 'ps') ) { 
        $view_file = ${$view.'_final'};
        $viewer = ${$view.'_previewer'};
        $viewer_update_method = ${$view.'_update_method'};
        $viewer_update_signal = ${$view.'_update_signal'};
        if (defined ${$view.'_update_command'}) {
           $viewer_update_command = ${$view.'_update_command'};
        }
    }
    # Specification of internal command for viewer update:
    my $PA_update = ['do_update_view', $viewer_update_method, $viewer_update_signal, 0, 1];

# For test_kind: Use file contents for latex and friends, but file time for the others.
# This is because, especially for dvi file, the contents of the file may contain
#    a pointer to a file to be included, not the contents of the file! 
    %rule_list = (
        'latex'     => [ 'primary',  "$latex",     '',            "%T",        $dvi_name,  "%R",   1, [$log_name] ],
        'pdflatex'  => [ 'primary',  "$pdflatex",  '',            "%T",        $pdf_name,  "%R",   1, [$log_name] ],
        'lualatex'  => [ 'primary',  "$lualatex",  '',            "%T",        $pdf_name,  "%R",   1, [$log_name] ],
        'xelatex'   => [ 'primary',  "$xelatex",   '',            "%T",        $xdv_name,  "%R",   1, [$log_name] ],
        'dvipdf'    => [ 'external', "$dvipdf",    'do_viewfile', $dvi_final,  $pdf_name,  "%Z%R", 2 ],
        'xdvipdfmx' => [ 'external', "$xdvipdfmx", 'do_viewfile', $xdv_final,  $pdf_name,  "%Z%R", 2 ],
        'dvips'     => [ 'external', "$dvips",     'do_viewfile', $dvi_final,  $ps_name,   "%Z%R", 2 ],
        'dvifilter' => [ 'external', $dvi_filter,  'do_viewfile', $dvi_name,   $dviF_name, "%Z%R", 2 ],
        'ps2pdf'    => [ 'external', "$ps2pdf",    'do_viewfile', $ps_final,   $pdf_name,  "%Z%R", 2 ],
        'psfilter'  => [ 'external', $ps_filter,   'do_viewfile', $ps_name,    $psF_name,  "%Z%R", 2 ],
        'print'     => [ 'external', "$print_cmd", 'if_source',   $print_file, "",         "",     2 ],
        'update_view' => [ 'external', $viewer_update_command, $PA_update,
                               $view_file,  "",        "",   2 ],
        'view'     => [ 'external', "$viewer",    'if_source',   $view_file,  "",        "",   2 ],
    );
} # END rdb_set_rule_templates 

#************************************************************

sub rdb_set_rule_net {
    # Set network of rules, including links
    &rdb_make_links;
    &rdb_classify_rules;
}

#************************************************************

sub rdb_make_links {
# ?? Problem if there are multiple rules for getting a file.  Notably pdf.
#    Which one to choose?
# ?? Problem: what if a rule is inactive,
#    e.g., bibtex because biber is in use,
#          or xelatex when pdflatex is in use
#          or bibtex when $bibtex_use is 0.
#    What if both latex and pdflatex are being used?
#      That has been allowed.  But .aux file (also
#      .log file) are made by both.

#  Other case: package (like bibtopic) creates bbl or other file when
#  it doesn't exist.  Later a rule is created by latexmk to make that
#  file.  Then the rule's main destination file should have priority
#  over non-main generated files from other rules.
    local %from_rules_old = %from_rules;
    &rdb_cache_generated;
    
    rdb_for_actives( 
        0,
        sub{ 
            if ( exists $from_rules_main{$file} ) {
                $$Pfrom_rule = $from_rules_main{$file};
            }
            elsif ( exists $from_rules{$file} ) {
                $$Pfrom_rule = $from_rules{$file};
            }
            if ( $$Pfrom_rule && (! rdb_rule_exists( $$Pfrom_rule ) ) ) {
                $$Pfrom_rule = '';
            }
        }
        );
    rdb_for_actives( \&rdb_set_source_rules );
#    print "=========In rdb_make_links: rules\n"; &rdb_show;
} # END rdb_make_links

#************************************************************

sub rdb_set_source_rules {
    # This applies to rules whose source file is a dvi or xdv file
    # Uses rule context
    my ($base, $path, $ext) = fileparseA( $$Psource );
    if ( ($ext eq '.dvi') || ($ext eq '.dviF') || ($ext eq '.xdv') ) {
        my $old_rule = $from_rules_old{$$Psource};
        my $new_rule = $from_rules{$$Psource};
        if ( defined $old_rule
             && defined $new_rule
             && ($old_rule eq $new_rule)
             && defined $$PHsource_rules{$new_rule}
            )
        {  # Nothing to do: source rule is correct.
        }
        else {
            if ( defined $old_rule ) { delete $$PHsource_rules{$old_rule}; }
            if ( defined $new_rule ) { $$PHsource_rules{$new_rule} = 0; }
        }
    }
}

#************************************************************

sub rdb_cache_generated {
    # Update %from_rules
    %from_rules = ();
    %from_rules_main = ();
    rdb_for_actives( \&one_from_main_rule_cache );
    rdb_for_actives( \&one_from_rule_cache );
} # END rdb_cache_generated

#------------

sub one_from_main_rule_cache {
    # Rule context assumed.
    # Set from_rules_main items for one rule
    if (! $$Pdest) { return; }
# Error message trigger:    if ( $$Pdest =~ /pdf$/) { $from_rules_main{$$Pdest} = 'pdflatexA'; }
    if ( exists $from_rules_main{$$Pdest} ) {
        my $old_rule = $from_rules_main{$$Pdest};
        if ( $old_rule eq $rule ) {
            # OK
        }
        else {
            warn "$My_name: Possible bug:\n",
                 "  In linking rules I already set from_rules_main{$$Pdest} to '$old_rule'\n",
                 "  But now I want to set it to '$rule'\n";
#            traceback( "================================\nFrom one_from_main_rule_cache" );
        }
    }
    $from_rules_main{$$Pdest} = $rule;
} # END one_from_main_rule_cache

#------------

sub one_from_rule_cache {
    # Rule context assumed.
    # Set from_rules items for one rule
    foreach (  @$PA_extra_gen, keys %$PHdest ) {
        # Error message trigger:  if ( $_ =~ /aux$/) { $from_rules{$_} = 'pdflatexA'; }
        if ( exists $from_rules{$_} ) {
            my $old_rule = $from_rules{$_};
            if ( $old_rule eq $rule ) {
                # OK
            }
            elsif ( exists $from_rules_main{$_} && ( $from_rules_main{$_} ne $rule ) ) {
                warn "$My_name: Possible bug:\n",
                     "  In linking rules, I already set from_rules_main{$_}\n".
                     "  to '$from_rules_main{$_}'\n",
                     "  But now I also have a different rule '$rule' that also made the file.\n";
            }
            elsif ( exists($possible_primaries{$old_rule}) && exists($possible_primaries{$rule}) ) {
                # This could be problematic.  But we'll let it go,
                # because it is a common case for .aux and .log files
                # (etc), and these cases do not appear to mess up
                # anything (by experience).
                # Once we allow an active flag for rules and only
                # examine active rules, the only case of this that
                # will appear (in the absence of other problems) will
                # be where two primary rules are active, notably a
                # latex rule to make dvi and a pdflatex (or other
                # rule) to make pdf.
            }
            else {
                warn "$My_name: Possible bug:\n",
                     "  In linking rules I already set from_rules{$_} to '$old_rule'\n",
                     "  But now I want to set it to '$rule'\n";
#            traceback( "================================\nFrom one_from__rule_cache" );
            }
        }
        $from_rules{$_} = $rule;
    }
} #END from_rule_cache

#************************************************************

sub set_trivial_aux_fdb {
    # 1. Write aux file as would be written if the tex file had no cross
    #    cross references, etc. i.e., a minimal .aux file, as would be
    #    written by latex with a simple document.
    #    That saves a run of latex on such simple documents.
    #    Before about 2020, latex only wrote one line, containing '\relax '
    #    in the aux file.  After that a reference to the last page was
    #    added.  So now I write what is written for a one page document.
    # 2. Write a corresponding fdb file
    # 3. Provoke a run of *latex (actually of all primaries). 

    local *aux_file;
    open( aux_file, '>', $aux_main )
        or die "Cannot write file '$aux_main'\n";
    print aux_file "\\relax \n";
    # The following is added by recent versions of latex for a
    # one page document
    print aux_file "\\gdef \\\@abspage\@last{1}\n";
    close(aux_file);

    foreach my $rule (keys %possible_primaries ) { 
        rdb_ensure_file( $rule, $texfile_name );
        rdb_ensure_file( $rule, $aux_main );
        rdb_one_rule(  $rule,  
                       sub{ $$Pout_of_date = 1; }
                    );
    }
    &rdb_write( $fdb_name );
} #END set_trivial_aux_fdb

#************************************************************
#### Particular actions
#************************************************************
#************************************************************

sub do_cusdep {
    # Unconditional application of custom-dependency
    # except that rule is not applied if the source file source 
    # does not exist, and an error is returned if the dest is not made.
    #
    # Assumes rule context for the custom-dependency, and that my first 
    # argument is the name of the subroutine to apply
    my $func_name = $_[0];
    my $return = 0;
    if ( !-e $$Psource ) {
        # Source does not exist.  Users of this rule will need to turn
        # it off when custom dependencies are reset
        if ( !$silent ) {
            warn "$My_name: In trying to apply custom-dependency rule\n",
            "  to make '$$Pdest' from '$$Psource'\n",
            "  the source file has disappeared since the last run\n";
        }
        # Treat as successful
    }
    elsif ( !$func_name ) {
        warn "$My_name: Possible misconfiguration or bug:\n",
        "  In trying to apply custom-dependency rule\n",
        "  to make '$$Pdest' from '$$Psource'\n",
        "  the function name is blank.\n";
    }
    elsif ( ! defined &$func_name ) {
        warn "$My_name: Misconfiguration or bug,",
        " in trying to apply custom-dependency rule\n",
        "  to make '$$Pdest' from '$$Psource'\n",
        "  function name '$func_name' does not exists.\n";
    }
    else {
        my $cusdep_ret = &$func_name( $$Pbase );
        if ( defined $cusdep_ret && ($cusdep_ret != 0) ) {
            $return = $cusdep_ret;
            if ($return) {
                warn "Rule '$rule', function '$func_name'\n",
                     "   failed with return code = $return\n";
            }
        }
        elsif ( !-e $$Pdest ) {
            # Destination non-existent, but routine failed to give an error
            warn "$My_name: In running custom-dependency rule\n",
            "  to make '$$Pdest' from '$$Psource'\n",
            "  function '$func_name' did not make the destination.\n";
            $return = -1;
        }
    }
    return $return;
}  # END do_cusdep

#************************************************************

sub do_viewfile {
    # Unconditionally make file for viewing, going through temporary file if
    # Assumes rule context

    my $return = 0;
    my ($base, $path, $ext) = fileparseA( $$Pdest );
    if ( &view_file_via_temporary ) {
        if ( $$Pext_cmd =~ /%D/ ) {
            my $tmpfile = tempfile1( "${root_filename}_tmp", $ext );
            warn "$My_name: Making '$$Pdest' via temporary '$tmpfile'...\n";
            $return = &Run_subst( undef, undef, undef, undef, $tmpfile );
            move( $tmpfile, $$Pdest );
        }
        else {
            warn "$My_name is configured to make '$$Pdest' via a temporary file\n",
                 "    but the command template '$$Pext_cmd' does not have a slot\n",
            "    to set the destination file, so I won't use a temporary file\n";
            $return = &Run_subst();
        }
    }
    else {
        $return = &Run_subst();
    }
    return $return;
} #END do_viewfile

#************************************************************

sub do_update_view {
    # Update viewer
    # Assumes rule context
    # Arguments: (method, signal, viewer_process)

    my $return = 0;

    # Although the process is passed as an argument, we'll need to update it.
    # So (FUDGE??) bypass the standard interface for the process.
    # We might as well do this for all the arguments.
    my $viewer_update_method = ${$PAint_cmd}[1];
    my $viewer_update_signal = ${$PAint_cmd}[2];
    my $Pviewer_process             = \${$PAint_cmd}[3];
    my $Pneed_to_get_viewer_process = \${$PAint_cmd}[4];
    
    if ($viewer_update_method == 2) {
        if ($$Pneed_to_get_viewer_process) {
            $$Pviewer_process = &find_process_id( $$Psource );
            if ($$Pviewer_process != 0) {
                $$Pneed_to_get_viewer_process = 0;
            }
        }
        if ($$Pviewer_process == 0) {
            print "$My_name: need to signal viewer for file '$$Psource', but didn't get \n",
                  "   process ID for some reason, e.g., no viewer, bad configuration, bug\n"
                if $diagnostics ;             
        }
        elsif ( defined $viewer_update_signal) {
            print "$My_name: signalling viewer, process ID $$Pviewer_process ",
                  "with signal $viewer_update_signal\n"
                if $diagnostics ;
            kill $viewer_update_signal, $$Pviewer_process;
        }
        else {
            warn "$My_name: viewer is supposed to be sent a signal\n",
                 "  but no signal is defined.  Misconfiguration or bug?\n";
            $return = 1;
        }
    }
    elsif ($viewer_update_method == 4) {
        if (defined $$Pext_cmd) {
            $return = &Run_subst();
        }
        else {
            warn "$My_name: viewer is supposed to be updated by running a command,\n",
                 "  but no command is defined.  Misconfiguration or bug?\n";
        }
    }
    return $return;
} #END do_update_view

#************************************************************

sub if_source {
    # Unconditionally apply rule if source file exists.
    # Assumes rule context
    if ( -e $$Psource ) {
        return &Run_subst();
    }
    else {
        warn "Needed source file '$$Psource' does not exist.\n";
        return -1;
    }
} #END if_source

#************************************************************
#### Subroutines
#************************************************************
#************************************************************

sub find_basename {
    # Finds the basename of the root file
    # Arguments:
    #  1 - Filename to breakdown
    #  2 - Where to place base file
    #  3 - Where to place tex file
    #  Returns non-zero if tex file does not exist

    my $fail = 0;
    local ( $given_name, $base_name, $ext, $path, $tex_name, $source_name );
    $given_name = $_[0];
    $source_name = '';
    $tex_name = $given_name;   # Default name if I don't find the tex file
    ($base_name, $path, $ext) = fileparseB( $given_name );

    # Treatment of extensions (in TeXLive 2019), with omission of path search:
    # Exists: always means exists as a file, i.e., not as a directory.
    #  A. Finding of tex file:
    #   1. If extension is .tex and given_name.tex exists, use it.
    #   2. Else if given_name.tex exists, use it.
    #   3. Else if givne_name exists, use it.
    # B. The base filename is obtained by deleting the path
    #    component and the extension.
    # C. The names of generated files (log, aux) are obtained by appending
    #    .log, .aux, etc to the basename.  Note that these are all in the
    #    CURRENT directory (or the output or aux directory, as appropriate).
    #    The drive/path part of the originally given filename is ignored.

    # Here we'll do:
    # 1. Find the tex file by the above method, if possible.
    # 2. If not, find a custom dependency with a source file that exists to
    #      make the tex file so that after the tex file is made, the above
    #      rules find the tex file.
    # 3. If that also fails, use kpsewhich on given_name to find the tex
    #      file
    # 4. If that also fails, report non-existent tex file.


    if ( ($ext eq '.tex') && (-f $given_name) ) {
       $tex_name = "$given_name";
    }
    elsif ( -f "$given_name.tex" ) {
       $tex_name = "$given_name.tex";
       $base_name .= $ext;
    }
    elsif ( -f $given_name ) {
       $tex_name = $given_name;
    }
    elsif ( ($ext eq '.tex') && find_cus_dep( $given_name, $source_name ) ) {
       $tex_name = $given_name;
    }
    elsif ( find_cus_dep( "$given_name.tex", \$source_name ) ) {
       $tex_name = "$given_name.tex";
       $base_name .= $ext;
    }
    elsif ( ($ext =~ /^\..+/) && find_cus_dep( $given_name, $source_name ) ) {
       $tex_name = $given_name;
    }
    else {
        my @kpse_result = kpsewhich( $given_name );
        if ($#kpse_result < 0) {
            $fail = 1;
        }
        else {
            $tex_name = $kpse_result[0];
            ($base_name) = fileparseB( $tex_name );
        }
    }

    $_[1] = $base_name;
    $_[2] = $tex_name;

    if ($diagnostics) {
       print "Given='$given_name', tex='$tex_name', base='$base_name', ext= $ext, source='$source_name'\n";
    }
    return $fail;

} #END find_basename

#************************************************************

sub make_preview_continuous {
    local @changed = ();
    local %changed_rules = ();
    local @changed_user = ();
    local @disappeared = ();
    local @no_dest = ();       # Non-existent destination files
    local @rules_never_run = ();
    local @rules_to_apply = ();

    local $failure = 0;
    local %rules_applied = ();
    local $updated = 0;

    print "======= Need to update make_preview_continuous for target files\n";
    
    $quell_uptodate_msgs = 1;

    if ( ($view eq 'dvi') || ($view eq 'pdf') || ($view eq 'ps') ) { 
        warn "Viewing $view\n";
    }
    elsif ( $view eq 'none' ) {
        warn "Not using a previewer\n";
        $view_file = '';
    }
    else {
        warn "$My_name:  BUG: Invalid preview method '$view'\n";
        exit 20;
    }

    my $viewer_running = 0;    # No viewer known to be running yet
    # Get information from update_view rule
    local $viewer_update_method = 0;
    # Pointers so we can update the following:
    local $Pviewer_process = undef;    
    local $Pneed_to_get_viewer_process = undef;
    rdb_one_rule( 'update_view', 
                  sub{ $viewer_update_method = $$PAint_cmd[1]; 
                       $Pviewer_process = \$$PAint_cmd[3]; 
                       $Pneed_to_get_viewer_process = \$$PAint_cmd[4]; 
                     } 
                );
    # Note that we don't get the previewer process number from the program
    # that starts it; that might only be a script to get things set up and the 
    # actual previewer could be (and sometimes IS) another process.

    if ( ($view_file ne '') && (-e $view_file) && !$new_viewer_always ) {
        # Is a viewer already running?
        #    (We'll save starting up another viewer.)
        $$Pviewer_process = &find_process_id( $view_file );
        if ( $$Pviewer_process ) {
            warn "$My_name: Previewer is already running\n" 
              if !$silent;
            $viewer_running = 1;
            $$Pneed_to_get_viewer_process = 0;
        }
    }

    # Loop forever, rebuilding .dvi and .ps as necessary.
    # Set $first_time to flag first run (to save unnecessary diagnostics)
    my $last_action_time = time();
    my $timed_out = 0;
CHANGE:
    for (my $first_time = 1; 1; $first_time = 0 ) {

        my %rules_to_watch = array_to_hash( &rdb_accessible );
        
        $updated = 0;
        $failure = 0;
        $failure_msg = '';
        if ( $MSWin_fudge_break && ($^O eq "MSWin32") ) {
            # Fudge under MSWin32 ONLY, to stop perl/latexmk from
            #   catching ctrl/C and ctrl/break, and let it only reach
            #   downstream programs. See comments at first definition of
            #   $MSWin_fudge_break.
            $SIG{BREAK} = $SIG{INT} = 'IGNORE';
        }
        if ($compiling_cmd) {
            Run_subst( $compiling_cmd );
        }
        $failure = &rdb_make;

        if ( $MSWin_fudge_break && ($^O eq "MSWin32") ) {
            $SIG{BREAK} = $SIG{INT} = 'DEFAULT';
        }
        # Start viewer if needed.
        if ( ($failure > 0) && (! $force_mode) ) {
            # No viewer yet
        }
        elsif ( ($view_file ne '') && (-e $view_file) && $updated && $viewer_running ) {
            # A viewer is running.  Explicitly get it to update screen if we have to do it:
            rdb_one_rule( 'update_view', \&rdb_run1 );
        }
        elsif ( ($view_file ne '') && (-e $view_file) && !$viewer_running ) {
            # Start the viewer
            if ( !$silent ) {
                if ($new_viewer_always) {
                    warn "$My_name: starting previewer for '$view_file'\n",
                         "------------\n";
                }
                else {
                    warn "$My_name: I have not found a previewer that ",
                         "is already running. \n",
                         "   So I will start it for '$view_file'\n",
                         "------------\n";
               }
            }
            local $retcode = 0;
            rdb_one_rule( 'view', sub { $retcode = &rdb_run1;} );
            if ( $retcode != 0 ) {
                if ($force_mode) {
                    warn "$My_name: I could not run previewer\n";
                }
                else {
                    &exit_msg1( "I could not run previewer", $retcode);
                }
            }
            else {
                $viewer_running = 1;
                $$Pneed_to_get_viewer_process = 1;
            } # end analyze result of trying to run viewer
        } # end start viewer
        if ( $failure > 0 ) {
            if ( !$failure_msg ) {
                $failure_msg = 'Failure to make the files correctly';
            }
            &rdb_set_rule_net;
            %rules_to_watch = array_to_hash( &rdb_accessible );

            # There will be files changed during the run that are irrelevant.
            # We need to wait for the user to change the files.

            # So set the GENERATED files from *latex as up-to-date:
            rdb_for_some( [keys %current_primaries], \&rdb_update_gen_files );

            # And don't watch for changes for post_primary rules (ps and pdf 
            # from dvi, etc haven't been run after an error in *latex, so
            # are out-of-date by filetime criterion, but they should not be run
            # until after another *latex run:
            foreach (@post_primary) { delete $rules_to_watch{$_}; }

            $failure_msg =~ s/\s*$//;  #Remove trailing space
            warn "$My_name: $failure_msg\n",
    "    ==> You will need to change a source file before I do another run <==\n";
            if ($failure_cmd) {
                Run_subst( $failure_cmd );
            }
        }
        else {
            if ( ($#primary_warning_summary > -1) && $warning_cmd ) {
                Run_subst( $warning_cmd );
            }
            elsif ( ($#primary_warning_summary > -1) && $warnings_as_errors && $failure_cmd ) {
                Run_subst( $failure_cmd );
            }
            elsif ($success_cmd) {
                Run_subst( $success_cmd );
            }
        }
        rdb_show_rule_errors();
        if ($rules_list) { rdb_list(); }
        if ($show_time && ! $first_time) { show_timing(); }
        if ( $dependents_list && ($updated || $failure) ) {
           my $deps_handle = new FileHandle "> $deps_file";
           if ( defined $deps_handle ) {
               deps_list($deps_handle);
               close($deps_handle);
           }
           else {
               warn "Cannot open '$deps_file' for output of dependency information\n";
           }
         }

        # Now wait for a file to change...
        &rdb_cache_generated;
        # During waiting for file changes, handle ctrl/C and ctrl/break here,
        #   rather than letting system handle them by terminating script (and
        #   code in the following command line to work: any script that calls
        #   it).  This allows, for example, the command cleanup in the following
        #   command line to work:
        #          latexmk -pvc foo; cleanup;
        &catch_break;
        $have_break = 0;
        $last_action_time = time();
        $waiting = 1;
        print "\n=== Watching for updated files. Use ctrl/C to stop ...\n";
  WAIT: while (1) {
           sleep( $sleep_time );
           if ($have_break) { last WAIT; }
           if ( rdb_user_changes(keys %rules_to_watch) ) { 
               if (!$silent) {
                   warn "$My_name: Need to remake files.\n";
                   &rdb_diagnose_changes( '  ' );
               }
               last WAIT;
           }
           #  Don't count waiting time in processing:
           $processing_time1 = processing_time();
        # Does this do this job????
           local $new_files = 0;
           rdb_for_some( [keys %current_primaries], sub{ $new_files += &rdb_find_new_files } );
           if ($new_files > 0) {
               warn "$My_name: New file(s) found.\n";
               last WAIT; 
           }
           if ($have_break) { last WAIT; }
           if ($pvc_timeout && ( time() > $last_action_time+60*$pvc_timeout_mins ) ) {
               $timed_out = 1;
               last WAIT;
           }
     } # end WAIT:
     &default_break;
     if ($have_break) { 
          print "$My_name: User typed ctrl/C or ctrl/break.  I'll finish.\n";
          return;
     }
     if ($timed_out) {
         print "$My_name: More than $pvc_timeout_mins mins of inactivity.  I'll finish.\n";
         return;
     }
     $waiting = 0; if ($diagnostics) { warn "NOT       WAITING\n"; }
  } #end infinite_loop CHANGE:
} #END sub make_preview_continuous

#************************************************************

sub process_rc_file {
    # Usage process_rc_file( filename )
    # NEW VERSION
    # Run rc_file whose name is given in first argument
    #    Exit with code 0 on success
    #    Exit with code 1 if file cannot be read or does not exist.
    #    Stop if there is a syntax error or other problem.
    # PREVIOUSLY: 
    #    Exit with code 2 if is a syntax error or other problem.
    my $rc_file = $_[0];
    my $ret_code = 0;
    push @rc_files_read, $rc_file;

    # I could use the do command of perl, but the preceeding -r test
    # to get good diagnostics gets the wrong result under cygwin
    # (e.g., on /cygdrive/c/latexmk/LatexMk)
    my $RCH = new FileHandle;
    if ( !-e $rc_file ) {
        warn "$My_name: The rc-file '$rc_file' does not exist\n";
        return 1;
    }
    elsif ( -d $rc_file ) {
        warn "$My_name: The supposed rc-file '$rc_file' is a directory; but it\n",
             "          should be a normal text file\n";
        return 1;
    }
    elsif ( open $RCH, "<$rc_file" ) {
        my $code = '';
        { local $/; $code = <$RCH>;}
        close $RCH;
        eval $code;
    }
    else {
        warn "$My_name: I cannot read the rc-file '$rc_file'\n";
        return 1;
    }
    # PREVIOUS VERSION
#    if ( ! -r $rc_file ) {
#        warn "$My_name: I cannot read the rc-file '$rc_file'\n",
#            "          or at least that's what Perl (for $^O) reports\n";
#        return 1;
#    }
#    do( $rc_file );
    if ( $@ ) {
        # Indent each line of possibly multiline message:
        my $message = prefix( $@, "     " );
        warn "$My_name: Initialization file '$rc_file' gave an error:\n",
             "$message\n";
        die "$My_name: Stopping because of problem with rc file\n";
        # Use the following if want non-fatal error.
        return 2;
    }
    return 0;
} #END process_rc_file

#************************************************************

sub execute_code_string {
    # Usage execute_code_string( string_of_code )
    # Run the perl code contained in first argument
    #    Halt if there is a syntax error or other problem.
    # ???Should I leave the exiting to the caller (perhaps as an option)?
    #     But I can always catch it with an eval if necessary.
    #     That confuses ctrl/C and ctrl/break handling.
    my $code = $_[0];
    warn "$My_name: Executing initialization code specified by -e:\n",
         "   '$code'...\n" 
        if  $diagnostics;
    eval $code;
    # The return value from the eval is not useful, since it is the value of 
    #    the last expression evaluated, which could be anything.
    # The correct test of errors is on the value of $@.

    if ( $@ ) {
        # Indent each line of possibly multiline message:
        my $message = prefix( $@, "    " );
        die "$My_name: ",
            "Stopping because executing following code from command line\n",
            "    $code\n",
            "gave an error:\n",
            "$message\n";
    }
} #END execute_code_string

#************************************************************

sub cleanup1 {
    # Usage: cleanup1( directory, exts_without_period, ... )
    #
    # The directory and the root file name are fixed names, so I must escape
    #   any glob metacharacters in them:
    my $dir = fix_pattern( shift );
    my $root_fixed = fix_pattern( $root_filename );
    foreach (@_) { 
        my $name = /%R/ ? $_ : "%R.$_";
        $name =~ s/%R/${root_fixed}/;
        $name = $dir.$name;
        unlink_or_move( my_glob( "$name" ) );
    }
} #END cleanup1

#************************************************************

sub cleanup_cusdep_generated {
    # Remove files generated by custom dependencies
    rdb_for_actives( \&cleanup_one_cusdep_generated );
} #END cleanup_cusdep_generated

#************************************************************

sub cleanup_one_cusdep_generated {
    # Remove destination file generated by one custom dependency
    # Assume rule context, but not that the rule is a custom dependency.
    # Only delete destination file if source file exists (so destination 
    #   file can be recreated)
    if ( $$Pcmd_type ne 'cusdep' ) {
       # NOT cusdep
       return;
    }
    if ( ! -e $$Psource ) {
        warn "$My_name: For custom dependency '$rule',\n",
             "    I won't delete destination file '$$Pdest'\n",
             "    and any other generated files,\n",
             "    because the source file '$$Psource' doesn't exist,\n",
             "    so the destination file may not be able to be recreated\n";
        return;
    }
    unlink_or_move( $$Pdest, keys %$PHdest );
} #END cleanup_one_cusdep_generated

#************************************************************
#************************************************************
#************************************************************

#   Error handling routines, warning routines, help

#************************************************************

sub die_trace {
    # Call: die_trace( message );
    &traceback;   # argument(s) passed unchanged
    die "\n";
} #END die_trace

#************************************************************

sub traceback {
    # Call: traceback() 
    # or traceback( message  )
    # NOT &traceback!!!
    my $msg = shift;
    if ($msg) { warn "$msg\n"; }
    warn "Traceback:\n";
    my $i=0;     # Start with immediate caller
    while ( my ($pack, $file, $line, $func) = caller($i++) ) {
        if ($func eq 'die_trace') { next; }
        warn "   $func called from line $line\n";
    }
} #END traceback

#************************************************************

sub exit_msg1
{
  # exit_msg1( error_message, retcode )
  #    1. display error message
  #    2. exit with retcode
  warn "\n------------\n";
  warn "$My_name: $_[0].\n";
  warn "-- Use the -f option to force complete processing.\n";

  my $retcode = $_[1];
  if ($retcode >= 256) {
     # Retcode is the kind returned by system from an external command
     # which is 256 * command's_retcode
     $retcode /= 256;
  }
  exit $retcode;
} #END exit_msg1

#************************************************************

sub warn_running {
   # Message about running program:
    if ( $silent ) {
        warn "$My_name: @_\n";
    }
    else {
        warn "------------\n@_\n------------\n";
    }
} #END warn_running

#************************************************************

sub exit_help
# Exit giving diagnostic from arguments and how to get help.
{
    warn "\n$My_name: @_\n",
         "Use\n",
         "   $my_name -help\nto get usage information\n";
    exit 10;
} #END exit_help


#************************************************************

sub print_help
{
  print
  "$My_name $version_num: Automatic LaTeX document generation routine\n\n",
  "Usage: $my_name [latexmk_options] [filename ...]\n\n",
  "  Latexmk_options:\n",
  "   -aux-directory=dir or -auxdir=dir \n",
  "                 - set name of directory for auxiliary files (aux, log)\n",
  "                 - Currently this only works with MiKTeX\n",
  "   -bibtex       - use bibtex when needed (default)\n",
  "   -bibtex-      - never use bibtex\n",
  "   -bibtex-cond  - use bibtex when needed, but only if the bib file exists\n",
  "   -bibtex-cond1 - use bibtex when needed, but only if the bib file exists;\n",
  "                   on cleanup delete bbl file only if bib file exists\n",
  "   -bibfudge or -bibtexfudge - change directory to output directory when running bibtex\n",
  "   -bibfudge- or -bibtexfudge- - don't change directory when running bibtex\n",
  "   -bm <message> - Print message across the page when converting to postscript\n",
  "   -bi <intensity> - Set contrast or intensity of banner\n",
  "   -bs <scale> - Set scale for banner\n",
  "   -commands  - list commands used by $my_name for processing files\n",
  "   -c     - clean up (remove) all nonessential files, except\n",
  "            dvi, ps and pdf files.\n",
  "            This and the other clean-ups are instead of a regular make.\n",
  "   -C     - clean up (remove) all nonessential files\n",
  "            including aux, dep, dvi, postscript and pdf files\n",
  "            and file of database of file information\n",
  "   -CA     - clean up (remove) all nonessential files.\n",
  "            Equivalent to -C option.\n",
  "   -CF     - Remove file of database of file information before doing \n",
  "            other actions\n",
  "   -cd    - Change to directory of source file when processing it\n",
  "   -cd-   - Do NOT change to directory of source file when processing it\n",
  "   -dependents or -deps - Show list of dependent files after processing\n",
  "   -dependents- or -deps- - Do not show list of dependent files\n",
  "   -deps-out=file - Set name of output file for dependency list,\n",
  "                    and turn on showing of dependency list\n",
  "   -dF <filter> - Filter to apply to dvi file\n",
  "   -dir-report  - Before processing a tex file, report aux and out dir settings\n",
  "   -dir-report- - Before processing a tex file, do not report aux and out dir settings\n",
  "   -dvi   - generate dvi\n",
  "   -dvi-  - turn off required dvi\n",
  "   -e <code> - Execute specified Perl code (as part of latexmk start-up\n",
  "               code)\n",
  "   -emulate-aux-dir  - emulate -aux-directory option for *latex\n",
  "   -emulate-aux-dir- - use -aux-directory option with *latex\n",
  "   -f     - force continued processing past errors\n",
  "   -f-    - turn off forced continuing processing past errors\n",
  "   -gg    - Super go mode: clean out generated files (-CA), and then\n",
  "            process files regardless of file timestamps\n",
  "   -g     - process at least one run of all rules\n",
  "   -g-    - Turn off -g and -gg\n",
  "   -h     - print help\n",
  "   -help - print help\n",
  "   -indexfudge or -makeindexfudge - change directory to output directory when running makeindex\n",
  "   -indexfudge- or -makeindexfudge- - don't change directory when running makeindex\n",
  "   -jobname=STRING - set basename of output file(s) to STRING.\n",
  "            (Like --jobname=STRING on command line for many current\n",
  "            implementations of latex/pdflatex.)\n",
  "   -l     - force landscape mode\n",
  "   -l-    - turn off -l\n",
  "   -latex=<program> - set program used for latex.\n",
  "                      (replace '<program>' by the program name)\n",
  "   -latexoption=<option> - add the given option to the *latex command\n",
  "   -logfilewarninglist or -logfilewarnings \n",
  "               give list of warnings after run of *latex\n",
  "   -logfilewarninglist- or -logfilewarnings- \n",
  "               do not give list of warnings after run of *latex\n",
  "   -lualatex     - use lualatex for processing files to pdf\n",
  "                   and turn dvi/ps modes off\n",
  "   -M     - Show list of dependent files after processing\n",
  "   -MF file - Specifies name of file to receives list dependent files\n",
  "   -MP    - List of dependent files includes phony target for each source file.\n",
  "   -makeindexfudge - change directory to output directory when running makeindex\n",
  "   -makeindexfudge-- don't change directory to output directory when running makeindex\n",
  "   -MSWinBackSlash  under MSWin use backslash (\\) for directory separators\n",
  "                    for filenames given to called programs\n",
  "   -MSWinBackSlash-  under MSWin use forward slash (/) for directory separators\n",
  "                     for filenames given to called programs\n",
  "   -new-viewer    - in -pvc mode, always start a new viewer\n",
  "   -new-viewer-   - in -pvc mode, start a new viewer only if needed\n",
  "   -nobibtex      - never use bibtex\n",
  "   -nobibfudge or -nobibtexfudge - don't change directory when running bibtex\n",
  "   -nodependents  - Do not show list of dependent files after processing\n",
  "   -noemulate-aux-dir - use -aux-directory option with *latex\n",
  "   -noindexfudge or -nomakeindexfudge - don't change directory when running makeindex\n",
  "   -norc          - omit automatic reading of system, user and project rc files\n",
  "   -output-directory=dir or -outdir=dir\n",
  "                  - set name of directory for output files\n",
  "   -output-format=FORMAT\n",
  "                  - if FORMAT is dvi, turn on dvi output, turn off others\n",
  "                  - if FORMAT is pdf, turn on pdf output, turn off others\n",
  "                  - otherwise error\n",    
  "   -pdf   - generate pdf by pdflatex\n",
  "   -pdfdvi - generate pdf by dvipdf\n",
  "   -pdflatex=<program> - set program used for pdflatex.\n",
  "                      (replace '<program>' by the program name)\n",
  "   -pdflualatex=<program> - set program used for lualatex.\n",
  "                      (replace '<program>' by the program name)\n",
  "   -pdfps - generate pdf by ps2pdf\n",
  "   -pdflua - generate pdf by lualatex\n",
  "   -pdfxe - generate pdf by xelatex\n",
  "   -pdfxelatex=<program> - set program used for xelatex.\n",
  "                      (replace '<program>' by the program name)\n",
  "   -pdf-  - turn off pdf\n",
  "   -ps    - generate postscript\n",
  "   -ps-   - turn off postscript\n",
  "   -pF <filter> - Filter to apply to postscript file\n",
  "   -p     - print document after generating postscript.\n",
  "            (Can also .dvi or .pdf files -- see documentation)\n",
  "   -pretex=<TeX code> - Sets TeX code to be executed before inputting source\n",
  "                    file, if commands suitable configured\n",    
  "   -print=dvi     - when file is to be printed, print the dvi file\n",
  "   -print=ps      - when file is to be printed, print the ps file (default)\n",
  "   -print=pdf     - when file is to be printed, print the pdf file\n",
  "   -pv    - preview document.  (Side effect turn off continuous preview)\n",
  "   -pv-   - turn off preview mode\n",
  "   -pvc   - preview document and continuously update.  (This also turns\n",
  "                on force mode, so errors do not cause $my_name to stop.)\n",
  "            (Side effect: turn off ordinary preview mode.)\n",
  "   -pvc-  - turn off -pvc\n",
  "   -pvctimeout    - timeout in pvc mode after period of inactivity\n",
  "   -pvctimeout-   - don't timeout in pvc mode after inactivity\n",
  "   -pvctimeoutmins=<time> - set period of inactivity (minutes) for pvc timeout\n",
  "   -quiet    - silence progress messages from called programs\n",
  "   -r <file> - Read custom RC file\n",
  "               (N.B. This file could override options specified earlier\n",
  "               on the command line.)\n",
  "   -rc-report  - After initialization, report names of rc files read\n",
  "   -rc-report- - After initialization, do not report names of rc files read\n",
  "   -recorder - Use -recorder option for *latex\n",
  "               (to give list of input and output files)\n",
  "   -recorder- - Do not use -recorder option for *latex\n",
  "   -rules    - Show list of rules after processing\n",
  "   -rules-   - Do not show list of rules after processing\n",
  "   -showextraoptions  - Show other allowed options that are simply passed\n",
  "               as is to latex and pdflatex\n",
  "   -silent   - silence progress messages from called programs\n",
  "   -stdtexcmds - Sets standard commands for *latex\n",    
  "   -time     - show CPU time used\n",
  "   -time-    - don't show CPU time used\n",
  "   -use-make - use the make program to try to make missing files\n",
  "   -use-make- - don't use the make program to try to make missing files\n",
  "   -usepretex - Sets commands for *latex to use extra code before inputting\n",
  "                source file\n",    
  "   -usepretex=<TeX code> - Equivalent to -pretex=<TeX code> -usepretex\n",
  "   -v        - display program version\n",
  "   -verbose  - display usual progress messages from called programs\n",
  "   -version      - display program version\n",
  "   -view=default - viewer is default (dvi, ps, pdf)\n",
  "   -view=dvi     - viewer is for dvi\n",
  "   -view=none    - no viewer is used\n",
  "   -view=ps      - viewer is for ps\n",
  "   -view=pdf     - viewer is for pdf\n",
  "   -Werror   - treat warnings from called programs as errors\n",
  "   -xelatex      - use xelatex for processing files to pdf\n",
  "                   and turn dvi/ps modes off\n",
  "\n",
  "   filename = the root filename of LaTeX document\n",
  "\n",
  "-p, -pv and -pvc are mutually exclusive\n",
  "-h, -c and -C override all other options.\n",
  "-pv and -pvc require one and only one filename specified\n",
  "All options can be introduced by '-' or '--'.  (E.g., --help or -help.)\n",
  " \n",
  "In addition, latexmk recognizes many other options that are passed to\n",
  "latex and/or pdflatex without interpretation by latexmk.  Run latexmk\n",
  "with the option -showextraoptions to see a list of these\n",
  "\n",
  "Report bugs etc to John Collins <jcc8 at psu.edu>.\n";

} #END print_help

#************************************************************

sub print_commands {
  warn "Commands used by $my_name:\n",
       "   To run latex, I use \"$latex\"\n",
       "   To run pdflatex, I use \"$pdflatex\"\n",
       "   To run lualatex, I use \"$lualatex\"\n",
       "   To run xelatex, I use \"$xelatex\"\n",
       "   To run biber, I use \"$biber\"\n",
       "   To run bibtex, I use \"$bibtex\"\n",
       "   To run makeindex, I use \"$makeindex\"\n",
       "   To make a ps file from a dvi file, I use \"$dvips\"\n",
       "   To make a ps file from a dvi file with landscape format, ",
           "I use \"$dvips_landscape\"\n",
       "   To make a pdf file from a dvi file, I use \"$dvipdf\"\n",
       "   To make a pdf file from a ps file, I use \"$ps2pdf\"\n",
       "   To make a pdf file from an xdv file, I use \"$xdvipdfmx\"\n",
       "   To view a pdf file, I use \"$pdf_previewer\"\n",
       "   To view a ps file, I use \"$ps_previewer\"\n",
       "   To view a ps file in landscape format, ",
            "I use \"$ps_previewer_landscape\"\n",
       "   To view a dvi file, I use \"$dvi_previewer\"\n",
       "   To view a dvi file in landscape format, ",
            "I use \"$dvi_previewer_landscape\"\n",
       "   To print a ps file, I use \"$lpr\"\n",
       "   To print a dvi file, I use \"$lpr_dvi\"\n",
       "   To print a pdf file, I use \"$lpr_pdf\"\n",
       "   To find running processes, I use \"$pscmd\", \n",
       "      and the process number is at position $pid_position\n";
   warn "Notes:\n",
        "  Command starting with \"start\" is run detached\n",
        "  Command that is just \"start\" without any other command, is\n",
        "     used under MS-Windows to run the command the operating system\n",
        "     has associated with the relevant file.\n",
        "  Command starting with \"NONE\" is not used at all\n";
} #END print_commands

#************************************************************

sub view_file_via_temporary {
    return $always_view_file_via_temporary 
           || ($pvc_view_file_via_temporary && $preview_continuous_mode);
} #END view_file_via_temporary

#************************************************************
#### Tex-related utilities

#**************************************************

sub check_biber_log {
    # Check for biber warnings:
    # Usage: check_biber_log( base_of_biber_run, \@biber_source )
    # return 0: OK;
    #        1: biber warnings;
    #        2: biber errors;
    #        3: could not open .blg file;
    #        4: failed to find one or more source files, except for bibfile;
    #        5: failed to find bib file;
    #        6: missing file, one of which is control file
    #       10: only error is missing \citation commands.
    #       11: Malformed bcf file (normally due to error in pdflatex run)
    # Side effect: add source files @biber_source
    my $base = $_[0];
    my $Pbiber_source = $_[1];
    my $blg_name = "$base.blg";
    my $blg_file = new FileHandle;
    open( $blg_file, "<$blg_name" )
      or return 3;
    my $have_warning = 0;
    my $have_error = 0;
    my $missing_citations = 0;
    my $no_citations = 0;
    my $error_count = 0;            # From my counting of error messages
    my $warning_count = 0;          # From my counting of warning messages
    # The next two occur only from biber
    my $bibers_error_count = 0;     # From biber's counting of errors
    my $bibers_warning_count = 0;   # From biber's counting of warnings
    my $not_found_count = 0;
    my $control_file_missing = 0;
    my $control_file_malformed = 0;
    my %remote = ();                # List of extensions of remote files
    while (<$blg_file>) {
        if (/> WARN /) { 
            print "Biber warning: $_"; 
            $have_warning = 1;
            $warning_count ++;
        }
        elsif (/> (FATAL|ERROR) /) {
            print "Biber error: $_"; 
            if ( /> (FATAL|ERROR) - Cannot find file '([^']+)'/    #'
                 || /> (FATAL|ERROR) - Cannot find '([^']+)'/ ) {  #'
                $not_found_count++;
                push @$Pbiber_source, $2;
            }
            elsif ( /> (FATAL|ERROR) - Cannot find control file '([^']+)'/ ) {  #'
                $not_found_count++;
                $control_file_missing = 1;
                push @$Pbiber_source, $2;
            }
            elsif ( /> ERROR - .*\.bcf is malformed/ ) {
                #  Special treatment: Malformed .bcf file commonly results from error
                #  in *latex run.  This error must be ignored.
                $control_file_malformed = 1;
            }
            else {
                $have_error = 1;
                $error_count ++;
                if ( /> (FATAL|ERROR) - The file '[^']+' does not contain any citations!/ ) { #'
                    $no_citations++;
                }
            }
        }
        elsif ( /> INFO - Data source '([^']*)' is a remote BibTeX data source - fetching/
            ){
            my $spec = $1;
            my ( $base, $path, $ext ) = fileparseA( $spec );
            $remote{$ext} = 1;
        }
        elsif ( /> INFO - Found .* '([^']+)'\s*$/
                || /> INFO - Found '([^']+)'\s*$/
                || /> INFO - Reading '([^']+)'\s*$/
                || /> INFO - Processing .* file '([^']+)'.*$/
                || /> INFO - Config file is '([^']+)'.*$/
            ) {
            my $file = $1;
            my ( $base, $path, $ext ) = fileparseA( $file );
            if ($remote{$ext} && ( $base =~ /^biber_remote_data_source/ ) && 1) {
                # Ignore the file, which appears to be a temporary local copy
                # of a remote file. Treating the file as a source file will
                # be misleading, since it will normally have been deleted by
                # biber itself.
            }
            elsif ( (defined $Pbiber_source) && (-e $file) ) {
                # Note that biber log file gives full path to file. (No search is
                # needed to find it.)  The file must have existed when biber was
                # run.  If it doesn't exist now, a few moments later, it must
                # have gotten deleted, probably by biber (e.g., because it is a
                # copy of a remote file).
                # So I have included a condition above that the file must
                # exist to be included in the source-file list.
                push @$Pbiber_source, $file;
            }
        }
        elsif ( /> INFO - WARNINGS: ([\d]+)\s*$/ ) {
            $bibers_warning_count = $1;
        }
        elsif ( /> INFO - ERRORS: ([\d]+)\s*$/ ) {
            $bibers_error_count = $1;
        }
    }
    close $blg_file;
    if ($control_file_malformed){return 11;} 

    my @not_found = &find_file_list1( $Pbiber_source, $Pbiber_source,
                                      '', \@BIBINPUTS );
    @$Pbiber_source = uniqs( @$Pbiber_source );

    if ( ($#not_found < 0) && ($#$Pbiber_source >= 0) ) {
        warn "$My_name: Found biber source file(s) [@$Pbiber_source]\n"
        unless $silent;
    }
    elsif ( ($#not_found == 0) && ($not_found[0] =~ /\.bib$/) ) {
        # Special treatment if sole missing file is bib file
        # I don't want to treat that as an error
        warn "$My_name: Biber did't find bib file [$not_found[0]]\n";
        return 5;
    }
    else {
        warn "$My_name: Failed to find one or more biber source files:\n";
        foreach (@not_found) { warn "    '$_'\n"; }
        if ($force_mode) {
            warn "==== Force_mode is on, so I will continue.  ",
                 "But there may be problems ===\n";
        }
        if ($control_file_missing) {
            return 6;
        }
        return 4;
    }
#    print "$My_name: #Biber errors = $error_count, warning messages = $warning_count,\n  ",
#          "missing citation messages = $missing_citations, no_citations = $no_citations\n";
    if ( ! $have_error && $no_citations ) {
        # If the only errors are missing citations, or lack of citations, that should
        # count as a warning.
        # HOWEVER: biber doesn't generate a new bbl.  So it is an error condition.
        return 10;
    }
    if ($have_error) {return 2;}
    if ($have_warning) {return 1;}
    return 0;
} #END check_biber_log

#**************************************************

sub run_bibtex {
    my $return = 999;
    # Prevent changes we make to environment becoming global:
    local %ENV = %ENV;

    my ( $base, $path, $ext ) = fileparseA( $$Psource );
    # Define source and dest base to include extension, no path.
    my $source_base = $base.$ext;
    my $dest_base = basename( $$Pdest );
    if ( $path && $bibtex_fudge ) {
        # Up to TeXLive 2018, the following was true; situation has changed since.
        #   When an output directory is specified and with a bibtex from 2018 or
        #   earlier, running 'bibtex output/main.aux' doesn't find subsidiary .aux
        #   files, as from \@include{chap.aux}.  To evade the bug, we change
        #   directory to the directory of the top-level .aux file to run bibtex.
        #   But we have to fix search paths for .bib and .bst, since they may be
        #   specified relative to the document directory.
        # There is also another problem: Depending on the exact
        #   specification of the aux dir, bibtex may refuse to write to the
        #   aux dir, for security reasons.
        my $cwd = good_cwd();
        foreach ( 'BIBINPUTS', 'BSTINPUTS' ) {
            if ( exists $ENV{$_} ) {
                $ENV{$_} = $cwd.$search_path_separator.$ENV{$_};
            }
            else {
                $ENV{$_} = $cwd.$search_path_separator;
            }
        }
        pushd( $path );
        if (!$silent) {
            print "$My_name: Change directory to '$path'.\n",
                  "To assist finding of files in document\n",
                  "directory, I set\n",
                  "  BIBINPUTS='$ENV{BIBINPUTS}'\n",
                  "  BSTINPUTS='$ENV{BSTINPUTS}'.\n";
        }
        # Override standard substitutions for source, dest, and base names in
        # default external command:
        $return = &Run_subst( undef, undef, '', $source_base, $dest_base, $base );
        popd();
        if (!$silent) {
            print "$My_name: Change directory back to '", cwd(), "'\n";
        }
    }
    else {
        # Use default substitutions etc for rule:
        $return = Run_subst();
    }
    return $return;
} #END run_bibtex

#**************************************************

sub run_makeindex {
    my $return = 999;
    my ( $base, $path, $ext ) = fileparseA( $$Psource );

    # Define source and dest base to include extension, no path.
    my $source_base = $base.$ext;
    my $dest_base = basename( $$Pdest );
    if ( $path && $makeindex_fudge ) {
        my $cwd = good_cwd();
        pushd( $path );
        if (!$silent) {
            print "$My_name: Change directory to '$path'.\n";
        }
        # Override standard substitutions for source, dest, and base names in
        # default external command:
        $return = &Run_subst( undef, undef, '', $source_base, $dest_base, $base );
        popd();
        if (!$silent) {
            print "$My_name: Change directory back to '", cwd(), "'\n";
        }
    }
    else {
        # Use default substitutions etc for rule:
        $return = Run_subst();
    }
    return $return;
} #END run_makeindex

#**************************************************

sub check_bibtex_log {
    # Check for bibtex warnings:
    # Usage: check_bibtex_log( base_of_bibtex_run )
    # return 0: OK, 1: bibtex warnings, 2: bibtex errors, 
    #        3: could not open .blg file.
    #       10: only error is missing \citation commands or a missing aux file
    #           (which would normally be corrected after a later run of 
    #           *latex).

    my $base = $_[0];
    my $blg_name = "$base.blg";
    my $blg_file = new FileHandle;
    open( $blg_file, "<$blg_name" )
      or return 3;
    my $have_warning = 0;
    my $have_error = 0;
    my $missing_citations = 0;
    my @missing_aux = ();
    my $error_count = 0;
    while (<$blg_file>) {
        if (/^Warning--/) { 
            #print "Bibtex warning: $_"; 
            $have_warning = 1;
        }
        elsif ( /^I couldn\'t open auxiliary file (.*\.aux)/ ) {
            push @missing_aux, $1;
        }
        elsif ( /^I found no \\citation commands---while reading file/ ) {
            $missing_citations++;
        }
        elsif (/There (were|was) (\d+) error message/) {
            $error_count = $2;
            #print "Bibtex error: count=$error_count $_"; 
            $have_error = 1;
        }
    }
    close $blg_file;
    my $missing = $missing_citations + $#missing_aux + 1;
    if ( $#missing_aux > -1 ) {
        # Need to make the missing files.
        warn "$My_name: One or more aux files is missing for bibtex. I'll try\n",
             "          to get *latex to remake them.\n";
        rdb_for_some( [keys %current_primaries], sub{ $$Pout_of_date = 1; } );
    }
    #print "Bibtex errors = $error_count, missing aux files and citations = $missing\n";
    if ($have_error && ($error_count <= $missing )
        && ($missing > 0) ) {
        # If the only error is a missing citation line, that should only
        # count as a warning.
        # Also a missing aux file should be innocuous; it will be created on
        # next run of *latex.  ?? HAVE I HANDLED THAT CORRECTLY?
        # But have to deal with the problem that bibtex gives a non-zero 
        # exit code.  So leave things as they are so that the user gets
        # a better diagnostic ??????????????????????????
#        $have_error = 0;
#        $have_warning = 1;
        return 10;
    }
    if ($have_error) {return 2;}
    if ($have_warning) {return 1;}
    return 0;
} #END check_bibtex_log

#**************************************************

sub normalize_force_directory {
    #  Usage, normalize_force_directory( dir, filename )
    #  Filename is assumed to be relative to dir (terminated with directory separator).
    #  Perform the following operations:
    #    Clean filename
    #    Prefix filename with dir
    #    Normalize filename
    #  Return result
    my $dir = $_[0];
    my $filename = clean_filename( $_[1] );
    $filename = "$dir$filename";
    return normalize_filename( $filename );
} #END normalize force_directory

#**************************************************

sub set_names {
    # Set names of standard files.  These are global variables.

    ## Remove extension from filename if was given.
    if ( find_basename($filename, $root_filename, $texfile_name) )  {
        if ( $force_mode ) {
           warn "$My_name: Could not find file '$texfile_name'\n";
        }
        else {
            &ifcd_popd;
            &exit_msg1( "Could not find file '$texfile_name'",
                        11);
        }
    }
    $tex_basename = $root_filename;  # Base name of TeX file itself
    if ($jobname ne '' ) {
        $root_filename = $jobname;
        $root_filename =~ s/%A/$tex_basename/g;
    }

    $aux_main = "%Y%R.aux";
    $log_name = "%Y%R.log";
    $fdb_name = "%Y%R.$fdb_ext";
    # Note: Only MiKTeX allows out_dir ne aux_dir. It puts
    #       .fls file in out_dir, not aux_dir, which seems
    #       not natural.
    $fls_name = "%Z%R.fls";

    $dvi_name  = "%Z%R.dvi";
    $dviF_name = "%Z%R.dviF";
    $ps_name   = "%Z%R.ps";
    $psF_name  = "%Z%R.psF";
    $pdf_name  = "%Z%R.pdf";
    ## It would be logical for a .xdv file to be put in the out_dir,
    ## just like a .dvi file.  But the only program, MiKTeX, that
    ## currently implements aux_dir, and hence allows aux_dir ne out_dir,
    ## puts .xdv file in aux_dir.  So we must use %Y not %Z:
    $xdv_name   = "%Y%R.xdv";

    foreach ( $aux_main, $log_name, $fdb_name, $fls_name,
              $dvi_name, $ps_name, $pdf_name, $xdv_name, $dviF_name, $psF_name ) {
        s/%R/$root_filename/g;
        s/%Y/$aux_dir1/;
        s/%Z/$out_dir1/;
    }

    $dvi_final = $dvi_name;
    $ps_final  = $ps_name;
    $pdf_final = $pdf_name;
    $xdv_final = $xdv_name;

    if ( length($dvi_filter) > 0) {
        $dvi_final = $dviF_name;
    }
    if ( length($ps_filter) > 0) {
        $ps_final = $psF_name;
    }
}

#**************************************************

sub move_out_files_from_aux {
    # Move output and fls files to out_dir
    # Omit 'xdv', that goes to aux_dir (as with MiKTeX). It's not final output.
    foreach my $ext ( 'fls', 'dvi', 'pdf', 'ps', 'synctex', 'synctex.gz' ) {
        # Include fls file, because MiKTeX puts it in out_dir, rather than
        # aux_dir, which would seem more natural.  We must maintain
        # compatibility.
        my $from =  "$aux_dir1$root_filename.$ext";
        my $to = "$out_dir1$root_filename.$ext" ;
        if ( test_gen_file( $from ) ) {
            if (! $silent) { warn "$My_name: Moving '$from' to '$to'\n"; }
            my $ret = move( $from, $to );
            if ( ! $ret ) { die "  That failed, with message '$!'\n";}
        }
    }
}

#***************************************************

sub parse_log {
# Scan log file for: dependent files
#    reference_changed, bad_reference, bad_citation
# Return value: 1 if success, 0 if no log file.
# Put results in UPDATES of global variables (which are normally declared
# local in calling routine, to be suitably scoped):
#   %dependents: maps definite dependents to code:
#      0 = from missing-file line
#            May have no extension
#            May be missing path
#      1 = from 'File: ... Graphic file (type ...)' line
#            no path.  Should exist, but may need a search, by kpsewhich.
#      2 = from regular '(...' coding for input file, 
#            Has NO path, which it would do if LaTeX file
#            Highly likely to be mis-parsed line
#      3 = ditto, but has a path character ('/').  
#            Should be LaTeX file that exists.
#            If it doesn't exist, we have probably a mis-parsed line.
#            There's no need to do a search.
#      4 = definitive, which in this subroutine is only done:
#             for default dependents, 
#             and for files that exist and are source of conversion
#                reported by epstopdf et al.
#      5 = Had a missing file line.  Now the file exists.
#      6 = File was written during run.  (Overrides 5)
#      7 = File was created during run to be read in.  (Overrides 5 and 6)
#          (e.g., by epstopdf)
# Treat the following specially, since they have special rules
#   @bbl_files to list of .bbl files.
#   %idx_files to map from .idx files to .ind files.
# %generated_log: keys give set of files written by *latex (e.g., aux, idx)
#   as determined by \openout = ... lines in log file.
# @missing_subdirs = list of needed subdirectories of aux_dir
#   These are needed for writing aux_files when an included file is in
#   a subdirectory relative to the directory of the main TeX file.
#   This variable is only set when the needed subdirectories don't exist,
#   and the aux_dir is non-trivial, which results in an error message in 
#   the log file
#  %conversions Internally made conversions from one file to another
#
#  These may have earlier found information in them, so they should NOT
#  be initialized.
#
# Also SET
#   $reference_changed, $bad_reference, $bad_citation
#   $pwd_latex
#
# Put in trivial or default values if log file does not exist/cannot be opened
#
# Input globals: $primary_out, $fls_file_analyzed
#
   
   
# Give a quick way of looking up custom-dependency extensions
    my %cusdep_from = ();
    my %cusdep_to = ();
    foreach ( @cus_dep_list ) {
        my ($fromext, $toext) = split;
        $cusdep_from{$fromext} = $cusdep_from{".$fromext"} = $_;
        $cusdep_to{$toext} = $cusdep_to{".$toext"} = $_;
    }
#    print "==== Cusdep from-exts:"; foreach (keys %cusdep_from) {print " '$_'";} print "\n";
#    print "==== Cusdep to-exts:"; foreach (keys %cusdep_to) {print " '$_'";} print "\n";



    # $primary_out is actual output file (dvi or pdf)
    # It is initialized before the call to this routine, to ensure
    # a sensible default in case of misparsing

    $reference_changed = 0;
    $mult_defined = 0;
    $bad_reference = 0;
    $bad_character = 0;
    $bad_citation = 0;

    my $log_file = new FileHandle;
    if ( ! open( $log_file, "<$log_name" ) ) {
        return 0;
    }
    print "$My_name: Examining '$log_name'\n"
        if not $silent;
    if ($log_file_binary) { binmode $log_file; }
# Collect lines of log file
    my @lines = ();
    my $line = 0;
    my $engine = 'pdfTeX';  # Simple default in case of problems
    while(<$log_file>) {
        $line++;
        # Could use chomp here, but that fails if there is a mismatch
        #    between the end-of-line sequence used by latex and that
        #    used by perl.  (Notably a problem with MSWin latex and
        #    cygwin perl!)
        s/[\n\r]*$//;
        # Handle wrapped lines:
        # They are lines brutally broken at exactly $log_wrap chars 
        #    excluding line-end.  Sometimes a line $log_wrap chars 
        #    long is an ordinary line, sometimes it is part of a line
        #    that was wrapped.  To handle all cases, I keep both
        #    options open by putting the line into @lines before
        #    and after appending the next line:  
        my $len = length($_);
        if ($line == 1) {
            if ( /^This is ([^,]+), / ) {
                $engine = $1;
                print "=== TeX engine is '$engine'\n"
                    if (!$silent);
                if ( /^This is ([^,]+), [^\(]*\(([^\)]+)\)/ ) {
                    $tex_distribution = $2;
                    print "=== TeX distribution is '$tex_distribution'\n"
                        if ($diagnostics);
                }
            }
            else {
                warn "$My_name: First line of .log file '$log_name' is not in standard format.\n";
            }
        }
        else {
            # Xetex and luatex sometimes wrap at longer line lengths:
            # LuaTeX sometimes at 80. Xetex 80 or longer with non-ascii characters.
            while ( ( ($len == $log_wrap)
                      || ( ($engine eq 'LuaTeX') && ($len == $log_wrap+1) )
                      || ( ($engine eq 'LuaHBTeX') && ($len == $log_wrap+1) )
                      || ( ($engine eq 'XeTeX') &&  ($len >= $log_wrap+1) )
                    )
                    && !eof($log_file) ) {
                push @lines, $_;
                my $extra = <$log_file>;
                $extra =~ s/[\n\r]*$//;
                $len = length($extra);
                $_ .= $extra;
            }
        }
        push @lines, $_;
    }
    close $log_file;

    push @lines, "";   # Blank line to terminate.  So multiline blocks 
              # are always terminated by non-block line, rather than eof.
    
    $line = 0;
    my $state = 0;   # 0 => before ** line,
                     # 1 => after **filename line, before next line (first file-reading line)
                     # 2 => pwd_log determined.
    # For parsing multiple line blocks of info
    my $current_pkg = "";   # non-empty string for package name, if in 
                            # middle of parsing multi-line block of form:
                            #       Package name ....
                            #       (name) ...
                            #       ...
    my $block_type = "";         # Specify information in such a block
    my $delegated_source = "";   # If it is a file conversion, specify source
    my $delegated_output = "";   #    and output file.  (Don't put in
                                 #    data structure until block is ended.)
    my %new_conversions = ();
    my @retries = ();
    my $log_silent = ($silent ||  $silence_logfile_warnings);
    my @warning_list = ();
LINE:
    while( ($line <= $#lines) || ($#retries > -1) ) { 
        if ($#retries > -1) {
            $_ = pop @retries;
        }
        else {
            $_ = $lines[$line];
            $line ++;
        }
        if ( /^! pdfTeX warning/ || /^pdfTeX warning/ ) {
            # This kind of warning is produced by some versions of pdftex
            # or produced by my reparse of warnings from other
            # versions.
            next;
        }
        elsif ( /^(.+)(pdfTeX warning.*)$/ ) {
            # Line contains a pdfTeX warnings that may have been
            # inserted directly after other material without an
            # intervening new line.  I think pdfTeX always inserts a
            # newline after the warning.  (From examination of source
            # code.) 
            push @retries, $1;
            # But continue parsing the original line, in case it was a
            # misparse, e.g., of a filename ending in 'pdfTeX';
        }
        if ( $line == 1 ){
            if ( /^This is / ) {
                # First line OK
                next LINE;
            } else {
                warn "$My_name: Error on first line of '$log_name'.\n".
                    "This is apparently not a TeX log file.  ",
                    "The first line is:\n$_\n";
                $failure = 1;
                $failure_msg = "Log file '$log_name' appears to have wrong format.";
                return 0;
            }
        }

        if ( ($state == 0) && /^\*\*(.*)$/ ) {
            # Line containing first line specified to tex
            # It's either a filename or a command starting with \
            my $first = $1;
            $state = 1;
            if ( ! /^\\/ ) {
                $source_log = $first;
                if ( -e "$source_log.tex" ) { $source_log .= '.tex'; }
            }
            else {
                $state = 2;
            }
            next LINE;
        }
        elsif ( $state == 1 ) {
            $state = 2;
            if (-e $source_log) {
                # then the string preceeding $source_log on the line after the
                # ** line is probably the PWD as it appears in filenames in the
                # log file, except if the file appears in two locations.
                if ( m{^\("([^"]*)[/\\]\Q$source_log\E"} ) {
                    unshift @pwd_log, $1;
                }
                elsif ( m{^\((.*)[/\\]\Q$source_log\E} ) {
                    unshift @pwd_log, $1;
                }
            }
        }

        if ( $block_type ) {
            # In middle of parsing block
            if ( /^\($current_pkg\)/ ) {
                # Block continues
                if ( ($block_type eq 'conversion') 
                     && /^\($current_pkg\)\s+Output file: <([^>]+)>/ ) 
                {
                    $delegated_output = normalize_clean_filename($1, @pwd_log);
                }
                next LINE;
            }
            # Block has ended.
            if ($block_type eq 'conversion') {
#print "=== $delegated_source -> $delegated_output\n";
                 $new_conversions{$delegated_source} =  $delegated_output;
            }
            $current_pkg = $block_type 
                 = $delegated_source = $delegated_output = "";
            # Then process current line
        }

        # Check for changed references, bad references and bad citations:
        if (/Rerun to get/) { 
            warn "$My_name: References changed.\n" if ! $log_silent;
            $reference_changed = 1;
        } 
        if (/^LaTeX Warning: (Reference[^\001]*undefined on input line .*)\./) {
            push @warning_list, $1;
            $bad_reference++;
        } 
        elsif (/^LaTeX Warning: (Label [^\001]* multiply defined.*)\./) {
            push @warning_list, $1;
            $mult_defined++;
        }
        elsif (/^LaTeX Warning: (Citation[^\001]*undefined on input line .*)\./) {
            push @warning_list, $1;
            $bad_citation++;
        }
        elsif (/^Package natbib Warning: (Citation[^\001]*undefined on input line .*)\./) {
            push @warning_list, $1;
            $bad_citation++;
        }
        elsif ( /^Missing character: There is no /
                || /^! Package inputenc Error: Unicode character /
                || /^! Bad character code /
            ) {
            $bad_character++;
        } 
        elsif ( /^Document Class: / ) {
            # Class sign-on line
            next LINE;
        }
        elsif ( /^\(Font\)/ ) {
            # Font info line
            next LINE;
        }
        elsif (/^No pages of output\./) {
            $primary_out = ''; 
            warn "$My_name: Log file says no output from latex\n";
            next LINE;
        }
        elsif ( /^Output written on\s+(.*)\s+\(\d+\s+page/ ) {
            $primary_out = normalize_clean_filename($1, @pwd_log);
            warn "$My_name: Log file says output to '$primary_out'\n"
               unless $silent;
            next LINE;
        }
        elsif ( /^Overfull / 
             || /^Underfull / 
             || /^or enter new name\. \(Default extension: .*\)/ 
             || /^\*\*\* \(cannot \\read from terminal in nonstop modes\)/
           ) {
            # Latex error/warning, etc.
            next LINE;
        }
        elsif ( /^\\openout\d+\s*=\s*(.*)\s*$/ ) {
            # \openout followed by filename followed by line end.
            # pdflatex and xelatex quote it and wrap,
            # lualatex leaves filename as is, and doesn't wrap.
            # Filename is always relative to aux_dir, given standard security
            # settings in TeXLive.
            my $cand = $1;
            if ( $cand =~ /\`\"([^\'\"]+)\"\'\.$/ ) {
                # One form of quoting by pdflatex, xelatex: `"..."'.
                $cand = $1;
            }
            elsif ( $cand =~ /\`([^\']+)\'\.$/ ) {
                # Another form of quoting by pdflatex, xelatex: `...'.
                $cand = $1;
            }
            if ( $cand =~ /[\`\'\"]/){
                # Bad quotes: e.g., incomplete wrapped line
                next LINE;
            }
            $generated_log{ normalize_force_directory($aux_dir1, $cand) } = 1;
            next LINE;
        }
        # Test for conversion produced by package:
        elsif ( /^Package (\S+) Info: Source file: <([^>]+)>/ ) {
            # Info. produced by epstopdf (and possibly others) 
            #    about file conversion
            $current_pkg = normalize_clean_filename($1, @pwd_log);
            $delegated_source = normalize_clean_filename($2, @pwd_log);
            $block_type = 'conversion';
            next LINE;
        }
#    Test for writing of index file.  The precise format of the message 
#    depends on which package (makeidx.sty , multind.sty or index.sty) and 
#    which version writes the message.
        elsif ( /Writing index file (.*)$/ ) {
            my $idx_file = '';
            if ( /^Writing index file (.*)$/ ) {
                # From makeidx.sty or multind.sty
                $idx_file = $1;
            }
            elsif ( /^index\.sty> Writing index file (.*)$/ ) {
                # From old versions of index.sty
                $idx_file = $1;
            }
            elsif ( /^Package \S* Info: Writing index file (.*) on input line/ ) {
                # From new versions of index.sty
                $idx_file = $1;                
            }
            else {
                warn "$My_name: Message indicates index file was written\n",
                     "  ==> but I do not know how to understand it: <==\n",
                     "  '$_'\n";
                next LINE;
            }
                # Typically, there is trailing space, not part of filename:
            $idx_file =~ s/\s*$//;
                #  When *latex is run with an -output-directory 
                #    or an -aux_directory, the file name does not contain
                #    the path. Fix this:
            $idx_file = normalize_force_directory( $aux_dir1, $idx_file );
            my ($idx_base, $idx_path, $idx_ext) = fileparseA( $idx_file );
            $idx_base = $idx_path.$idx_base;
            $idx_file = $idx_base.$idx_ext;
            if ( $idx_ext eq '.idx' ) {
                warn "$My_name: Index file '$idx_file' was written\n"
                  unless $silent;
                $idx_files{$idx_file} = [ "$idx_base.ind", $idx_base ];
            }
            elsif ( exists $cusdep_from{$idx_ext} ) {
                if ( !$silent ) {
                    warn "$My_name: Index file '$idx_file' was written\n";
                    warn "   Cusdep '$cusdep_from{$idx_ext}' should be used\n";
                }
                # No action needed here
            }
            else {
                warn "$My_name: Index file '$idx_file' written\n",
                     "  ==> but it has an extension I do not know how to handle <==\n";
            }

            next LINE;
        }
        elsif ( /^No file (.*?\.bbl)./ ) {
            # Filename is always relative to aux_dir, given standard security
            # settings in TeXLive.
            my $bbl_file = normalize_force_directory( $aux_dir1, $1 );
            warn "$My_name: Missing bbl file '$bbl_file' in following:\n $_\n";
            $dependents{$bbl_file} = 0;
            push @bbl_files, $bbl_file;
            next LINE;
        }
        foreach my $pattern (@file_not_found) {
            if ( /$pattern/ ) {
                my $file = clean_filename($1);
                warn "$My_name: Missing input file '$file' (or dependence on it) from following:\n  '$_'\n"
                    unless $silent;
                $dependents{normalize_filename($file, @pwd_log)} = 0;
                my $file1 = $file;
                if ( $aux_dir && ($aux_dir ne '.') ) {
                    # Allow for the possibility that latex generated
                    # a file in $aux_dir, from which the missing file can
                    # be created by a cusdep (or other) rule that puts
                    # the result in $out_dir.  If the announced missing file
                    # has no path, then it would be effectively a missing
                    # file in $aux_dir, with a path.  So give this alternate
                    # location.
                    # It is also possible to have a file that is in a directory
                    # relative to the aux_dir, so allow for that as well
                    my $file1 = normalize_force_directory( $aux_dir1, $file );
                    $dependents{$file1} = 0;
                }
                next LINE;
            }
        }
        if ( (! $fls_file_analyzed)
             && /^File: (.+) Graphic file \(type / ) {
            # First line of message from includegraphics/x
            # But this does NOT include full path information
            #   (if exact match is not found and a non-trivial
            #   kpsearch was done by *latex).
            # But the source-file information is in the fls file,
            #   if we are using it.
            $dependents{normalize_clean_filename($1, @pwd_log)} = 1;
            next LINE;
        }
        # Now test for generic lines to ignore, only after special cases!
        if ( /^File: / ) {
           # Package sign-on line. Includegraphics/x also produces a line 
           # with this signature, but I've already handled it.
           next LINE;
        }
        if ( /^Package: / ) {
            # Package sign-on line
            next LINE;
        }
        if (/^\! LaTeX Error: / ) {
            next LINE;
        }
        if ( m[^! I can't write on file `(.*)/([^/']*)'.\s*$] ) {
            my $dir = $1;
            my $file = $2;
            my $full_dir = $aux_dir1.$dir;
            if ( ($aux_dir ne '') && (! -e $full_dir) && ( $file =~ /\.aux$/) ) {
                warn "$My_name: === There were problems writing to '$file' in '$full_dir'\n",
                     "    I'll try to make the subdirectory later.\n"
                  if $diagnostics;
                push @missing_subdirs, $full_dir;
            }
            else {
                warn "$My_name: ====== There were problems writing to",
                     "----- '$file' in '$full_dir'.\n",
                     "----- But this is not the standard situation of\n",
                     "----- aux file to subdir of output directory, with\n",
                     "----- non-existent subdir\n",
            }
        }

        if ( ($fls_file_analyzed) && (! $analyze_input_log_always) ) {
            # Skip the last part, which is all about finding input
            # file names which should all appear more reliably in the
            # fls file.
            next LINE;
        }
        
        my @new_includes = ();
        
   GRAPHICS_INCLUDE_CANDIDATE:
        while ( /<([^>]+)(>|$)/g ) {
            if ( -f $1 ) { push @new_includes, $1; }
         }  # GRAPHICS_INCLUDE_CANDIDATE:

   INCLUDE_CANDIDATE:
        while ( /\((.*$)/ ) {
        # Filename found by
        # '(', then filename, then terminator.
        # Terminators: obvious candidates: ')':  end of reading file
        #                                  '(':  beginning of next file
        #                                  ' ':  space is an obvious separator
        #                                  ' [': start of page: latex
        #                                        and pdflatex put a
        #                                        space before the '['
        #                                  '[':  start of config file
        #                                        in pdflatex, after
        #                                        basefilename.
        #                                  '{':  some kind of grouping
        # Problem: 
        #   All or almost all special characters are allowed in
        #   filenames under some OS, notably UNIX.  Luckily most cases
        #   are rare, if only because the special characters need
        #   escaping.  BUT 2 important cases are characters that are
        #   natural punctuation
        #   Under MSWin, spaces are common (e.g., "C:\Program Files")
        #   Under VAX/VMS, '[' delimits directory names.  This is
        #   tricky to handle.  But I think few users use this OS
        #   anymore.
        #
        # Solution: use ' [', but not '[' as first try at delimiter.
        # Then if candidate filename is of form 'name1[name2]', then
        #   try splitting it.  If 'name1' and/or 'name2' exists, put
        #   it/them in list, else just put 'name1[name2]' in list.
        # So form of filename is now:
        #  '(', 
        # then any number of characters that are NOT ')', '(', or '{'
        #   (these form the filename);
        # then ' [', or ' (', or ')', or end-of-string.
        # That fails for pdflatex
        # In log file:
        #   '(' => start of reading of file, followed by filename
        #   ')' => end of reading of file
        #   '[' => start of page (normally preceeded by space)
        # Remember: 
        #    filename (on VAX/VMS) may include '[' and ']' (directory
        #             separators) 
        #    filenames (on MS-Win) commonly include space.
        #    filenames on UNIX can included space.
        #    Miktex quotes filenames
        #    But web2c doesn't.  Then 
        #       (string  message
        #    is ambiguous: is the filename "string" or "string message".
        #    Allow both as candidates, since user filenames with spaces 
        #    are rare.  System filenames with spaces are common, but
        #    they are normally followed by a newline rather than messages. 

        # First step: replace $_ by whole of line after the '('
        #             Thus $_ is putative filename followed by other stuff.
            $_ = $1; 
            # Array of new candidate include files; sometimes more than one.
            my $quoted = 0;
            if ( /^\"([^\"]+)\"/ ) {
               # Quoted file name, as from MikTeX
                $quoted = 1;
            }
            elsif ( /^\"/ ) {
                # Incomplete quoted file, as in wrapped line before appending
                # next line
                next LINE;
            }
            elsif ( /^([^\(^\)]*?)\s+[\[\{\<]/ ) {
                # Terminator: space then '[' or '{' or '<'
                # Use *? in condition: to pick up first ' [' (etc) 
                # as terminator
            }
            elsif ( /^([^\(^\)]*)\s+(?=\()/ ) {
                # Terminator is ' (', but '(' isn't in matched string,
                # so we keep the '(' ready for the next match
            }
            elsif  ( /^([^\(^\)]*)(\))/ ) {
                # Terminator is ')'
            }
            else {
                #Terminator is end-of-string
            }
            $_ = $';       # Put $_ equal to the unmatched tail of string '
            my $include_candidate = $1;
            $include_candidate =~ s/\s*$//;   # Remove trailing space.
            if ($quoted) {
            # Remove quotes around filename.
                $include_candidate =~ s/^\"(.*)\"$/$1/;
            }
            elsif ( !$quoted && ($include_candidate =~ /(\S+)\s/ ) ){
                # Non-space-containing filename-candidate
                # followed by space followed by message
                # (Common)
                push @new_includes, $1;
            }
            if ($include_candidate =~ /[\"\'\`]/) {
                # Quote inside filename.  Probably misparse.
                next INCLUDE_CANDIDATE;
            }
            if ( $include_candidate eq "[]" ) {
                # Part of overfull hbox message
                next INCLUDE_CANDIDATE;
            }
            if ( $include_candidate =~ /^\\/ ) {
                # Part of font message
                next INCLUDE_CANDIDATE;
            }

            push @new_includes, $include_candidate;
            if ( $include_candidate =~ /^(.+)\[([^\]]+)\]$/ ) {
                # Construct of form 'file1[file2]', as produced by pdflatex
                if ( -e $1 ) {
                    # If the first component exists, we probably have the
                    #   pdflatex form
                    push @new_includes, $1, $2;
                }
                else {
                    # We have something else.
                    # So leave the original candidate in the list
                }
            }
        } # INCLUDE_CANDIDATE

    INCLUDE_NAME:
        foreach my $include_name (@new_includes) {
            if ($include_name =~ /[\"\'\`]/) {
                # Quote inside filename.  Probably misparse.
                next INCLUDE_NAME;
            }
            $include_name = normalize_filename( $include_name, @pwd_log );
            if ( ! defined $include_name )  { next INCLUDE_NAME; }
            my ($base, $path, $ext) = fileparseB( $include_name );
            if ( ($path eq './') || ($path eq '.\\') ) {
                $include_name = $base.$ext;
            }
            if ( $include_name !~ m'[/|\\]' ) {
                # Filename does not include a path character
                # High potential for misparsed line
                $dependents{$include_name} = 2;
            } else {
                $dependents{$include_name} = 3;
            }
            if ( $ext eq '.bbl' ) {
                warn "$My_name: Found input bbl file '$include_name'\n"
                   unless $silent;
                push @bbl_files, $include_name;
            }
        } # INCLUDE_NAME
    } # LINE

    # Default includes are always definitive:
    foreach (@default_includes) { $dependents{$_} = 4; }

    ###print "New parse: \n";
    ###foreach (sort keys %dependents) { print "  '$_': $dependents{$_}\n"; }

    my @misparsed = ();
    my @missing = ();
    my @not_found = ();

    my %kpsearch_candidates = ();
CANDIDATE:
    foreach my $candidate (keys %dependents) {
        my $code = $dependents{$candidate};
        if ( -d $candidate ) {
            #  If $candidate is directory, it was presumably found from a 
            #     mis-parse, so remove it from the list.  (Misparse can 
            #     arise, for example from a mismatch of latexmk's $log_wrap
            #     value and texmf.cnf value of max_print_line.)
            delete $dependents{$candidate};
        }
        elsif ( -e $candidate ) {
            if ( exists $generated_log{$candidate} ){
                $dependents{$candidate} = 6;
            }
            elsif ($code == 0) {
                $dependents{$candidate} = 5;
            }
            else {
                $dependents{$candidate} = 4;
            }
        }
        elsif ($code == 1) {
            # Graphics file that is supposed to have been read.
            # Candidate name is as given in source file, not as path
            #   to actual file.
            # We have already tested that file doesn't exist, as given.
            #   so use kpsewhich.  
            # If the file still is not found, assume non-existent;
            $kpsearch_candidates{$candidate} = 1;
            delete $dependents{$candidate};
        }
        elsif ($code == 2) {
            # Candidate is from '(...' construct in log file, for input file
            #    which should include pathname if valid input file.
            # Name does not have pathname-characteristic character (hence
            #    $code==2.
            # We get here if candidate file does not exist with given name
            # Almost surely result of a misparsed line in log file.
            delete $dependents{$candidate};
            push @misparse, $candidate;
        }
        elsif ($code == 3) {
            # Candidate is from '(...' construct in log file, for input file
            #    which should include pathname if valid input file.
            # Name does have pathname-characteristic character (hence
            #    $code==3.
            # But we get here only if candidate file does not exist with 
            # given name.  
            # Almost surely result of a misparsed line in log file.
            # But with lower probability than $code == 2
            delete $dependents{$candidate};
            push @misparse, $candidate;
        }
        elsif ($code == 0) {
            my ($base, $path, $ext) = fileparseA($candidate);
            $ext =~ s/^\.//;
            if ( ($ext eq '') && (-e "$path$base.tex") ) {
                # I don't think the old version was correct.
                # If the missing-file report was of a bare
                #    extensionless file, and a corresponding .tex file
                #    exists, then the missing file does not correspond
                #    to the missing file, unless the .tex file was
                #    created during the run.  
                # OLD $dependents{"$path$base.tex"} = 4;
                # OLD delete $dependents{$candidate};
                # NEW:
                $dependents{"$path$base.tex"} = 4;
            }
            push @missing, $candidate;
        }
    }

    my @kpsearch_candidates = keys %kpsearch_candidates;
    if (@kpsearch_candidates) {
        foreach my $result ( kpsewhich( @kpsearch_candidates ) ) {
            $dependents{$result} = 4;
        }
    }
        
CANDIDATE_PAIR:
    foreach my $delegated_source (keys %new_conversions) {
        my $delegated_output = $new_conversions{$delegated_source};
        my $rule = "Delegated $delegated_source, $delegated_output";
        # N.B. $delegated_source eq '' means the output file
        #      was created without a named input file.
        foreach my $candidate ($delegated_source, $delegated_output) {
            if (! -e $candidate ) {
                # The file might be somewhere that can be found
                #   in the search path of kpathsea:
                my @kpse_result = kpsewhich( $candidate,);
                if ($#kpse_result > -1) {
                    $candidate = $kpse_result[0];
                }
            }
        }
        if ( ( (-e $delegated_source) || ($delegated_source eq '') )
              && (-e $delegated_output) )
        {
            $conversions{$delegated_output} = $delegated_source;
            $dependents{$delegated_output} = 7;
            if ($delegated_source) {
                $dependents{$delegated_source} = 4;
            }
        }
        elsif (!$silent) {
            print "Logfile claimed conversion from '$delegated_source' ",
                  "to '$delegated_output'.  But:\n";
            if (! -e $delegated_output) {
                print  "   Output file does not exist\n";
            }
            if ( ($delegated_source ne '') && (! -e $delegated_source) ) {
                print  "   Input file does not exist\n";
            }
        }
    }

    if ( ($#warning_list >= 0) && !$log_silent ) {
        @warning_list = uniqs( @warning_list );
        show_array( "$My_name: List of undefined refs and citations:",
                    @warning_list );
    }
    
    if ( $diagnostics ) {
        @misparse = uniqs( @misparse );
        @missing = uniqs( @missing );
        @not_found = uniqs( @not_found );
        my @dependents = sort( keys %dependents );

        my $dependents = $#dependents + 1;
        my $misparse = $#misparse + 1;
        my $missing = $#missing + 1;
        my $not_found = $#not_found + 1;
        my $exist = $dependents - $not_found - $missing;
        my $bbl = $#bbl_files + 1;

        print "$dependents dependent files detected, of which ",
              "$exist exist, $not_found were not found,\n",
              "   and $missing appear not to exist.\n";
        print "Dependents:\n";
        foreach (@dependents) { 
            print "   '$_' "; 
            if ( $dependents{$_} == 6 ) { print " written by *latex";}
            if ( $dependents{$_} == 7 ) { print " converted by *latex";}
            print "\n";
        }
        if ($not_found > 0) {
            print "Not found:\n";
            foreach (@not_found) { print "   $_\n"; }
        }
        if ($missing > 0) {
            print "Not existent:\n";
            foreach (@missing) { print "   $_\n"; }
        }
        if ( $bbl > 0 ) {
            print "Input bbl files:\n";
            foreach (@bbl_files) { print "   $_\n"; }
        }

        if ( $misparse > 0 ) {
            print "Possible input files, perhaps from misunderstood lines in .log file:\n";
            foreach ( @misparse ) { print "   $_\n"; }
        }
    }
    return 1;
} #END parse_log

#************************************************************

sub find_set_log {
    # Locate the log file, if possible.  This allows for possible configuration
    # errors, e.g., because the command for (*)latex was such that it did not 
    # do the setting of -output-directory or -aux-directory that the user intended,
    # or because the version used did not support one or other of these options.
    # Put result in $where_log (see its initial declaration/definition for details).
    # Change $aux_dir and/or $out_dir as appropriate, and make consequent changes.
    #
    # Probably further attention to location of output file (.dvi, .pdf, or .xdv)
    # could be done, to get $out_dir and $$Pdest more accurately set.
    #
    # Typical configuration errors that lead to the need for this subroutine:
    #        %O not used in command definition, so directory options don't getpassed
    #           to (*)latex.
    #        Use of $aux_dir different to $out_dir, when (*)latex doesn't support
    #           the -aux-directory option (notably with TeXLive distribution).
    if ($where_log == 1) {
        # .log file was found in correct place on previous run.
        # So there's no need to repeat search, since if the location were to
        # change from run to run, we'd have other serious difficulties that are
        # to hard to deal with.
        return;
    }
    if ( test_gen_file( "$aux_dir1$root_filename.log" ) ) {
        # .log file is in expected place.
        $where_log = 1;
    }
    elsif ( test_gen_file( "$out_dir1$root_filename.log" ) ) {
        # .log file is in out_dir not in aux_dir.
        # Presumably there is a configuration error
        # that prevents aux_dir from being used by latex.
        warn "$My_name: .log file in '$out_dir' instead of expected '$aux_dir'\n";
        if ($emulate_aux) {
            warn "    But emulate_aux is on, so that should not happen\n",
                 "    I'll switch aux_dir to equal out_dir\n";
            $where_log = 2;
            $aux_dir = $out_dir;
        }
        else {
            warn "    But emulate_aux is off.  So I'll turn it on.\n";
            $emulate_aux = 1;
            $emulate_aux_switched = 1;
            foreach ( $$Pext_cmd ) {
                s/ -output-directory=[^ ]*(?= )//g;
                s/ -aux(-directory=[^ ]*)(?= )/ -output$1/g;
            }
        }
    }
    elsif ( test_gen_file( "$root_filename.log" ) ) {
        # .log file is not in out_dir nor in aux_dir, but is in cwd.
        # Presumably there is a configuration error
        # that prevents the directories from being used by latex.
        # So change $aux_dir to the actually used value.
        $where_log = 3;
        $aux_dir = "";
    }
    else {
        # No .log file found
        $failure = 1;
        $$Plast_result = 2;
        $where_log = 0;
        $failure_msg 
            = "*LaTeX didn't generate the expected log file '$log_name'\n";
    }
    if ($where_log > 1) {
        warn "$My_name: Changed aux_dir from '$aux_dir_requested' to '$aux_dir'\n".
             "          to allow for probable configuration error\n";
        # Allow for the changes associated with change of $aux_dir:
        &normalize_aux_out_ETC;
        &set_names;
        warn "$My_name: Actual .log file is\n",
             "     '$log_name'\n",
             "  instead of the value\n",
             "     '$aux_dir_requested/$root_filename.log'\n",
             "   that seemed to be intended.\n";
    }
} #END find_set_log

#************************************************************

sub parse_fls {
    my $start_time = processing_time();  
    my ($fls_name, $Pinputs, $Poutputs, $Pfirst_read_after_write, $Ppwd_latex ) = @_;
    %$Pinputs = %$Poutputs = %$Pfirst_read_after_write = ();
    my $fls_file = new FileHandle;
    # Make a note of current working directory
    # I'll update it from the fls file later
    # Currently I don't use this, but it would be useful to use
    # this when testing prefix for cwd in a filename, by
    # giving *latex's best view of the cwd.  Note that the
    # value given by the cwd() function may be mangled, e.g., by cygwin
    # compared with native MSWin32.
    #
    # Two relevant forms of cwd exist: The system one, which we can find, and
    # the one reported by *latex in the fls file.  It will be
    # useful to remove leading part of cwd in filenames --- see the
    # comments in sub rdb_set_latex_deps.  Given the possible multiplicity
    # of representations of cwd, the one reported in the fls file should
    # be definitive in the fls file.

    my $cwd = good_cwd();
    if ( ! open ($fls_file, "<$fls_name") ) {
        return 1;
    }

    my $pdf_base = basename($pdf_name);
    my $log_base = basename($log_name);
    my $out_base = basename($$Pdest);

    foreach $_ ( <$fls_file> ) {
        # Remove trailing CR and LF. Thus we get correct behavior when an fls file
        #  is produced by MS-Windows program (e.g., in MiKTeX) with CRLF line ends,
        #  but is read by Unix Perl (which treats LF as line end, and preserves CRLF
        #  in read-in lines):
        $_ =~ s/[\n\r]*$//;
        if (/^\s*PWD\s+(.*)$/) {
            my $cwd_fls = $1;
            $$Ppwd_latex = $cwd_fls;
            if ( $cwd_fls =~ /\"/ ) {
                warn "$My_name: The working directory has a '\"' character in its name:\n",
                     "  '$cwd'\n  This can cause me trouble. Beware!\n";
            }
            if ( normalize_filename($cwd_fls) ne normalize_filename($cwd) ) {
                print "$My_name: ============== Inequiv cwd_fls cwd '$cwd_fls' '$cwd'\n";
            }
        }
        elsif (/^\s*INPUT\s+(.*)$/) {
            # Take precautions against aliasing of foo, ./foo and other possibilities for cwd.
            my $file = $1;
            # Remove exactly pwd reported in this file, and following separator.
            # MiKTeX reports absolute pathnames, and this way of removing PWD insulates
            #   us from coding issues if the PWD contains non-ASCII characters.  What
            #   coding scheme (UTF-8, code page, etc) is used depends on OS, TeX
            #   implementation, ...
            if ( defined $$Ppwd_latex ) { 
                $file =~ s(^\Q$$Ppwd_latex\E[\\/])();
            }
            $file = normalize_filename( $file );
            if ( (exists $$Poutputs{$file}) && (! exists $$Pinputs{$file}) ) {
                $$Pfirst_read_after_write{$file} = 1;
            }
            # Take precautions against main destination file being listed as INPUT file
            # This results, e.g., from hyperxmp (2020/10/05 v. 5.6) reading the pdf file
            # size, and triggers an infinite loop, unless we omit the pdf file from the 
            # list of input files.  (Hyperxmp v. 5.7 2010/11/01 doesn't give this problem.)
            # There's a related issue with the log file, when acmart.cls is used with
            # xelatex.  (I don't work out what causes this, e.g., what package.)
            # Test on basenames rather than full name to evade in a simple-minded way
            # alias issues with the directory part.
            if ( basename($file) eq $pdf_base ) {
                warn "$My_name: !!!!!!!!!!! Fls file lists main pdf **output** file as an input\n",
                     "   file for rule '$rule'. I won't treat as a source file, since that leads\n",
                     "   to an infinite loop.\n",
                    "    This can be caused by the hyperxmp package in an old version.\n",
                    "    You should update to hyperxmp in ver. 5.7 or higher\n";
            } elsif ( basename($file) eq $out_base ) {
                warn "$My_name: !!!!!!!!!!! Fls file lists main **output** file as an input\n",
                     "   file for rule '$rule'. I won't treat as a source file, since that leads\n",
                     "   to an infinite loop.\n",
                    "    This can be caused by the hyperxmp package in an old version.\n",
                    "    You should update to hyperxmp in ver. 5.7 or higher\n";
            } elsif ( basename($file) eq $log_base ) {
                warn "$My_name: !!!!!!!!!!! Fls file lists log file as an input\n",
                     "   file for rule '$rule'. I won't treat it as a source file, since\n",
                    "   there appear to be no good uses for it.\n",
                    "   This behavior happens at least under acmart.cls with xelatex\n";
            } else {
                $$Pinputs{$file} = 1;
            }
        }
        elsif (/^\s*OUTPUT\s+(.*)$/) {
            # Take precautions against aliasing of foo, ./foo and other possibilities for cwd.
            my $file = $1;
            $file =~ s(^\Q$$Ppwd_latex\E[\\/])();
            $file = normalize_filename( $file );
            $$Poutputs{$file} = 1;
        }
    }
    close( $fls_file );
    return 0;
} #END parse_fls

#************************************************************

sub dirname_no_tail {
    my $dirname = $_[0];
    foreach ($dirname) {
        # Normalize name to use / to separate directory components:
        #   (Note both / and \ are allowed under MSWin.)
        s(\\)(/)g;
        # Change multiple trailing / to single /
        #   (Note internal // or \\ can have special meaning on MSWin)
        s(/+$)(/);
        # Remove trailing /,
        # BUT **not** if that changes the semantics, i.e., if name is "/" or "C:/".
        if ( m(/$) ) {
            if ( ( ! m(^/+$) ) && ( ! m(:/+$) ) ) {
                s(/$)();
            }
        }
    }
    return $dirname;
}

#************************************************************

sub clean_filename {
    # Convert quoted filename as found in log file to filename without quotes
    # Allows arbitrarily embedded double-quoted substrings, includes the
    # cases
    # 1. `"string".ext', which arises e.g., from \jobname.bbl:
    #    when the base filename contains spaces, \jobname has quotes.
    #    and from \includegraphics with basename specified.
    #    Also deals with filenames written by asymptote.sty
    # 2. Or "string.ext" from \includegraphcs with basename and ext specified.
    #    and from MiKTeX logfile for input files with spaces. 
    # Doubled quotes (e.g., A""B) don't get converted.
    # Neither do unmatched quotes.
    my $filename = $_[0];
    while ( $filename =~ s/^([^\"]*)\"([^\"]+)\"(.*)$/$1$2$3/ ) {}
    return $filename;
}

# ------------------------------

sub normalize_filename {
   # Usage: normalize_filename( filename [, extra forms of name of cwd] )
   # Returns filename with removal of various forms for cwd, and
   # with conversion of directory separator to '/' only.
   # Also when filename is name of a directory, with a trailing '/',
   #   the trailing '/' is removed.
   #
   my ( $file, @dirs ) = @_;
   my $file1 = $file;   # Saved original value
   my $cwd = good_cwd();
   # Normalize files to use / to separate directory components:
   # (Note both / and \ are allowed under MSWin.)
   foreach ($cwd, $file,  @dirs) {
       s(\\)(/)g;
       # If this is directory name of form :.../", remove unnecessary
       # trailing directory separators:
       $_ = dirname_no_tail( $_ );
   }
   
   # Remove initial component equal to current working directory.
   # Use \Q and \E round directory name in regex to avoid interpretation
   #   of metacharacters in directory name:
   foreach my $dir ( @dirs, '.', $cwd ) {
       if ( $dir =~ /^\s*$/ ) {
           # All spaces, nothing to do.
           next;
       }
       if ($file eq $dir) {
           # Filename equals cwd, so it is . relative to cwd:
           $file = '.';
           last;
       }
       if ( $file =~ s(^\Q$dir\E/)() ) {
           last;
     }
   }
   if ($file eq '' ) {
       # This only occurs for $file equal to a directory that
       # is the cwd. Our convention is always to set it to '.'
       # 
       $file = '.';
   }
   return $file;
} #END normalize_filename

# ------------------------------

sub normalize_filename_abs {
    # Convert filename to be either
    # absolute path in canonical form
    # or relative to cwd.
    return normalize_filename( abs_path($_[0]) );
}

#-----------------------------

sub normalize_clean_filename {
   # Usage: normalize_clean_filename( filename [, extra forms of name of cwd] )
   # Same as normalize_filename, but first remove any double quotes, as
   # done by clean_filename, which is appropriate for filenames from log file.
    my ($file, @dirs) = shift;
    return normalize_filename( clean_filename( $file ) , @dirs );
}

#************************************************************

sub fix_pattern {
   # Escape the characters [ and {, to give a pattern for use in glob
   #    with these characters taken literally.
   my $pattern = shift;
   $pattern =~ s/\[/\\\[/g;
   $pattern =~ s/\{/\\\{/g;
   return $pattern;
}

#************************************************************

sub parse_aux {
    #Usage: parse_aux( $aux_file, \@new_bib_files, \@new_aux_files, \@new_bst_files )
    # Parse aux_file (recursively) for bib files, and bst files.  
    # If can't open aux file, then
    #    Return 0 and leave @new_bib_files empty
    # Else set @new_bib_files from information in the aux files
    #    And:
    #    Return 1 if no problems
    #    Return 2 with @new_bib_files empty if there are no \bibdata
    #      lines. 
    #    Return 3 if I couldn't locate all the bib_files
    # Set @new_aux_files to aux files parsed

    my $aux_file = $_[0];
    local $Pbib_files = $_[1];
    local $Paux_files = $_[2];
    local $Pbst_files = $_[3];
   
    @$Pbib_files = ();
    @$Pbst_files = ();
    @$Paux_files = ();

    parse_aux1( $aux_file );
    if ($#{$Paux_files} < 0) {
       return 0;
    }
    @$Pbib_files = uniqs( @$Pbib_files );
    @$Pbst_files = uniqs( @$Pbst_files );

    if ( $#{$Pbib_files} == -1 ) {
        warn "$My_name: No .bib files listed in .aux file '$aux_file' \n",
        return 2;
    }
    my @not_found = &find_file_list1( $Pbib_files, $Pbib_files,
                                      '.bib', \@BIBINPUTS );
    @$Pbib_files = uniqs( @$Pbib_files );
    &find_file_list1( $Pbst_files, $Pbst_files, '.bst' );
    @$Pbst_files = uniqs( @$Pbst_files );
    my @bad_bib = ();
    foreach ( @$Pbib_files ) {
        if ( /\s/ ) { push @bad_bib, $_; }
    }
    if ($#bad_bib >= 0)  {
            warn "$My_name: White space in an argument list for \\bibliography.\n",
                 "    which is not allowed by bibtex.  Bad arguments:\n";
            foreach (@bad_bib ) { warn "    '$_'\n"; }
            return 3;
    }
    if ( $#not_found < 0) {
        warn "$My_name: Found bibliography file(s) [@$Pbib_files]\n"
        unless $silent;
    }
    else {
        warn "$My_name: Failed to find one or more bibliography files:\n";
        foreach (@not_found) { warn "    '$_'\n"; }
        if ($force_mode) {
            warn "==== Force_mode is on, so I will continue.  ",
                 "But there may be problems ===\n";
        }
        return 3;
    }
    return 1;
} #END parse_aux

#************************************************************

sub parse_aux1
# Parse single aux file for bib files.  
# Usage: &parse_aux1( aux_file_name )
#   Append newly found bib_filenames in @$Pbib_files, already 
#        initialized/in use.
#   Append aux_file_name to @$Paux_files if aux file opened
#   Recursively check \@input aux files
#   Return 1 if success in opening $aux_file_name and parsing it
#   Return 0 if fail to open it
{
   my $aux_file = $_[0];
   my $aux_fh = new FileHandle;
   if (! open($aux_fh, $aux_file) ) { 
       warn "$My_name: Couldn't find aux file '$aux_file'\n";
       return 0; 
   }
   push @$Paux_files, $aux_file;
AUX_LINE:
   while (<$aux_fh>) {
      if ( /^\\bibdata\{(.*)\}/ ) { 
          # \\bibdata{comma_separated_list_of_bib_file_names}
          # These are normally without the '.bib' extension.
          push @$Pbib_files, split /,/, $1;
      }
      elsif ( /^\\bibstyle\{(.*)\}/ ) { 
          # \\bibstyle{bst_file_name}
          # Normally without the '.bst' extension.
          push @$Pbst_files, split /,/, $1;
      }
      elsif ( /^\\\@input\{(.*)\}/ ) { 
          # \\@input{next_aux_file_name}
          &parse_aux1( $aux_dir1.$1 );
      }
      else {
          foreach my $Psub (@aux_hooks) {
              &$Psub;
          }
      }
   }
   close($aux_fh);
   return 1;
} #END parse_aux1

#************************************************************

#************************************************************
#************************************************************
#************************************************************

#   Manipulations of main file database:

#************************************************************

sub fdb_get {
    # Call: fdb_get(filename [, check_time])
    # Returns an array (time, size, md5) for the current state of the
    #    named file.
    # The optional argument check_time is either the run_time of some command
    #    that may have changed the file or the last time the file was checked
    #    for changes --- see below.
    # For non-existent file, deletes its entry in fdb_current, 
    #    and returns (0,-1,0) (whatever is in @nofile).
    # As an optimization, the md5 value is taken from the cache in 
    #    fdb_current, if the time and size stamp indicate that the 
    #    file has not changed.
    # The md5 value is recalculated if
    #    the current filetime differs from the cached value: 
    #               file has been written
    #    the current filesize differs from the cached value: 
    #               file has definitely changed
    # But the file can also be rewritten without change in filetime when 
    #    file processing happens within the 1-second granularity of the 
    #    timestamp (notably for aux files from latex on a short source file).
    # The only case that concerns us is when the file is an input to a program
    #    at some runtime t, the file is rewritten later by the same or another
    #    program, with timestamp t, and when the initial file also has 
    #    timestamp t.
    # A test is applied for this situation if the check_time argument is
    #    supplied and is nonzero.

    my ($file, $check_time) = @_;
    if ( ! defined $check_time ) { $check_time = 0;}
    my ($new_time, $new_size) = get_time_size($file);
    if ( $new_size < 0 ) {
        delete $fdb_current{$file};
        return @nofile;
    }
    my $recalculate_md5 = 0;
    if ( ! exists $fdb_current{$file} ) {
        # Ensure we have a record.  
        $fdb_current{$file} = [@nofile];
        $recalculate_md5 = 1;
    }
    my $file_data = $fdb_current{$file};
    my ( $time, $size, $md5 ) = @$file_data;

    if ( ($new_time != $time) || ($new_size != $size) 
         || ( $check_time && ($check_time == $time ) )
       ) {
        # Only force recalculation of md5 if time or size changed.
        # However, the physical file time may have changed without
        #   affecting the value of the time coded in $time, because
        #   times are computed with a 1-second granularity.
        #   The only case to treat specially is where the file was created,
        #   then used by the current rule, and then rewritten, all within
        #   the granularity size, otherwise the value of the reported file
        #   time changed, and we've handled it.  But we may have already
        #   checked this at an earlier time than the current check.  So the
        #   only dangerous case is where the file time equals a check_time,
        #   which is either the run_time of the command or the time of a
        #   previous check.
        # Else we assume file is really unchanged.
        $recalculate_md5 = 1;
    }
    if ($recalculate_md5) {
        @$file_data = ( $new_time, $new_size, get_checksum_md5( $file ) );
    }
    return @$file_data;;
} #END fdb_get

#************************************************************

sub fdb_set {
    # Call: fdb_set(filename, $time, $size, $md5 )
    # Set data in file data cache, i.e., %fdb_current
    my ($file, $time, $size, $md5 ) = @_;
    if ( ! exists $fdb_current{$file} ) {
        $fdb_current{$file} = [@nofile];
    }
    @{$fdb_current{$file}} = ( $time, $size, $md5 );
} #END fdb_set

#************************************************************

sub fdb_show {
    # Displays contents of fdb
    foreach my $file ( sort keys %fdb_current ) {
        print "'$file': @{$fdb_current{$file}}\n";
    }
} #END fdb_show

#************************************************************
#************************************************************
#************************************************************

# Routines for manipulating rule database

#************************************************************

sub rdb_read {
    # Call: rdb_read( $in_name  )
    # Sets rule database from saved file, in format written by rdb_write.
    # Returns -1 if file could not be read else number of errors.
    # Thus return value on success is 0
    # Requires: Rule database initialized with standard rules, with
    #             conditions corresponding to requests determined by
    #             initialization and command line options.
    # Asssumption: Normally the fdb_latexmk file contains state of
    #                rules and files corresponding to end of last
    #                compilation, and the rules in the file were
    #                active on that run.
    # Complications arise when that state does not correspond to current
    #   rule set:
    #   (a) Configuration etc may have changed: e.g., different out_dir,
    #       different target rules and files, including different tex engine.
    #   (b) Output extension of primary rule may be different from current
    #       initialized one, because of document properties (use of
    #       \pdfoutput etc).
    #   (c) The same may arise because of misconfigured rules, a situation
    #       that may or may not have changed in current run.
    #   (d) The primary engine requested may not be the one used in
    #       the previous run, possibly because (i) request has
    #       changed, or (ii) document metacommand was obeyed to change
    #       engine. (The last is not currently implemented, but
    #       may/should be in the future.)
    #   (e) Something else, e.g., copying/editing of fdb_latexmk file.
    #
    local $in_name = $_[0];
    my $in_handle = new FileHandle;
    $in_handle->open( $in_name, '<' )
        or return ();
    my $errors = 0;
    my $state = -1;   # Values: -1: before start; 0: outside rule;
                      # 1: in source section;
                      # 2: in generated file section;
                      # 10: ignored rule.
    my $rule = '';
    local $run_time = 0;
    local $source = '';
    local $dest = '';
    my $base = '';
    my %old_actives = (); # Hash: keys are rules in fdb_latexmk file
    local %new_sources = ();  # Hash: rule => { file=>[ time, size, md5, fromrule ] }
    my $new_source = undef;   # Reference to hash of sources for current rule
LINE:
    while ( <$in_handle> ) {
        # Remove leading and trailing white space.
        s/^\s*//;
        s/\s*$//;
        if ($state == -1) {
            if ( ! /^# Fdb version ([\d]+)$/ ) {
                warn "$My_name: File-database '$in_name' is not of correct format\n";
                return 1;
            }
            if ( $1 > $fdb_ver) {
                warn "$My_name: File-database '$in_name' is of too new version, $1 > $fdb_ver\n";
                return 1;
            }
            $state = 0;
        }
        # Ignore blank lines and comments
        if ( /^$/ || /^#/ || /^%/ ) { next LINE;}
        if ( /^\[\"([^\"]+)\"\]/ ) {
            # Start of section
            $rule = $1;
            my $tail = $'; #'  Single quote in comment tricks the parser in
                           # emacs from misparsing an isolated single quote
            $run_time = $check_time = 0;
            $source = $dest = $base = '';
            $old_actives{$rule} = 1;
            if ( $tail =~ /^\s*(\S+)\s*$/ ) {
                $run_time = $1;
            }
            elsif ( $tail =~ /^\s*(\S+)\s+\"([^\"]*)\"\s+\"([^\"]*)\"\s+\"([^\"]*)\"\s*$/ ) {
                $run_time = $1;
                $source = $2;
                $dest = $3;
                $base = $4;
            }
            elsif ( $tail =~ /^\s*(\S+)\s+\"([^\"]*)\"\s+\"([^\"]*)\"\s+\"([^\"]*)\"\s+(\S+)\s*$/ ) {
                $run_time = $1;
                $source = $2;
                $dest = $3;
                $base = $4;
                $check_time = $5;
            }
            if ( rdb_rule_exists( $rule ) ) {
                rdb_one_rule( $rule, \&rdb_read_set_rule );
            }
            elsif ($rule =~ /^cusdep\s+(\S+)\s+(\S+)\s+(.+)$/ ) {
                # Create custom dependency
                my $fromext = $1;
                my $toext = $2;
                my $base = $3;
                $source = "$base.$fromext";
#                $dest =   "$base.$toext";
                my $func_name = '';
                foreach my $dep ( @cus_dep_list ) {
                    my ($tryfromext,$trytoext,$must,$try_func_name) = split('\s+',$dep);
                    if ( ($tryfromext eq $fromext) && ($trytoext eq $toext) ) {
                        $func_name = $try_func_name;
                    }
                }
                if ($func_name) {
                    my $PAnew_cmd = ['do_cusdep', $func_name];
                    # Set source file as non-existent.  
                    # If it existed on last run, it will be in later 
                    #    lines of the fdb file
                    rdb_create_rule( $rule, 'cusdep', '', $PAnew_cmd, 1, 
                                     $source, $dest, $base, 0, $run_time, $check_time, 1 );
                }
                else {
                    warn "$My_name: In file-database '$in_name', the custom-dependency rule\n",
                         "  '$rule' is not available in this session.\n",
                         "  Presumably it's no longer in your configuration for latexmk.\n";
                    $state = 10;
                    next LINE;
                }
            }
            elsif ( $rule =~ /^(makeindex|bibtex|biber)\s*(.*)$/ ) {
                my $PA_extra_gen = [];
                my $rule_generic = $1;
                my $int_cmd = '';
                if ( ! $source ) {
                    # If fdb_file was old-style (v. 1)
                    $source = $2;
                    my $path = '';
                    my $ext = '';
                    ($base, $path, $ext) = fileparseA( $source );
                    $base = $path.$base;
                    if ($rule_generic eq 'makeindex') {
                        $dest = "$base.ind";
                    }
                    elsif ($rule_generic eq 'bibtex') {
                        $dest = "$base.bbl";
                        $source = "$base.aux";
                    }
                    elsif ($rule_generic eq 'biber') {
                        $dest = "$base.bbl";
                        $source = "$base.bcf";
                    }
                }
                if ($rule =~ /^makeindex/) { $PA_extra_gen = [ "$base.ilg" ]; }
                if ($rule =~ /^(bibtex|biber)/) { $PA_extra_gen = [ "$base.blg" ]; }
                if ($rule =~ /^bibtex/) { $int_cmd = "run_bibtex"; }
                if ($rule =~ /^makeindex/) { $int_cmd = "run_makeindex"; }
                warn "$My_name: File-database '$in_name': setting rule '$rule'\n"
                   if $diagnostics;
                my $cmd_type = 'external';
                my $ext_cmd = ${$rule_generic};
                warn "  Rule kind = '$rule_generic'; ext_cmd = '$ext_cmd';\n",
                     "  int_cmd = '$int_cmd';\n",
                     "  source = '$source'; dest = '$dest'; base = '$base';\n"
                   if $diagnostics;
                # Set source file as non-existent.  
                # If it existed on last run, it will be in later 
                #    lines of the fdb file
                rdb_create_rule( $rule, $cmd_type, $ext_cmd, $int_cmd, 1, 
                                 $source, $dest, $base, 0, $run_time,  $check_time, 1, $PA_extra_gen );
            }
            else {
                if ($diagnostics) {
                    warn "$My_name: In file-database '$in_name' rule '$rule'\n",
                        "   is not in use in this session\n";
                }
                $new_source = undef;
                $state = 10;
                next LINE;
            }
            $new_source = $new_sources{$rule} = {};
            $state = 1;  #Reading a section, source part
        }
        elsif ( ($state <=0) || ($state >= 3) ) {
            next LINE;
        }
        elsif ( /^\(source\)/ ) { $state = 1; next LINE; }
        elsif ( /^\(generated\)/ ) { $state = 2; next LINE; }
        elsif ( ($state == 1) && /^\"([^\"]*)\"\s+(\S+)\s+(\S+)\s+(\S+)\s+\"([^\"]*)\"/ ) {
            # Source file line
            my $file = $1;
            my $time = $2;
            my $size = $3;
            my $md5 = $4;
            my $from_rule = $5;
            if ($state != 1) {
                warn "$My_name: In file-database '$in_name' ",
                     "line $. is outside a section:\n   '$_'\n";
                $errors++;
                next LINE;
            }
            # Set file in database.  But ensure we don't do an unnecessary 
            #    fdb_get, which can trigger a new MD5 calculation, which is
            #    lengthy for a big file.  Ininitially flagging the file
            #    as non-existent solves the problem:
            rdb_ensure_file( $rule, $file, undef, 1 ); 
            rdb_set_file1( $rule, $file, $time, $size, $md5 );
            fdb_set( $file, $time, $size, $md5 );
            # Save the rest of the data, especially the from_rule until we know all 
            #   the rules, otherwise the from_rule may not exist.
            # Also we'll have a better chance of looping through files.
            ${$new_source}{$file} = [ $time, $size, $md5, $from_rule ];
        }
        elsif ( ($state == 2) && /^\"([^\"]*)\"/ ) {
            my $file = $1;
            rdb_one_rule( $rule, sub{ rdb_add_generated($file); } );
        }
        else {
            warn "$My_name: In file-database '$in_name' ",
                 "line $. is of wrong format:\n   '$_'\n";
            $errors++;
            next LINE;
        }
    }
    undef $in_handle;
    # Set cus dependencies.
    &rdb_set_dependents( keys %rule_db );
    &rdb_set_rule_net;

    return $errors;
}  # END rdb_read

#************************************************************

sub rdb_read_set_rule {
    # Rule context assumed.  Implicit passing of $dest, $run_time, $check_time,
    # $in_name used as local variables in calling routine rdb_read;
    if ($$Ptest_kind == 3) { $$Ptest_kind = 1; }
    $$Prun_time = $run_time;
    $$Pcheck_time = $check_time;
    # Deal with possibility that destination in fdb_latexmk has different name
    # than the default one.  The only case that concerns us is where
    # the extension is changed (by \pdfoutput, e.g., in tex file).  But
    # it is possible out and aux directories have been chosen differently,
    # and the user choice there MUST OVERRIDE the value in the fdb_latexmk file.
    if ($dest ne $$Pdest) {
        if (! $possible_primaries{$rule} ) {
            warn "$My_name: In reading rule '$rule' in '$in_name',\n",
                 "  name of destination file is not current one; I'll flag rule as out of date.\n";
            $$Pout_of_date = 10;
        }
        elsif ( ! rdb_is_active($rule) ) {
            warn "$My_name: In reading rule '$rule' in '$in_name',\n",
                 "  rule is not currently active.\n";
            # No fixup now. Causes to be analyzed:
            # Change of requested files: no action needed.
            # Obeying of metacommand: not implemented yet.
        }
        else {
            # Get here if rule is active and primary and destination is different
            warn "$My_name: In reading rule '$rule' in '$in_name',\n",
                 "  destination has different name than configured...\n";
            my ($oldbase, $oldpath, $oldext) = fileparseA( $dest );
            my ($newbase, $newpath, $newext) = fileparseA( $$Pdest );
            if ($oldext ne $newext) {
                if ( ! exists $allowed_output_ext{$oldext} ) {
                    warn "  Old extension '$oldext' not allowed.\n";
                    $$Pout_of_date = 10;
                }
                else {
                    warn "  ===== CHANGING output type from '$newext' to '$oldext' in '$rule'\n";
                    my $switch_error =  switch_output( $rule, $oldext, $newext );
                    if ($switch_error) {
                        warn "   I could not accommodate the changed output extension.\n",
                             "   That is either because the configuration does not allow it\n",
                             "   or because there is a conflict with implicit or explicit requested filetypes.\n",
                             "   (Typically that is about .dvi and/or .ps filetypes.)\n",
                             "===> There may be subsequent warnings, which may or may not be ignorable.\n",
                             "===> If necessary, clean out generated files and try again\n";
                    }
                }
            }
            if ( ($oldbase ne $newbase) || ($oldpath ne $newpath) ) {
                # There are further issues (e.g., change of out_dir).
                # Need rerun to correct:
                $$Pout_of_date = 10;
            }
        }
    }
}  #END rdb_read_set_rule

#************************************************************

sub rdb_write {
    # Call: rdb_write( $out_name )
    # Writes to the given file name the database of file and rule data
    #   for all rules needed to make final output
    # Returns 1 on success, 0 if file couldn't be opened.
    local $out_name = $_[0];
    local $out_handle = new FileHandle;
    if ( ($out_name eq "") || ($out_name eq "-") ) {
        # Open STDOUT
        $out_handle->open( '>-' );
    }
    else {
       $out_handle->open( $out_name, '>' );
    }
    if (!$out_handle) { return 0; }

    &rdb_set_rule_net;

    print $out_handle "# Fdb version $fdb_ver\n";
    my @rules = sort &rdb_accessible;
    rdb_for_some(
       \@rules,
       sub { 
           # Omit data on a unused and never-run primary rule:
           if ( ($$Prun_time == 0) 
                && exists( $possible_primaries{$rule} )
                && ! exists( $current_primaries{$rule} )
              )
           { 
               return;
           }
           print $out_handle "[\"$rule\"] $$Prun_time \"$$Psource\" \"$$Pdest\" \"$$Pbase\" $$Pcheck_time\n";
           rdb_do_files(
             sub { print $out_handle "  \"$file\" $$Ptime $$Psize $$Pmd5 \"$$Pfrom_rule\"\n"; }
           );
           print $out_handle "  (generated)\n";
           foreach (keys %$PHdest) {
               print $out_handle "  \"$_\"\n";
           }
       }
    );
    undef $out_handle;
    return 1;
} #END rdb_write

#************************************************************

sub rdb_set_latex_deps {
    # Assume primary rule context.  
    # This is intended to be applied only for a primary (LaTeX-like) rule.
    # Set its dependents etc, using information from log, aux, and fls files.
    # Use fls file only if $recorder is set, and the fls file was generated
    # on this run.

    # N.B.  A complication which we try and handle in determining
    #   dependent files is that there may be aliasing of file names,
    #   especially when characters are used in file and directory
    #   names that are not pure 7-bit-ASCII.  Here is a list of some
    #   of the difficulties that do arise, between, on the one hand,
    #   the filenames specified on latexmk's and the cwd found by
    #   latexmk from the system, and, on the other hand, the filenames
    #   and their components reported by *latex in the fls and log
    #   files:
    #      1. Whether the separator of path components is / or \ in
    #         MSWin.
    #      2. Whether the LFN or the SFN is provided.
    #      3. Whether the filenames include the cwd or whether they
    #         are relative to the current directory.
    #      4. Under cygwin, whether the absolute filenames are
    #         specified by UNIX or native MSWin conventions.
    #         (With cygin, the programs used, including the Perl that
    #         executes latexmk, can be any combination of native MSWin
    #         programs and cygwin programs with their UNIX-like
    #         behavior.)
    #      5. Whether UTF-8 or some other coding is used, and under
    #         which circumstances: e.g., in calls to the OS to access
    #         files, in files output by programs, on latexmk's command
    #         line, on other programs' command lines, by the command
    #         interpreterS. 
    #      6. If UTF-8 is used, what kind of canonicalization is used,
    #         if any.  (This is a particular bugbear when files are
    #         transferred between different OSes.)
    #      7. Whether the name of a file in the current directory is
    #         reported as the simple filename or whether it is
    #         preceeded by ".\" or "./".
    #      8. How is it determined whether a pathname is absolute or
    #         relative?  An absolute pathname in MSWin may start with
    #         a drive letter and a colon, but under UNIX-type systems,
    #         the colon is an ordinary character.
    #      9. Whether a filename reported in an fls or log file can be
    #         used as is by perl to access a file, or on the command
    #         line to invoke another program, and whether the use on a
    #         command line depends on whether the command line is
    #         executed by a CLI, and by which CLI.  (E.g., cmd.exe,
    #         v. sh v. tcsh, etc.)
    #     10. Whether such a filename for the filename on *latex's
    #         file agrees with the one on the command line.
    #   The above questions have arisen from actual experiences and
    #   tests.
    #
    #   In any case, when determining dependent files, we will try to
    #   remove an initial directory string from filenames found in the
    #   fls and log files, whenever it denotes the current
    #   directory. The directory string may be an absolute pathname,
    #   such as MiKTeX writes in both fls and log files, or it may be
    #   simply "./" as given by TeXLive in its log file. There are
    #   several reasons for removing a directory string when possible:
    #
    #      1. To avoid having multiple names referring to the same
    #         file in the list of dependents.
    #      2. Because the name may be in a different coding.  Thus
    #         under MSWin 7, cmd.exe and perl (by default) work in an
    #         "ANSI" coding with some code page, but the filenames
    #         written by MiKTeX are UTF-8 coded (and if they are non-ASCII
    #         can't be used for file-processing by Perl without some
    #         trouble).  This is a particular problem if the pathname
    #         contains non-ASCII characters; the directory names may not
    #         even be under the user's control, unlike typical filenames.
    #      3. When it comes to filenames that are then used in calls to
    #         bibtex and makeindex, it is bad to use absolute pathnames
    #         instead of clearly relative pathnames, because the default
    #         security settings are to prohibit writing files to the
    #         corresponding directories, which makes the calls to these
    #         programs unnecessarily fail.
    #
    #   In removing unnecessary directory-specifying strings, to
    #   convert a filename to a simple specification relative to the
    #   current directory, it will be important to preferentially use
    #   a determination of the current directory from the file being
    #   processed.  In the fls file, there is normally a PWD line.  In
    #   the log file, if *latex is started with a filename instead
    #   of a command-executing first line, then this can be determined
    #   from the first few lines of the log file -- see parse_log.
    #   This gives a more reliable determination of the relevant path
    #   string; this is especially important in cases where there is a
    #   mismatch of coding of the current directory, particularly
    #   notable in the above-mentioned case of non-ASCII characters
    #   under MSWin.  Other inconsistencies happen when there is a
    #   mixure of cygwin and native MSWin software. There can also be
    #   inconsistencies between whether the separator of pathname
    #   components is "/" or "\".  So we will allow for this.  The
    #   necessary normalizations of filenames are handled by the
    #   subroutines normalize_filename and normalize_clean_filename.
    #
    #   I have not tried to handle the (currently rare) cases that the
    #   OS is neither UNIX-like nor MSWin-like.
    #
    #   Assumption: the list of generated files in %PHdest was already initialized earlier.
    #     In principle, I should do it here, but useful possibilities (e.g.,
    #     see pythontex-latexmk) for subroutine called to process a .tex to add items to
    #     %PHdest. So initializing here is too late.

    # Rules should only be primary
    if ( $$Pcmd_type ne 'primary' ) {
        warn "\n$My_name: ==========$My_name: Probable BUG======= \n   ",
             "   rdb_set_latex_deps called to set files ",
             "for non-primary rule '$rule'\n\n";
        return;
    }

#??    # We'll prune this by all files determined to be needed for source files.
#??    my %unneeded_source = %$PHsource;

    # Parse fls and log files to find relevant filenames
    # Result in the following variables:
    local %dependents = ();    # Maps files to status
    local @bbl_files = ();
    local %idx_files = ();     # Maps idx_file to (ind_file, base)
    local %generated_log = (); # Lists generated files found in log file
    local %generated_fls = (); # Lists generated files found in fls file
    local %source_fls = ();    # Lists source files found in fls file
    local %first_read_after_write = (); # Lists source files that are only read
                                  # after being written (so are not true
                                  # source files.
    local $primary_out = $$Pdest;  # output file (dvi or pdf)
    local %conversions = ();   # *latex-performed conversions.
                     # Maps output file created and read by *latex
                     #    to source file of conversion.
    local @missing_subdirs = ();  # Missing subdirectories in aux_dir

    local $pwd_latex = undef;     # Cwd as reported in fls file by *latex

    local %created_rules = ();    # Maps files to rules existing or created to
                                  #  make them. Use to avoid misunderstood
                                  #  dependencies when a package creates a
                                  #  missing file during *latex compliation
                                  #  instead of just allowing to be made later
                                  #  by another rule. 
    
    # The following are also returned by parsing routines, but are global,
    # to be used by caller:
    # $reference_changed, $bad_reference, $bad_character, $bad_citation, $mult_defined

    # Do I have my own eps-to-pdf conversion?
    my $epspdf_cusdep = 0;
    foreach (@cus_dep_list) {
        if ( /^eps pdf / ) { $epspdf_cusdep = 1; last; }
    }

    # Analyze fls file first.  It tells us the working directory as seen by *latex
    # But we'll use the results later, so that they take priority over the findings
    # from the log file.
    local $fls_file_analyzed = 0;
    if ($recorder && test_gen_file($fls_name) ) {
        $fls_file_analyzed = 
            (0== parse_fls( $fls_name, \%source_fls, \%generated_fls, \%first_read_after_write, \$pwd_latex ));
        if (! $fls_file_analyzed ) {
            warn "$My_name: fls file '$fls_name' appears to have been made but it couldn't be opened.\n";
        }
    }
 
    &parse_log;

    my $missing_dirs = 'none';      # Status of missing directories
    if (@missing_subdirs) {
        $missing_dirs = 'success';
        if ($allow_subdir_creation) {
            foreach my $dir ( uniqs( @missing_subdirs ) ) {
                if ( -d $dir ) {
                    $missing_dirs = 'failure';
                    warn "$My_name: ==== Directory '$dir' is said to be missing\n",
                         "     But it exists!\n";
                }
                elsif ( (-e $dir) && (!-d $dir) ) {
                    $missing_dirs = 'failure';
                    warn "$My_name: ==== Directory '$dir' is said to be missing\n",
                         "     But a non-directory file of this name exists!\n";
                }
                else {
                    if (mkdir $dir) {
                        warn "$My_name: Directory '$dir' created\n";
                    }
                    else {
                        $missing_dirs = 'failure';
                        warn "$My_name: Couldn't create directory '$dir'.\n",
                             "    System error: '$!'\n";
                    }
                }
            }
        }
        else {
            $missing_dirs = 'not allowed';
            warn "$My_name: There are missing subdirectories, but their creation\n",
                 "    is not allowed.  The subdirectories are:\n";
            foreach my $dir ( uniqs( @missing_subdirs ) ) {
                warn "   '$dir'\n";
            }
       }
    }
    # Use results from fls file.  (N.B. The hashes will be empty if the fls file
    # wasn't used/analyzed, so we don't need a test as to whether the fls file was
    # used.
    foreach (keys %source_fls) {
        if (! -e ) {
            # File is listed in .fls file as read, but doesn't exist now.
            # Therefore it is not a true source file, surely.
            # Sometimes this is caused by a bug (e.g., lualatex in TeXLive 2016, 
            #   2017) when there is an incorrect line in .fls file.  (This
            #   would deserve a warning.)
            # But sometimes (e.g., with minted package), the file could be
            #  created during a run, read, and then deleted.
           next;
        }
        $dependents{$_} = 4;
        if ( /\.bbl$/ ) { push @bbl_files, $_; }
    }
    foreach (keys %generated_fls) {
        if (! -e ) {
            # File is listed in .fls file as written, but doesn't exist now.
            # Therefore it is not a true externally visible generated file.
            # (Typically, e.g., with the minted package, it is a temporary
            #   file created during a run and then deleted during the run.)
            next;
        }
        rdb_add_generated( $_ );
        if ( exists($dependents{$_}) ) {
            $dependents{$_} = 6;
        }
     }

    for my $conv (sort keys %conversions) {
        my $conv_source = $conversions{$conv};
        if ( $conv =~ /^(.*)-eps-converted-to\.pdf$/ ) {
            # Check all the conditions for pdflatex's conversion eps to pdf
            # are valid; if they are, treat the converted file as not a
            # source file.
            my $base = $1;
            if ( (-e $conv_source) && (-e $conv) && ( $conv_source eq "$base.eps" ) ) {
                # $conv isn't a real source of *latex
                rdb_remove_files( $rule, $conv );
                delete $dependents{$conv};
                if ($epspdf_cusdep) {
                    $dependents{"$base.pdf"} = ((-e "$base.pdf") ? 4 : 0 );
                }
            }
        }
    }



# ?? !! Should also deal with .run.xml file

    # Handle result on output file:
    #   1.  Non-existent output file, which is because of no content.
    #         This could either be because the source file has genuinely
    #         no content, or because of a missing input file.  Since a
    #         missing input file might be correctable by a run of some
    #         other program whose running is provoked AFTER a run of
    #         *latex, we'll set a diagnostic and leave it to the
    #         rdb_make to handle after all circular dependencies are
    #         resolved. 
    #   2.  The output file might be of a different kind than expected
    #         (i.e., dvi instead of pdf, or vv).  This could
    #         legitimately occur when the source file (or an invoked
    #         package or class) sets \pdfoutput. 
    $missing_dvi_pdf = '';
    if ($primary_out eq '')  {
        warn "$My_name: For rule '$rule', no output was made\n";
        $missing_dvi_pdf = $$Pdest;
    }
    elsif ($primary_out ne normalize_filename($$Pdest) ) {
        my ($actual_base, $actual_path, $actual_ext) = fileparseA( $primary_out );
        my ($intended_base, $intended_path, $intended_ext) = fileparseA( $$Pdest );
        if ( $actual_ext ne $intended_ext ) {
            warn "$My_name: ===For rule '$rule', the extensions differ between the\n",
                 "   actual output file '$primary_out',\n",
                 "   and the expected output '$$Pdest'.\n";
            if ( ! exists $allowed_output_ext{$actual_ext} ) {
                warn "   Actual output file has an extension '$actual_ext' that\n",
                     "   is not one I know about. I cannot handle this\n";
            }
            else {
                my $switch_error = switch_output( $rule, $actual_ext, $intended_ext );
                if ( $switch_error ) { 
                    warn "   I could not accommodate the changed output extension\n",
                         "   (either because the configuration does not allow it\n",
                         "   or because there is a conflict with requested filetypes).\n";
                    $failure = 1;
                    $failure_msg = 'Could not handle change of output extension';
                }
                else {
                    warn "   Rule structure will be changed suitably.\n";
                }
            }
        }
    }

  IDX_FILE:
    foreach my $idx_file ( keys %idx_files ) {
        my ($ind_file, $ind_base) = @{$idx_files{$idx_file}};
        my $from_rule = "makeindex $idx_file";
        if ( ! rdb_rule_exists( $from_rule ) ){
            print "!!!===Creating rule '$from_rule': '$ind_file' from '$idx_file'\n"
                  if ($diagnostics);
            rdb_create_rule( $from_rule, 'external', $makeindex, 'run_makeindex', 1, 
                             $idx_file, $ind_file, $ind_base, 1, 0, 0, 1, [ "$ind_base.ilg" ] );
            print "  ===Source file '$ind_file' for '$rule'\n"
                  if ($diagnostics);
            rdb_ensure_file( $rule, $ind_file, $from_rule );
        }
        # Make sure the .ind file is treated as a detected source file;
        # otherwise if the log file has it under a different name (as
        # with MiKTeX which gives full directory information), there
        # will be problems with the clean-up of the rule concerning
        # no-longer-in-use source files:
        $dependents{$ind_file} = 4;
        if ( ! -e $ind_file ) { 
            # Failure was non-existence of makable file
            # Leave failure issue to other rules.
            $failure = 0;
        }
        $created_rules{$ind_file} = $from_rule;
    }

    local %processed_aux_files = ();
  BBL_FILE:
    foreach my $bbl_file ( uniqs( @bbl_files ) ) {
        my ($bbl_base, $bbl_path, $bbl_ext) = fileparseA( $bbl_file );
        $bbl_base = $bbl_path.$bbl_base;
        my @new_bib_files = ();
        my @new_aux_files = ();
        my @new_bst_files = ();
        my @biber_source = ( "$bbl_base.bcf" );
        my $bib_program = 'bibtex';
        if ( test_gen_file( "$bbl_base.bcf" ) ) {
             $bib_program = 'biber';
        }
        my $from_rule = "$bib_program $bbl_base";
        print "=======  Dealing with '$from_rule'\n" if ($diagnostics);
        # Don't change to use activation and deactivation here, rather than
        # creation and removal of rules.  This is because rules are to be
        # created on the fly here with details corresponding to current. So
        # activating a previously inactive rule, which is out-of-date, may
        # cause trouble.
        if ($bib_program eq 'biber') {
            check_biber_log( $bbl_base, \@biber_source );
            # Remove OPPOSITE kind of bbl generation:
            rdb_remove_rule( "bibtex $bbl_base" );
        }
        else {
            parse_aux( "$bbl_base.aux", \@new_bib_files, \@new_aux_files, \@new_bst_files );
            # Remove OPPOSITE kind of bbl generation:
            rdb_remove_rule( "biber $bbl_base" );
        }
        if ( ! rdb_rule_exists( $from_rule ) ){
            print "   ===Creating rule '$from_rule'\n" if ($diagnostics);
            if ( $bib_program eq 'biber' ) {
                rdb_create_rule( $from_rule, 'external', $biber, '', 1,
                                 "$bbl_base.bcf", $bbl_file, $bbl_base, 1, 0, 0, 1, [ "$bbl_base.blg" ]  );
            }
            else {
                rdb_create_rule( $from_rule, 'external', $bibtex, 'run_bibtex', 1,
                                  "$bbl_base.aux", $bbl_file, $bbl_base, 1, 0, 0, 1, [ "$bbl_base.blg" ]  );
            }
        }
        $created_rules{$bbl_file} = $from_rule;
        local %old_sources = ();
        rdb_one_rule( $from_rule, sub { %old_sources = %$PHsource; } );
        my @new_sources = ( @new_bib_files, @new_aux_files, @new_bst_files );
        if ( $bib_program eq 'biber' ) {
            push @new_sources, @biber_source;
        }
        foreach my $source ( @new_sources ) {
            print "  ===Source file '$source' for '$from_rule'\n"
               if ($diagnostics);
            rdb_ensure_file( $from_rule, $source );
            delete $old_sources{$source};
        }
        foreach my $source ( @new_aux_files ) {
            $processed_aux_files{$source} = 1;
        }
        if ($diagnostics) {
            foreach ( keys %old_sources ) {
                print "Removing no-longer-needed dependent '$_' from rule '$from_rule'\n";
            }
        }
        rdb_remove_files( $from_rule, keys %old_sources );
        print "  ===Source file '$bbl_file' for '$rule'\n"
            if ($diagnostics);
        rdb_ensure_file( $rule, $bbl_file, $from_rule );
        if ( ! -e $bbl_file ) { 
            # Failure was non-existence of makable file
            # Leave failure issue to other rules.
            $failure = 0;
        }
    }

    if ( ($#aux_hooks > -1) && ! exists $processed_aux_files{$aux_main} ) {
        my @new_bib_files = ();
        my @new_aux_files = ();
        my @new_bst_files = ();
        parse_aux( $aux_main, \@new_bib_files, \@new_aux_files, \@new_bst_files );
        foreach my $source ( @new_aux_files ) {
            $processed_aux_files{$source} = 1;
        }
    }

NEW_SOURCE:
    foreach my $new_source (keys %dependents) {
        print "  ===Source file for rule '$rule': '$new_source'\n"
            if ($diagnostics);
        if ( exists $first_read_after_write{$new_source} ) {
            if ( dep_at_start($new_source) ) {
                #warn "--- READ ONLY AFTER WRITE OF '$new_source'\n";
                $dependents{$new_source} = 7;
            }
            else {
                #warn "--- READ ONLY AFTER CREATE OF '$new_source'\n";
                $dependents{$new_source} = 6;
            }
        }
        if ( ($dependents{$new_source} == 5)
             || ($dependents{$new_source} == 6)
            ) {
            # (a) File was detected in "No file..." line in log file. 
            #     Typically file was searched for early in run of 
            #     latex/pdflatex, was not found, and then was written 
            #     later in run.
            # or (b) File was written during run. 
            # In both cases, if file doesn't already exist in database, we 
            #    don't know its previous status.  Therefore we tell 
            #    rdb_ensure_file that if it needs to add the file to its 
            #    database, then the previous version of the file should be 
            #    treated as non-existent, to ensure another run is forced.
            rdb_ensure_file( $rule, $new_source, undef, 1 );
        }
        elsif ( $dependents{$new_source} == 7 )  {
            # File was result of conversion by *latex.
            my $cnv_source = $conversions{$new_source};
            rdb_ensure_file( $rule, $new_source );
#            if ($cnv_source && ($cnv_source !~ /\"/ ) ) {
             if ($cnv_source ) {
                # Conversion from $cnv_source to $new_source
                #   implies that effectively $cnv_source is a source
                #   of the *latex run.
                rdb_ensure_file( $rule, $cnv_source );
            }
            # Flag that changes of the generated file during a run 
            #    do not require a rerun:
            rdb_one_file( $new_source, sub{ $$Pcorrect_after_primary = 1; } );
        }
        else {
            # But we don't need special precautions for ordinary user files 
            #    (or for files that are generated outside of latex/pdflatex). 
            rdb_ensure_file( $rule, $new_source );
        }
        if ( ($dependents{$new_source} == 6) 
             || ($dependents{$new_source} == 7) 
            ) {
            rdb_add_generated($new_source);
        }
    }

    foreach my $Psub (@latex_file_hooks) {
         &$Psub;
    }

    # Some packages (e.g., bibtopic) generate a dummy error-message-providing
    #   bbl file when a bbl file does not exist.  Then the fls and log files
    #   show the bbl file as created by the primary run and hence as a
    #   generated file.  Since we now have a rule to create a real bbl file,
    #   the information in the fls and log files no longer represents a
    #   correct dependency, so the bbl file is to be removed from the
    #   generated files.
    foreach (keys %created_rules) { rdb_remove_generated( $_ );  }

    my @more_sources = &rdb_set_dependents( $rule );
    my $num_new = $#more_sources + 1;
    foreach (@more_sources) { 
        $dependents{$_} = 4;
        if ( ! -e $_ ) { 
            # Failure was non-existence of makable file
            # Leave failure issue to other rules.
            $failure = 0; 
            $$Pchanged = 1; # New files can be made.  Ignore error.
        }
    }
    if ($diagnostics) {
        if ($num_new > 0 ) {
            print "$num_new new source files for rule '$rule':\n";
            foreach (@more_sources) { print "   '$_'\n"; }
        }
        else {
            print "No new source files for rule '$rule':\n";
        }
        my @first_read_after_write = sort keys %first_read_after_write;
        if ($#first_read_after_write >= 0) {
            print "The following files were only read after being written:\n";
            foreach (@first_read_after_write) {
                print "   '$_'\n";
            }
          }
    }
    my @files_not_needed = ();
    foreach (keys %$PHsource) { 
        if ( ! exists $dependents{$_} ) {
            print "Removing no-longer-needed dependent '$_' from rule '$rule'\n"
              if $diagnostics;
            push @files_not_needed, $_;
        }
    }
    rdb_remove_files( $rule, @files_not_needed );

    return ($missing_dirs, [@missing_subdirs] );

} # END rdb_set_latex_deps

#************************************************************

sub switch_output {
    # Usage: switch_output( primary_rule, actual_ext, intended_ext )
    # Rearrange rules to deal with changed extension of output file of
    # the specified primary rule (one of *latex).
    # Return 0 on success, non-zero error code on failure

    my ( $rule, $actual_ext, $intended_ext ) = @_;
    if ( $actual_ext eq $intended_ext ) { return 0; }
    if ( ! $can_switch ) { return 1; }

    if (! defined $possible_primaries{$rule} ) {
        warn "$My_name: BUG: subroutine switch_output called with non-primary rule '$rule'\n";
        return 1;
    }

    rdb_deactivate_derequest( 'dvipdf', 'pspdf', 'xdvipdfmx', keys %possible_primaries );
    
    rdb_activate_request( $rule );

    if ( $actual_ext eq '.dvi' ) {
        rdb_activate_request( 'dvipdf' );
        $input_extensions{$rule} = $standard_input_extensions{latex};
    }
    elsif ( $actual_ext eq '.xdv' ) {
        rdb_activate_request( 'xdvipdfmx' );
        $input_extensions{$rule} = $standard_input_extensions{xelatex};
    }
    else {
        $input_extensions{$rule} = $standard_input_extensions{pdflatex};
    }

    my $old_dest = $$Pdest;
    my $new_dest = $$Pdest;
    $new_dest =~ s/$intended_ext$/$actual_ext/;
    # Compensate for MiKTeX's behavior: dvi and pdf are put in out_dir, but xdv is put in aux_dir:
    if ( ($actual_ext eq '.xdv') && ($out_dir ne $aux_dir) ){ $new_dest =~ s/^$out_dir1/$aux_dir1/; }
    if ( ($intended_ext eq '.xdv') && ($out_dir ne $aux_dir) ){ $new_dest =~ s/^$aux_dir1/$out_dir1/; }

    rdb_change_dest( $new_dest );
        
    # Some fixes to avoid spurious error conditions:
    $switched_primary_output = 1;
    if (-e $$Pdest) {
        $missing_dvi_pdf = '';
        if ($$Plast_result == 1 ) { $$Plast_result = 0; }
    }
    else { $missing_dvi_pdf = $$Pdest; }

    return 0;
} #END switch_output

#************************************************************

sub test_gen_file {
    # Usage: test_gen_file( filename )
    # Tests whether the file was generated during a run of *latex.
    # Assumes context for primary rule.
    # Two kinds of test are used:
    # a. From %generated_log, which works after the log file has been parsed,
    #    but only for certain files and for those TeX engines (not MiKTeX)
    #    that put \openout lines in log file.
    # b. By the file existing and being at least as new as the system
    #    time at the start of the run. But we allow for a measured
    #    offset between filetime and system time, which could be
    #    nonzero if the file is on a different, remote system than the
    #    one running latexmk. We must also allow a threshold in the
    #    comparisons of filetimes to allow for the inaccuracy of the
    #    offset measurement.
    my $file = shift;
    return exists $generated_log{$file}
           || ( -e $file && ( get_mtime( $file ) >= $$Prun_time + $filetime_offset - $filetime_causality_threshold));
}

#************************************************************

sub dep_at_start {
    # Usage: dep_at_start( filename )
    # Tests whether the file was source file and existed at start of run.
    # Assumes context for primary rule.
    my $time = undef;
    rdb_one_file( shift, sub{ $time = $$Ptime; } );
    return (defined $time) && ($time != 0);
}

#************************************************************

sub rdb_find_new_files {
    # Call: rdb_find_new_files
    # Assumes rule context for primary rule.
    # Deal with files which were missing and for which a method
    # of finding them has become available:
    #   (a) A newly available source file for a custom dependency.
    #   (b) When there was no extension, a file with appropriate
    #       extension
    #   (c) When there was no extension, and a newly available source 
    #       file for a custom dependency can make it.

    my %new_includes = ();

MISSING_FILE:
    foreach my $missing ( keys %$PHsource ) {
        next if ( $$PHsource{$missing} != 0 ); 
        my ($base, $path, $ext) = fileparseA( $missing );
        $ext =~ s/^\.//;
        if ( -e "$missing.tex" ) { 
            $new_includes{"$missing.tex"} = 1;
        }
        elsif ( -e $missing ) { 
            $new_includes{$missing} = 1;
        }
        elsif ( $ext ne "" ) {
            foreach my $dep (@cus_dep_list){
               my ($fromext,$toext) = split('\s+',$dep);
               if ( ( "$ext" eq "$toext" )
                    && ( -f "$path$base.$fromext" )
                  )  {
                  # Source file for the missing file exists
                  # So we have a real include file, and it will be made
                  # next time by rdb_set_dependents
                  $new_includes{$missing} = 1;
               }
               else {
                   # no point testing the $toext if the file doesn't exist.
               }
               next MISSING_FILE;
            }
       }
       else {
           # $_ doesn't exist, $_.tex doesn't exist,
           # and $_ doesn't have an extension
           foreach my $dep (@cus_dep_list){
              my ($fromext,$toext) = split('\s+',$dep);
              if ( -f "$path$base.$fromext" ) {
                  # Source file for the missing file exists
                  # So we have a real include file, and it will be made
                  # next time by &rdb__dependents
                  $new_includes{"$path$base.$toext"} = 1;
#                  next MISSING_FILE;
              }
              if ( -f "$path$base.$toext" ) {
                  # We've found the extension for the missing file,
                  # and the file exists
                  $new_includes{"$path$base.$toext"} = 1;
#                  next MISSING_FILE;
              }
           }
       }
    } # end MISSING_FILES

    # Sometimes bad line-breaks in log file (etc) create the
    # impression of a missing file e.g., ./file, but with an incorrect
    # extension.  The above tests find the file with an extension,
    # e.g., ./file.tex, but it is already in the list.  So now I will
    # remove files in the new_include list that are already in the
    # include list.  Also handle aliasing of file.tex and ./file.tex.
    # For example, I once found:
# (./qcdbook.aux (./to-do.aux) (./ideas.aux) (./intro.aux) (./why.aux) (./basics
#.aux) (./classics.aux)

    my $found = 0;
    foreach my $file (keys %new_includes) {
#       if ( $file =~ /\"/ ) {next; }
        my $stripped = $file;
        $stripped =~ s{^\./}{};
        if ( exists $PHsource{$file} ) {
            delete $new_includes{$file};
        }
        else {
            $found ++;
            rdb_ensure_file( $rule, $file );
        }
    }

    if ( $diagnostics && ( $found > 0 ) ) {
        warn "$My_name: Detected previously missing files:\n";
        foreach ( sort keys %new_includes ) {
            warn "   '$_'\n";
        }
    }
    return $found;
} # END rdb_find_new_files

#************************************************************

sub rdb_set_dependents {
    # Call rdb_set_dependents( rules ...)
    # Returns array (sorted), of new source files.
    local @new_sources = ();
    local @deletions = ();

# Shouldn't recurse.  The definite rules to be examined are given.
    rdb_for_some( [@_],  0, \&rdb_one_dep );
# OLD    rdb_recurse( [@_],  0, \&rdb_one_dep );
    foreach (@deletions) {
        my ($rule, $file) = @$_;
        rdb_remove_files( $rule, $file );
    }
    &rdb_make_links;
    return uniqs( @new_sources );
} #END rdb_set_dependents

#************************************************************

sub rdb_find_source_file {
    # Helper for searching dependencies in all paths inside the TEXINPUTS
    # environment variable.
    my $test = "$_[0].$_[1]";
    if ( -e $test ) {
        return $_[0];
    }
    if ( exists $ENV{TEXINPUTS} ) {
        foreach my $searchpath (split $search_path_separator, $ENV{TEXINPUTS}) {
            my $file = File::Spec->catfile($searchpath,$_[0]);
            my $test = "$file.$_[1]";
            if ( -e $test ) {
                return $file;
            }
        }
    }
    return "$_[0]";
}

#************************************************************

sub rdb_one_dep {
    # Helper for finding dependencies.  One case, $rule and $file given
    # Assume file (and rule) context for DESTINATION file.

    # Only look for dependency if $rule is primary rule (i.e., latex
    # or pdflatex) or is a custom dependency:
    if ( (! exists $possible_primaries{$rule}) && ($rule !~ /^cusdep/) ) {
        return;
    }
#print "=============ONE_DEP: '$rule' '$file'\n";
    local $new_dest = $file;
    my ($base_name, $path, $toext) = fileparseA( $new_dest );
    $base_name = $path.$base_name;
    $toext =~ s/^\.//;
    my $Pinput_extensions = $input_extensions{$rule};
DEP:
    foreach my $dep ( @cus_dep_list ) {
        my ($fromext,$proptoext,$must,$func_name) = split('\s+',$dep);
        if ( $toext eq $proptoext ) {
            $base_name = rdb_find_source_file($base_name, $fromext);
            my $source = "$base_name.$fromext";
            # Found match of rule
            if ($diagnostics) {
                print "Found cusdep:  $source to make $rule:$new_dest ====\n";
            }
            if ( -e $source ) {
                $$Pfrom_rule = "cusdep $fromext $toext $base_name";
                my $new_new_dest = "$base_name.$toext";
                if ($new_new_dest ne $new_dest) {
                    rdb_ensure_file( $rule, $new_new_dest );
                    $new_dest = $new_new_dest;
                }
                local @PAnew_cmd = ( 'do_cusdep', $func_name );
                if ( !-e $new_dest ) {
                    push @new_sources, $new_dest;
                }
                if (! rdb_rule_exists( $$Pfrom_rule ) ) {
                    print "$My_name: === Creating rule '$$Pfrom_rule'\n" if $diagnostics;
                    rdb_create_rule( $$Pfrom_rule, 'cusdep', '', \@PAnew_cmd, 3, 
                                     $source, $new_dest, $base_name, 0 );
                }
                return;
            }
            else {
                # Source file does not exist
                if ( !$force_mode && ( $must != 0 ) ) {
                    # But it is required that the source exist ($must !=0)
                    $failure = 1;
                    $failure_msg = "File '$base_name.$fromext' does not exist ".
                                   "to build '$base_name.$toext'";
                    return;
                }
                elsif ( $$Pfrom_rule =~ /^cusdep $fromext $toext / )  {
                    # Source file does not exist, destination has the rule set.
                    # So turn the from_rule off
                    $$Pfrom_rule = '';
                }
                else {
                }
            }
        }
        elsif ( ($toext eq '') 
                && (! -e $file ) 
                && (! -e "$base_name.$proptoext" ) 
                && exists $$Pinput_extensions{$proptoext}
              ) {
            # Empty extension and non-existent destination
            #   This normally results from  \includegraphics{A}
            #    without graphics extension for file, when file does
            #    not exist.  So we will try to find something to make it.
            $base_name = rdb_find_source_file($base_name, $fromext);
            my $source = "$base_name.$fromext";
            if ( -e $source ) {
                $new_dest = "$base_name.$proptoext";
                my $from_rule = "cusdep $fromext $proptoext $base_name";
                push @new_sources, $new_dest;
                print "Ensuring rule for '$from_rule', to make '$new_dest'\n"
                    if $diagnostics > -1;
                local @PAnew_cmd = ( 'do_cusdep', $func_name );
                if (! rdb_rule_exists( $from_rule ) ) {
                    print "$My_name: === Creating rule '$$Pfrom_rule'\n" if $diagnostics;
                    rdb_create_rule( $from_rule, 'cusdep', '', \@PAnew_cmd, 3, 
                                     $source, $new_dest, $base_name, 0 );
                }
                rdb_ensure_file( $rule, $new_dest, $from_rule );
                # We've now got a spurious file in our rule.  But don't mess
                # with deleting an item we are in the middle of!
                push @deletions, [$rule, $file];
                return;
            }
        } # End of Rule found
    } # End DEP
    if ( (! -e $file) && $use_make_for_missing_files ) {
        # Try to make the missing file
        #Set character to surround filenames in commands:
        if ( $toext ne '' ) {
             print "$My_name: '$rule': source file '$file' doesn't exist. I'll try making it...\n";
             &Run_subst( "$make $quote$file$quote" );
             if ( -e $file ) {
                 return;
             }
        }
        else {
             print "$My_name: '$rule': source '$file' doesn't exist.\n",
                   "   I'll try making it with allowed extensions \n";
             foreach my $try_ext ( keys %$Pinput_extensions ) {
                 my $new_dest = "$file.$try_ext";
                 &Run_subst( "$make $quote$new_dest$quote" );
                 if ( -e $new_dest ) {
                     print "SUCCESS in making '$new_dest'\n";
                     # Put file in rule, without a from_rule, but
                     # set its state as non-existent, to correspond
                     # to file's state before the file was made
                     # This ensures a rerun of *latex is provoked.
                     rdb_ensure_file( $rule, $new_dest, undef, 1 );
                     push @new_sources, $new_dest;
                     push @deletions, [$rule, $file];
                     # Flag need for a new run of *latex despite
                     # the error due to a missing file.
                     $$Pout_of_date_user = 1;
                     return;
                 }
           }
        }
    }
} #END rdb_one_dep

#************************************************************

sub rdb_list {
    # Call: rdb_list()
    # List rules and their source files
    print "===Rules:\n";
    local $count_rules = 0;
    my @accessible_all = &rdb_accessible;
    rdb_for_some( 
        \@accessible_all,
        sub{ $count_rules++; 
             print "Rule '$rule' depends on:\n"; 
           },
        sub{ print "    '$file'\n"; },
        sub{ print "  and generates:\n";
             foreach (keys %$PHdest) { print "    '$_'\n"; }
#             print "  default_extra_generated:\n";
#             foreach (@$PA_extra_gen) { print "    '$_'\n"; }
           },
    );
    if ($count_rules <= 0) {
        print "   ---No rules defined\n";
    }
} #END rdb_list

#************************************************************

sub deps_list {
    # Call: deps_list(fh)
    # List dependent files to file open on fh
    my $fh = $_[0];
    print $fh "#===Dependents, and related info, for $filename:\n";
    my @dest_exts = ();
    if ($pdf_mode) {push @dest_exts, '.pdf';}
    if ($dvi_mode) {push @dest_exts, '.dvi';}
    if ($postscript_mode) {push @dest_exts, '.ps';}
    my %source = ( $texfile_name => 1 );
    my @generated = ();
    my @accessible_all = &rdb_accessible;
    rdb_for_some(
        \@accessible_all,
        sub{ push @generated, keys %$PHdest; },
        sub{ $source{$file} = 1; }
    );
    foreach (keys %generated_exts_all) {
        (my $name = /%R/ ? $_ : "%R.$_") =~ s/%R/${aux_dir1}${root_filename}/;
        push @generated, $name;
    }
    show_array( "Generated:", @generated )  if $diagnostics;
    foreach (@generated) {
        delete $source{$_};
    }
    show_array( "Sources:", keys %source ) if $diagnostics;
    foreach my $ext (@dest_exts) {
         # Don't insert name of deps file in targets.
         # The previous behavior of inserting the name of the deps file
         # matched the method recommended by GNU make for automatically
         # generated prerequisites -- see Sec. "Generating Prerequisites
         # Automatically" of GNU make manual (v. 4.2).  But this can
         # cause problems in complicated cases, and as far as I can see,
         # it doesn't actually help, despite the reasoning given.
         # The only purpose of the deps file is to to determine source
         # files for a particular rule.  The files whose changes make the
         # deps file out-of-date are the same as those that make the real
         # target file (e.g., .pdf) out-of-date. So the GNU method seems
         # completely unnecessary.
       print $fh "${out_dir1}${root_filename}${ext} :";
       foreach (sort keys %source) {
           print $fh "\\\n    $_";
       }
       print $fh "\n";
    }
    print $fh "#===End dependents for $filename:\n";
    if ($dependents_phony) {
        print $fh "\n#===Phony rules for $filename:\n\n";
        foreach (sort keys %source) {
            print $fh "$_ :\n\n";
        }
        print $fh "#===End phony rules for $filename:\n";
    }
} #END deps_list

#************************************************************

sub rdb_show {
    # Call: rdb_show()
    # Displays contents of rule data base.
    # Side effect: Exercises access routines!
    print "===Rules:\n";
    local $count_rules = 0;
    rdb_for_actives( 
        sub{ $count_rules++; 
             my @int_cmd = @$PAint_cmd;
             foreach (@int_cmd) {
                 if ( !defined($_) ) { $_='undef';}
             }
             print "  [$rule]: '$$Pcmd_type' '$$Pext_cmd' '@int_cmd' $$Ptest_kind ",
                   "'$$Psource' '$$Pdest' '$$Pbase' $$Pout_of_date $$Pout_of_date_user\n"; },
        sub{ print "    '$file': $$Ptime $$Psize $$Pmd5 '$$Pfrom_rule'\n"; }
    );
    if ($count_rules <= 0) {
        print "   ---No rules defined\n";
    }
} #END rdb_show

#************************************************************

sub rdb_target_array {
    # Returns array of all rules implicated by %target_rules and %target_files
    my %rules = &rdb_target_hash;
    return keys %rules;
} # End rdb_target_array

#************************************************************

sub rdb_target_hash {
    # Returns hash mapping to 1 all rules implicated by %target_rules and %target_files
    my %rules = %target_rules;
    foreach (keys %target_files) {
        if (exists $from_rules{$_}) { $rules{$from_rules{$_}} = 1; }
    }
    return %rules;
} # End rdb_target_hash

#************************************************************

sub rdb_accessible {
    # Call: &rdb_accessible
    # Returns array of rules accessible from target rules and rules to make target files

    local %accessible_rules = &rdb_target_hash;
    rdb_recurse( [keys %accessible_rules], sub{ $accessible_rules{$rule} = 1; } );
    return keys %accessible_rules;
} #END rdb_accessible

#************************************************************
#************************************************************
#************************************************************

sub rdb_make {
    # Call: &rdb_make
    # Makes the targets and prerequisites.  
    # Leaves one-time rules to last.
    # Does appropriate repeated makes to resolve dependency loops

    # Returns 0 on success, nonzero on failure.

    # General method: Find all accessible rules, then repeatedly make
    # them until all accessible rules are up-to-date and the source
    # files are unchanged between runs.  On termination, all
    # accessible rules have stable source files.
    #
    # One-time rules are view and print rules that should not be
    # repeated in an algorithm that repeats rules until the source
    # files are stable.  It is the calling routine's responsibility to
    # arrange to call them, or to use them here with caution.
    #
    # Note that an update-viewer rule need not be considered
    # one-time.  It can be legitimately applied everytime the viewed
    # file changes.
    #
    # Note also that the criterion of stability is to be applied to
    # source files, not to output files.  Repeated application of a
    # rule to IDENTICALLY CONSTANT source files may produce different
    # output files.  This may be for a trivial reason (e.g., the
    # output file contains a time stamp, as in the header comments for
    # a typical postscript file), or for a non-trivial reason (e.g., a
    # stochastic algorithm, as in abcm2ps).   
    #
    # This caused me some actual trouble.  In general, circular
    # dependencies produce non-termination, and the the following
    # situation is an example of a generic situation where certain
    # rules must be obeyed in order to obtain proper results:
    #    1.  A/the latex source file contains specifications for
    #        certain postprocessing operations.  Standard *latex 
    #        already has this, for indexing and bibliography.
    #    2.  In the case in point that caused me trouble, the
    #        specification was for musical tunes that were contained
    #        in external source files not directly input to
    #        *latex.  But in the original version, there was a
    #        style file (abc.sty) that caused latex itself to call
    #        abcm2ps to make .eps files for each tune that were to be
    #        read in on the next run of latex. 
    #    3.  Thus the specification can cause a non-terminating loop
    #        for latexmk, because the output files of abcm2ps changed
    #        even with identical input.  
    #    4.  The solution was to 
    #        a. Use a style file abc_get.sty that simply wrote the
    #           specification on the tunes to the .aux file in a
    #           completely deterministic fashion.
    #        b. Instead of latex, use a script abclatex.pl that runs
    #           latex and then extracts the abc contents for each tune
    #           from the source abc file.  This is also
    #           deterministic. 
    #        c. Use a cusdep rule in latexmk to convert the tune abc
    #           files to eps.  This is non-deterministic, but only
    #           gets called when the (deterministic) source file
    #           changes.
    #        This solves the problem.  Latexmk works.  Also, it is no
    #        longer necessary to enable write18 in latex, and multiple
    #        unnecessary runs of abcm2ps are no longer used. 
    #
    # The order of testing and applying rules is chosen by the
    # following heuristics: 
    #    1.  Both latex and pdflatex may be used, but the resulting
    #        aux files etc may not be completely identical.  Define
    #        latex and pdflatex as primary rules.  Apply the general
    #        method of repeated circulating through all rules until
    #        the source files are stable for each primary rule
    #        separately.  Naturally the rules are all accessible
    #        rules, but excluding primary rules except for the current
    #        primary.
    #    2.  Assume that the primary rules are relatively
    #        time-consuming, so that unnecessary passes through them
    #        to check stability of the source files should be avoided.
    #    3.  Assume that although circular dependencies exist, the
    #        rules can nevertheless be thought of as basically
    #        non-circular, and that many rules are strictly or
    #        normally non-circular.  In particular cusdep rules are
    #        typically non-circular (e.g., fig2eps), as are normal
    #        output processing rules like dvi2ps.  
    #    4.  The order for the non-circular approximation is
    #        determined by applying the assumption that an output file
    #        from one rule that is read in for an earlier stage is
    #        unchanged. 
    #    HOWEVER, at a first attempt, the ordering is not needed.  It
    #    only gives an optimization
    #    5.  (Note that these assumptions could be violated, e.g., if
    #        $dvips is arranged not only to do the basic dvips
    #        command, but also to extract information from the ps file
    #        and feed it back to an input file for *latex.)
    #    6.  Nevertheless, the overall algorithm should allow
    #        circularities.  Then the general criterion of stability
    #        of source files covers the general case, and also
    #        robustly handles the case that the USER changes source
    #        files during a run.  This is particularly important in
    #        -pvc mode, given that a full make on a large document can
    #        be quite lengthy in time, and moreover that a user
    #        naturally wishes to make corrections in response to
    #        errors, particularly latex errors, and have them apply
    #        right away.
    # This leads to the following approach:
    #    1.  Classify accessible rules as: primary, pre-primary
    #        (typically cusdep, bibtex, makeindex, etc), post-primary
    #        (typically dvips, etc), and one-time
    #    2.  Then stratify the rules into an order of application that
    #        corresponds to the basic feedforward structure, with the
    #        exclusion of one-time rules.
    #    3.  Always require that one-time rules are among the
    #        explicitly requested rules, i.e., the last to be applied,
    #        were we to apply them.  Anything else would not match the
    #        idea of a one-time rule.  
    #    4.  Then work as follows:
    #        a. Loop over primaries
    #        b. For each primary, examine each pre-primary rule and
    #           apply if needed, then the primary rule and then each
    #           post-primary rule.  The ordering of the pre-primary
    #           and post-primary rules was found in step 2.
    #      BUT applying the ordering is not essential
    #        c. Any time that a pre-primary or primary rule is
    #           applied, loop back to the beginning of step b.  This
    #           ensures that bibtex etc are applied before rerunning
    #           *latex, and also covers changing source files, and
    #           gives priority to quick pre-primary rules for changing
    #           source files against slow reruns of latex.
    #        d. Then apply post-primary rules in order, but not
    #           looping back after each rule.  This non-looping back
    #           is because the rules are normally feed-forward only.
    #      BUT applying the ordering is not essential
    #        e. But after completing post-primary rules do loop back
    #           to b if any rules were applied.  This covers exotic
    #           circular dependence (and as a byproduct, changing
    #           source files).
    #        f. On each case of looping back to b, re-evaluate the
    #           dependence setup to allow for the effect of changing
    #           source files.  
    #    


    &rdb_set_rule_net;

    local %pass = ();
    local $failure = 0;        # General accumulated error flag
    local $missing_dvi_pdf = ''; # Did primary run fail to make its output file?
    local $runs = 0;
    local $too_many_passes = 0;
    local %rules_applied = ();
    local $switched_primary_output = 0;
    my $retry_msg = 0;         # Did I earlier say I was going to attempt 
                               # another pass after a failure?
    rdb_for_some ( [keys %rule_db],
                   sub{ $pass{$rule} = 0; 
                        foreach (keys %$PHsource_rules) {
                            $$PHsource_rules{$_} = 0;
                        }
                   }
                 );
    PASS:
    while (1==1) {
        # Exit condition at end of body of loop.
        $runs = 0;
        $switched_primary_output = 0;
        my $previous_failure = $failure;
        $failure = 0;
        local $newrule_nofile = 0;  # Flags whether rule created for
                           # making currently non-existent file, which
                           # could become a needed source file for a run
                           # and therefore undo an error condition
        foreach my $rule (keys %rule_db) {
            # Update %pass in case new rules have been created
            if (! exists $pass{$rule} ) { $pass{$rule} = 0; }
        }
        if ($diagnostics) {
            print "Make: doing pre_primary and primary...\n";
        }
        # Do the primary run if it is needed. On return $runs == 0
        #       signals that nothing was run (and hence no output
        #       files changed), either because no input files
        #       changed and no run was needed, or because the
        #       number of passes through the rule exceeded the
        #       limit.  In the second case $too_many_runs is set.
        rdb_for_some( [@pre_primary, $current_primary], \&rdb_make1 );
        if ($switched_primary_output) {
            print "=========SWITCH OF OUTPUT WAS DONE.\n";
            next PASS;
        }
        if ( ($runs > 0) && ! $too_many_passes ) {
            $retry_msg = 0;
            if ( $force_mode || (! $failure) || $switched_primary_output ) {
                next PASS;
            }
            # Get here on failure, without being in force_mode
            if ( $newrule_nofile ) { 
                $retry_msg = 1;
                print "$My_name: Error on run, but found possibility to ",
                      "make new source files\n";
                next PASS;
            }
            else { last PASS; }
        }
        if ($runs == 0) {
            # $failure not set on this pass, so use value from previous pass:
            $failure = $previous_failure;
            if ($retry_msg) {
                print "But in fact no new files made\n";
                }
            if ($failure && !$force_mode ) { last PASS; }
        }
        if ( $missing_dvi_pdf ) { 
            # No output from primary, after completing circular dependence
            warn "Failure to make '$missing_dvi_pdf'\n";
            $failure = 1; 
            last PASS;
        }    
        if ($diagnostics) {
            print "Make: doing post_primary...\n";
        }
        rdb_for_some( [@post_primary], \&rdb_make1 );
        if ( ($runs == 0) || $too_many_passes ) {
            # If $too_many_passes is set, it should also be that
            # $runs == 0; but for safety, I also checked
            # $too_many_passes.
            last PASS;
        }
     }
     continue {
         # Re-evaluate rule classification and accessibility,
         # but do not change primaries.
         # Problem is that %current_primaries gets altered
         &rdb_set_rule_net;
    }  #End PASS

    rdb_for_some( [@unusual_one_time], \&rdb_make1 );
    rdb_write( $fdb_name );

    if ($#primary_warning_summary > -1) {
        # N.B. $mult_defined, $bad_reference, $bad_character, $bad_citation also available here.
        show_array( "$My_name: Summary of warnings from last run of *latex:", 
                    @primary_warning_summary );
    }
    if (! $silent) {
        if ($failure && $force_mode) {
            print "$My_name: Errors, in force_mode: so I tried finishing targets\n";
        }
        elsif ($failure) {
            print "$My_name: Errors, so I did not complete making targets\n";
        }
        else {
#            local @dests = ( keys %current_primaries, @pre_primary, @post_primary, @unusual_one_time );
            local @rules = ( keys %current_primaries, @post_primary, @unusual_one_time );
            local @dests = ();
            rdb_for_some( [@rules], sub{ push @dests, $$Pdest if ($$Pdest); } );
            print "$My_name: All targets (@dests) are up-to-date\n";
        }
    }
    rdb_for_some ( [keys %rule_db],
                   sub{ 
                        foreach my $s_rule (keys %$PHsource_rules) {
                            $$PHsource_rules{$s_rule} = $pass{$s_rule};
                        }
                   }
                );
    return $failure;
} #END rdb_make

#-------------------

sub rdb_show_rule_errors {
    local @errors = ();
    local @warnings = ();
    rdb_for_actives( 
               sub{
                   if ($$Plast_message ne '') {
                       if ($$Plast_result == 200) {
                          push @warnings, "$rule: $$Plast_message";
                       }
                       else {
                          push @errors, "$rule: $$Plast_message";
                       }
                   }
                   elsif ($$Plast_result == 1) {
                       push @errors, "$rule: failed to create output file";
                   }
                   elsif ($$Plast_result == 2) {
                       push @errors, "$rule: gave an error";
                   }
                   elsif ($$Prun_time == 0) {
                       #  This can have innocuous causes.  So don't report
                   }
               }
              );
    if ($#warnings > -1) { 
        warn "Collected warning summary (may duplicate other messages):\n";
        foreach (@warnings){
            warn "  $_\n";
        }
    }
    if ($#errors > -1) { 
        warn "Collected error summary (may duplicate other messages):\n";
        foreach (@errors){
            warn "  $_\n";
        }
    }
    return $#errors+1;
}

#-------------------

sub rdb_make1 {
    # Call: rdb_make1
    # Helper routine for rdb_make.
    # Carries out make at level of given rule (all data available).
    # Assumes contexts for recursion, make, and rule, and
    # assumes that source files for the rule are to be considered
    # up-to-date.
    if ($diagnostics) { print "  Make1 $rule\n"; }
    if ($failure & ! $force_mode) {return;}
    if ( ! defined $pass{$rule} ) {$pass{$rule} = 0; } 

    # Special fix up for bibtex:
    my $bibtex_not_run = -1;   # Flags status as to whether this is a
        # bibtex rule and if it is, whether out-of-date condition is to
        # be ignored.
        #  -1 => not a bibtex rule
        #   0 => no special treatment
        #   1 => don't run bibtex because of non-existent bibfiles
        #           (and setting to do this test)
        #   2 => don't run bibtex because of setting
    my @missing_bib_files = ();
    if ( $rule =~ /^(bibtex|biber)/ ) {
        $bibtex_not_run = 0;
        if ($bibtex_use == 0) {
           $bibtex_not_run = 2;
        }
        elsif ( ($bibtex_use == 1) || ($bibtex_use == 1.5) ) {
            foreach ( keys %$PHsource ) {
                if ( ( /\.bib$/ ) && (! -e $_) ) {
                    push @missing_bib_files, $_;
                    $bibtex_not_run = 1;
                }
            }
        }
    }

    if ( ($$Prun_time == 0) && exists($possible_primaries{$rule}) ) {
        push @rules_never_run, $rule;
        $$Pout_of_date = 1;
        $$Plast_result = -1;
    }
    else {
        if ( $$Pdest && (! -e $$Pdest) ) {
            # With a non-existent destination, if we haven't made any passes
            #   through a rule, rerunning the rule is good, because the file
            #   may fail to exist because of being deleted by the user (for ex.)
            #   rather than because of a failure on a previous run. 
            # (We could do better with a flag in fdb file.)
            # But after the first pass, the situation is different.  
            #   For a primary rule *latex, the lack of a destination file 
            #      could result from there being zero content due to a missing
            #      essential input file.  The input file could be generated 
            #      by a program to be run later (e.g., a cusdep or bibtex), 
            #      so we should wait until all passes are completed before 
            #      deciding a non-existent destination file is an error.
            #   For a custom dependency, the rule may be obsolete, and
            #      if the source file does not exist also, we should simply
            #      not run the rule, but not set an error condition.
            #      Any error will arise at the *latex level due to a 
            #      missing source file at that level.
            if ( $$Psource && (! -e $$Psource)
                 && ( ( $$Pcmd_type ne 'primary') )
               ) {
                # Main source file doesn't exist, and rule is NOT primary.
                # No action, since a run is pointless.  Primary is different:
                # file might be found elsewhere (by kpsearch from *latex),
                # while non-existence of main source file is a clear error.
            }
            elsif ( $$Pcmd_type eq 'delegated' ) {
                # Delegate to destination rule
            }
            elsif ( $pass{$rule}==0) {
                push @no_dest, $$Pdest;
                $$Pout_of_date = 1;
            }
            if ( $$Pcmd_type eq 'primary' ) {
                $missing_dvi_pdf = $$Pdest;
            }
        }
    }

    &rdb_clear_change_record;
    &rdb_flag_changes_here(0);

    if (!$$Pout_of_date) {
        return;
    }
    if ($diagnostics) { print "     remake\n"; }
    if (!$silent) { 
        print "$My_name: applying rule '$rule'...\n"; 
        &rdb_diagnose_changes( "Rule '$rule': " );
    }

    # We are applying the rule, so its source file state for when it
    # was last made is as of now:
    # ??IS IT CORRECT TO DO NOTHING IN CURRENT VERSION?

    # The actual run
    my $return = 0;   # Return code from called routine
    # Rule may have been created since last run:
    if ( ! defined $pass{$rule} ) {$pass{$rule} = 0; }
    if ( $pass{$rule} >= $max_repeat ) {
        # Avoid infinite loop by having a maximum repeat count
        # Getting here represents some kind of weird error.
        warn "$My_name: Maximum runs of $rule reached ",
             "without getting stable files\n";
        $too_many_passes = 1;
        # Treat rule as completed, else in -pvc mode get infinite reruns:
        $$Pout_of_date = 0;
        $failure = 1;
        $failure_msg = "'$rule' needed too many passes";
        return;
    }

    $rules_applied{$rule} = 1;
    $runs++;

    $pass{$rule}++;
    if ($bibtex_not_run > 0) {
        if ($bibtex_not_run == 1 ) {
            show_array ("$My_name: I WON'T RUN '$rule' because I don't find the following files:",
                        @missing_bib_files);
        }
        elsif ($bibtex_not_run == 2 ) {
            warn "$My_name: I AM CONFIGURED/INVOKED NOT TO RUN '$rule'\n"; 
        }
        $return = &rdb_dummy_run0;
    }
    else {
        warn_running( "Run number $pass{$rule} of rule '$rule'" );
        if ($$Pcmd_type eq 'primary' ) { 
            $return = &rdb_primary_run;
        }
        else { $return = &rdb_run1; }
    }
    if ($$Pchanged) {
        $newrule_nofile = 1;
        $return = 0;
    }
    elsif ( $$Pdest && ( !-e $$Pdest ) && (! $failure) ){
        # If there is a destination to make, but for some reason
        #    it did not get made, and no other error was reported, 
        #    then a priori there appears to be an error condition:
        #    the run failed.   But there are some important cases in
        #    which this is a wrong diagnosis.
        if ( ( $$Pcmd_type eq 'cusdep') && $$Psource && (! -e $$Psource) ) {
            # However, if the rule is a custom dependency, this is not by
            #  itself an error, if also the source file does not exist.  In 
            #  that case, we may have the situation that (1) the dest file is no
            #  longer needed by the tex file, and (2) therefore the user
            #  has deleted the source and dest files.  After the next
            #  latex run and the consequent analysis of the log file, the
            #  cusdep rule will no longer be needed, and will be removed.

            # So in this case, do NOT report an error          
            $$Pout_of_date = 0;
        }
        elsif ($$Pcmd_type eq 'primary' ) { 
            # For a primary rule, i.e., *latex, not to produce the 
            #    expected output file may not be an error condition.  
            # Diagnostics were handled in parsing the log file.
            # Special action in main loop in rdb_make
            $missing_dvi_pdf = $$Pdest;
        }
        elsif ($return == -2) {
           # Missing output file was reported to be NOT an error
           $$Pout_of_date = 0;
        }
        elsif ( ($bibtex_use <= 1.5) && ($bibtex_not_run > 0) ) {
           # Lack of destination file is not to be treated as an error
           # for a bibtex rule when latexmk is configured not to treat
           # this as an error, and the lack of a destination file is the
           # only error.
           $$Pout_of_date = 0;
        }
        else {
            $failure = 1;
        }
    }
    if ( ($return != 0) && ($return != -2) ) {
        $failure = 1; 
        $$Plast_result = 2;
        if ( !$$Plast_message ) {
            $$Plast_message = "Run of rule '$rule' gave a non-zero error code";
        }
    }
    foreach ( keys %$PHsource_rules ) {
        $$PHsource_rules{$_} = $pass{$_};
    }
}  #END rdb_make1

#************************************************************

sub rdb_classify_rules {
    # Usage: &rdb_classify_rules
    # Assume the following variables are available (global or local):
    # Input:
    #    %target_rules    # Set to target rules
    #    %target_files    # Set to target files
    #    %possible_primaries
    
    # Output:
    #    %current_primaries    # Keys are actual primaries
    #    @pre_primary          # Array of rules
    #    @post_primary         # Array of rules
    #    @unusual_one_time     # Array of rules
    # @pre_primary and @post_primary are in natural order of application.

    local @requested_targets = &rdb_target_array;
    local $state = 0;       # Post-primary
    local @classify_stack = ();

    %current_primaries = ();
    @pre_primary = ();
    @post_primary = ();
    @unusual_one_time = ();

    rdb_recurse( \@requested_targets, \&rdb_classify1, 0,0, \&rdb_classify2 );

    # Reverse, as tendency is to find last rules first.
    @pre_primary = reverse @pre_primary;
    @post_primary = reverse @post_primary;

    my @current_primaries = keys %current_primaries;
    if ($#current_primaries < 0) {
        die "$My_name: No active primary rules found.  I have to stop.\n";
    }
    elsif ($#current_primaries > 0) {
        die "$My_name: More than one active primary rule found.  I have to stop.\n",
            "  Primary rules: @current_primaries\n";
    }
    $current_primary = $current_primaries[0];

    if ($diagnostics) {
        print "Rule classification: \n";
        if ($#requested_targets < 0) {
            print "  No requested rules\n";
        }
        else {
            print "  Requested rules:\n";
            foreach ( @requested_targets ) { print "    $_\n"; }
        }
        if ($#pre_primary < 0) {
            print "  No pre-primaries\n";
        }
        else {
            print "  Pre-primaries:\n";
            foreach (@pre_primary) { print "    $_\n"; }
        }
        print "  Primaries:\n";
        foreach (keys %current_primaries) { print "    $_\n"; }
        if ($#post_primary < 0) {
            print "  No post-primaries\n";
        }
        else {
            print "  Post-primaries:\n";
            foreach (@post_primary) { print "    $_\n"; }
        }
        if ($#unusual_one_time < 0) {
            print "  No inner-level one_time rules, as expected\n";
        }
        else {
            print "  Inner-level one_time rules:\n";
            foreach ( @unusual_one_time ) { print "    $_\n"; }
        }
        my @normal_one_time = keys %one_time;
        if ($#normal_one_time < 0) {
            print "  No outer-level one_time rules\n";
        }
        else {
            print "  Outer-level one_time rules:\n";
            foreach ( @normal_one_time ) { print "    $_\n"; }
        }
    } #end diagnostics

} #END rdb_classify_rules

#-------------------

sub rdb_classify1 {
    # Helper routine for rdb_classify_rules
    # Applied as rule_act1 in recursion over rules
    # Assumes rule context, and local variables from rdb_classify_rules
    push @classify_stack, [$state];
    if ( exists $possible_one_time{$rule} ) {
        # Normally, we will have already extracted the one_time rules,
        # and they will never be accessed here.  But just in case of
        # problems or generalizations, we will cover all possibilities:
        if ($depth > 1) {
           warn "ONE TIME rule not at outer level '$rule'\n";
        }
        push @unusual_one_time, $rule;
    }
    elsif ($state == 0) {
       if ( exists $possible_primaries{$rule} ) {
           $state = 1;   # In primary rule
           $current_primaries{ $rule } = 1;
       }
       else {
           push @post_primary, $rule;
       }
    }
    else {
        $state = 2;     # in post-primary rule
        push @pre_primary, $rule;
    }
} #END rdb_classify1

#-------------------

sub rdb_classify2 {
    # Helper routine for rdb_classify_rules
    # Applied as rule_act2 in recursion over rules
    # Assumes rule context
    ($state) = @{ pop @classify_stack };
} #END rdb_classify2

#************************************************************


sub rdb_run1 {
    # Assumes context for: rule.
    # Unconditionally apply the rule
    # Returns return code from applying the rule.
    # Otherwise: 0 on other kind of success, 
    #            -1 on error, 
    #            -2 when missing dest_file is to be ignored

    # Source file data, by definition, correspond to the file state just
    # before the latest run, and the run_time to the time just before the run:
    &rdb_update_files;
    $$Prun_time = time();
    $$Pchanged = 0;       # No special changes in files
    $$Plast_result = 0;
    $$Plast_message = '';

    # Return values for external command:
    my $return = 0;

    # Find any internal command
    my @int_args = @$PAint_cmd;
    
    my $int_cmd = shift @int_args;
    my @int_args_for_printing = @int_args;
    foreach (@int_args_for_printing) {
        if ( ! defined $_ ) { $_ = 'undef'; }
    }

    # The actual execution of the command:
    my $time = processing_time();
    if ($int_cmd) {
        print "For rule '$rule', use internal command '\&$int_cmd( @int_args_for_printing )' ...\n"
            if $diagnostics;
        $return = &$int_cmd( @int_args ); 
    }
    elsif ($$Pext_cmd) {
        $return = &Run_subst() / 256;
    }
    else {
        warn "$My_name: Either a bug OR a configuration error:\n",
             "    No command provided for '$rule'\n";
        traceback();
        $return = -1;
        $$Plast_result = 2;
        $$Plast_message = "Bug or configuration error; incorrect command type";
    }
    $time = processing_time() - $time;
    push @timings, "'$_[0]': time = $time\n";            

    if ( $rule =~ /^biber/ ) {
        my @biber_source = ( );
        my $retcode = check_biber_log( $$Pbase, \@biber_source );
        foreach my $source ( @biber_source ) {
#           if ( $source =~ /\"/ ) {next; }
            print "  ===Source file '$source' for '$rule'\n"
               if ($diagnostics);
            rdb_ensure_file( $rule, $source );
        }
        if ($retcode == 5) {
        # Special treatment if sole missing file is bib file
        # I don't want to treat that as an error
            $return = 0;
            $$Plast_result = 200;
            $$Plast_message = "Could not find bib file for '$$Pbase'";
            push @warnings, "Bib file not found for '$$Pbase'";
        }
        elsif ($retcode == 6) {
           # Missing control file.  Need to remake it (if possible)
           # Don't treat missing bbl file as error.
           warn "$My_name: bibtex control file missing.  Since that can\n",
                "   be recreated, I'll try to do so.\n";
           $return = -2;
           rdb_for_some( [keys %current_primaries], sub{ $$Pout_of_date = 1; } );
        }
        elsif ($retcode == 4) {
            $$Plast_result = 2;
            $$Plast_message = "Could not find all biber source files for '$$Pbase'";
            push @warnings, "Not all biber source files found for '$$Pbase'";
        }
        elsif ($retcode == 3) {
            $$Plast_result = 2;
            $$Plast_message = "Could not open biber log file for '$$Pbase'";
            push @warnings, $$Plast_message;
        }
        elsif ($retcode == 2) {
            $$Plast_message = "Biber errors: See file '$$Pbase.blg'";
            push @warnings, $$Plast_message;
        }
        elsif ($retcode == 1) {
            push @warnings, "Biber warnings for '$$Pbase'";
        }
        elsif ($retcode == 10) {
            push @warnings, "Biber found no citations for '$$Pbase'";
            # Biber doesn't generate a bbl file in this situation.
            $return = -2;
        }
        elsif ($retcode == 11) {
            push @warnings, "Biber: malformed bcf file for '$$Pbase'.  IGNORE";
            if (!$silent) {
               warn "$My_name: biber found malformed bcf file for '$$Pbase'.\n",
                    "  I'll ignore error, and delete any bbl file.\n";
            }
            # Malformed bcf file is a downstream consequence, normally,
            # of an error in *latex run.  So this is not an error
            # condition in biber itself.
            # Current version of biber deletes bbl file.
            # Older versions (pre-2016) made an incorrect bbl file, which
            # tended to cause latex errors, and give a self-perpetuating error.
            # To be safe, ensure the bbl file doesn't exist.
            unlink $$Pdest;
            # The missing bbl file is now not an error:
            $return = -2;
# ??????? BCF
# Following is intended to work, but creates infinite loop
# in malformed bcf file situation under -pvc.
# since on each check for change in ANY file, pvc finds changed file
# Need to restrict pvc reruns to case of changed USER files
#           # To give good properties for *latex rule, it is best
#           # to have a valid bbl file that exists:
#           create_empty_file( $$Pdest );
#            $return = 0;
            
        }
    }
    if ( $rule =~ /^bibtex/ ) {
        my $retcode = check_bibtex_log($$Pbase);
        if ( ! -e $$Psource ) {
            $retcode = 10;
            rdb_for_some( [keys %current_primaries], sub{ $$Pout_of_date = 1; } );
        }
        if ($retcode == 3) {
            $$Plast_result = 2;
            $$Plast_message = "Could not open bibtex log file for '$$Pbase'";
            push @warnings, $$Plast_message;
        }
        elsif ($retcode == 2) {
            $$Plast_message = "Bibtex errors: See file '$$Pbase.blg'";
            $failure = 1;
            push @warnings, $$Plast_message;
        }
        elsif ($retcode == 1) {
            push @warnings, "Bibtex warnings for '$$Pbase'";
        }
        elsif ($retcode == 10) {
            push @warnings, "Bibtex found no citations for '$$Pbase',\n",
                            "    or bibtex found a missing aux file\n";
            if (! -e $$Pdest ) {
                warn "$My_name: Bibtex did not produce '$$Pdest'.  But that\n",
                     "     was because of missing files, so I will continue.\n";
                $return = -2;
            }
            else {
                $return = 0;
            }
        }
    }

    if ( ($$Pcmd_type eq 'primary') && ( $aux_dir ne $out_dir ) ) {
        &move_out_files_from_aux;
    }
    $updated = 1;
    if ($$Ptest_kind == 3) { 
        # We are time-criterion first time only.  Now switch to
        # file-change criterion
        $$Ptest_kind = 1; 
    }
    $$Pout_of_date = $$Pout_of_date_user = 0;

    if ( ($$Plast_result == 0) && ($return != 0) && ($return != -2) ) {
        $$Plast_result = 2;
        if ($$Plast_message eq '') {
            $$Plast_message = "Command for '$rule' gave return code $return";
            if ($rule =~ /^(pdf|lua|xe|)latex/) {
                $$Plast_message .= "\n      Refer to '$log_name' for details";
            }
            elsif ($rule =~ /^makeindex/) {
                $$Plast_message .= "\n      Refer to '${aux_dir1}${root_filename}.ilg' for details";
            }
        }
    }
    elsif ( $$Pdest && (! -e $$Pdest) && ($return != -2) ) {
        $$Plast_result = 1;
    }
    return $return;
}  # END rdb_run1

#-----------------

sub rdb_dummy_run0 {
    # Assumes contexts for: rule.
    # Update rule state as if the rule ran successfully,
    #    but don't run the rule.
    # Returns 0 (success code)

    # Source file data, by definition, correspond to the file state just before 
    # the latest run, and the run_time to the time just before the run:
    &rdb_update_files;
    $$Prun_time = time();
    $$Pchanged = 0;       # No special changes in files
    $$Plast_result = 0;
    $$Plast_message = '';

    if ($$Ptest_kind == 3) { 
        # We are time-criterion first time only.  Now switch to
        # file-change criterion
        $$Ptest_kind = 1; 
    }
    $$Pout_of_date = $$Pout_of_date_user = 0;

    return 0;
}  # END rdb_dummy_run0

#-----------------

sub Run_subst {
    # Call: Run_subst( cmd, msg, options, source, dest, base )
    # Runs command with substitutions.
    # If an argument is omitted or undefined, it is replaced by a default:
    #    cmd is the command to execute
    #    msg is whether to print a message: 
    #           0 for not, 1 according to $silent setting, 2 always
    #    options, source, dest, base: correspond to placeholders.
    # Substitutions:
    #    %S=source, %D=dest, %B=base, %R=root=base for latex, %O=options, 
    #    %T=texfile,
    #    %V=$aux_dir, %W=$out_dir, %Y=$aux_dir1, %Z=$out_dir1
    # This is a globally usable subroutine, and works in a rule context,
    #    and outside.
    # Defaults:
    #     cmd: $PPext_cmd if defined, else '';
    #     msg: 1
    #     options: ''
    #     source:  $$Psource if defined, else $texfile_name;
    #     dest:    $$Pdest if defined, else $view_file, else '';
    #     base:    $$Pbase if defined, else $root_filename;

    my ($ext_cmd, $msg, $options, $source, $dest, $base ) = @_;

    $ext_cmd ||= ( $Pext_cmd ? $$Pext_cmd : '' );
    $msg     =   ( defined $msg ? $msg : 1 );
    $options ||= '';
    $source  ||= ( $Psource ? $$Psource : $texfile_name );
    $dest    ||= ( $Pdest ? $$Pdest : ( $view_file || '' ) );
    $base    ||= ( $Pbase ? $$Pbase : $root_filename );

    if ( $ext_cmd eq '' ) {
         return 0;
    }

    #Set character to surround filenames:
    my %subst = ( 
       '%A' => $quote.$tex_basename.$quote,
       '%B' => $quote.$base.$quote,
       '%D' => $quote.$dest.$quote,
       '%O' => $options,
       '%S' => $quote.$source.$quote,
       '%R' => $quote.$root_filename.$quote,
       '%S' => $quote.$source.$quote,
       '%T' => $quote.$texfile_name.$quote,
       '%V' => $quote.$aux_dir.$quote,
       '%W' => $quote.$out_dir.$quote,
       '%Y' => $quote.$aux_dir1.$quote,
       '%Z' => $quote.$out_dir1.$quote,
       '%%' => '%'         # To allow literal %B, %R, etc, by %%B.
        );
    if ($pre_tex_code) {
        $subst{'%U'} = $quote.$pre_tex_code.$quote;
        $subst{'%P'} = "$quote$pre_tex_code\\input{$source}$quote";
    }
    else {
        $subst{'%U'} = '';
        $subst{'%P'} = $subst{'%S'};
    }
    if ( ($^O eq "MSWin32" ) && $MSWin_back_slash ) {
        foreach ( '%R', '%B', '%T', '%S', '%D', '%Y', '%Z' ) {
            $subst{$_} =~ s(/)(\\)g;
        }
    }

    my @tokens = split /(%.)/, $ext_cmd;
    foreach (@tokens) {
        if (exists($subst{$_})) { $_ = $subst{$_}; }
    }
    $ext_cmd = join '', @tokens;

    my ($pid, $return) = 
          ( ($msg == 0) || ( ($msg == 1) && $silent ) )
             ? &Run($ext_cmd)
             : &Run_msg($ext_cmd);
    return $return;
} #END Run_subst

#-----------------

sub rdb_primary_run {
    # Call: rdb_primary_run
    # Assumes contexts for: recursion, make, & rule.
    # Assumes (a) the rule is a primary, 
    #         (b) a run has to be made,
    #         (c) source files have been made.
    # This routine carries out the run of the rule unconditionally,
    # and then parses log file etc.
    my $return = 0;

    if ( ! $filetime_offset_measured ) {
        $filetime_offset = get_filetime_offset( $aux_dir1."tmp" );
        if ( (abs($filetime_offset) > $filetime_offset_report_threshold)
             && ($diagnostics || ! $silent) )
        {
            warn "$My_name: I am working around an offset relative to my system time by\n",
                 "   $filetime_offset secs for file times in directory '$aux_dir1'.\n";
        }
        $filetime_offset_measured = 1;
    }

    # Need to reset the list of generated files.  If we don't it can contain
    # out-of-date items from previous run.  (Think bibtopic, which writes
    # bbl files!)
    &rdb_initialize_generated;
    my $return_latex = &rdb_run1;

    # Need to worry about changed directory, changed output extension
    # Where else is $missing_dvi_pdf set?  Was it initialized?
    if (-e $$Pdest) { $missing_dvi_pdf = '';}

    # Handle case that log file is caused to be in an unexpected place,
    #   from a configuration error:
    &find_set_log;

    if ($recorder) {
        # Handle problem that some version of *latex give fls files
        #    of name latex.fls or pdflatex.fls instead of $root_filename.fls.
        # Also that setting of -output-directory -aux-directory is not 
        #    respected by *latex, at least in some versions.
        my $std_fls_file = $fls_name;
        my @other_fls_names = ( );
        if ( $rule =~ /^pdflatex/ ) {
            push @other_fls_names, "pdflatex.fls";
        }
        else {
            push @other_fls_names, "latex.fls";
        }
        if ( $aux_dir1 ne '' ) {
            push @other_fls_names, "$root_filename.fls";
            # MiKTeX uses out_dir for .fls. However, it seems logical to
            # me for .fls to be in aux_dir.  So I'll allow for this
            # Possibility, although I don't know if it has been used.
            push @other_fls_names, "$aux_dir1$root_filename.fls";
        }
        # Find the first non-standard fls file and copy it to the standard
        # place. But only do this if the file time is compatible with being
        # generated in the current run, and if the standard fls file hasn't
        # been made in the current run,  as tested by the use of
        # test_gen_file; that avoids problems with fls files leftover from
        # earlier runs with other versions of latex.
        if ( ! test_gen_file( $std_fls_file ) ) {
            foreach my $cand (@other_fls_names) {
                if ( test_gen_file( $cand ) ) {
                    copy $cand, $std_fls_file;
                    last;
                }
            }
        }
        if ( ! test_gen_file( $std_fls_file ) ) {
            warn "$My_name: fls file doesn't appear to have been made.\n";
        }
    }

    # Find current set of source files:
    my ($missing_dirs, $PA_missing_subdirs) = &rdb_set_latex_deps;

    # For each file of the kind made by epstopdf.sty during a run, 
    #   if the file has changed during a run, then the new version of
    #   the file will have been read during the run.  Unlike the usual
    #   case, we will NOT need to redo the primary run because of the
    #   change of this file during the run.  Therefore set the file as
    #   up-to-date:
    rdb_do_files( sub { if ($$Pcorrect_after_primary) {&rdb_update1;} } );

    $updated = 1;    # Flag that some dependent file has been remade

    if ( $diagnostics ) {
        print "$My_name: Rules after run: \n";
        rdb_show();
    }

    $return = $return_latex;

# ???? Is the following needed?
    if ($return_latex && $$Pout_of_date_user) {
       print "Error in *LaTeX, but change of user file(s), ",
             "so ignore error & provoke rerun\n"
          if (! $silent);
       $return = 0;
    }
    if ($return_latex && ($missing_dirs ne 'none') ) {
       print "Error in *LaTeX, but needed subdirectories in output directory\n",
             "   were missing and successfully created, so try again.\n"
          if (! $silent);
       $return = 0;
    }
    # Summarize issues that may have escaped notice:
    @primary_warning_summary = ();
    if ($bad_reference) {
        push @primary_warning_summary,
             "Latex failed to resolve $bad_reference reference(s)";
    }
    if ($mult_defined) {
        push @primary_warning_summary,
             "Latex found $mult_defined multiply defined reference(s)";
    }
    if ($bad_character) {
        push @primary_warning_summary,
            "=====Latex reported missing or unavailable character(s).\n".
            "=====See log file for details.";
    }
    if ($bad_citation) {
        push @primary_warning_summary,
             "Latex failed to resolve $bad_citation citation(s)";
    }
    if ( $diagnostics && ($#primary_warning_summary > -1) ) {
       show_array( "$My_name: Summary of warnings:", @primary_warning_summary );
    }
    return $return;
} #END rdb_primary_run

#************************************************************

sub rdb_clear_change_record {
    # Initialize diagnostics for reasons for running rule.
    @changed = ();
    %changed_rules = ();
    @changed_user = ();
    @disappeared = ();
    @no_dest = ();          # We are not now using this
    @rules_never_run = ();
    @rules_to_apply = ();   # This is used in recursive application
                            # of rdb_flag_changes_here, to list
                            # rules that were out-of-date for some reason.
} #END rdb_clear_change_record 

#************************************************************

sub rdb_flag_changes_here {
    # Flag changes in current rule.  
    # Assumes rule context.
    # Usage: rdb_flag_changes_here( ignore_run_time )
    # Argument: if true then fdb_get shouldn't do runtime test
    #             for recalculation of md5
    local $ignore_run_time = $_[0];
    if ( ! defined $ignore_run_time ) { $ignore_run_time = 0; }

    $$Pcheck_time = time();

    local $dest_mtime = 0;
    $dest_mtime = get_mtime($$Pdest) if ($$Pdest);
    rdb_do_files( \&rdb_file_change1);
    while ( my ($s_rule, $l_pass) = each %$PHsource_rules ) {
        if ( defined $pass{$s_rule}
             && ($pass{$s_rule} > $l_pass)
            )
        {
            $changed_rules{$s_rule} = $rule;
            $$Pout_of_date = 1;
        }
    }
    if ($$Pout_of_date) {
        push @rules_to_apply, $rule;
    }
} #END rdb_flag_changes_here

#************************************************************

sub rdb_file_change1 {
    # Call: &rdb_file_change1
    # Assumes rule and file context.  Assumes $dest_mtime set.
    # Flag whether $file in $rule has changed or disappeared.
    # Set rule's make flag if there's a change.

    my $check_time_argument = 0;
    if (! $ignore_run_time ) {
        $check_time_argument = max( $$Pcheck_time, $$Prun_time );
    }
    my ($new_time, $new_size, $new_md5) = fdb_get($file, $check_time_argument );
    my $ext_no_period = ext_no_period( $file );
    my $generated = exists $from_rules{$file};
    if ( ($new_size < 0) && ($$Psize >= 0) ) {
        # print "Disappeared '$file' in '$rule'\n";
        push @disappeared, $file;
        # No reaction is good.  
        #$$Pout_of_date = 1;
        # ??? 1 Sep. 2008: I do NOT think so, for cusdep no-file-exists issue
        # ??? 30 Sep 2008: I think I have this fixed.  There were other changes
        #  needed.  No-change-flagged is correct.  The array @disappeared flags 
        #  files that have disappeared, if I need to know.  But having a source
        #  file disappear is not a reason for a remake unless I know how to 
        #  make the file.  If the file is a destination of a rule, that rule
        #  will be rerun.  It may be that the user is changing another source 
        #  in such a way that the disappeared file won't be needed.  Before the
        #  change is applied we get a superfluous infinite loop.
        return;
    }
    if ( ($new_size < 0) && ($$Psize < 0) ) {
        return;
    }
    # Primarily use md5 signature to determine whether file contents have
    #   changed.
    # Backup by file size change, but only in the case where there is
    #   no pattern of lines to ignore in testing for a change
    if ( ($new_md5 ne $$Pmd5) 
         || (
              (! exists $hash_calc_ignore_pattern{$ext_no_period})
              && ($new_size != $$Psize)   
            )
       ) {
        push @changed, $file;
        $$Pout_of_date = 1;
        if ( ! $generated ) {
            push @changed_user, $file;
            $$Pout_of_date_user = 1;
        }
    }
    elsif ( $new_time != $$Ptime ) {
        $$Ptime = $new_time;
    }
    if ( ( ($$Ptest_kind == 2) || ($$Ptest_kind == 3) )
         && (! $generated)
         && ( $new_time > $dest_mtime )
        ) {
            push @changed, $file;
            $$Pout_of_date = $$Pout_of_date_user = 1;
    }
} #END rdb_file_change1

#************************************************************

sub rdb_user_changes {
    # Argument(s): a set of top level rules.
    # Aim: Find any changed user files for those rules and all ancestors.
    # Assumption: List of from_rules for files is up-to-date.
    &rdb_clear_change_record;
    rdb_recurse( [@_], sub{ &rdb_flag_changes_here(1); } );
    if ($#changed_user >=0) { show_array( 'User changed files', @changed_user ); }
    return ($#changed_user >= 0);
} #END rdb_user_changes

#************************************************************

sub rdb_diagnose_changes {
    # Call: rdb_diagnose_changes or rdb_diagnose_changes( heading )
    # List changes on STDERR
    # Precede the message by the optional heading, else by "$My_name: " 
    my $heading = defined($_[0]) ?   $_[0]  :  "$My_name: "; 

    if ($#rules_never_run >= 0) {
        warn "${heading}Rules & subrules not known to be previously run:\n";
        foreach (@rules_never_run) { warn "   $_\n"; }
    }
    if ( ($#changed >= 0) || (keys %changed_rules > 0) || ($#disappeared >= 0) || ($#no_dest >= 0) ) {
        warn "${heading}File changes, etc:\n";
        if ( $#changed >= 0 ) {
            warn "   Changed files, or newly in use since previous run(s):\n";
            foreach (uniqs(@changed)) { warn "      '$_'\n"; }
        }
        if ( $#disappeared >= 0 ) {
            warn "   No-longer-existing files:\n";
            foreach (uniqs(@disappeared)) { warn "      '$_'\n"; }
        }
        if ( $#no_dest >= 0 ) {
            warn "   Non-existent destination files:\n";
            foreach (uniqs(@no_dest)) { warn "      '$_'\n"; }
        }
        if ( keys %changed_rules > 0 ) {
            warn "   Rule(s) that have been run and require run of dependent rule:\n";
            while (my ($s_rule, $d_rule) = each %changed_rules) {
                warn "      '$s_rule' which requires run of '$d_rule'\n";
            }
        }
    }
    elsif ($#rules_to_apply >=0) {
         warn "${heading}The following rules & subrules became out-of-date:\n";
         foreach (@rules_to_apply) { warn "      '$_'\n"; }
    }
    else {
        warn "${heading}No file changes\n";
    }
}     #END rdb_diagnose_changes


#************************************************************
#************************************************************
#************************************************************
#************************************************************

#************************************************************
#************************************************************
#************************************************************
#************************************************************

# Routines for convenient looping and recursion through rule database
# ================= NEW VERSION ================

# There are several places where we need to loop through or recurse
# through rules and files.  This tends to involve repeated, tedious
# and error-prone coding of much book-keeping detail.  In particular,
# working on files and rules needs access to the variables involved,
# which either involves direct access to the elements of the database,
# and consequent fragility against changes and upgrades in the
# database structure, or involves lots of routines for reading and
# writing data in the database, then with lots of repetitious
# house-keeping code.
#
# The routines below provide a solution.  Looping and recursion
# through the database are provided by a set of basic routines where
# each necessary kind of looping and iteration is coded once.  The
# actual actions are provided as references to action subroutines.
# (These can be either actual references, as in \&routine, or
# anonymous subroutines, as in sub{...}, or aas a zero value 0 or an
# omitted argument, to indicate that no action is to be performed.)
#
# When the action subroutine(s) are actually called, a context for the
# rule and/or file (as appropriate) is given by setting named
# variables to REFERENCES to the relevant data values.  These can be
# used to retrieve and set the data values.  As a convention,
# references to scalars are given by variables named start with "$P",
# as in "$Pdest", while references to arrays start with "$PA", as in 
# "$PAint_cmd", and references to hashes with "$PH", as in "$PHsource".
# After the action subroutine has finished, checks for data
# consistency may be made. 
#
# The only routines that actually use the database structure and need
# to be changed if that is changed are:  (a) the routines rdb_one_rule
# and rdb_one_file that implement the calling of the action subroutines,
# (b) routines for creation of single rules and file items, and (c) to
# a lesser extent, the routine for destroying a file item.  
#
# Note that no routine is provided for destroying a rule.  During a
# run, a rule, with its source files, may become inaccessible or
# unused.  This happens dynamically, depending on the dependencies
# caused by changes in the source file or by error conditions that
# cause the computation of dependencies, particular of latex files, to
# become wrong.  In that situation the files certainly come and go in
# the database, but subsidiary rules, with their content information
# on their source files, need to be retained so that their use can be
# reinstated later depending on dynamic changes in other files.
#
# However, there is a potential memory leak unless some pruning is
# done in what is written to the fdb file.  (Probably only accessible
# rules and those for which source files exist.  Other cases have no
# relevant information that needs to be preserved between runs.)

#
#


#************************************************************

# First the top level routines for recursion and iteration

#************************************************************

sub rdb_recurse {
    # Call: rdb_recurse( rule | [ rules],
    #                    \&rule_act1, \&file_act1, \&file_act2, 
    #                    \&rule_act2 )
    # The actions are pointers to subroutines, and may be null (0, or
    # undefined) to indicate no action to be applied.
    # Recursively acts on the given rules and all ancestors:
    #   foreach rule found:
    #       apply rule_act1
    #       loop through its files:
    #          apply file_act1
    #          act on its ancestor rule, if any
    #          apply file_act2
    #       apply rule_act2
    # Guards against loops.  
    # Access to the rule and file data by local variables, only
    #   for getting and setting.

    # This routine sets a context for anything recursive, with @heads,
    # %visited  and $depth being set as local variables.

    local @heads = ();
    my $rules = shift;

    # Distinguish between single rule (a string) and a reference to an
    # array of rules:
    if ( ref $rules eq 'ARRAY' ) { @heads = @$rules; }
    else { @heads = ( $rules ); }

    # Keep a list of visited rules, used to block loops in recursion:
    local %visited = (); 
    local $depth = 0;

    foreach $rule ( @heads ) {
        if ( rdb_is_active($rule) ) { rdb_recurse_rule( $rule, @_ ); }
    }

} #END rdb_recurse

#************************************************************

sub rdb_for_actives {
    # Call: rdb_for_actives( \&rule_act1, \&file_act, \&rule_act2 )
    # Loops through all rules and their source files, using the 
    #   specified set of actions, which are pointers to subroutines.
    # Sorts rules alphabetically.
    # See rdb_for_some for details.
#    rdb_for_some( [ sort keys %rule_db ], @_);
    rdb_for_some( [ sort &rdb_actives ], @_);
} #END rdb_for_actives

#************************************************************

sub rdb_for_some {
    # Call: rdb_for_some( rule | [ rules],
    #                    \&rule_act1, \&file_act, \&rule_act2)
    # Actions can be zero, and rules at tail of argument list can be
    # omitted.  E.g. rdb_for_some( rule, 0, \&file_act ).  
    # Anonymous subroutines can be used, e.g., rdb_for_some( rule, sub{...} ).  
    #
    # Loops through rules and their source files, using the 
    # specified set of rules:
    #   foreach rule:
    #       apply rule_act1
    #       loop through its files:
    #          apply file_act
    #       apply rule_act2
    #
    # Rule data and file data are made available in local variables 
    # for access by the subroutines.

    local @heads = ();
    my $rules = shift;
    # Distinguish between single rule (a string) and a reference to an
    # array of rules:
    if ( ref $rules eq 'ARRAY' ) { @heads = @$rules; }
    else { @heads = ( $rules ); }

    foreach $rule ( @heads ) {
        # $rule is implicitly local
        &rdb_one_rule( $rule, @_ );
    }
}  #END rdb_for_some

#************************************************************

sub rdb_for_one_file {
    my $rule = shift;
    # Avoid name collisions with general recursion and iteraction routines:
    local $file1 = shift;
    local $action1 = shift;
    rdb_for_some( $rule, sub{rdb_one_file($file1,$action1)} );
} #END rdb_for_one_file


#************************************************************

#   Routines for inner part of recursion and iterations

#************************************************************

sub rdb_recurse_rule {
    # Call: rdb_recurse_rule($rule, \&rule_act1, \&file_act1, \&file_act2, 
    #                    \&rule_act2 )
    # to do the work for one rule, recurisvely called from_rules for
    # the sources of the rules.
    # Assumes recursion context, i.e. that %visited, @heads, $depth.
    # We are overriding actions:
    my ($rule, $rule_act1, $new_file_act1, $new_file_act2, $rule_act2)
        = @_;
    if (! rdb_is_active($rule)) { return; }
    # and must propagate the file actions:
    local $file_act1 = $new_file_act1;
    local $file_act2 = $new_file_act2;
    # Prevent loops:
    if ( (! $rule) || exists $visited{$rule} ) { return; }
    $visited{$rule} = 1;
    # Recursion depth
    $depth++;
    # We may need to repeat actions on dependent rules, without being
    # blocked by the test on visited files.  So save %visited:
    # NOT CURRENTLY USED!!    local %visited_at_rule_start = %visited;
    # At end, the last value set for %visited wins.
    rdb_one_rule( $rule, $rule_act1, \&rdb_recurse_file, $rule_act2 );
    $depth--;
 } #END rdb_recurse_rule 

#************************************************************

sub rdb_recurse_file {
    # Call: rdb_recurse_file to do the work for one file.
    # This has no arguments, since it is used as an action subroutine,
    # passed as a reference in calls in higher-level subroutine.
    # Assumes contexts set for: Recursion, rule, and file
    &$file_act1 if $file_act1;
    rdb_recurse_rule( $$Pfrom_rule, $rule_act1, $file_act1, $file_act2,
                      $rule_act2 )
        if $$Pfrom_rule;
    &$file_act2 if $file_act2;
} #END rdb_recurse_file

#************************************************************

sub rdb_do_files {
    # Assumes rule context, including $PHsource.
    # Applies an action to all the source files of the rule.
    local $file_act = shift;
    my @file_list = sort keys %$PHsource;
    foreach my $file ( @file_list ){
        rdb_one_file( $file, $file_act );
    }
} #END rdb_do_files

#************************************************************

# Routines for action on one rule and one file.  These are the main
# places (in addition to creation and destruction routines for rules
# and files) where the database structure is accessed.

#************************************************************

sub rdb_one_rule {
    # Call: rdb_one_rule( $rule, $rule_act1, $file_act, $rule_act2 )
    # Sets context for rule and carries out the actions.
#===== Accesses rule part of database structure =======

    local ( $rule, $rule_act1, $file_act, $rule_act2 ) = @_;
    if ( (! $rule) || ! rdb_rule_exists($rule) ) { return; }

    local ( $PArule_data, $PHsource, $PHdest, $PHsource_rules ) = @{$rule_db{$rule}};
    local ($Pcmd_type, $Pext_cmd, $PAint_cmd, $Ptest_kind, 
           $Psource, $Pdest, $Pbase,
           $Pout_of_date, $Pout_of_date_user, $Prun_time, $Pcheck_time,
           $Pchanged,
           $Plast_result, $Plast_message, $PA_extra_gen )
        = Parray( $PArule_data );

    &$rule_act1 if $rule_act1;
    &rdb_do_files( $file_act ) if $file_act;
    &$rule_act2 if $rule_act2;
} #END rdb_one_rule

#************************************************************

sub rdb_activate {
    # Usage rdb_activate( rule_names )
    # Turns on active flag for the rules
    foreach ( @_ ) {
        if ( rdb_rule_exists($_) ) { $actives{$_} = 1; }
    }
}

#--------------------------------------------------

sub rdb_deactivate {
    # Usage rdb_deactivate( rule_names )
    # Turns off active flag for the rules
    foreach ( @_ ) { delete $actives{$_}; }
}

#--------------------------------------------------

sub rdb_activate_request {
    # Usage rdb_activate_request( rule_names )
    # Turns on active flag for the rules.
    # Adds rules to target_rules list
    foreach ( @_ ) {
        if ( rdb_rule_exists($_) ) { $actives{$_} = 1; $target_rules{$_} = 1; }
    }
}

#--------------------------------------------------

sub rdb_deactivate_derequest {
    # Usage rdb_deactivate_derequest( rule_names )
    # Turns off active flag for the rules
    # Removes rules from target_rules list
    foreach ( @_ ) { delete $actives{$_}; delete $target_rules{$_}; }
}

#--------------------------------------------------
sub rdb_is_active {
    # Usage rdb_is_active( rule_name )    
    if ( (exists $actives{$_[0]}) && rdb_rule_exists($_[0]) ) { return 1; }
    else { return 0; }
}

#--------------------------------------------------

sub rdb_actives {
    # Returns array of active rules
    return keys %actives;
}

#************************************************************

sub rdb_one_file {
    # Call: rdb_one_file($file, $file_act)
    # Sets context for file and carries out the action.
    # Assumes $rule context set.
#===== Accesses file part of database structure =======
    local ($file, $file_act) = @_;
    if ( (!$file) ||(!exists ${$PHsource}{$file}) ) { return; }
    local $PAfile_data = ${$PHsource}{$file};
    local ($Ptime, $Psize, $Pmd5, $Pfrom_rule, $Pcorrect_after_primary ) 
          = Parray( $PAfile_data );
    &$file_act() if $file_act;
    if ( ! rdb_rule_exists( $$Pfrom_rule ) ) {
        $$Pfrom_rule = '';
    }
} #END rdb_one_file

#************************************************************

# Routines for creation of rules and file items, and for removing file
# items. 

#************************************************************

sub rdb_remove_rule {
    # rdb_remove_rule( rule, ...  )
    foreach my $key (@_) {
       delete $rule_db{$key};
       delete $actives{$key};
    }
}

#************************************************************

sub rdb_create_rule {
    # rdb_create_rule( rule, command_type, ext_cmd, int_cmd, test_kind,
    #                  source, dest, base, 
    #                  needs_making, run_time, check_time, set_file_not_exists,
    #                  ref_to_array_of_specs_of_extra_generated_files )
    # int_cmd is either a string naming a perl subroutine or it is a
    # reference to an array containing the subroutine name and its
    # arguments. 
    # Makes rule.  Update rule if it already exists.
    # Omitted arguments: replaced by 0 or '' as needed.
    # Rule is made active
# ==== Sets rule data ====
    my ( $rule, $cmd_type, $ext_cmd, $PAint_cmd, $test_kind, 
         $source, $dest, $base, 
         $needs_making, $run_time, $check_time, $set_file_not_exists, $extra_gen ) = @_;
    my $active = 1;
    my $changed = 0;

    # Set defaults, and normalize parameters:
    foreach ( $cmd_type, $ext_cmd, $PAint_cmd, $source, $dest, $base, 
              $set_file_not_exists ) {
        if (! defined $_) { $_ = ''; }
    }
    if ( ($source =~ /\"/) || ($dest =~ /\"/) || ($base =~ /\"/) ) {
        die "$My_name: Error. In rdb_create_rule to create rule\n",
            "    '$rule',\n",
            "  there is a double quote in one of source, destination or base parameters:\n",
            "    '$source'\n",
            "    '$dest'\n",
            "    '$base'\n",
            "  I cannot handle this.  Cause is probably a latexmk bug.  Please report it.\n";
    }
    foreach ( $needs_making, $run_time, $check_time, $test_kind ) {
        if (! defined $_) { $_ = 0; }
    }
    if (!defined $test_kind) {
        # Default to test on file change
        $test_kind = 1; 
    }
    if ( ref( $PAint_cmd ) eq '' ) {
        #  It is a single command.  Convert to array reference:
        $PAint_cmd = [ $PAint_cmd ];
    }
    else {
        # COPY the referenced array:
        $PAint_cmd = [ @$PAint_cmd ];
    }
    my $PA_extra_gen = [];
    if ($extra_gen) {
        @$PA_extra_gen = @$extra_gen;
    }
    $rule_db{$rule} = 
        [  [$cmd_type, $ext_cmd, $PAint_cmd, $test_kind, 
            $source, $dest, $base,
            $needs_making, 0, $run_time, $check_time, $changed,
            -1, '', $PA_extra_gen ],
           {},
           {},
           {}
        ];
    if ($source) {
       rdb_ensure_file( $rule, $source, undef, $set_file_not_exists );  
    }
    rdb_one_rule( $rule, \&rdb_initialize_generated );
    if ($active) { rdb_activate($rule); }
    else { rdb_deactivate($rule); }
} #END rdb_create_rule

#************************************************************

sub rdb_initialize_generated {
# Assume rule context.
# Initialize hash of generated files
    %$PHdest = ();
    if ($$Pdest) { rdb_add_generated($$Pdest); }
    rdb_add_generated(@$PA_extra_gen);
} #END rdb_initialize_generated

#************************************************************

sub rdb_add_generated {
# Assume rule context.
# Add arguments to hash of generated files, and to global cache
    foreach (@_) {
        $$PHdest{$_} = 1;
        $from_rules{$_} = $rule;
    }
} #END rdb_add_generated

#************************************************************

sub rdb_remove_generated {
# Assume rule context.
# Remove arguments from hash of generated files
    foreach (@_) { delete $$PHdest{$_}; }
} #END rdb_remove_generated

#************************************************************

sub rdb_ensure_file {
    # rdb_ensure_file( rule, file[, fromrule[, set_not_exists]] )
    # Ensures the source file item exists in the given rule.
    # Then if the fromrule is specified, set it for the file item.
    # If the item is created, then:
    #    (a) by default initialize it to current file state.
    #    (b) but if the fourth argument, set_not_exists, is true, 
    #        initialize the item as if the file does not exist.
    #        This case is typically used when the log file for a run
    #        of latex/pdflatex claims that the file was non-existent
    #        at the beginning of a run. 
#============ rule and file data set here ======================================
    my $rule = shift;
    local ( $new_file, $new_from_rule, $set_not_exists ) = @_;
    if ( ! rdb_rule_exists( $rule ) ) {
        die_trace( "$My_name: BUG in call to rdb_ensure_file: non-existent rule '$rule'" );
    }
    if ( ! defined $new_file ) {
        die_trace( "$My_name: BUG in call to rdb_ensure_file: undefined file for '$rule'" );
    }
    if ( $new_file =~ /\"/ ) {
        warn "$My_name: in rdb_ensure_file for rule '$rule', there is a double quote in\n",
             "  the filename: '$new_file'.\n",
             "  I cannot handle this, will ignore this file.\n";
        return;
    }
    if ( ! defined $set_not_exists ) { $set_not_exists = 0; }
    rdb_one_rule( $rule, 
                  sub{
                      if (! exists ${$PHsource}{$new_file} ) {
                          if ( $set_not_exists ) {
                              ${$PHsource}{$new_file} = [@nofile, '', 0];
                          }
                          else {
                              ${$PHsource}{$new_file} 
                              = [fdb_get($new_file, $$Prun_time), '', 0];
                          }
                      }
                  }
    );
    if (defined $new_from_rule ) {
        rdb_for_one_file( $rule, $new_file, sub{ $$Pfrom_rule = $new_from_rule; });
    }
} #END rdb_ensure_file 

#************************************************************

sub rdb_remove_files {
    # rdb_remove_file( rule, file, ... )
    # Removes file(s) for the rule.  
    my $rule = shift;
    if (!$rule) { return; }
    local @files = @_;
    rdb_one_rule( $rule, 
                  sub{ foreach (@files) { delete ${$PHsource}{$_}; }  }
    );
} #END rdb_remove_files

#************************************************************

sub rdb_list_source {
    # rdb_list_source( rule )
    # Return array of source files for rule.
    my $rule = shift;
    my @files = ();
    rdb_one_rule( $rule, 
                  sub{ @files = keys %$PHsource; }
    );
    return @files;
} #END rdb_list_source

#************************************************************

sub rdb_set_source {
    # rdb_set_source( rule, file, ... )
    my $rule = shift;
    if (!$rule) { return; }
    my %files = ();
    foreach (@_) {
#       if ( /\"/ ) {next; }
        rdb_ensure_file( $rule, $_ );
        $files{$_} = 1;
    }
    foreach ( rdb_list_source($rule) ) {
        if ( ! exists $files{$_} ) { rdb_remove_files( $rule, $_ ); }
    }    
    return;
} #END rdb_list_source

#************************************************************

sub rdb_change_dest {
   # Assumes rule context.
   # Usage change_dest( new_dest [, flag] )
   # Changes destination for this rule. Fixes from_rule links.
   # If flag set, make the new_dest a source file in any rule
   # for which the old destination is already set.
   # No action if there's no change of destination.
   local ($new_dest, $flag) = @_;
   local $old_dest = $$Pdest;
   if ($old_dest eq $new_dest) { return; }
#   if ( $new_dest =~ /\"/ ) { return; }
   rdb_remove_generated( $old_dest );
   rdb_add_generated( $new_dest );
   if ($flag) {
      print "rdb_change_dest: fixing dependencies\n";
      rdb_for_actives( sub{ if ( rdb_file_exists( $rule, $old_dest ) ) {
                            rdb_ensure_file( $rule, $new_dest );
                            rdb_remove_files( $rule, $old_dest );
                        }
                      }
                 );
   }
   $$Pdest = $new_dest;
   # ??? Do I need to fix from_rule setting?
   #&rdb_make_links;
   return;
} #END rdb_change_dest

#************************************************************

sub rdb_rule_exists { 
    # Call rdb_rule_exists($rule): Returns whether rule exists.
    my $rule = shift;
    if (! $rule ) { return 0; }
    return exists $rule_db{$rule}; 
} #END rdb_rule_exists

#************************************************************

sub rdb_file_exists { 
    # Call rdb_file_exists($rule, $file): 
    # Returns whether source file item in rule exists.
    local ( $rule, $file ) = @_;
    local $exists = 0;
    rdb_one_rule( $rule, 
                  sub{ $exists =  exists( ${$PHsource}{$file} ) ? 1:0; } 
                );
    return $exists; 
} #END rdb_file_exists

#************************************************************

sub rdb_update_gen_files {
    # Assumes rule context.  Update source files of rule to current state.
    rdb_do_files( 
        sub{
            if ( exists $generated_exts_all{ ext_no_period($file) }
                 || exists $$PHdest{$file}
                ) {
                &rdb_update1;
            }
        }
    );
} #END rdb_update_gen_files

#************************************************************

sub rdb_update_files {
    # Call: rdb_update_files
    # Assumes rule context.  Update source files of rule to current state.
    rdb_do_files( \&rdb_update1 );
}

#************************************************************

sub rdb_update1 {
    # Call: rdb_update1.  
    # Assumes file context.  Updates file data to correspond to
    # current file state on disk
    ($$Ptime, $$Psize, $$Pmd5) = fdb_get($file);
}

#************************************************************

sub rdb_set_file1 {
    # Call: fdb_file1(rule, file, new_time, new_size, new_md5)
    # Sets file time, size and md5.
    my $rule = shift;
    my $file = shift;
    local @new_file_data = @_;
    rdb_for_one_file( $rule, $file, sub{ ($$Ptime,$$Psize,$$Pmd5)=@new_file_data; } );
}

#************************************************************

sub rdb_dummy_file {
    # Returns file data for non-existent file
# ==== Uses rule_db structure ====
    return (0, -1, 0, '');
}

#************************************************************
#************************************************************

# Predefined subroutines for custom dependency

sub cus_dep_delete_dest {
    # This subroutine is used for situations like epstopdf.sty, when
    #   the destination (target) of the custom dependency invoking
    #   this subroutine will be made by the primary run provided the
    #   file (destination of the custom dependency, source of the
    #   primary run) doesn't exist.
    # It is assumed that the resulting file will be read by the
    #   primary run.

    # Remove the destination file, to indicate it needs to be remade:
    unlink_or_move( $$Pdest );
    # Arrange that the non-existent destination file is not treated as
    #   an error.  The variable changed here is a bit misnamed.
    $$Pchanged = 1;
    # Ensure a primary run is done
    &cus_dep_require_primary_run;
    # Return success:
    return 0;
}

#************************************************************

sub cus_dep_require_primary_run {
    # This subroutine is used for situations like epstopdf.sty, when
    #   the destination (target) of the custom dependency invoking
    #   this subroutine will be made by the primary run provided the
    #   file (destination of the custom dependency, source of the
    #   primary run) doesn't exist.
    # It is assumed that the resulting file will be read by the
    #   primary run.

    local $cus_dep_target = $$Pdest;
    # Loop over all rules and source files:
    rdb_for_actives( 0, 
                 sub { if ($file eq $cus_dep_target) {
                            $$Pout_of_date = 1;
                            $$Pcorrect_after_primary = 1;
                       }
                     }
               );
    # Return success:
    return 0;
}


#************************************************************
#************************************************************
#************************************************************
#
#      UTILITIES:
#

#************************************************************
# Miscellaneous

sub show_array {
# For use in diagnostics and debugging. 
#  On stderr, print line with $_[0] = label.  
#  Then print rest of @_, one item per line preceeded by some space
    warn "$_[0]\n";
    shift;
    if ($#_ >= 0) {
        foreach (@_){
           if (defined $_ ) { warn "  $_\n"; }
           else { warn "  undef\n"; }
        }
    }
    else { warn "  NONE\n"; }
}


#************************************************************

sub array_to_hash {
    # Call: array_to_hash( items )
    # Returns: hash mapping items to 1
    my %hash = ();
    foreach (@_) {$hash{$_} = 1; }
    return %hash;
}
    
#************************************************************

sub Parray {
    # Call: Parray( \@A )
    # Returns array of references to the elements of @A
    # But if an element of @A is already a reference, the
    # reference will be returned in the output array, not a
    # reference to the reference.
    my $PA = shift;
    my @P = (undef) x (1+$#$PA);
    foreach my $i (0..$#$PA) {
        $P[$i] = (ref $$PA[$i]) ? ($$PA[$i]) : (\$$PA[$i]);
      }
    return @P;
}

#************************************************************

sub glob_list1 {
    # Glob a collection of filenames.  
    # But no sorting or elimination of duplicates
    # Usage: e.g., @globbed = glob_list1(string, ...);
    # Since perl's glob appears to use space as separator, I'll do a special check
    # for existence of non-globbed file (assumed to be tex like)

    my @globbed = ();
    foreach my $file_spec (@_) {
        # Problem, when the PATTERN contains spaces, the space(s) are
        # treated as pattern separaters.
        # Solution: I now the glob from use File::Glob.
        # The following hack avoids issues with glob in the case that a file exists
        # with the specified name (possibly with extension .tex):
        if ( -e $file_spec || -e "$file_spec.tex" ) { 
           # Non-globbed file exists, return the file_spec.
           # Return $file_spec only because this is not a file-finding subroutine, but
           #   only a globber
           push @globbed, $file_spec; 
        }
        else { 
            push @globbed, my_glob( "$file_spec" );
        }
    }
    return @globbed;
} #END glob_list1

#************************************************************
# Miscellaneous

sub prefix {
   #Usage: prefix( string, prefix );
   #Return string with prefix inserted at the front of each line
   my @line = split( /\n/, $_[0] );
   my $prefix = $_[1];
   for (my $i = 0; $i <= $#line; $i++ ) {
       $line[$i] = $prefix.$line[$i]."\n";
   }
   return join( "", @line );
} #END prefix


#===============================

sub parse_quotes {
    # Split string into words.
    # Words are delimited by space, except that strings
    # quoted all stay inside a word.  E.g., 
    #   'asdf B" df "d "jkl"'
    # is split to ( 'asdf', 'B df d', 'jkl').
    # An array is returned.
    my @results = ();
    my $item = '';
    local $_ = shift;
    pos($_) = 0;
  ITEM:
    while() {
        /\G\s*/gc;
        if ( /\G$/ ) {
            last ITEM;
        }
        # Now pos (and \G) is at start of item:
      PART:
        while () {
            if (/\G([^\s\"]*)/gc) {
                $item .= $1;
            }
            if ( /\G\"([^\"]*)\"/gc ) {
                # Match balanced quotes
                $item .= $1;
                next PART;
            }
            elsif ( /\G\"(.*)$/gc ) {
                # Match unbalanced quote
                $item .= $1;
                warn "====Non-matching quotes in\n    '$_'\n";
            }
            push @results, $item;
            $item = '';
            last PART;
        }
    }
    return @results;
} #END parse_quotes

#************************************************************
#************************************************************
#      File handling utilities:


#************************************************************

sub get_latest_mtime
# - arguments: each is a filename.
# - returns most recent modify time.
{
  my $return_mtime = 0;
  foreach my $include (@_)
  {
    my $include_mtime = &get_mtime($include);
    # The file $include may not exist.  If so ignore it, otherwise
    # we'll get an undefined variable warning.
    if ( ($include_mtime) && ($include_mtime >  $return_mtime) )
    {
      $return_mtime = $include_mtime;
    }
  }
  return $return_mtime;
}

#************************************************************

sub get_mtime_raw
{ 
  my $mtime = (stat($_[0]))[9];
  return $mtime;
}

#************************************************************

sub get_mtime { 
    return get_mtime0($_[0]);
}

#************************************************************

sub get_mtime0 {
   # Return time of file named in argument
   # If file does not exist, return 0;
   if ( -e $_[0] ) {
       return get_mtime_raw($_[0]);
   }
   else {
       return 0;
   }
}

#************************************************************

sub get_size {
   # Return time of file named in argument
   # If file does not exist, return 0;
   if ( -e $_[0] ) {
       return get_size_raw($_[0]);
   }
   else {
       return 0;
   }
}

#************************************************************

sub get_size_raw
{ 
  my $size = (stat($_[0]))[7];
  return $size;
}

#************************************************************

sub get_time_size {
   # Return time and size of file named in argument
   # If file does not exist, return (0,-1);
   if ( -e $_[0] ) {
       return get_time_size_raw($_[0]);
   }
   else {
       return (0,-1);
   }
}

#************************************************************

sub get_time_size_raw
{ 
  my $mtime = (stat($_[0]))[9];
  my $size = (stat($_[0]))[7];
  return ($mtime, $size);
}

#************************************************************

sub processing_time
{  my ($user, $system, $cuser, $csystem) = times();
   return $user + $system + $cuser + $csystem;
}

#************************************************************

sub get_checksum_md5 {
    my $source = shift;
    my $input = new FileHandle;
    my $md5 = Digest::MD5->new;
    my $ignore_pattern = undef;

#warn "======= GETTING MD5: $source\n";
    if ( -d $source ) {
        # We won't use checksum for directory
        return 0;
    }
    else {
        open( $input, '<:bytes', $source )
        or return 0;
        my ($base, $path, $ext) = fileparseA( $source );
        $ext =~ s/^\.//;
        if ( exists $hash_calc_ignore_pattern{$ext} ) {
            $ignore_pattern = $hash_calc_ignore_pattern{$ext};
        }
    }
    if ( defined $ignore_pattern ) {
        while (<$input>) {
            if ( ! /$ignore_pattern/ ){
                $md5->add($_);
            }
        }
    }
    else {
        $md5->addfile($input);
    }
    close $input;
    return $md5->hexdigest();
}

#************************************************************
#************************************************************

sub create_empty_file {
    my $name = shift;
    my $h = new FileHandle ">$name"
        or return 1;
    close ($h);
    return 0;
}

#************************************************************
#************************************************************

sub find_file1 {
    # Usage: find_file1(name, ref_to_array_search_path)
    # Modified find_file, which doesn't die.
    # Given filename and path, return array of:
    #             full name 
    #             retcode
    # On success: full_name = full name with path, retcode = 0
    # On failure: full_name = given name, retcode = 1

    my $name = $_[0];
    # Make local copy of path, since we may rewrite it!
    my @path = ();
    if ($_[1]) {
        @path = @{$_[1]};
    }
    if ( $name =~ /^\// ) {
        # Absolute path (if under UNIX)
        # This needs fixing, in general
        if (-e $name) { return( $name, 0 );}
        else { return( $name, 1 );}
    }
    foreach my $dir ( @path ) {
        # Make $dir concatenatable, and empty for current dir:
        if ( $dir eq '.' ) { 
            $dir = ''; 
        }
        elsif ( $dir =~ /[\/\\:]$/ ) { 
            #OK if dir ends in / or \ or :
        }
        elsif ( $dir ne '' ) { 
            #Append directory separator only to non-empty dir
            $dir = "$dir/"; 
        }
        if (-e "$dir$name") {
            return("$dir$name", 0);
        }
    }
    my @kpse_result = kpsewhich( $name );
    if ($#kpse_result > -1) {
        return( $kpse_result[0], 0);
    }
    return("$name" , 1);
} #END find_file1

#************************************************************

sub find_file_list1 {
    # Modified version of find_file_list that doesn't die.
    # Given output and input arrays of filenames, a file suffix, and a path, 
    # fill the output array with full filenames
    # Return array of not-found files.
    # Usage: find_file_list1( ref_to_output_file_array,
    #                         ref_to_input_file_array,
    #                         suffix,
    #                         ref_to_array_search_path
    #                       )
    # SPECIAL TREATMENT TO .bib extension, because of behavior of bibtex
    # OTHER SPECIAL TREATMENT IF EXTENSION IS GIVEN.

  my $ref_output = $_[0];
  my $ref_input  = $_[1];
  my $suffix     = $_[2];
  my $ref_search = $_[3];
  my @not_found = ();

  my @return_list = ();    # Generate list in local array, since input 
                           # and output arrays may be same
  my $retcode = 0;
  foreach my $file1 (@$ref_input) {
    my $file = $file1;
    if ($suffix eq '.bib') { $file =~ s/\.bib$//; }
    my ($tmp_file, $find_retcode) = &find_file1( "$file$suffix", $ref_search );
    if ($tmp_file)  {
        push @return_list, $tmp_file;
    }
    if ( $find_retcode != 0 ) {
        push @not_found, $file.$suffix;
    }
  }
  @$ref_output = @return_list;
  return @not_found;
} #END find_file_list1

#************************************************************

sub unlink_or_move {
    if ( $del_dir eq '' ) {
        foreach (@_) {
            if (!-e) {next;}
            if (-d) {
                if (!rmdir) {
                    warn "$My_name: Cannot remove directory '$_'\n";
                }
            }
            else { 
                if (!unlink) {
                    warn "$My_name: Cannot remove file '$_'\n";
                }
            }
        }
    }
    else {
        foreach (@_) {
            if (-e $_ && ! move $_, "$del_dir/$_" ) {
                warn "$My_name: Cannot move '$_' to '$del_dir/$_'\n";
            }
        }
    }
}

#************************************************************

sub make_path_mod {
    my $dir = $_[0];
    my $title = $_[1];
    my $ret = 0;
    if ( -d $dir ) {}
    elsif ( (! -e $dir) && (! -l $dir) ) {
        # N.B. A link pointing to a non-existing target
        # returns false for -e, so we must also check -l
        warn "$My_name: making $title directory '$dir'\n"
            if ! $silent;
        # Error handling from File::Path documentation:
        make_path( $dir, {error => \my $err} );
        if ($err && @$err) {
             for my $diag (@$err) {
                 my ($file, $message) = %$diag;
                 if ($file eq '') {
                     print "general error in making dir: $message\n";
                 }
                 else {
                      print "problem making path $file: $message\n";
                }
             }
             $ret = 1;
        }
    }
    else {
        $ret = 2;
        warn "$My_name: you requested $title directory '$dir',\n",
            "    but a non-directory file/symlink of the same name exists.\n";
    }
    return $ret;
}

#************************************************************

sub kpsewhich {
# Usage: kpsewhich( filespec, ...)
# Returns array of files with paths as found by kpsewhich
#    kpsewhich( 'try.sty', 'jcc.bib' );
# With standard use of kpsewhich (i.e., without -all option), the array
# has either 0 or 1 element.
# Can also do, e.g.,
#    kpsewhich( '-format=bib', 'trial.bib', 'file with spaces');
    my $cmd = $kpsewhich;
    my @args = @_;
    if ( ($cmd eq '') || ( $cmd =~ /^NONE($| )/ ) ) {
        # Kpsewhich not set up.
        warn "$My_name: Kpsewhich command needed but not set up\n";
        return ();
    }
    foreach (@args) {
        if ( ! /^-/ ) {
            $_ = "\"$_\"";
        }
    }
    $cmd =~ s/%[RBTDO]//g;
    $cmd =~ s/%S/@args/g;
    my @found = ();
    local $fh;
    if ( $kpsewhich_show || $diagnostics ) {
        print "$My_name.kpsewhich: Running '$cmd'...\n";
    }
    open $fh, "$cmd|"
        or die "Cannot open pipe for \"$cmd\"\n";
    while ( <$fh> ) {
        s/[\r\n]*$//;
        push @found, $_;
    }
    close $fh;
    if ( $kpsewhich_show || $diagnostics ) {
        show_array( "$My_name.kpsewhich: '$cmd' ==>", @found );
    }
    return @found;
}

####################################################

sub add_cus_dep {
    # Usage: add_cus_dep( from_ext, to_ext, flag, sub_name )
    # Add cus_dep after removing old versions
    my ($from_ext, $to_ext, $must, $sub_name) = @_;
    remove_cus_dep( $from_ext, $to_ext );
    push @cus_dep_list, "$from_ext $to_ext $must $sub_name";
}

####################################################

sub remove_cus_dep {
    # Usage: remove_cus_dep( from_ext, to_ext )
    my ($from_ext, $to_ext) = @_;
    my $i = 0;
    while ($i <= $#cus_dep_list) {
        # Use \Q and \E round directory name in regex to avoid interpretation
        #   of metacharacters in directory name:
        if ( $cus_dep_list[$i] =~ /^\Q$from_ext $to_ext \E/ ) {
            splice @cus_dep_list, $i, 1;
        }
        else {
            $i++;
        }
    }
}

####################################################

sub show_cus_dep {
    show_array( "Custom dependency list:", @cus_dep_list );
}

####################################################

sub find_cus_dep {
    # Usage find_cus_dep( dest, source )
    # Given dest, if a cus_dep to make it is found, set source.
    # Return 1 or 0 on success or failure.
    #
    my $dest = $_[0];
    my ($base, $path, $ext) = fileparseB( $dest );
    $ext =~ s/^\.//;
    if (! $ext ) { return 0; }
    foreach my $dep ( @cus_dep_list ) {
        my ($fromext, $toext) = split( '\s+', $dep );
        if ( ( "$ext" eq "$toext" ) && ( -f "$path$base.$fromext" ) ) {
            # We have a way of making $dest
            $_[1] = "$path$base.$fromext";
            return 1
        }
    }
    return 0;
}

####################################################
####################################################

sub add_aux_hook {
    # Usage: add_aux_hook( sub_name )
    # Add the name subroutine to the array of hooks for
    # processing lines of aux files.
    # The argument is either a string naming the subroutine, e.g.
    #     add_aux_hook( 'subname' );
    # or a Perl reference to the subroutine, e.g.,
    #     add_aux_hook( \&subname );
    # It is also possible to use an anonymous subroutine, e.g.,
    #     add_aux_hook( sub{  code of subroutine... } );
    my ($sub_name) = @_;
    push @aux_hooks, $sub_name;
}

####################################################

sub add_latex_file_hook {
    # Usage: add_latex_file_hook( sub_name )
    # Add the name subroutine to the array of hooks for
    # processing list of possible dependency files after a run of *latex.
    # The argument is either a string naming the subroutine, e.g.
    #     add_latex_file_hook( 'subname' );
    # or a Perl reference to the subroutine, e.g.,
    #     add_latex_file_hook( \&subname );
    # It is also possible to use an anonymous subroutine, e.g.,
    #     add_latex_file_hook( sub{  code of subroutine... } );
    my ($sub_name) = @_;
    push @latex_file_hooks, $sub_name;
}

####################################################

sub set_input_ext {
    # Usage: set_input_ext( rule, ext, ... )
    # Set list of extension(s) (specified without a leading period) 
    # for the given rule ('latex', 'pdflatex', etc).  
    # These extensions are used when an input
    # file without an extension is found by *latex, as in
    # \input{file} or \includegraphics{figure}.  When latexmk searches
    # custom dependencies to make the missing file, it will assume that
    # the file has one of the specified extensions.
    my $rule = shift;
    $input_extensions{$rule} = {};
    my $Prule = $input_extensions{$rule};
    foreach (@_) { $$Prule{$_} = 1; }
}

####################################################

sub show_input_ext {
    # Usage: show_input_ext( rule )
    my $rule = shift;
    show_array ("Input extensions for rule '$rule': ", 
                keys %{$input_extensions{$rule}} );
}

####################################################

sub find_dirs1 {
   # Same as find_dirs, but argument is single string with directories
   # separated by $search_path_separator
   find_dirs( &split_search_path( $search_path_separator, ".", $_[0] ) );
}


#************************************************************

sub find_dirs {
# @_ is list of directories
# return: same list of directories, except that for each directory 
#         name ending in //, a list of all subdirectories (recursive)
#         is added to the list.
#   Non-existent directories and non-directories are removed from the list
#   Trailing "/"s and "\"s are removed
    local @result = ();
    my $find_action 
        = sub 
          { ## Subroutine for use in File::find
            ## Check to see if we have a directory
               if (-d) { push @result, $File::Find::name; }
          };
    foreach my $directory (@_) {
        my $recurse = ( $directory =~ m[//$] );
        # Remove all trailing /s, since directory name with trailing /
        #   is not always allowed:
        $directory =~ s[/+$][];
        # Similarly for MSWin reverse slash
        $directory =~ s[\\+$][];
        if ( ! -e $directory ){
            next;
        }
        elsif ( $recurse ){
            # Recursively search directory
            find( $find_action, $directory );
        }
        else {
            push @result, $directory;
        }
    }
    return @result;
}

#************************************************************

sub uniq 
# Read arguments, delete neighboring items that are identical,
# return array of results
{
    my @sort = ();
    my ($current, $prev);
    my $first = 1;
    while (@_)
    {
        $current = shift;
        if ($first || ($current ne $prev) )
        {
            push @sort, $current; 
            $prev = $current;
            $first = 0;
        }
    }
    return @sort;
}

#==================================================

sub uniq1 {
   # Usage: uniq1( strings )
   # Returns array of strings with duplicates later in list than
   # first occurence deleted.  Otherwise preserves order.

    my @strings = ();
    my %string_hash = ();

    foreach my $string (@_) {
        if (!exists( $string_hash{$string} )) { 
            $string_hash{$string} = 1;
            push @strings, $string; 
        }
    }
    return @strings;
}

#************************************************************

sub uniqs {
    # Usage: uniq2( strings )
    # Returns array of strings sorted and with duplicates deleted
    return uniq( sort @_ );
}

#************************************************************

sub ext {
    # Return extension of filename.  Extension includes the period
    my $file_name = $_[0];
    my ($base_name, $path, $ext) = fileparseA( $file_name );
    return $ext;
 }

#************************************************************

sub ext_no_period {
    # Return extension of filename.  Extension excludes the period
    my $file_name = $_[0];
    my ($base_name, $path, $ext) = fileparseA( $file_name );
    $ext =~ s/^\.//;
    return $ext;
 }

#************************************************************

sub fileparseA {
    # Like fileparse but replace $path for current dir ('./' or '.\') by ''
    # Also default second argument to get normal extension.
    my $given = $_[0];
    my $pattern = '\.[^\.]*';
    if  ($#_ > 0 ) { $pattern = $_[1]; }
    my ($base_name, $path, $ext) = fileparse( $given, $pattern );
    if ( ($path eq './') || ($path eq '.\\') ) { 
        $path = ''; 
    }
    return ($base_name, $path, $ext);
}

#************************************************************

sub fileparseB {
    # Like fileparse but with default second argument for normal extension
    my $given = $_[0];
    my $pattern = '\.[^\.]*';
    if  ($#_ > 0 ) { $pattern = $_[1]; }
    my ($base_name, $path, $ext) = fileparse( $given, $pattern );
    return ($base_name, $path, $ext);
}

#************************************************************

sub split_search_path 
{
# Usage: &split_search_path( separator, default, string )
# Splits string by separator and returns array of the elements
# Allow empty last component.
# Replace empty terms by the default.
    my $separator = $_[0]; 
    my $default = $_[1]; 
    my $search_path = $_[2]; 
    my @list = split( /$separator/, $search_path);
    if ( $search_path =~ /$separator$/ ) {
        # If search path ends in a blank item, the split subroutine
        #    won't have picked it up.
        # So add it to the list by hand:
        push @list, "";
    }
    # Replace each blank argument (default) by current directory:
    for ($i = 0; $i <= $#list ; $i++ ) {
        if ($list[$i] eq "") {$list[$i] = $default;}
    }
    return @list;
}

#################################

sub get_filetime_offset {
    # Usage: get_filetime_offset( prefix, [suffix] )
    # Measures offset between filetime in a directory and system time
    # Makes a temporary file of a unique name, and deletes in.
    # Filename is of form concatenation of prefix, an integer, suffix.
    # Prefix is normally of form dir/ or dir/tmp.
    # Default default suffix ".tmp".
    my $prefix = $_[0];
    my $suffix = $_[1] || '.tmp';
    my $tmp_file_count = 0;
    while (1==1) {
        # Find a new temporary file, and make it.
        $tmp_file_count++;
        my $tmp_file = "${prefix}${tmp_file_count}${suffix}";
        if ( ! -e $tmp_file ) {
            open( TMP, ">$tmp_file" ) 
                or die "$My_name.get_filetime_offset: In measuring filetime offset, couldn't write to\n",
                       "    temporary file '$tmp_file'\n";
            my $time = time();
            close(TMP);
            my $offset = get_mtime($tmp_file) - $time;
            unlink $tmp_file;
            return $offset;
         }
     }
     die "$My_name.get_filetime_offset: BUG TO ARRIVE HERE\n";
}

#################################

sub tempfile1 {
    # Makes a temporary file of a unique name.  I could use file::temp,
    # but it is not present in all versions of perl.
    # Filename is of form $tmpdir/$_[0]nnn$suffix, where nnn is an integer
    my $tmp_file_count = 0;
    my $prefix = $_[0];
    my $suffix = $_[1];
    while (1==1) {
        # Find a new temporary file, and make it.
        $tmp_file_count++;
        my $tmp_file = "${tmpdir}/${prefix}${tmp_file_count}${suffix}";
        if ( ! -e $tmp_file ) {
            open( TMP, ">$tmp_file" ) 
               or next;
            close(TMP);
            return $tmp_file;
         }
     }
     die "$My_name.tempfile1: BUG TO ARRIVE HERE\n";
}

#################################

#************************************************************
#************************************************************
#      Process/subprocess routines

sub Run_msg {
    # Same as Run, but give message about my running
    warn_running( "Running '$_[0]'" );
    return Run($_[0]);
} #END Run_msg

#==================

sub Run_time {
    # This is wrapper around Run to capture timing information
    my $time1 = processing_time();
    my ($pid, $return) = Run($_[0]);
    my $time = processing_time() - $time1;
    push @timings, "'$_[0]': time = $time\n"; 
    return ($pid, $return);
} #END Run_time

#==================

sub Run {
# Usage: Run_no_time ("command string");
#    or  Run_no_time ("one-or-more keywords command string");
# Possible keywords: internal, NONE, start, nostart.
#
# A command string not started by keywords just gives a call to system with
#   the specified string, I return after that has finished executing.
# Exceptions to this behavior are triggered by keywords.
# The general form of the string is
#    Zero or more occurences of the start keyword,
#    followed by at most one of the other key words (internal, nostart, NONE),
#    followed by (a) a command string to be executed by the systerm
#             or (b) if the command string is specified to be internal, then
#                    it is of the form
#
#                       routine arguments
#
#                    which implies invocation of the named Perl subroutine
#                    with the given arguments, which are obtained by splitting
#                    the string into words, delimited by spaces, but with
#                    allowance for double quotes.
#
# The meaning of the keywords is:
#
#    start: The command line is to be running detached, as appropriate for
#             a previewer.  The method is appropriate for the operating system
#             (and the keyword is inspired by the action of the start command
#             that implements in under MSWin).
#           HOWEVER: the start keyword is countermanded by the nostart,
#             internal, and NONE keywords.  This allows rules that do
#             previewing to insert a start keyword to create a presumption
#             of detached running unless otherwise.
#   nostart: Countermands a previous start keyword; the following command
#             string is then to be obeyed by the system, and any necessary
#             detaching (as of a previewer) is done by the executed command(s).
#   internal: The following command string, of the form 'routine arguments'
#             specifies a call to the named Perl subroutine.
#   NONE:   This does not run anything, but causes an error message to be
#             printed.  This is provided to allow program names defined in the
#             configuration to flag themselves as unimplemented.
# Note that if the word "start" is duplicated at the beginning, that is
#   equivalent to a single "start".
#
# Return value is a list (pid, exitcode):
#   If a process is spawned sucessfully, and I know the PID,
#       return (pid, 0),
#   else if process is spawned sucessfully, but I do not know the PID,
#       return (0, 0),
#   else if process is run, 
#       return (0, exitcode of process)
#   else if I fail to run the requested process
#       return (0, suitable return code)
#   where return code is 1 if cmdline is null or begins with "NONE" (for
#       an unimplemented command)
#       or the return value of the Perl subroutine.
    my $cmd_line = $_[0];
    if ( $cmd_line eq '' ) {
        traceback( "$My_name: Bug OR configuration error\n".
                   "   In run of '$rule', attempt to run a null program" );
        return (0, 1);
    }
    # Deal with latexmk-defined pseudocommands 'start' and 'NONE' 
    # at front of command line:
    my $detach = 0;
    while ( $cmd_line =~ s/^start +// ) {
        # But first remove extra starts (which may have been inserted
        # to force a command to be run detached, when the command
        # already contained a "start").
        $detach = 1;
    }
    if ( $cmd_line =~ s/^nostart +// ) {
        $detach = 0;
    }
    if ( $cmd_line =~ /^internal\s+([a-zA-Z_]\w*)\s+(.*)$/ ) {
        my $routine = $1;
        my @args = parse_quotes( $2 );
        warn "$My_name: calling $routine( $2 )\n"
            if (! $silent);
        return ( 0, &$routine( @args ) );
    }
    elsif ( $cmd_line =~ /^internal\s+([a-zA-Z_]\w*)\s*$/ ) {
        my $routine = $1;
        warn "$My_name: calling $routine()\n"
            if (! $silent);
        return ( 0, &$routine() );
    }
    elsif ( $cmd_line =~ /^NONE/ ) {
        warn "$My_name: ",
             "Program not implemented for this version.  Command line:\n";
        warn "   '$cmd_line'\n";
        return (0, 1);
    }
    elsif ($detach) {
        # Run detached.  How to do this depends on the OS
        return &Run_Detached( $cmd_line );
    }
    else { 
       # The command is given to system as a single argument, to force shell
       # metacharacters to be interpreted:
       return( 0, system( $cmd_line ) );
   }
}  #END Run

#************************************************************

sub Run_Detached {
# Usage: Run_Detached ("program arguments ");
# Runs program detached.  Returns 0 on success, 1 on failure.
# Under UNIX use a trick to avoid the program being killed when the 
#    parent process, i.e., me, gets a ctrl/C, which is undesirable for pvc 
#    mode.  (The simplest method, system("program arguments &"), makes the 
#    child process respond to the ctrl/C.)
# Return value is a list (pid, exitcode):
#   If process is spawned sucessfully, and I know the PID,
#       return (pid, 0),
#   else if process is spawned sucessfully, but I do not know the PID,
#       return (0, 0),
#   else if I fail to spawn a process
#       return (0, 1)

    my $cmd_line = $_[0];

##    warn "Running '$cmd_line' detached...\n";
    if ( $cmd_line =~ /^NONE / ) {
        warn "$My_name: ",
             "Program not implemented for this version.  Command line:\n";
        warn "   '$cmd_line'\n";
        return (0, 1);
    }

    if ( "$^O" eq "MSWin32" ){
        # Win95, WinNT, etc: Use MS's start command:
        # Need extra double quotes to deal with quoted filenames: 
        #    MSWin start takes first quoted argument to be a Window title. 
        return( 0, system( "start \"\" $cmd_line" ) );
    } else {
        # Assume anything else is UNIX or clone
        # For this purpose cygwin behaves like UNIX.
        ## warn "Run_Detached.UNIX: A\n";
        my $pid = fork();
        ## warn "Run_Detached.UNIX: B pid=$pid\n";
        if ( ! defined $pid ) {
            ## warn "Run_Detached.UNIX: C\n";
            warn "$My_name: Could not fork to run the following command:\n";
            warn "   '$cmd_line'\n";
            return (0, 1);
        }
        elsif( $pid == 0 ){
           ## warn "Run_Detached.UNIX: D\n";
           # Forked child process arrives here
           # Insulate child process from interruption by ctrl/C to kill parent:
           #     setpgrp(0,0);
           # Perhaps this works if setpgrp doesn't exist 
           #    (and therefore gives fatal error):
           eval{ setpgrp(0,0);};
           exec( $cmd_line );
           # Exec never returns; it replaces current process by new process
           die "$My_name forked process: could not run the command\n",
               "  '$cmd_line'\n";
        }
        ##warn "Run_Detached.UNIX: E\n";
        # Original process arrives here
        return ($pid, 0);
    }
    # NEVER GET HERE.
    ##warn "Run_Detached.UNIX: F\n";
} #END Run_Detached

#************************************************************

sub find_process_id {
# find_process_id(string) finds id of process containing string and
# being run by the present user.  In all the uses in latexmk, the string is
# the name of a file that is expected to be on the command line.
#
# On success, this subroutine returns the process ID.
# On failure, it returns 0.
#
# This subroutine only works on UNIX systems at the moment.

    if ( $pid_position < 0 ) {
        # I cannot do a ps on this system
        return (0);
    }

    my $looking_for = $_[0];
    my @ps_output = `$pscmd`;
    my @ps_lines = ();

# There may be multiple processes.  Find only latest, 
#   almost surely the one with the highest process number
# This will deal with cases like xdvi where a script is used to 
#   run the viewer and both the script and the actual viewer binary
#   have running processes.
    my @found = ();

    shift(@ps_output);  # Discard the header line from ps
    foreach (@ps_output)   {
        next unless ( /$looking_for/ ) ;
        s/^\s*//;
        my @ps_line = split ('\s+');
        push @found, $ps_line[$pid_position];
        push @ps_lines, $_;
    }

    if ($#found < 0) {
       # No luck in finding the specified process.
       return(0);
    }
    @found = reverse sort @found;
    if ($diagnostics) {
       print "Found the following processes concerning '$looking_for'\n",
             "   @found\n",
             "   I will use $found[0]\n";
       print "   The relevant lines from '$pscmd' were:\n";
       foreach (@ps_lines) { print "   $_"; }
    }
    return $found[0];
}

#************************************************************
#************************************************************
#************************************************************

#============================================

sub cache_good_cwd {
    # Set cached value of cwd to current cwd.
    # Under cygwin, the cached value is converted to a native MSWin path so
    # that the result can be used for input to MSWin programs as well
    # as cygwin programs.
    # Similarly for msys.
    my $cwd = getcwd();
    if ( $^O eq "cygwin" ) {
        my $cmd = "cygpath -w \"$cwd\"";
        my $Win_cwd = `$cmd`;
        chomp $Win_cwd;
        if ( $Win_cwd ) {
            $cwd = $Win_cwd;
        }
        else {
            warn "$My_name: Could not correctly run command\n",
                 "      '$cmd'\n",
                 "  to get MSWin version of cygwin path\n",
                 "     '$cwd'\n",
                 "  The result was\n",
                 "     '$Win_cwd'\n";
        }
    }
    elsif ( $^O eq "msys" ) {
        $cwd =~ s[^/([a-z])/][\u$1:/];
    }
    # Normalized
    if ($normalize_names) {
        $cwd = abs_path($cwd);
    }
    $cache{cwd} = $cwd;
}  # END cache_good_cwd

#============================================

sub good_cwd {
    # Return cwd, but under cygwin (or ...), convert to MSWin path.
    # Use cached result, to save a possible expensive computation (running 
    #  of extenal program under cygwin).
    return $cache{cwd};
}  # END good_cwd

#============================================

#   Directory stack routines

sub pushd {
    push @dir_stack, [cwd(), $cache{cwd}];
    if ( $#_ > -1) {
        local $ret = 0;
        eval {
            if ( -d $_[0] ) {
                $ret = chdir dirname_no_tail( $_[0] );
            }
            else {
                print "$my_name: Can't change directory to '$_[0]'\n",
                      "   A directory of the same name does not exist.\n";
            }
        };
        if ( ($ret == 0) || $@ ) {            
            if ($@) {
                print "Error:\n  $@" ;
            }
            die "$My_name: Error in changing directory to '$_[0]'.  I must stop\n";
        }
        &cache_good_cwd;
    }
}

#************************************************************

sub popd {
    if ($#dir_stack > -1 ) { 
        my $Parr = pop @dir_stack;
        chdir $$Parr[0];
        $cache{cwd} = $$Parr[1];
    }
}

#************************************************************

sub ifcd_popd {
    if ( $do_cd ) {
        warn "$My_name: Undoing directory change\n"
          if !$silent;
        &popd;
    }
}

#************************************************************

sub finish_dir_stack {
    while ($#dir_stack > -1 ) { &popd; }
}

#************************************************************
#************************************************************
# Break handling routines (for wait-loop in preview continuous)

sub end_wait {
    #  Handler for break: Set global variable $have_break to 1.
    # Some systems (e.g., MSWin reset) appear to reset the handler.
    # So I'll re-enable it
    &catch_break;
    $have_break = 1;
}

#========================

sub catch_break {
# Capture ctrl/C and ctrl/break.
# $SIG{INT} corresponds to ctrl/C on LINUX/?UNIX and MSWin
# $SIG{BREAK} corresponds to ctrl/break on MSWin, doesn't exist on LINUX
    $SIG{INT} = \&end_wait;
    if ( exists $SIG{BREAK} ) {
        $SIG{BREAK} = \&end_wait;
    }
}

#========================

sub default_break {
# Arrange for ctrl/C and ctrl/break to give default behavior
    $SIG{INT} = 'DEFAULT';
    if ( exists $SIG{BREAK} ) {
        $SIG{BREAK} = 'DEFAULT';
    }
}

#************************************************************
#************************************************************


==> related.tex <==
\section{Related Work} \label{related_work}

{\bf Regret Bounds for Multi-Armed Bandit:} Prior works for K = 1 extensively study the problem and involves a lower limit on regret  \citep{lai1985asymptotically}, and efficient algorithms like UCB  \citep{auer2002finite,auer2010ucb}, and MOSS  \citep{audibert2009minimax}. The authors of \citep{thompson1933likelihood} gave the first algorithm for Multi Armed Bandits using a Bayesian approach, which was proven to be efficient in \citep{agrawal2012analysis}. %The authors of \citep{Even-Dar:2006:AES:1248547.1248586} analyzed the problem in terms of the number of samples. 
Recent research in this area involves reducing space complexity at the cost of regret bounds \citep{pmlr-v84-liau18a}. Our work aims to reduce space complexity, since approaches cannot be directly applied  as they loop over the entire $\binom{N}{K}$ action space. % which is not the case in this paper. %they still loop over the entire action space.

Based on the type of environment, and how it generates rewards, the multi-armed bandit problem is divided into two classes, namely stochastic and adversarial \citep{audibert2009minimax}. In stochastic bandits, the rewards follow a stochastic process, whose distribution may not change on taking a particular action. However in adversarial bandits, the environment acts as an adversary, and can try to beat the agent by changing the distribution of the rewards by learning the strategy of the agent. Agent, in such a case, randomizes its actions to beat the adversary \citep{doi:10.1137/S0097539701398375}. %Under such strategy, the probability to select the action which generating the highest expected reward is highest.

{\bf Adversarial Combinatorial Bandits:} Adversarial Combinatorial Bandits have been studied where the agent chooses $K$ of the $N$ arms in each round  \citep{DBLP:conf/colt/DaniHK08,NIPS2007_3371,Cesa-Bianchi:2012:CB:2240304.2240495,Audibert:2014:ROC:2765232.2765234}. In these works, it is assumed that the reward function in each round is linear in the different arms. Due to this linear function, the problem is also called  online linear optimization. The algorithm proposed in this works uses the linearity of the reward function to estimate the rewards of individual arms, and achieve a regret of $O{\sqrt{T}}$. The weights are assigned to each of the $\binom{N}{K}$ actions to decide the action in the next round, and thus the approach is not computationally efficient for large $N$. 

%Scenarios where an adversary chooses the reward of individual actions, the gain is a linear combination of the arms played in a round are well studied by \citep{DBLP:conf/colt/DaniHK08}, \citep{NIPS2007_3371}, \citep{Cesa-Bianchi:2012:CB:2240304.2240495}, and \citep{Audibert:2014:ROC:2765232.2765234}. The linear combination of the rewards earned the problem its name of Online linear optimization. The algorithm achieves regret of $O{\sqrt{T}}$ uses of the linear nature of reward combining and tries to estimate the rewards of individual arms to update the weights. However, the algorithm needs to assign weights to all actions and is not computationally efficient for large number of base arms.

{\bf Stochastic Combinatorial Bandits:} For stochastic multi-armed bandits, the authors of \citep{gai2010learning} provided an UCB style algorithm when the rewards of each of the $K$ arms is also observed in each round, with the aggregate reward as the sum of individual rewards. Such setup, where the rewards of each of the $K$ arms is also available to agent, is referred to as a semi-bandit problem. The authors of \citep{kveton2015tight} showed that the UCB algorithm  provides a tight regret bound for semi-bandit combinatorial bandit problem with linear reward function. The authors of \citep{pmlr-v28-chen13a} considered combinatorial semi-bandit problem with non-linear rewards  using a UCB style analysis. The authors of \citep{pmlr-v32-lind14} assumed combinatorial bandit problem with non-linear reward function and feedback, where the feedback  is a linear combination of rewards of the $K$ arms. Such feedback of linear function of rewards allows recovery of individual rewards. In contrast, this paper does not consider the availability of individual arm rewards or a linear feedback. With non-linear feedback, it might not be possible to obtain the exact values of the rewards of base arms. 

%analyze the non linear rewards setting however they considered the partial feedback to be available which is a linear combination of rewards of base arms which made it possible to recover the individual rewards of base arms.

%For combinatorial stochastic multi-armed bandits prior works involve works of \citep{gai2010learning} who provided an UCB style algorithm to solve the problem. However in their framework, rewards of all the K arms chosen were observed simultaneously. This setting is referred as semi-bandit problem. \citep{kveton2015tight} provided the analysis that the UCB algorithm indeed provides a tight regret bound. \citep{pmlr-v28-chen13a} did regret analysis for non linear rewards using a UCB style analysis however their problem under consideration was semi-bandit. \citep{pmlr-v32-lind14} analyze the non linear rewards setting however they considered the partial feedback to be available which is a linear combination of rewards of base arms which made it possible to recover the individual rewards of base arms.

%As compared to the works mentioned above, our algorithm solves the problem of non linear rewards with non linear feedback of arms. Under the setting of non linear feedback, it might not be possible to obtain the exact values of the rewards of base arms. The algorithm proposed works on a linear space in number of base arms, and provide regret bounds which is sublinear in time, number of base arms, and number of arms simultaneously chosen.

==> result.tex <==
\section{Regret Analysis of the proposed algorithm} \label{main_results}
In this section, we will present the main result of the paper, related to the regret analysis of the proposed algorithm. Our main result is presented in Theorem \ref{final_theorem_for_regret_bound}, which states that \NAM\ algorithm achieves a sub linear expected regret. %, while simultaneously reducing space and time complexity to polynomial order in problem size.

\begin{theorem} \label{final_theorem_for_regret_bound}
\NAM\ algorithm described in Algorithm \ref{alg:dama} has an expected regret accumulated during the entire time horizon upper bounded as
	\begin{equation}
	W(T) = \tilde{O}\left(N^\frac{1}{3}K^\frac{1}{2}T^\frac{2}{3}\right)
	\end{equation}
\end{theorem}

In order to prove the result, we will first prove a few lemmas to show the correctness of the algorithm, to bound the number of rounds, and to bound the maximum error. This will be followed by the proof of \cref{final_theorem_for_regret_bound}. 
%Then we will go over proof of main result.

\input{algos_merge.tex}

\input{keylemmas}

\input{sortmergetime}
\input{explore_time}

\subsection{Proof of Theorem \ref{final_theorem_for_regret_bound}}
In this subsection, we will prove Theorem \ref {final_theorem_for_regret_bound}. We note that the expected regret till time $T$ is sum of expected regret accumulated at each round. We can rewrite it as sum of two phases of the algorithm which are exploration and exploitation as,
    \begin{eqnarray}
        W(T)&=& \sum^{T}_{t = 1}\mathbb{E}\left[R(t)\right]\\
        &=& \sum^{T_{exp}}_{t = 1}\mathbb{E}\left[R(t)\right] + \left(T-T_{exp}\right)\times\mathbb{E}\left[\Delta_{\hat{{\bf a}}^*}\right] \label{eq:max_regret_explore_exploit}\\
        &\le & \sum^{T_{exp}}_{t = 1}\mathbb{E}\left[R(t)\right] + T\mathbb{E}\left[\Delta_{\hat{{\bf a}}^*}\right] \label{eq:max_regret_exploit_time}\\
        &\leq& \sum^{T_{exp}}_{t = 1}\max\left(R(t)\right) + T\mathbb{E}\left[\Delta_{\hat{{\bf a}}^*}\right] \label{eq:max_regret_max_explore}\\
        &\leq& T_{exp}\max\left(R(t)\right) + T\mathbb{E}\left[\Delta_{\hat{{\bf a}}^*}\right], \label{eq:max_explore_regret} 
    \end{eqnarray}
    where  (\ref{eq:max_regret_explore_exploit}) follows from splitting the regret into exploration-exploitation phase,  (\ref{eq:max_regret_exploit_time}) follows since $T-T_{exp}\le T$, and  (\ref{eq:max_regret_max_explore}) follows since mean is at most the maximum. 
    
 %   by making regret in each round to be the maximum regret possible and (\ref{eq:max_explore_regret}) follows if time for exploration uses the maximum time for which the \cref{alg:dama} can explore.
    Using the values for maximum regret in any round, Lemma \ref{exploitation_regret_bound}, inequality (\ref{eq:pbound}), maximum exploration time from Lemma \ref{exploration_time_bound}, and maximum exploitation regret from Lemma \ref{exploitation_regret_bound}, we have,
    \begin{eqnarray}
        W(T)&\leq& U\sqrt{K}\frac{128NU^2\log{2NT}}{\lambda^2} + T\left(U\lambda\sqrt{K} + \frac{U\sqrt{K}}{NT^2}\right)\\
        &=& \left(\frac{128NU^3\sqrt{K}\log{2NT}}{\lambda^2} + TU\lambda\sqrt{K}\right) + \frac{U\sqrt{K}}{NT}.
    \end{eqnarray}
    Choosing the value of $\lambda$ as defined in  (\ref{eq:define_lambda}), we have the total regret of the algorithm as
    \begin{eqnarray}
        W(T)&\leq& 
        3U\sqrt{K}\left(256NU^2\log{2NT}\right)^{\frac{1}{3}}T^{\frac{2}{3}} + \frac{U\sqrt{K}}{NT}
    \end{eqnarray}
This proves the result as in the statement of the Theorem. 

\subsection{Discussion}\label{disc}

We now compare the regret bound with the one that would be achieved by using the UCB approach on each of the $\binom{N}{K}$ actions. 

\begin{lemma}[UCB Regret, \cite{auer2010ucb}] 
    For a Multi Armed Bandit setting with action space $\mathcal{A}$, time horizon T, and precision $\lambda \approx \sqrt{\frac{|\mathcal{A}|\log{|\mathcal{A}|}}{T}}$, expected regret accumulated during entire time horizon T using improved UCB algorithm is upper bounded by 
    \begin{equation}
        \sqrt{|\mathcal{A}|T}\frac{\log{\left(|\mathcal{A}|\log{|\mathcal{A}|}\right)}}{\sqrt{\log{|\mathcal{A}|}}}
    \end{equation}
\end{lemma}

Bounding the size of action space by using Stirling's approximation \citep{slomson1997introduction}, we get expected regret accumulated regret at time $T$ of UCB algorithm as,
\begin{eqnarray}
W_{UCB}(T) = \tilde{O}\left(\left(\frac{eN}{K}\right)^{\frac{K}{2}}T^{\frac{1}{2}}\right)
\end{eqnarray}

%In order outperform \NAM, time horizon $T$ for which both algorithm runs is of exponential order in $K$. Mathematically,
For UCB approach to outperform \NAM, $T$ has to be very large. More formally, 
\begin{eqnarray}
W(T) > W_{UCB}(T),
\text{ when }T = \Tilde{\Omega}\left(\frac{e^{3K}N^{3K-2}}{K^{3K+3}}\right)
\end{eqnarray}

Even for an agent which can play $10^{12}$ actions per second, this will take about $10$ million years to outperform \NAM\ for a setup with $N=30$ and $K=15$. Hence, for all practical problems when an agent have large number simultaneously arms to play, \NAM\ algorithm will outperform UCB algorithm.

==> social_influence.tex <==
% \newpage
\section{Application to Social Influence Maximization} \label{evaluation}

We now apply \NAM\ and evaluate it for solving the problem of Social Influence Maximization, which in the words of Domingos \& Richardson \citep{domingos2001mining} is defined as follows: ``if we can try to convince a subset of individuals in a social network to adopt a new product or innovation, and the goal is to trigger a large cascade of further adoptions, which set of individuals should we target?''

\subsection{Problem Description}

Consider a social network $G=(V,E,P)$, where $V$ is the node set representing individuals, $E=\{(u,v): u,v \in V\}$ is the set of directed ($u$ to $v$) connections among the individuals, and $P=\{p_{e}: e \in E\}$ is the set the strengths/weights of the connections in $E$. % Note that, $p_{(u,v)}=0$ can be seen as absence of a directed connection from $u$ to $v$.

For the standard influence maximization problem \citep{kempe2003maximizing}, we select a `seed' set $S$ of $K>0$ individuals to initiate a cascade.  Analogous to diseases spreading between individuals, the set of users $S$ will attempt to influence their neighbors in the social network $G$, and those infected neighbors will attempt to influence their neighbors, and so on.  We consider the simple, discrete-time \emph{independent cascades} diffusion model.  In this model, if individual $u$ becomes influenced, then at the next time step, individual $u$ attempts to influence each of his neighbors $v$ in the network with probability $p_{(u,v)}$.  All the influence attempts are statistically independent of each other.  Our goal in picking the seed set $S$ is to have a large cascade.  Let $y^{(v)} = 1$ denote that  node $v$ was influenced in the cascade and $y^{(v)} = 0$ otherwise. Let $\sigma(S)$ denote the expected cascade size when $S$ is the seed set,  
\begin{eqnarray}
\sigma(S) &=& \mathbb{E}\left[\sum_{v \in V} y^{(v)} \bigg | \text{individuals in } S %\right.\nonumber\\&&\left. 
\text{ were initially influenced}  \right].
\end{eqnarray}  The goal is to find $\argmax_{S\subseteq V:\ |S|=K} \sigma(S)$. 


Note that the word time-step in the above diffusion model is different from the word time-step in an adaptive/online algorithm. In fact, for every time-step in an adaptive algorithm, the entire diffusion (all time-steps of the aforementioned independent cascade model) takes place.


In the traditional problem, $G$ is fully known, not only the edge set $E$ but also the diffusion parameters $P$.  Here, we consider an adaptive version of the problem, \emph{where only the individuals (node set $V$) are known.}  At each time $t$, we  select a seed set $S_t$ and observe a single resulting cascade $\{y^{(v)}_t\}_{v\in V}$. Using the information from those outcomes, at time $t+1$ we select a (possibly new) seed set, and so on.  We want to maximize the average, expected %\footnote{\hl{expected or actual?}; also check notation consistent with earlier parts; state not denoting time within a cascade?} cascade size, 
\begin{eqnarray}
\argmax_{ \{S_t \subseteq V: |S_t|=K\}_{t=1}^T} \ \frac{1}{T} &&\sum_{t=1}^T \ \mathbb{E}\left[\sum_{v \in V} y_t^{(v)} \bigg | \text{individuals in } S_t %\right.\nonumber\\&&\left. 
\text{ were initially influenced} \right]  
\end{eqnarray}

Recent works on adaptive influence maximization assume semi-bandit feedback, such as which specific nodes were influenced or even along which edges influence propagated \citep{wen2017online, vaswani2017model}.  In \citep{lei2015online}, $\epsilon$-greedy strategies are proposed for adaptive influence maximization although assumptions are made on edge parameter distributions. 

\subsection{Algorithms}  \label{social_algorithms} We propose  to solve the adaptive influence maximization problem using \NAM . Note that \NAM\ is a general procedure for CMAB problems and does not use any special properties of network diffusion models or knowledge about the edge set $E$ or parameters $P$.  

The reward $r_{\bf a}(t)$ for an action ${\bf a}$ of choosing seed set $S$ at time $t$ is the count of infected individuals in a cascade run at time $t$ where only nodes in $S$ were initially infected,
\[r_{\bf a}(t) = \sum_{v \in V} y_t^{(v)}   \  \text{ where only } v \in S \text{ were initially influenced}  .\]
%
%\color{blue}
The aggregate reward function $r_{\bf a}(t)$ cannot be decomposed into a function of ``rewards'' for individual nodes like  $f({\bf d}_{{\bf a}_t})$ in \eqref{eq:R_at_t}.  Thus, it does not strictly satisfy the assumptions used to prove performance guarantees for \NAM.  However, the reward function $r_{\bf a}(t)$ satisfies properties related to those in the assumptions.  We discuss this in more detail in Appendix \ref{appendix_social_influence3}.

% It is not clear that the aggregate reward function $r_{\bf a}(t)$ can be decomposed into a function of ``rewards'' for individual nodes like  $f({\bf d}_{{\bf a}_t})$ in \eqref{eq:R_at_t}.  One approach for doing so is using the marginal influence, such as setting the individual reward $X_{i,t}$ of person $i$ at time $t$  as the resulting cascade size if $i$  alone was initially influenced in cascade $t$; then letting the reward $r_{\bf a}(t)$ for the set $S$ be the count of nodes influenced by at least one of the $v \in S$ (e.g., combine the cascades of individual seeds). However, the corresponding reward $r_{\bf a}(t)$ would depend on the overlap of the cascade subgraphs, which depends in part on which seeds $i$ are in $S$ and their relative locations in the network, not just the sizes $\{X_{i,t}\}_{i\in S}$ of the individual cascades.  Thus, defining individual rewards in this way would lead to $r_{\bf a}(t)$ not satisfying the form \eqref{eq:R_at_t} in general, where $f(\cdot)$ should not depend on the specific indices $i \in {\bf a}$. We note that even though the influence function does not satisfy the assumptions used to prove performance guarantees for \NAM, yet it nonetheless performs well empirically. 


% In Appendix \ref{appendix_social_influence3}, we explain the assumptions satisfied by the Social Influence Maximization problem. Additionally, even though stochastic dominance does not hold for influence maximization in social networks,  we empirically found that a related property  does hold with non-negligible probability.  That is discussed further in Appendix \ref{appendix_social_influence3}.


    We compare the performance of \NAM\ against an $\epsilon$-greedy version of the \textit{credit distribution model} \cite{goyal2011data}, we call it $\epsilon$-CD. The credit distribution model was proposed to infer influences from historical data without knowledge of the diffusion parameters.  It does require the edge set $E$; to provide a fair comparison to \NAM, we provide the credit distribution method  with the edge set of the complete directed graph (for which edges $e' \not \in E$ have $p_{e'} = 0$).
        
    The $\epsilon$-CD algorithm follows standard $\epsilon$-greedy method for bandits. For a fraction $\epsilon$ of the total time horizon $T$, a random size $K$ subset of nodes is chosen.  For the rest of the time horizon it exploits the best seed set of size $K$ chosen by the credit-distribution algorithm using the diffusion history obtained from $\epsilon T$ time steps.  The  credit-distribution algorithm uses the list of infected nodes from the $t-1$ previous cascades and when exactly did they get infected within those cascades to estimate the expected reward of different size $K$ seed sets.  The seed set it estimates as best is then used at time $t$.  Note that the proposed algorithm CMAB uses more limited feedback--only the number of nodes infected in each cascade.
        
    It is also of interest to understand that how close does \NAM \ get to the actual optimal set. However, for large networks, it can be computationally intractable to find the optimal set. Hence, instead of the optimal set, we compare \NAM \ with the greedy-best optimal set obtained by the simulation-based greedy algorithm which is guaranteed \citep{kempe2003maximizing} to have an influence of at least $1-\frac{1}{e}$ times the influence of the actual optimal set. Moreover, the simulation-based greedy algorithm is computationally very expensive as compared to \NAM \ as it involves large number of costly Monte-Carlo simulations.

% The simulation-based greedy algorithm guarantees an expected influence of at least .66 times the optimal expected influence.


% To compare against \NAM, we use an $\epsilon$-greedy 

% lei2015online 
% wen2017online  -- edge knowledge
% vaswani2017model -- similar to edge knowledge

\subsection{Experimental Setup}

For our experiments, we considered the \textit{Facebook Friends network} \cite{leskovec2012learning} which has 4039 nodes with 88234 undirected edges. We  used a representative community (sub-network) of the Facebook network which has 534 nodes and 8158 undirected edges. It was identified using the the Louvain method for community detection \cite{blondel2008fast}.    The selected community originally had one node with extremely high degree of 533 within the selected community, which was removed.  Each undirected edge was then replaced by two directed edges. Following \cite{kempe2003maximizing},  for each node $v\in V$, the parameter of each edge entering $v$ was set to $1/\text{indegree}(v)$.  We used a time horizon of $T=100,000$. At each time step $t$, each method selected a seed set $S_t$, which was used to run a single cascade.  The total number of influenced users was set as the reward.
    
For the $\epsilon$-CD algorithm, we used the exploration probabilities $\epsilon=0.10,0.25$.  For the offline greedy algorithm, we averaged 1000 Monte-Carlo diffusions for each candidate subset. 
    
We used seed-set sizes $K = 2,4,8$.  Performance of each algorithm was measured using observed reward, averaged over 10 runs. For aesthetic reasons, we  smoothed the average across runs  using a simple moving average of the data for previous 500 time points.

For the simulation-based greedy algorithm, we have calculated the expected influence of any subset as Monte-Carlo average of the observed influences based on 1000 diffusions. 

\begin{figure}
   \subfigure[$K=2$]{
       % \centering
        \input{figures/sim_reward_plot_k_2_fb4_new}
     %   \caption{$K=2$}
        \label{fig:K_2_fb}
   }
%\hspace{.1in}
   \subfigure[$K=4$]{
    %    \centering
        \input{figures/sim_reward_plot_k_4_fb4_new}
    %    \caption{$K=4$}
        \label{fig:K_4_fb}}
%\hspace{.1in}
   \subfigure[$K=8$]{
     %   \centering
        \input{figures/sim_reward_plot_k_8_fb4_new}
    %    \caption{$K=8$}
        \label{fig:K_8_fb}}
\caption{Averaged observed reward for different algorithms for different seed set sizes for the \textit{Facebook friends network}.} \label{fig:figure_facebook_reward}
\end{figure}

\subsection{Results}
The observed reward for each algorithm, averaged over 10 independent runs and further smoothed using moving average filter on the time-axis, is shown in Figure \ref{fig:figure_facebook_reward}, separately for each $K=2,4,8$. 
        
For all values of $K$, \NAM \  significantly out-performs  the UCB algorithm.  For the size of this problem ($N=534$ and $K\in\{2,4,8\}$), the UCB algorithm is unable to even finish sampling each possible set of $K$ nodes once, even for $K=2$.  Thus, although for sufficiently large $T$ the UCB algorithm should eventually find the optimal set, it needs a much larger time horizon $T$ to do so.   The efficient divide-and-conquer strategy of \NAM \ allows it to do well while the exhaustive-search based UCB algorithm is still in the exploration phase.
        
For all values of $K$, \NAM \ achieves a lower cumulative reward than the $\epsilon$-CD algorithms (area under the curves in Figure \ref{fig:figure_facebook_reward}). Recall that the $\epsilon$-CD algorithms are domain-specific and receive significantly more feedback than our proposed domain-agnostic algorithm \NAM \ does, so we expect that the $\epsilon$-CD algorithms would do better.  We note that the \NAM\ algorithm is in SORT phase until around $t=4\times 10^4$. The \NAM\ algorithm finishes exploration around  $t=9 \times 10^4$ which is consistent with Lemma $14$ of the main text with $\lambda$ defined in Equation $19$.
       
However, despite \NAM \ being domain-agnostic and receiving less feedback,  the final seed sets selected by \NAM \ are significantly better than those selected by the $\epsilon$-CD algorithms for $K=2$ and $K=8$, and slightly better for $K=4$.  In fact, for $K=2$, despite having no explicit knowledge of the underlying network or diffusion dynamics, and receiving minimal feedback, \NAM \ finds the same set as the greedy offline method, which is provably near-optimal.     This result may in part be due to  probabilistic stochastic dominance holding with a high probability, especially for $K=2$. 

%\color{black}
We do not formally compare empirical run-times of the different algorithms because we wrote Python3 implementations for \NAM \ and UCB, but for $\epsilon$-CD, we used Python3 code that called an executable for the credit distribution method \citep{CDcode} which required extensive disk I/O.  In Table \ref{run_time_table}, we provide complexity bounds,  suggesting $\epsilon$-CD is inherently slower than \NAM. In terms of both time and space complexity, \NAM \ algorithm outperforms $\epsilon$-CD algorithm (a domain-specific algorithm) and UCB algorithm (a bandit-specific algorithm). 

%\color{blue}
        We compare the amortized time-complexity for all the algorithms. We do so because exactly once for the entire time-horizon, the $\epsilon$-CD algorithm scrapes through the history of independent-cascade diffusions accumulated over $\epsilon T$ time steps where each diffusion can be of the length $N$ in the worst-case. Hence, $\epsilon N T $ amount of time consumed by this bottleneck step is effectively distributed over $T$ time steps. However, the space-complexity cannot be distributed across all time steps, as we would need a computer of at least worst-case space-complexity to store the history of independent-cascade diffusions accumulated over $\epsilon T$ time steps. Hence, we compare the worst-case space complexity for all algorithms.

\begin{table}[h!]
	\caption{Computational complexities of  the different algorithms}\label{run_time_table}
	\centering
	\begin{tabular}{c c c}
		\hline \hline
		Algorithm & Amortized Time-Complexity & Worst-Case Space-Complexity \\
		\hline
		CMAB &    $O(K \log K)$ &    $O(N)$\\
		$\epsilon$-CD &  $\Omega(\epsilon N)$ &    $\Omega\left(\epsilon NT \right)$\\
		UCB &    $O( N^K K \log N )$ &   $O( N^K)$ \\
		\hline
	\end{tabular}
\end{table}
    
\begin{remark}
    For sufficient exploration time, there is an additional factor of $T^{-\frac{1}{3}}$ in amortized time-complexity of the \NAM\ algorithm as the exploration, and sorting of actions, only happens for $O(T^\frac{2}{3})$ steps.
\end{remark}
%\color{black}

==> sortmergetime1.tex <==
\subsection{Number of time steps in SORT and MERGE subroutines}

In this subsection, we will bound the number of exploration time steps that are spent in SORT and MERGE subroutines. The next result bounds the number of time steps spent in a group $G$ in the SORT subroutine to obtain an ordering on the actions and thus on arms (by Lemma \ref{ordering_from_expectation}). 

\begin{lemma}[Sort time requirement] \label{sort_requirements}
	SORT subroutine (\cref{alg:da}) gives correct ordering on $K+1$ actions in a group $G$ with probability $1-\frac{K}{N^2T^2}$, for a threshold $\lambda$ defined in equation (\ref{eq:define_lambda}), where the actions are chosen for at most % total play requirement at most
	\begin{equation}
	O\left(\sum_{i=1}^{K+1} \frac{U^2}{\max(\delta_{G(i)}^2, \lambda^2)}\right)
	\end{equation}
	time steps, where 
	\begin{eqnarray}
	\delta_{G(i)} = \left\{\begin{array}{cr}\mathbb{E}\left[X_{G(i)}\right] - \mathbb{E}\left[X_{G(i+1)}\right], &i = 1 \\
	\min\left\{\mathbb{E}\left[X_{G(i-1)}\right] - \mathbb{E}\left[X_{G(i)}\right], \mathbb{E}\left[X_{G(i)}\right] - \mathbb{E}\left[X_{G(i+1)}\right]\right\}, &i \in {2,...,K}\\
	\mathbb{E}\left[X_{G(i)}\right] - \mathbb{E}\left[X_{G(i+1)}\right], &i = K+1 \end{array}\right. \label{eq:delta_i_def}
	\end{eqnarray}
\end{lemma} 
\begin{proof}
	Let $G(i)$   for all $ i \in {1, 2, \cdots,K+1}$ be the different arms of group $G$ that we aim to sort using the SORT subroutine. Let $\hat{\mu}_{{\bf a}^G_{-i}}$ be the estimate of action made using all arms in $G$ except  arm $G(i)$. We want to identify the number of time steps spent in SORT subroutine, and the error probability in the ordering.   
	
	%action ${\bf a}^G_{-i}$, and the error probability for ranking.
	
	%We consider a group $G$ with arms $G(i) \forall i \in {1, 2,...,K+1}$ which is to be sorted. Let $\hat{\mu}_{{\bf a}^G_{-i}}$ be estimate of action made using all but $G(i)$ arm. We want to identify the number of plays required for action ${\bf a}^G_{-i}$, and the error probability for ranking.
	
	The algorithm proceeds in rounds starting from $r = 1$. We define $\Delta_r \triangleq 2^{-r}$, and each un-sorted action in round $r$ is played for $n_r \triangleq \frac{\log{2NT}}{\Delta^2_r}$ time steps. Using Hoeffding's Inequality, the expected reward estimate of each action lies in the range $\left[\hat{\mu}_{{\bf a}^G_{-i}} - \Delta_r, \hat{\mu}_{{\bf a}^G_{-i}} + \Delta_r\right]$ with probability bound given as 
	\begin{eqnarray}
	P\left(\big|\mu_{{\bf a}^G_{-i}} - \hat{\mu}_{{\bf a}^G_{-i}}\big| \geq \Delta_r  \right) &\leq& 2e^{-2\frac{\log{2NT}}{\Delta^2_r}\Delta^2_r} \label{eq:hoeffding_error_bound}\\
	%        &=& 2\times\frac{1}{(2NT)^2}\\
	&=& \frac{1}{2N^2T^2}\label{eq:hoeffding_error_boundl}
	\end{eqnarray}
	%   Inequality (\ref{eq:hoeffding_error_bound}) follows from the definition of $\Delta_r$, $n_r$, and Lemma \ref{Hoeffding_lemma}. 
	Thus,  the expected reward estimate of each action lies in the range $\left[\hat{\mu}_{{\bf a}^G_{-i}} - \Delta_r, \hat{\mu}_{{\bf a}^G_{-i}} + \Delta_r\right]$ with probability  at least $1- \frac{1}{2N^2T^2}$. Let it take $r_i$ rounds to be able to sort ${\bf a}^G_{-i}$ in its correct position, which implies that all other actions can be well separated from this action.  When two actions are separated, upper confidence bound for the action with a lower estimated reward is less than the lower confidence bound of action with higher estimated reward, which gives the following inequality
	\begin{eqnarray}
	\hat{\mu}_{{\bf a}^G_{-i}} + \Delta_{r_i} &<& \hat{\mu}_{{\bf a}^G_{-j}} -\Delta_{r_i}. \label{eq:estimate_deltas}
	\end{eqnarray}
	This further means that the actions ${\bf a}^G_{-i}$ and ${\bf a}^G_{-j}$ were inseparable in round $r_i -1$, thus the following holds.
	\begin{eqnarray}
	\hat{\mu}_{{\bf a}^G_{-i}} + \Delta_{r_i-1} &\geq& \hat{\mu}_{{\bf a}^G_{-j}} -\Delta_{r_i-1} \label{eq:estimate_deltas_r_1}
	\end{eqnarray}
	However, using Lemma \ref{Hoeffding_lemma}, $\hat{\mu}_{{\bf a}^G_{-i}}$ lies between the confidence region around the true mean as $\hat{\mu}_{{\bf a}^G_{-i}} \in \left[\mu_{{\bf a}^G_{-i}} - \Delta_{r_i-1}, \mu_{{\bf a}^G_{-i}} + \Delta_{r_i-1}\right]$. The same is true for $\hat{\mu}_{{\bf a}^G_{-j}}$. Using the upper limits of estimated mean rewards, we can rewrite inequality (\ref{eq:estimate_deltas_r_1}) as 
	\begin{eqnarray}
	\mu_{{\bf a}^G_{-i}} + 2\Delta_{r_i-1} &\geq&\mu_{{\bf a}^G_{-j}} - 2\Delta_{r_i-1} \label{eq:true_deltas}
	\end{eqnarray} 
	From inequality (\ref{eq:true_deltas}), we get $\Delta_{r_i}$ in terms of the difference of expected rewards of the two arms as follows. 
	\begin{eqnarray}
	4\Delta_{r_i-1} &\geq& \mu_{{\bf a}^G_{-j}}-\mu_{{\bf a}^G_{-i}} \label{eq:true_deltas_v2}\\
	%        &\geq& \frac{1}{U}\Big|\Big|\mathbb{E}\left[{\bf d}_{{\bf a}^G_{-j}}\right] - \mathbb{E}\left[{\bf d}_{{\bf a}^G_{-i}}\right]\Big|\Big|_2 \label{eq:cont_vect_diff}\\
	&\geq& \frac{1}{U}\left(\mathbb{E}\left[X_{G(i)}\right] - \mathbb{E}\left[X_{G(j)}\right]\right), \label{eq:cont_arm_diff}
	\end{eqnarray} 
	where the last step follows from corollary \ref{double_sided_continuity}. 
	% Inequality (\ref{eq:true_deltas_v2}) is by shuffling the terms to get the confidence bound in terms of difference of expected reward of two actions. Inequality (\ref{eq:cont_vect_diff}) follows from assumption \ref{continuous_assumption}, and inequality (\ref{eq:cont_lower_defn}). And, (\ref{eq:cont_arm_diff}) is obtained as $\mathbb{E}\left[{\bf d}_{\bf a}\right]$ is a column vector in individual rewards of arms in action ${\bf a}$.
	%  We now try to find the number of rounds $r_i$ needed to separate the actions.
	Using the definition of $\Delta_r$ and the upper bound obtained in inequality (\ref{eq:cont_arm_diff}), we have
	\begin{eqnarray}
	2^{-(r_i-1)} &=& \Delta_{r_i-1} \label{eq:delta_r_i_def}\\
	&\geq& \frac{\left(\mathbb{E}\left[X_{G(i)}\right] - \mathbb{E}\left[X_{G(j)}\right]\right)}{4U} \label{eq:delta_r_i_up_lim}
	\end{eqnarray} 
    %    Equation (\ref{eq:delta_r_i_def}) follows from the definition of confidence region, and (\ref{eq:delta_r_i_up_lim}) follows from inequality (\ref{eq:cont_arm_diff}). 
	Taking logarithm with base $2$, we obtain a lower bound on the number of rounds needed as 
	\begin{eqnarray}
	r_i - 1 &\leq& \log_2{\left(\frac{4U}{\left(\mathbb{E}\left[X_{G(i)}\right] - \mathbb{E}\left[X_{G(j)}\right]\right)}\right)}. \label{eq:r_upper_lim}
	\end{eqnarray} 
	
	The term $\left(\mathbb{E}\left[X_{G(i)}\right] - \mathbb{E}\left[X_{G(j)}\right]\right)$ will be lowest for $j=i+1$ or $i-1$ since the arms closest to $i$ will result in the lowest gap. Thus, we define  $\delta_i$ for arm $G(i)$ as 
	\begin{eqnarray}
	\delta_i &\triangleq& \min\left\{\mathbb{E}\left[X_{G(i)}\right] - \mathbb{E}\left[X_{G(i+1)}\right], \mathbb{E}\left[X_{G(i-1)}\right] - \mathbb{E}\left[X_{G(i)}\right]\right\}
	\end{eqnarray}
	Number of rounds to correctly rank arm $G(i)$ can thus be upper bounded as follows. 
	\begin{eqnarray}
	r_i &\leq& \log_2{\left(\frac{8U}{\delta_i}\right)}.  \label{eq:r_i_upper_delta}
	\end{eqnarray}
	Having bounded the number of rounds to rank ${\bf a}^G_{-i}$, we  find the number of time steps each action is played till round $r_i$ as follows.
	
	%   Now we need to find number of plays obtained while going till round $r_i$. From the definition of number of plays $n_r$ and using the value of $r_i$, we get,
	\begin{eqnarray}
	n_{r_i} &=& \frac{\log{2NT}}{\Delta^2_{r_i}} \label{eq:n_r_i_Delta}\\
	&=& 2^{2{r_i}}\log{2NT} \label{eq:n_r_i_rounds}\\
	&\le& 2^{2\log_2{\left(\frac{8U}{\delta_i}\right)}}\log{2NT} \label{eq:n_r_i_exp_delta}\\
	&=& \frac{64U^2\log{2NT}}{\delta^2_i} \label{eq:n_r_i_frac_delta}
	\end{eqnarray}
	This provides the number of times  action ${\bf a}^G_{-i}$ is played. Let $\lambda$ be chosen as a threshold, which is the precision level below which we cannot correctly order two actions. Using  $\lambda$ as a lower bound for $\delta_i$, each of the $K+1$ action is chosen for $n_{r_i}$ times, where $\delta_i$ is replaced by $\max(\delta_i,\lambda)$. Thus, the total time steps any of the action is selected is given as 
	
	%    we have the maximum number of time steps in round limited by
	\begin{eqnarray}
	n' &\le& \sum_{i=1}^{K+1}\frac{64U^2\log{2NT}}{\max(\delta^2_i, \lambda^2)}   \end{eqnarray}
	which proves the number of time steps as in the statement of the Lemma.
	%Thus, the total time the action is chosen, $n'$, is given as follows. 
	
	%    Thus, we get the number of plays required for an individual action. After an action is ranked correctly, we will not play it again, so the total number of plays $n'$ as the sum of all plays required for all actions in terms of $\delta_i$ as
	%  \begin{eqnarray}
	%    n' &=& \sum_{i = 1}^{K+1}\frac{64U^2\log{2NT}}{\delta^2_i}
	% \end{eqnarray}
	%  where delta is defined in equation (\ref{eq:delta_i_def}). 
	
	For $K+1$ arms, there can be $\binom{K+1}{2}$ ordered pairs denoting the edges of a complete graph, where each edge is the ordering of the two vertices. However, the ordering is preserved by a sub-graph which is a tree by just keeping the edges which connect two immediately ordered vertices. The number of edges thus becomes $(K+1) - 1 = K$. Thus, there are $K$ orderings in a group, and all of them should be correct to make the algorithm work. The probability of error in sorting  group $G$ can then be written as
	\begin{eqnarray}
	P\left(\{\text{any arm is incorrectly sorted}\}\right) &=& 1 - P\left(\{\text{all arms are correctly sorted}\}\right)\\
	&\le& 1 - \left(1-\frac{1}{2N^2T^2}\right)^K\\
	&<& 1 - \left(1 -\frac{K}{2N^2T^2} \right)\\
	&=& \frac{K}{2N^2T^2}, \label{eq:sort_prob_error}
	\end{eqnarray} 
	where the probability that any two arms are incorrectly sorted is bounded by $\frac{1}{2N^2T^2}$ as given in \eqref{eq:hoeffding_error_boundl}. This proves the probability of correct ordering as in the statement of the Lemma. 
\end{proof}

Having understood the number of time steps spent in the SORT subroutine, and the error probability of ranking arms in each group, we now consider the MERGE subroutine. In the following lemma, we find the number of time steps it takes to merge two groups, with an error probability on the ordering in the combined group.  

\begin{lemma}[Merge time requirement] \label{Merge_requirements}
	MERGE subroutine (\cref{alg:ma}) merges arms in two groups $G_1$ and $G_2$ to $G$ correctly with probability $1-\frac{K}{N^2T^2}$, for a threshold $\lambda$ as defined in equation (\ref{eq:define_lambda}), where the total number of time steps needed to merge is at most 
	\begin{eqnarray}
	&O\left(\sum_{i=1}^{K+1} \frac{U^2}{\max(\delta_{G(i)}^2, \lambda^2)} \right),\text{ where }&\\
	&\delta_{G(i)} = \Bigg\{\begin{array}{cr}\mathbb{E}\left[X_{G(i)}\right] - \mathbb{E}\left[X_{G(i+1)}\right], &i = 1 \\
	\min\left\{\mathbb{E}\left[X_{G(i-1)}\right] - \mathbb{E}\left[X_{G(i)}\right], \mathbb{E}\left[X_{G(i)}\right] - \mathbb{E}\left[X_{G(i+1)}\right]\right\}, &i \in {2,...,K}\\
	\mathbb{E}\left[X_{G(i)}\right] - \mathbb{E}\left[X_{G(i+1)}\right], &i = K+1 \end{array}&
	\end{eqnarray}
\end{lemma} 
\begin{proof}
In the MERGE subroutine, we use the sorted groups $G_1$ and $G_2$ to construct a group $G$ of $K$ elements such that arms in group $G$ are sorted. We maintain two counters $i$ and $j$ for the groups $G_1$ and $G_2$ respectively. We replace arm $G_2(j)$ by $G_1(i)$ in group $G_1$ to create a new action. We play both actions in rounds starting from $r=1$. At the end of  round $r$, the deviation of estimated mean reward and true expected rewards is $\Delta_r \triangleq 2^{-r}$. By round $r$, each action has been played for $n_r \triangleq \frac{\log{2NT}}{\Delta_r^2}$ time steps similar to \cref{alg:da}. Two actions are separated when the upper confidence bound of worse action is lesser than the lower confidence bound of better action. We then add the arm corresponding to better action to group $G$ and increment the counter for the corresponding group from which arm was picked and continue comparing new actions. This is continued till we have $K$ arms in $G$.
	
Since the fundamental concept of comparison of two actions in  \cref{alg:ma} is the same as that in  \cref{alg:da}, similar analysis follows and the number of time steps required to merge the groups is 
	\begin{eqnarray}
	n' &\le& \sum_{i=1}^{K+1} \frac{1}{U^2\max{(\delta_{G(i)}^2,\lambda^2)}}, %\text{where}
	\end{eqnarray}
%	\begin{eqnarray}
%	\delta_{G(i)} = \Bigg\{\begin{array}{cr}\mathbb{E}\left[X_{G(i)}\right] - \mathbb{E}\left[X_{G(i+1)}\right], &i = 1 \\
%	\min\left\{\mathbb{E}\left[X_{G(i-1)}\right] - \mathbb{E}\left[X_{G(i)}\right], \mathbb{E}\left[X_{G(i)}\right] - \mathbb{E}\left[X_{G(i+1)}\right]\right\}, &i \in {2,...,K}\\
%	\mathbb{E}\left[X_{G(i)}\right] - \mathbb{E}\left[X_{G(i+1)}\right], &i = K+1 \end{array}&        
%	\end{eqnarray}
	where $G(K+1)$ is the last arm with which comparison was made but not added to group $G$. The same argument as in the proof of Lemma \ref{sort_requirements} can be used to bound the error probability of a single run of \cref{alg:ma} by $\frac{K}{2N^2T^2}$.
\end{proof}

